Near Delay-Optimal Scheduling of Batch Jobs in Multi-Server Systems

We study a class of scheduling problems, where each job is divided into a batch of unit-size tasks and these tasks can be executed in parallel on multiple servers with New-Better-than-Used (NBU) service time distributions. While many delay optimality results are available for single-server queueing systems, generalizing these results to the multi-server case has been challenging. This motivated us to investigate near delay-optimal scheduling of batch jobs in multi-server queueing systems. We consider three lowcomplexity scheduling policies: the Fewest Unassigned Tasks first (FUT) policy, the Earliest Due Date first (EDD) policy, and the First-Come, First-Served (FCFS) policy. We prove that for arbitrary number, batch sizes, arrival times, and due times of the jobs, these scheduling policies are near delay-optimal in stochastic ordering for minimizing three classes of delay metrics among all causal and non-preemptive policies. In particular, the FUT policy is within a constant additive delay gap from the optimum for minimizing the mean average delay, and the FCFS policy within twice of the optimum for minimizing the mean maximum delay and the mean p-norm of delay. The key proof tools are several novel samplepath orderings, which can be used to compare the sample-path delay of different policies in a near-optimal sense.

==> appendices.tex <==
% !TEX root = ./replication.tex
\ifreport
\appendices
\else
\appendix
\fi
\section{Proofs of Lemmas~1-3 and Corollaries 1-2} \label{app0}
\ifreport
\begin{proof}[Proof of Lemma \ref{lem1}]
\else
\begin{proof}[of Lemma \ref{lem1}]
\fi
First, fix the sequence of task completion times as $\bm{T}(\pi)=\bm{t}$ for all $\pi\in\Pi$. Because a job is completed at the time that the last task of the job is completed, each job completion time $C_i(\pi)$ must be equal to one element of $\bm{t}$. Using condition 2 and the sample-path optimality of the preemptive SRPT discipline \cite{Schrage68,Smith78}, one can obtain that for all $\pi\in\Pi$ and $\bm{t}\geq\bm{0}$
\begin{align}
[\bm{C}_{\uparrow} (P')|\bm{T}(P')=\bm{t}] \leq[\bm{C}_{\uparrow} (\pi)|\bm{T}(\pi)=\bm{t}],\nonumber
\end{align} 
where $\bm{C}_{\uparrow} (\pi)= (C_{(1)}(\pi),\ldots,$ $C_{(n)}(\pi))$ is the increasing time sequence of job completions. In addition, using the proof arguments in \cite{Schrage68,Smith78}, we can show that $[\bm{C}_{\uparrow} (P') | \bm{T}(P')=\bm{t}]$ is an increasing function of $\bm{t}$. This implies
\begin{align}\label{eq_order}
[\bm{C}_{\uparrow} (P')|\bm{T}(P')=\bm{t}] \leq[\bm{C}_{\uparrow} (\pi)|\bm{T}(\pi)=\bm{t}'],
\end{align} 
whenever $\bm{0}\leq\bm{t}\leq \bm{t}'$. On the other hand, condition 1 tells us that for all $\pi\in\Pi$ and $\mathcal{I}$
\begin{align}\label{eq_order_}
[\bm{T}(P')|\mathcal{I}] \leq_{\text{st}}[\bm{T}(\pi)|\mathcal{I}].
\end{align} 
%Therefore, 
%\begin{align}
%[{D}_{\text{avg}}(\bm{C}_{} (P))|\mathcal{I}] \leq_{\text{st}}[{D}_{\text{avg}}(\bm{C}_{} (\pi))|\mathcal{I}].\nonumber
%\end{align} 
According to Theorem 6.B.3 and Theorem 6.B.16(c) of \cite{StochasticOrderBook}, we can obtain from  \eqref{eq_order} and \eqref{eq_order_} that
\begin{align}\label{eq_order_1}
[\bm{C}_{\uparrow} (P')|\mathcal{I}] \leq_{\text{st}}[\bm{C}_{\uparrow} (\pi)|\mathcal{I}].
\end{align} 
Combining this and condition 3, we can get
\begin{align}
[\bm{U}_{\uparrow} (P)|\mathcal{I}] \leq_{\text{st}}[\bm{C}_{\uparrow} (\pi)|\mathcal{I}].\nonumber
\end{align} 
Since ${D}_{\text{avg}}\in \mathcal{D}_{\text{sym}}$ is symmetric and increasing, we can obtain that for all $\pi\in\Pi$ and $\mathcal{I}$
\begin{align}
&[{D}_{\text{avg}}(\bm{U} (P))|\mathcal{I}]=[{D}_{\text{avg}}(\bm{U}_{\uparrow} (P))|\mathcal{I}] \nonumber\\
\leq_{\text{st}}&[{D}_{\text{avg}}(\bm{C}_{\uparrow} (\pi))|\mathcal{I}] = [{D}_{\text{avg}}(\bm{C} (\pi))|\mathcal{I}],\nonumber
\end{align} 
where the inequality follows from Theorem 6.B.16(a) of \cite{StochasticOrderBook}. By this, \eqref{eq_lem1_1} is proven.

If condition 3 is replaced by $P'=P$, then \eqref{eq_lem1_2} follows from \eqref{eq_order_1} and Theorem 6.B.16(a) of \cite{StochasticOrderBook}. This completes the proof.
%In addition, 
%
%Let $[{D}_{\text{avg},\pi} |\mathcal{I}, (t_{1,\pi},\ldots,t_{J,\pi}) = (t_1,$ $\ldots, t_J)]$ denote the average delay of policy $\pi$ for given parameters $\mathcal{I}$ and task completion instants $(t_1,\ldots, t_J)$. According to the sample-path optimality of the preemptive SRPT discipline \cite{Schrage68,Smith78}, $[{D}_{\text{avg},\pi} | \mathcal{I}, (t_{1,\pi},\ldots,t_{J,\pi}) = (t_1,\ldots,$ $ t_J)]$ is minimized among all policies in $\Pi$, if each completed task belongs to a job with the fewest remaining tasks. By condition 2, policy $P$ satisfies this requirement, and hence
%\begin{align}
%&~~~[{D}_{\text{avg},P} | \mathcal{I}, (t_{1,P},\ldots,t_{J,P}) = (t_1,\ldots, t_J)] \nonumber\\
%&\leq [{D}_{\text{avg},\pi} | \mathcal{I}, (t_{1,\pi},\ldots,t_{J,\pi}) = (t_1,\ldots, t_J)],~\forall~\pi\in\Pi.\nonumber
%\end{align}
%Further, $[{D}_{\text{avg},\pi} | \mathcal{I}, (t_{1,\pi},\ldots,t_{J,\pi}) = (t_1,\ldots, t_J)]$ is an increasing function of $(t_1,\ldots, t_J)$, because if task completions are postponed, the job completions are also postponed.
%Therefore, for any $\pi\in\Pi$, we have
%\begin{align}\label{eq_order}
%&~~~[{D}_{\text{avg},P} | \mathcal{I}, (t_{1,P},\ldots,t_{J,P}) = (t_1,\ldots, t_J)] \nonumber\\
%&\leq [{D}_{\text{avg},\pi} | \mathcal{I}, (t_{1,\pi},\ldots,t_{J,\pi}) = (t_1',\ldots,t_J')],\nonumber\\
%&~~~~~~~~~~~~~~~~~~~~\text{whenever}~(t_1,\ldots, t_J)\leq (t_1',\ldots,t_J').
%\end{align}
%By condition 1, we can obtain 
%\begin{align}\label{eq_order_}
%(t_{1,P},\ldots,t_{J,P})\leq_{\text{st}}(t_{1,\pi},\ldots,t_{J,\pi}),~\forall~\pi\in\Pi.
%\end{align}
%With \eqref{eq_order} and \eqref{eq_order_}, we can use the standard construction argument
% in Theorem 6.B.3 of \cite{StochasticOrderBook} to show that for all $\pi\in\Pi$
%\begin{align}\label{eq_order1}
%\!\!\!\![{D}_{\text{avg},P}, (t_{1,P},\ldots,t_{J,P})| \mathcal{I}] \leq_{\text{st}} [{D}_{\text{avg},\pi}, (t_{1,\pi},\ldots,t_{J,\pi}) | \mathcal{I}].\!\!\!\!
%\end{align}
%Then, \eqref{eq_thm1} follows from \eqref{eq_order1} and Theorem 6.B.16 (c) of \cite{StochasticOrderBook}. 
%Finally, \eqref{eq_thm1_1} follows from condition 3, \eqref{eq_thm1}, and Eq (6.B.4) of \cite{StochasticOrderBook}.
%By Theorem \ref{thm1}, for all $\mathcal{I}$, we have
%\begin{align}
%\mathbb{E}[{D}_{\text{avg},P'}| \mathcal{I}]  \leq \mathbb{E}[{D}_{\text{avg},\pi}| \mathcal{I}],~\forall~\pi\in\Pi.\nonumber
%\end{align}
%%Hence,
%%\begin{align}
%%[{D}_{\text{avg},P'}| \mathcal{I}]  \leq_{\text{st}} [{D}_{\text{avg},\pi}| \mathcal{I}],~\forall~\pi\in\Pi.\nonumber
%%\end{align}
%%
%%Because $G$ is independent of $P$, $P'$, and $\mathcal{I}$, by Theorem 1.A.3 (b) of \cite{StochasticOrderBook}, we have
%%\begin{align}
%%[{D}_{\text{avg},P'}| \mathcal{I}] +G  \leq_{\text{st}} [{D}_{\text{avg},\pi}| \mathcal{I}] + G,~\forall~\pi\in\Pi.\nonumber
%%\end{align}
%This, together with condition 3, implies %\eqref{eq_thm2}. Finally, 
%\eqref{eq_thm2_1}. % follows from \eqref{eq_thm2} and Eq (6.B.4) of \cite{StochasticOrderBook}.
\end{proof}
\ifreport
\begin{proof}[Proof of Corollary \ref{coro1}]
\else
\begin{proof}[of Corollary \ref{coro1}]
\fi
Corollary \ref{coro1} is proven by replacing ${D}_{\text{avg}}$ in the proof of Lemma \ref{lem1} with any $f\in\mathcal{D}_{\text{sym}}$.
\end{proof}


\ifreport
\begin{proof}[Proof of Lemma \ref{lem2}]
\else
\begin{proof}[of Lemma \ref{lem2}]
\fi

First, fix the sequence of task completion times such that $\bm{T}(P')=\bm{T}(\pi)=\bm{t}$ for all $\pi\in\Pi$. Using condition 2 and the sample-path optimality of the preemptive earliest due date (EDD) discipline \cite{Jackson55}, one can obtain that for all $\pi\in\Pi$ and $\bm{t}\geq\bm{0}$
\begin{align}
[L_{\max}(\bm{C}(P'))|\bm{T}(P')=\bm{t}] \leq[L_{\max}(\bm{C}(\pi))|\bm{T}(\pi)=\bm{t}].\nonumber
\end{align} 
In addition, one can show that $[L_{\max}(\bm{C}(P')) | \bm{T}(P')=\bm{t}]$ is increasing in $\bm{t}$. Hence,
\begin{align}\label{eq_lem2_order1}
[L_{\max}(\bm{C}(P'))|\bm{T}(P')=\bm{t}] \leq[L_{\max}(\bm{C}(\pi))|\bm{T}(\pi)=\bm{t}'],
\end{align} 
whenever $\bm{0}\leq\bm{t}\leq \bm{t}'$. On the other hand, condition 1 tells us that for all $\pi\in\Pi$ and $\mathcal{I}$
\begin{align}\label{eq_lem2_order2}
[\bm{T}(P')|\mathcal{I}] \leq_{\text{st}}[\bm{T}(\pi)|\mathcal{I}].
\end{align} 
Using \eqref{eq_lem2_order1}, \eqref{eq_lem2_order2}, Theorem 6.B.3, and Theorem 6.B.16(c) of \cite{StochasticOrderBook}, yields that for all $\pi\in\Pi$ and $\mathcal{I}$
\begin{align}\label{eq_lem2_order3}
[L_{\max}(\bm{C}(P'))|\mathcal{I}] \leq_{\text{st}}[L_{\max}(\bm{C}(\pi))|\mathcal{I}].
\end{align} 
Using condition 3, the fact that $L_{\max}$ is increasing, and Theorem 6.B.16(a) of \cite{StochasticOrderBook}, we can obtain 
\begin{align}\label{eq_lem2_order4}
[L_{\max}(\bm{U}(P))|\mathcal{I}]\leq_{\text{st}} [L_{\max}(\bm{C}(P'))|\mathcal{I}].
\end{align} 
Combining \eqref{eq_lem2_order3} and \eqref{eq_lem2_order4}, \eqref{eq_lem2_1} follows. If condition 3 is replaced by $P'=P$, then 
\eqref{eq_lem2_2} follows from \eqref{eq_lem2_order3}. This completes the proof.
\end{proof}
\ifreport
\begin{proof}[Proof of Corollary \ref{coro2}]
\else
\begin{proof}[of Corollary \ref{coro2}]
\fi
We need the rearrangement partial ordering $\leq^{\text{a}}$ defined in \cite[Sec. 6.F]{Marshall2011}: Consider two $n$-vector $\bm{x}$ and $\bm{y}$, $\bm{x}$ is said to \emph{immediately precede} $\bm{y}$ by one pairwise interchange, denote $\bm{x}<^{\text{p}}\bm{y}$, if for some index $i$, $1\leq i\leq n-1$,
\begin{align}
y_i<y_{i+1}, ~x_i= y_{i+1}, ~x_{i+1}=y_i, ~x_l= y_l,~l\neq i,i+1.\nonumber
\end{align}
Let $\leq^{\text{b}}$ denote the ordering of successive interchanges, such that $\bm{x}\leq^{\text{b}}\bm{y}$ if $\bm{x}=\bm{y}$ or if there exists a finite chain $\bm{z}^1,\ldots,\bm{z}^k$ of permutations such that
\begin{align}
\bm{x}<^{\text{p}}\bm{z}^1<^{\text{p}}\ldots<^{\text{p}}\bm{z}^k<^{\text{p}}\bm{y}.\nonumber
\end{align}
Suppose that $\bm{x}$ is a permutation of $\bm{u}$ and $\bm{y}$ is a permutation of $\bm{v}$ such that $\bm{x}_{\uparrow}=\bm{u}_{\uparrow}$ and $\bm{y}_{\uparrow}=\bm{v}_{\uparrow}$. Then, $(\bm{x},\bm{y})\leq^{\text{a}} (\bm{u},\bm{v})$ if there exists permutation matrices $W$ and $U$ such that
\begin{align}
\bm{x}W = \bm{u} U=\bm{x}_{\uparrow},~~~\text{and}~~ \bm{y} W \leq^{\text{b}} \bm{v} U.\nonumber
\end{align}
Hence, one can obtain
\begin{align}
(\bm{x}_{\uparrow},\bm{y}_{\downarrow})\leq^{\text{a}}(\bm{x},\bm{y})\leq^{\text{a}}(\bm{x}_{\uparrow},\bm{y}_{\uparrow}).\nonumber
\end{align}
The following rearrangement inequality is an immediate consequence of Theorem F.14 in Chapter 6 of \cite{Marshall2011}:
\begin{lemma}\label{lem_coro_2}
If \emph{$(\bm{x},\bm{y})\geq^{\text{a}} (\bm{u},\bm{v})$}, then
\begin{align}
\bm{x}-\bm{y}\prec \bm{u}-\bm{v}.\nonumber
\end{align}
\end{lemma}

Now, we are ready to prove Corollary \ref{coro2}. As before, we first fix the sequence of task completion times such that $\bm{T}(P')=\bm{T}(\pi)=\bm{t}$ for all $\pi\in\Pi$. Since $k_1=\ldots=k_n=1$, $\bm{C}(P')$ and $\bm{C}(\pi)$ are permutations of $\bm{t}$. According to condition 2 of Lemma \ref{lem2}, each completed job of policy $P'$ has the smallest due time $d_i$ among all unfinished jobs in the queue. Hence,
\begin{align}
[(\bm{C}(P'), \bm{d}) |\bm{T}(P')=\bm{t}] \geq^{\text{a}} [(\bm{C}(\pi), \bm{d}) |\bm{T}(\pi)=\bm{t}].\nonumber
\end{align}
Then, Lemma \ref{lem_coro_2} tells us that for all $\pi\in\Pi$
\begin{align}\label{eq_coro2_4}
&[\bm{L} (P') |\bm{T}(P')=\bm{t}]\nonumber\\
=&[\bm{C}(P') - \bm{d}|\bm{T}(P')=\bm{t}]\nonumber\\
\prec& [\bm{C}(\pi) - \bm{d}|\bm{T}(\pi)=\bm{t}] \nonumber\\
=&[\bm{L}(\pi)|\bm{T}(\pi)=\bm{t}]. 
\end{align} 
%it is easy to show that $t_{i}\leq {C}_{(i)}(\pi)$ for all $i=1,2,\ldots, n$ and $\pi\in\Pi$. Using condition 2 of Lemma \ref{lem2}, we can obtain that for all $\pi\in\Pi$
%\begin{align}\label{eq_coro2_1}
%[\bm{C}_{\uparrow}(P')|\bm{T}(P')=\bm{t}] = (t_1,t_{2},\ldots,t_{n}) \leq [\bm{C}_{\uparrow}(\pi)|\bm{T}(\pi)=\bm{t}].
%\end{align} 
%On the other hand, the rearrangement inequality \cite[Theorem F.14 of Sec. 6]{Marshall2011} implies that for all $\pi\in\Pi$
%\begin{align}\label{eq_coro2_2}
%\bm{C}_{\uparrow}(\pi) - \bm{d}_{\uparrow} \prec \bm{C}(\pi) - \bm{d}.
%\end{align} 
%In addition, condition 2 of Lemma \ref{lem2} tells us that the jobs are completed in the increasing order of $\bm{d}$. Hence, the job completed at time $C_{(i)}(P')$ has a due time $d_{(i)}$ for all $i=1,\ldots,n$. This implies
%\begin{align}\label{eq_coro2_3}
%\bm{L}_{\uparrow} (P')= \bm{C}_{\uparrow}(P') - \bm{d}_{\uparrow}.
%\end{align} 
%Combining \eqref{eq_coro2_1}-\eqref{eq_coro2_3}, yields for all $\pi\in\Pi$
%\begin{align}\label{eq_coro2_4}
%&[\bm{L}_{\uparrow} (P') |\bm{T}(P')=\bm{t}]\nonumber\\
%=&[\bm{C}_{\uparrow}(P') - \bm{d}_{\uparrow}|\bm{T}(P')=\bm{t}]\nonumber\\
%\leq&[\bm{C}_{\uparrow}(\pi)- \bm{d}_{\uparrow}|\bm{T}(\pi)=\bm{t}]\nonumber\\
%\prec& [\bm{C}(\pi) - \bm{d}|\bm{T}(\pi)=\bm{t}] \nonumber\\
%=&[\bm{L}(\pi)|\bm{T}(\pi)=\bm{t}]. 
%\end{align} 
For any $f\in\mathcal{D}_{\text{Sc}}$, define $g(\bm{x})=f(\bm{x}+\bm{d})$. Then, $g$ is Schur convex. For $\pi\in\Pi$, we can obtain
\begin{align}
&[f(\bm{C} (P')) |\bm{T}(P')=\bm{t}]\nonumber\\
=&[g(\bm{L} (P') ) |\bm{T}(P')=\bm{t}]\nonumber\\
\leq&[g(\bm{L} (\pi)) |\bm{T}(\pi)=\bm{t}]\nonumber\\
=&[f(\bm{C} (\pi)) |\bm{T}(\pi)=\bm{t}],\nonumber
\end{align}
where the inequality is due to \eqref{eq_coro2_4} and the definition of Schur convex functions. The remaining proof is the same as \eqref{eq_lem2_order1}-\eqref{eq_lem2_order4}, where we will need to use the fact that $f$ is increasing.
\end{proof}

%\begin{proof}[of Lemma \ref{thm1}]
%
%\end{proof}
%
%\begin{proof}[of Lemma \ref{thm3}]
%Let $[L_{\max,\pi} | \mathcal{I}, (t_{1,\pi},\ldots,t_{J,\pi}) = (t_1,$ $\ldots, t_J)]$ denote the maximum lateness of policy $\pi$ for given parameters $\mathcal{I}$ and task completion instants $(t_1,\ldots, t_J)$. According to the sample-path optimality of the preemptive Earliest Due Date (EDD) discipline \cite{Jackson55}, $[L_{\max,\pi} | \mathcal{I}, (t_{1,\pi},\ldots,$ $t_{J,\pi}) = (t_1,\ldots, t_J)]$ is minimized among all policies in $\Pi$, if each completed task belongs to the job with the earliest due date. By condition 2, policy $R$ satisfies this requirement, and hence
%\begin{align}
%&~~~[L_{\max,R} | \mathcal{I}, (t_{1,R},\ldots,t_{J,R}) = (t_1,\ldots, t_J)] \nonumber\\
%&\leq [L_{\max,\pi} | \mathcal{I}, (t_{1,\pi},\ldots,t_{J,\pi}) = (t_1,\ldots, t_J)],~\forall~\pi\in\Pi.\nonumber
%\end{align}
%%Further, $[L_{\max,\pi} | \mathcal{I}, (t_{1,\pi},\ldots,t_{J,\pi}) = (t_1,\ldots, t_J)]$ is an increasing function of $(t_1,\ldots, t_J)$, because if task completions are postponed, the job completions are also postponed. 
%The remaining proof steps are the same with Theorem \ref{thm1}.
%%Therefore, for all $\pi\in\Pi$, we have
%%\begin{align}\label{eq_order2}
%%&~~~~[L_{\max,R} | \mathcal{I}, (t_{1,R},\ldots,t_{J,R}) = (t_1,\ldots, t_J)] \nonumber\\
%%&\leq [L_{\max,\pi} | \mathcal{I}, (t_{1,\pi},\ldots,t_{J,\pi}) = (t_1',\ldots,t_J')],\nonumber\\
%%&~~~~~~~~~~~~~~~~~~~~\text{whenever}~(t_1,\ldots, t_J)\leq (t_1',\ldots,t_J').
%%\end{align}
%%Using condition 1, \eqref{eq_order2}, and the proof arguments of Theorem 6.B.3 of \cite{StochasticOrderBook}, we can obtain that  for all $\pi\in\Pi$
%%\begin{align}\label{eq_order3}
%%(L_{\max,R},t_{1,R},t_{2,R},\ldots) \leq_{\text{st}} (L_{\max,\pi}, t_{1,\pi},t_{2,\pi},\ldots).
%%\end{align}
%%Then, \eqref{eq_thm3} follows from \eqref{eq_order3} and Theorem 6.B.16 (c) of \cite{StochasticOrderBook}. Finally, \eqref{eq_thm3_1} follows from \eqref{eq_thm3} and Eq (6.B.4) of \cite{StochasticOrderBook}.
%\end{proof}



%\begin{proof}[of Lemma \ref{thm4}]
%The proof steps are the same with Theorem \ref{thm2}.
%\end{proof}

\ifreport
\begin{proof}[Proof of Lemma \ref{lem3}]
\else
\begin{proof}[of Lemma \ref{lem3}]
\fi
Using \eqref{eq_lem3_1} and $\bm{U}(\pi)\leq\bm{C}(\pi)$, we can obtain $[\bm{U}(P)|\mathcal{I}] \leq_{\text{st}} [\bm{C}(\pi)|\mathcal{I}]$ for all $\pi\in\Pi_{PL}$. By this, Theorem 6.B.4.(a) of \cite{StochasticOrderBook}, and the fact that $f$ is increasing, \eqref{eq_lem3_2} follows. This completes the proof.
\end{proof}

==> appendices_2.tex <==


\section{Proofs of Theorem~1 and Corollary 3} \label{app1}
\subsection{Proof of {\large \eqref{eq_delaygap1}} in Theorem \ref{thm1}} \label{sec_app_thm1_1}
We prove \eqref{eq_delaygap1} by using the sufficient conditions in Lemma \ref{lem1} and Corollary \ref{coro1}. The proof steps are as follows:

{\bf Construction of Policy $P'$:}
We construct an {infeasible} policy $P'$. \emph{First, in policy $P'$, all servers are busy whenever the queue is not empty.} If the number of tasks is less than $m$, some tasks are replicated over multiple servers. 
\emph{Second, the task completion times of policy $P'$ are constructed as if there is no task cancellations.} Suppose that at any time $t$, server $l$ has processed a task for $\tau$ seconds, and another copy of this task is completed at time $t$ on another server. In policy $P'$, server $l$ will cancel this task and process a new task. More specifically, in policy $P'$, server $l$ will not process the new task from scratch; instead, it is assumed that the new task assigned to server $l$ has already been processed for $\tau$ seconds by time $t$ (which is infeasible),~and server $l$ will serve the task from this progress point. If two task copies are completed at the same time on two servers, they are assumed to be distinct tasks, instead of two replicated copy of the same task. 
\emph{Finally, the completed tasks of policy $P'$ are relabelled such that each completed task is from the job with the fewest remaining tasks}. (This relabeling operation might be infeasible, because the tasks from different jobs may be simultaneously processed on parallel servers.) 
By this, policy $P'$ is constructed.


%\emph{In policy $P'$, all servers are working whenever the queue is not empty, and task cancellations do not affect the task completion times in policy $P'$.} More specifically, if the number of remaining tasks is larger than 0 and less than the number of servers $m$, some of the tasks are replicated over multiple servers to make sure that all servers are working. 

%In both policy $P'$ and FUT-NR, all servers are busy whenever the queue is not empty. 
%
%Suppose that at any time $t$, server $l$ has processed a task for $\tau$ seconds, and another copy of this task is completed at time $t$ on another server. In FUT-NR, after canceling the task with some delay overhead, server $l$ will process a new task that have not been served. 
%%In policy $P'$, task cancellations are implemented for two cases: If server $l$ is an NWU server, server $l$ will process a new task that have not been served (the same as FUT-NR). If server $l$ is an NBU server, 
%In policy $P'$, server $l$ will not process a new task from scratch; instead, it is assumed that at time $t$, the next task assigned to server $l$ is already processed for $\tau$ seconds by a genie (which is infeasible!) and server $l$ will serve the task from this progress point. Therefore, in policy $P'$, the task completion times of NBU servers are constructed as if there is no task cancellations. Finally, the completed tasks in policy $P'$ are relabelled such that each completed task is from the job with the fewest remaining tasks (which is also infeasible, because the tasks from different jobs are processed simultaneously). Note that both policy $P'$ and FUT-NR are work-conserving.

Next, we prove the conditions of Lemma \ref{lem1} one by one.

\textbf{Condition 1:} \emph{Policy $P'$ is more {work-efficient} than any policy $\pi\in\Pi$}. 
%Recall that $\bm{T}(\pi)=(T_1(\pi),\ldots, T_{k_{\text{sum}}}(\pi))$ is the sequence of task completion times of the system. 
\ifreport
\begin{proof}[Proof of Condition 1]
\else
\begin{proof}[of Condition 1]
\fi
We prove condition 1 by induction. Consider the first task completion time $T_1(\pi)$. Job 1 arrives at time $a_1=0$. 
If policy $\pi$ is non-preemptive and work-conserving, then
\begin{align}
[T_1(\pi)|\mathcal{I}]=\min_{l=1,\ldots,m} X_l.\nonumber
\end{align} 
If policy $\pi$ is preemptive and work-conserving, then some  servers may cancel the current task and switch to process a new task at time $t\in[0,T_1(\pi))$, then Lemma \ref{lem_property_MNBUMNWU} tells us that
\begin{align}\label{eq_condition1_2_1}
\min_{l=1,\ldots,m} X_l \leq_{\text{st}}[T_1(\pi)|\mathcal{I}].
\end{align}
If policy $\pi$ is non-work-conserving, then \eqref{eq_condition1_2_1} still holds, because of the possibility of server idleness. Since policy $P'$ is non-preemptive and work-conserving, we can obtain that for all $\pi\in\Pi$
\begin{align}\label{eq_condition1_2}
[T_1(P')|\mathcal{I}]=\min_{l=1,\ldots,m} X_l\leq_{\text{st}}[T_1(\pi)|\mathcal{I}].
\end{align} 



Next, consider the update from $T_j(\pi)$ to $T_{j+1}(\pi)$. Recall that $s_j$ is the $j$-th task arrival time of the system. If $s_{j+1}>T_j(\pi)$, the first $j$ tasks are completed before the $(j+1)$-th task arrives, hence all servers are idle during $[T_j(\pi),s_{j+1})$; otherwise, if $s_{j+1}\leq T_j(\pi)$, the servers can keep working after $T_j(\pi)$. For any work-conserving policy $\pi$, we can obtain
\begin{eqnarray}\label{eq_thm1_2}
T_{j+1}(\pi)\!=\max\{s_{j+1},T_j(\pi)\} + \!\min_{l=1,\ldots,m} R_{j,l}(\pi),
\end{eqnarray}
where $R_{j,l}(\pi)$ is the time duration for server $l$ to complete a task after time $\max\{s_{j+1},T_j(\pi)\}$. 



Suppose that $s_{j+1}\leq T_j(\pi)$ and server $l$ has spent $\tau_l$ ($\tau_l\geq0$) seconds on a task by time $T_j(\pi)$. 
In policy $P'$,  the task completion times are constructed as if there is no task cancellations. Hence, the tail probability for the servers to complete a task after time $T_j(P')$ is 
\begin{align}\label{eq_thm1_7}
&\Pr\Big[\min_{l=1,\ldots,m} R_{j,l}(P')>t\Big]\nonumber\\
=& \Pr\Big[\min_{l=1,\ldots,m}(X_l-\tau_l)>t\Big|\bm{X}> \bm{\tau} \Big].
\end{align}
If $\pi$ is a non-preemptive work-conserving policy, some servers may cancel the tasks they are processing  at time $T_j(\pi)$. If the servers in $\mathcal{S}^c$ cancel the current task and switch to process a new task at time $T_j(\pi)$, then the tail probability for the servers to complete a task after time $T_j(\pi)$ is 
\begin{align}\label{eq_thm1_8}
&\Pr\Big[\min_{l=1,\ldots,m} R_{j,l}(\pi)>t\Big]\nonumber\\
=&\Pr\!\Big[\min\Big\{\min_{l\in\mathcal{S}}(X_l-\tau_l),\min_{l\in\mathcal{S}^c}X_l\Big\}\!>t \Big| \bm{X}_{\mathcal{S}}> \bm{\tau}_{\mathcal{S}}\Big].
\end{align} 
Combining \eqref{eq_thm1_7}, \eqref{eq_thm1_8}, and Lemma \ref{lem_property_MNBUMNWU}, yields 
\begin{align}\label{eq_min}
\min_{l=1,\ldots,m} R_{j,l}(P') \leq_{\text{st}} \min_{l=1,\ldots,m} R_{j,l}(\pi).
\end{align}
If $\pi$ is a preemptive work-conserving policy, then some servers may cancel the current task and switch to process a new task at a particular time $t\in[T_j(\pi),T_{j+1}(\pi))$.
In this case, we can use Lemma \ref{lem_property_MNBUMNWU} to show that \eqref{eq_min} holds. Hence, \eqref{eq_min} holds for all work-conserving policy $\pi$. 

Suppose that $s_{j+1}> T_j(\pi)$, then the servers start to process new tasks at time $s_{j+1}$. In this case, we can show that
\eqref{eq_min} also holds for all work-conserving policy $\pi$. 

Using \eqref{eq_thm1_2}, \eqref{eq_min}, and the fact that $s_j$ is uniquely determined by $\mathcal{I}$, it follows that for all work-conserving policy $\pi$
\begin{align}\label{eq_thm1_4}
[T_{j+1}(P') | \mathcal{I},  T_j(P') = t_j] \leq_{\text{st}} [T_{j+1}(\pi) | \mathcal{I},  T_j(\pi) = t_j'] \nonumber\\
\text{whenever}~ t_j \leq t_j',j=1,2,\ldots
\end{align}
If policy $\pi$ is non-work-conserving, \eqref{eq_thm1_2} becomes
\begin{eqnarray}\label{eq_thm1_2_1}
T_{j+1}(\pi)\!\geq\max\{s_{j+1},T_j(\pi)\} + \!\min_{l=1,\ldots,m} R_{j,l}(\pi),\nonumber
\end{eqnarray}
because of the possibility of server idleness. In this case, \eqref{eq_thm1_4} still holds. Hence, \eqref{eq_thm1_4} holds for all $\pi\in\Pi$.
Then, combining \eqref{eq_condition1_2}, \eqref{eq_thm1_4}, and Theorem 6.B.3 of \cite{StochasticOrderBook}, yields
\begin{align}%\label{eq_thm1_5}
[(T_1(P'),\ldots,T_j(P'))|\mathcal{I}] \leq_{\text{st}} [(T_1(\pi),\ldots,T_j(\pi))|\mathcal{I}],~\forall~\pi\in\Pi.\nonumber
\end{align}
Hence, condition 1 is proven.
\end{proof}

\textbf{Condition 2:} \emph{Each completed task of policy $P'$ belongs to the job with the fewest remaining tasks}. Condition 2 directly follows from the construction of policy $P'$.

\textbf{Condition 3:} \emph{It holds that} 
%\begin{align}
%\mathbb{E}\left[{D}_{\text{avg,FUT-NR}}\right]\leq \mathbb{E}\left[{D}_{\text{avg}}(P')| \mathcal{I}\right] \nonumber\\
%+\frac{1}{N}\sum_{h=1}^N \max_{\substack{S: |S|\leq k_i\\
%S\subseteq\{1,\ldots,m\}}}\!\!\mathbb{E}\left[\max_{l\in S} X_l\right].
%\end{align}
\begin{align}\label{eq_condition3}
[\bm{U}_{\uparrow}(\text{FUT-NR})|\mathcal{I}] \leq_{\text{st}} [\bm{C}_{\uparrow}(P')|\mathcal{I}].
\end{align}
We prove condition 3 by a \emph{sample-path ordering} technique, which is motivated by the second proof of the  optimality of SRPT in single-server queueing systems \cite{Smith78}. The generalization from \cite{Smith78} to this {sample-path ordering} technique is non-trivial and unexpected when this research started.


%It is difficult to compare policies $P'$ and FUT-NR directly.~Hence, we will construct an intermediate policy called
%Fewest Positive Unassigned Tasks first with Virtual Tasks (FUT-VT), and prove the following results:
%\begin{align}\label{eq_condition3_1}
%&[{D}_{\text{avg,FUT-NR}}|\mathcal{I}]  \leq_{\text{st}} [{D}_{\text{avg,FUT-VT}}| \mathcal{I}],\\
%&[{D}_{\text{avg,FUT-VT}}|\mathcal{I}]  \leq_{\text{st}} [{D}_{\text{avg}}(P')| \mathcal{I}] + G.\label{eq_condition3_2}
%\end{align}
%Then, \eqref{eq_condition3} follows from \eqref{eq_condition3_1} and \eqref{eq_condition3_2}. 
%
%First, we construct the sample path of policy FUT-VT. In FUT-VT, there are always $m$ virtual tasks in the system, each belongs to a virtual job. Because of these $m$ virtual tasks, the total number of remaining tasks is always no smaller than $m$. Hence, there is no task replications in FUT-VT. In the meanwhile, the task completion times of policy $P'$ are constructed as if there is no task cancellations. Therefore, the task completion sample paths of policies $P'$ and FUT-VT can be aligned (see Fig. \ref{fig_compare} for an illustration): Consider a busy period $[\tau,\nu)$ of policy $P'$. If all $m$ servers start to process new tasks at time $\tau$ in both policies $P'$ and FUT-VT, the task completion times of the two policies are exact the same during the period $[\tau,\nu)$. At time $\nu$, the queue of policy $P'$ is empty, and hence all severs becomes empty.  
%
%An illustration of FUT-NR, FUT-VT, and the lower bound policy $P'$ is provided in .
%
% policy $P'$
%
%On the other hand, there is no virtual task in FUT-NR and hence the servers can spend time to process replicated task copies, instead of wasting time on virtual tasks. By this, \eqref{eq_condition3_1} follows. 
%
%Next, we compare policies $P'$ and FUT-VT. Consider the completion times $(T_1(\pi),\ldots,T_j(\pi))$ of the first $J$ tasks in policies $P'$ and FUT-VT. Note that virtual tasks are completed in FUT-VT, which is not counted in job completion time. We will show that 
%\begin{align}
%[(t_{1,\text{FUT-VT}},\ldots,t_{J,\text{FUT-VT}})|\mathcal{I}] \leq_{\text{st}} [(T_1(P'),\ldots,T_j(P'))|\mathcal{I}].
%\end{align}


First, we define the system states of policies $P'$ and FUT-NR. 
\begin{definition}\label{def_state_P}
The system state of  policy $P'$ is specified by an infinite vector $\bm{\beta}=(\beta_1,\beta_2,\ldots)$ with non-negative, non-increasing components. At any time, the coordinates of $\bm{\beta}$ are interpreted as follows: $\beta_1$ is the maximum number of remaining tasks among all jobs in the queue, $\beta_2$ is the next greatest number of remaining tasks among all jobs in the queue, and so on, with duplications being explicitly repeated. If there are $l$ unfinished jobs in the system, then it holds that
\begin{eqnarray}
\beta_1\geq\beta_2\geq\ldots\geq\beta_l>0 = \beta_{l+1} =\beta_{l+2}=\ldots.\nonumber
\end{eqnarray}
\end{definition}

\begin{definition}\label{def_state}
The system state of FUT-NR is specified by a pair of infinite vectors $\bm{\alpha}=(\alpha_1,\alpha_2,\ldots)$ and $\bm{\delta}=(\delta_1,\delta_2,$ $\ldots)$ with non-negative components. At any time, the coordinates of $\bm{\alpha}$ and $\bm{\delta}$ are interpreted as follows: $\alpha_h$ is the number of unfinished tasks of the job associated to the $h$-th coordinate, and $\delta_h$ out of these $\alpha_h$ tasks are being processed on some servers. Hence, 
\begin{align}\label{eq_def_state}
\delta_h \leq \alpha_h\leq k_{\max},~\sum_{h=1}^\infty \delta_h\leq m. 
\end{align}
The coordinates of $\bm{\alpha}$ and $\bm{\delta}$ are sorted in the non-increasing order of $\alpha_h-\delta_h$, with duplications being explicitly repeated. 
%When $\alpha_h-\delta_h=\alpha_{i+1}-\delta_{i+1}$, the coordinates are sorted such that $\alpha_h\geq \alpha_{i+1}$. 
If there are $l$ unfinished jobs in the system, then there exists an integer $r$ ($0\leq r\leq l$) such that 
\begin{eqnarray}
&&\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\alpha_1-\delta_1\geq\ldots\geq \alpha_{r}-\delta_{r}>0= \alpha_{r+1}-\delta_{r+1}=\ldots,\\
&&\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\alpha_h \left\{\begin{array}{l l} >0, &\text{if}~ h\leq l;\\
  =0, &\text{if}~ h\geq l+1,\end{array}\right.~~\delta_h \left\{\begin{array}{l l} \geq0, &\text{if}~ h\leq l;\\
  =0, &\text{if}~ h\geq l+1.\end{array}\right.
  \end{eqnarray}
\end{definition}

Let $\{\bm{\beta}(t),t\geq0\}$ be the state process of policy $P'$ and $\{\bm{\alpha}(t),\bm{\delta}(t),t\geq0\}$ be the state process of FUT-NR, which are assumed to be right-continuous. One key result of the sample-path ordering technique is the following lemma:



\begin{lemma}\label{lemG4}
Suppose that $\bm{\alpha}(0^-) = \bm{\delta}(0^-)=\bm{\beta}(0^-)=\bm{0}$ and the job parameters $\mathcal{I}$ are given. For any sample path of policy $P'$, there exists a sample path of FUT-NR with the same probability density such that
\begin{eqnarray}\label{eq_lemG4}
\sum_{h=j}^\infty [\alpha_h(t)- \delta_h(t)]\leq \sum_{h=j}^\infty \beta_h(t)
\end{eqnarray}
holds for all $t\geq0$ and j = $1,2,\ldots$
\end{lemma}

The following lemmas are needed to prove Lemma \ref{lemG4}:

\begin{lemma}\label{lem_non_prmp1}
Suppose that, under policy FUT-NR, $\{\bm{\alpha}',\bm{\delta}'\}$ is obtained by completing a task on one server in the system whose state is $\{\bm{\alpha},\bm{\delta}\}$. Further, suppose that, under policy $P'$, $\bm{\beta}'$ is obtained by completing a task on one server in the system whose state is $\bm{\beta}$.
If
\begin{eqnarray}\label{eq_non_prmp_41}
\sum_{h=j}^\infty [\alpha_h - \delta_h]\leq \sum_{h=j}^\infty \beta_h, ~\forall~j=1,2,\ldots,\nonumber
\end{eqnarray}
then
\begin{eqnarray}\label{eq_non_prmp_40}
\sum_{h=j}^\infty [\alpha'_h - \delta'_h]\leq \sum_{h=j}^\infty \beta'_h, ~\forall~j=1,2,\ldots
\end{eqnarray}
\end{lemma}

\begin{proof}
The proof is similar to that of Lemma 2 in \cite{Smith78}.
If $\sum_{h=j}^\infty [\alpha'_h - \delta'_h]=0$, then the inequality \eqref{eq_non_prmp_40} follows naturally. 
If $\sum_{h=j}^\infty [\alpha'_h - \delta'_h]>0$, then there exist some tasks that have not been assigned to any server. 
In FUT-NR, a server that has just completed a task will be allocated to process an unassigned task from the job with the minimum positive $\alpha'_h - \delta'_h$. Hence,
$\sum_{h=j}^\infty [\alpha'_h - \delta'_h]=\sum_{h=j}^\infty [\alpha_h - \delta_h] - 1 \leq \sum_{h=j}^\infty \beta_h -1 \leq \sum_{h=j}^\infty \beta'_h$.
\end{proof}


\begin{lemma}\label{lem_non_prmp2}
Suppose that, under policy FUT-NR, $\{\bm{\alpha}',\bm{\delta}'\}$ is obtained by adding a job with $b$ tasks to the system whose state is $\{\bm{\alpha},\bm{\delta}\}$. Further, suppose that, under policy $P'$, $\bm{\beta}'$ is obtained by adding a job with $b$ tasks to the system whose state is $\bm{\beta}$.
If
\begin{eqnarray}
\sum_{h=j}^\infty [\alpha_h - \delta_h]\leq \sum_{h=j}^\infty \beta_h, ~\forall~j=1,2,\ldots,\nonumber
\end{eqnarray}
then
\begin{eqnarray}
\sum_{h=j}^\infty [\alpha'_h - \delta'_h]\leq \sum_{h=j}^\infty \beta'_h, ~\forall~j=1,2,\ldots\nonumber
\end{eqnarray}
\end{lemma}

\begin{proof}
The proof is similar to that of Lemma 3 in \cite{Smith78}.
Without loss of generalization, we suppose that after the job arrival, $b$ is the $l$-th coordinate of $\bm{\alpha}'$ and the $m$-th coordinate of $\bm{\beta}'$. Hence, $\alpha'_l = \beta'_m= b$. Because no server completes a task at this time instant, $\delta'_l =0$. We consider the following four cases:

{Case 1}: $l<j, m<j$. We can obtain $\sum_{h=j}^\infty [\alpha'_h - \delta'_h] = \sum_{h=j-1}^\infty [\alpha_h - \delta_h] \leq \sum_{h=j-1}^\infty \beta_h= \sum_{h=j}^\infty \beta_h'$.

{Case 2}: $l<j, m\geq j$. We have $\sum_{h=j}^\infty [\alpha'_h - \delta'_h] =\sum_{h=j-1}^\infty $ $[\alpha_h - \delta_h] \leq b + \sum_{h=j}^\infty [\alpha_h - \delta_h] \leq b + \sum_{h=j}^\infty \beta_h = \sum_{h=j}^\infty \beta_h'$.

{Case 3}: $l\geq j, m<j$. We have $\sum_{h=j}^\infty [\alpha'_h - \delta'_h] = b + \sum_{h=j}^\infty [\alpha_h - \delta_h] \leq \sum_{h=j-1}^\infty [\alpha_h - \delta_h] \leq \sum_{h=j-1}^\infty \beta_h = \sum_{h=j}^\infty \beta_h'$.

{Case 4}: $l\geq j, m\geq j$. We have $\sum_{h=j}^\infty [\alpha'_h - \delta'_h] = b + \sum_{h=j}^\infty [\alpha_h - \delta_h] \leq b + \sum_{h=j}^\infty \beta_h = \sum_{h=j}^\infty \beta_h'$.
\end{proof}


\ifreport
\begin{proof}[Proof of Lemma \ref{lemG4}]
\else
\begin{proof}[of Lemma \ref{lemG4}]
\fi
Consider any busy period $[\tau,\nu)$ of policy $P'$. Then, in policy $P'$, all servers are busy during $[\tau,\nu)$, and are idle at time $\tau^-$ and time $\nu$. We prove \eqref{eq_lemG4} for $t\in[\tau,\nu)$ by considering two cases:

\emph{Case 1: At time $t=\tau^-$, policy FUT-NR has $m$ tasks and the service of these tasks has just started.} Consider the system states of both policies at time $\tau^-$. The system state of policy FUT-NR satisfies 
\begin{align}\label{proof_lemG4_1}
\sum_{h=1}^\infty \alpha_h(\tau^-)= m, ~\bm{\alpha}(\tau^-)=\bm{\delta}(\tau^-).
\end{align}
In policy $P'$, there is no task in the system at time $\tau^-$ such that 
\begin{align}\label{proof_lemG4_5}
\bm{\beta}(\tau^-)=\bm{0}. 
\end{align}
Consider the evolutions of both policies during $[\tau,\nu)$. 
In policy $P'$, all servers are busy if there is at least one task. On the other hand, in policy FUT-NR, there is no task replication. Hence, all servers are busy if there are no less than $m$ tasks. Because the servers become busy in policy $P'$ at time $\tau$, a job must has arrived. By \eqref{proof_lemG4_1} and \eqref{proof_lemG4_5}, it holds that for $t=\tau$
%^there are no less than $m$ tasks in policy FUT-NR at time $\tau^-$.
\begin{align}\label{proof_lemG4_4}
\sum_{h=1}^\infty \alpha_h(t)= \sum_{h=1}^\infty \beta_h(t) +m\geq m+1.
\end{align}
Therefore,  the servers are all busy in policy $P'$ and policy FUT-NR at time $\tau$. Hence, for any sample path of policy $P'$, there is a sample path of policy FUT-NR such that for sufficiently small $\Delta t$ the task arrival times and task completion times of the two policies are exactly the same during $[\tau,\tau+\Delta t)$, and \eqref{proof_lemG4_4} holds during $[\tau,\tau+\Delta t)$. By induction over time, we can show that for any sample path of policy $P'$, there is a sample path of policy FUT-NR with the same probability density such that the task arrival times and task completion times of the two policies are exactly the same  during $[\tau,\nu)$, and \eqref{proof_lemG4_4} holds for all $t\in[\tau,\nu)$. Using Lemma \ref{lem_non_prmp1}, Lemma \ref{lem_non_prmp2}, and the initial states at time $\tau^-$, we can prove that \eqref{eq_lemG4} holds for all $t\in[\tau,\nu)$ on these two sample paths.

%In general, suppose that at some time $t\in[\tau,\nu)$
%\begin{align}
%\sum_{h=1}^\infty \alpha_h(t)= \sum_{h=1}^\infty \beta_h(t) +m\geq m+1.\nonumber
%\end{align}
%Then, the scheduling decisions of policies $P'$ and policy FUT-NR are the same at time $t$. This further implies that for any sample path of policy $P'$, we can construct a sample path of policy FUT-NR such that 
%\begin{align}
%\sum_{h=1}^\infty \alpha_h(t^+)= \sum_{h=1}^\infty \beta_h(t^+) +m\geq m+1.\nonumber
%\end{align}
%Therefore, 
%
%Using Lemma \ref{lem_non_prmp1} and Lemma \ref{lem_non_prmp2}, and we can prove that 
%\begin{align}
%\sum_{h=1}^\infty \alpha_h(t^+)= \sum_{h=1}^\infty \beta_h(t^+) +m.\nonumber
%\end{align}
%
%For any sample path of policy $P'$ during $[\tau,\nu)$, we can construct a sample path of policy FUT-NR during $[\tau,\nu)$ with the same probability density such that the task arrival times and task completion times of the two policies are exactly the same. In particular, if 
%
%
%if policy $P'$ has $b$ tasks at time $t\in[\tau,\nu)$, policy FUT-NR has $m+b$ tasks at time $t$. Hence, the scheduling decisions of policies $P'$ and policy FUT-NR are the same at time $t$. Therefore, we can obtain
%\begin{align}
%\sum_{h=1}^\infty \alpha_h(t)= \sum_{h=1}^\infty \beta_h(t) +m,~\forall~t\in [\tau,\nu).\nonumber
%\end{align}
%Because the task arrivals and departures of policies $P'$ and FUT-NR are aligned during $[\tau,\nu)$, using Lemma \ref{lem_non_prmp1}, Lemma \ref{lem_non_prmp2}, and the initial states at time $\tau^-$, we can prove by induction that \eqref{eq_lemG4} holds for $t\in[\tau,\nu)$.

\emph{Case 2: At time $t=\tau^-$, policy FUT-NR has less than $m$ tasks or the service of these tasks started before time $\tau^-$}. In both \emph{Case 1} and \emph{Case 2}, the sample path evolutions of policy $P'$ are the same. On the other hand, in policy FUT-NR, the tasks are completed earlier in \emph{Case 2} than in \emph{Case 1}. Therefore, \eqref{eq_lemG4} also holds in \emph{Case 2} for $t\in[\tau,\nu)$.

%Note that the case that policy FUT-NR has more than $m$ tasks at time $\tau^-$ will not happen. This will be clear 
Let $[\tau_1,\nu_1)$ be the next busy period of policy $P'$ with $\nu<\tau_1$. Then, $[\nu,\tau_1)$ is an idle period of policy $P'$. We prove \eqref{eq_lemG4} during the idle period $[\nu,\tau_1)$. 
Because all servers are idle during $[\nu,\tau_1)$ in policy $P'$, it follows that 
\begin{align}\label{proof_lemG4_2}
\bm{\beta}(t)=\bm{0},~t\in[\nu,\tau_1).
\end{align}
Hence, there is no task arrival during $[\nu,\tau_1)$; otherwise, \eqref{proof_lemG4_2} cannot be true.
On the other hand, at time $\nu$ there are no more than $m$ tasks in policy FUT-NR such that 
\begin{align}
\bm{\alpha}(\nu)=\bm{\delta}(\nu).\nonumber
\end{align}
Because there is no task arrival during $[\nu,\tau_1)$, policy FUT-NR satisfies
\begin{align}\label{proof_lemG4_3}
\bm{\alpha}(t)=\bm{\delta}(t),~t\in[\nu,\tau_1).
\end{align}
By \eqref{proof_lemG4_2} and \eqref{proof_lemG4_3}, \eqref{eq_lemG4} holds during $[\nu,\tau_1)$.
Further, from \eqref{proof_lemG4_3}, we can obtain
\begin{align}
\sum_{h=1}^\infty \alpha_h(\tau_1^-)=\sum_{h=1}^\infty \delta(\tau_1^-)\leq m,
\end{align}
such that there are no more than $m$ tasks at time $t=\tau_1^-$ in policy FUT-NR. Hence, either \emph{Case 1} or \emph{Case 2} is satisfied at time $t=\tau_1^-$. Then, we can use the above arguments to prove that  \eqref{eq_lemG4} holds during the next busy period $[\tau_1,\nu_1)$ of policy $P'$.


Finally, by taking an induction over the busy and idle periods of policy $P'$,  Lemma \ref{lemG4} is proven.
%Let $[\nu,\tau_1)$ and $[\tau_1,\nu_1)$ be the next idle and busy periods of policy $P'$, respectively. Because policy $P'$ is work-conserving, all $m$ servers are idle in policy $P'$ during $[\nu,\tau_1)$. Hence, there is no job arrival during $[\nu,\tau_1)$. At time $\nu$, we have
%\begin{align}
%\sum_{h=j}^\infty [\alpha_h(\nu)- \delta_h(\nu)]\leq 0.\nonumber
%\end{align}
%This and $\alpha_h(\nu)\geq\delta_h(\nu)$ imply that $\alpha_h(\nu)=\delta_h(\nu)$ for all $h=1,2,\ldots$ Since no job arrives during $[\nu,\tau_1)$, we can obtain that $\alpha_h(t)=\delta_h(t)$ for all $t\in[\nu,\tau_1)$ and $h=1,2,\ldots$ Hence, \eqref{eq_lemG4} holds during $[\nu,\tau_1)$. 
%
%Because there is no job arrival during $[\nu,\tau_1)$, there are no more than $m$ remaining tasks in FUT-NR at time $\tau_1$ and each remaining task has been processed by a certain amount of time. Similar with the case of $[\tau,\nu)$, we can prove that \eqref{eq_lemG4} holds in the busy period $[\tau_1,\nu_1)$.
%By taking an induction over the busy and idle periods of policy $P'$, Lemma \ref{lemG4} follows.
\end{proof}

\ifreport
\begin{proof}[Proof of Condition 3]
\else
\begin{proof}[of Condition 3]
\fi
%Let the evolution of the system state under some scheduling policy be on a space $(\Omega,\mathcal{F},P)$. Each $\omega\in\Omega$ corresponds to a sample path of policy $P'$ and a sample path of policy FUT-NR. The job arrival parameters $\mathcal{I}$ is fixed for all $\omega\in\Omega$. 
%Let $(C_{(1)}(P'),\ldots,c_{N:N}(P'))$ be a permute of the job completion time sequence $(c_{1}(P'),\ldots,c_{N}(P'))$ in the increasing order, such that $c_{i:N}(P')\leq c_{i+1:N}(P')$. 

%Pick any $\omega\in\Omega$ and consider the first job completion time $C_{(1)}(P')$ of policy $P'$. Suppose that there are $y$ job arrivals during $[0,C_{(1)}(P'))$. 

We will prove Condition 3 by induction. Consider the sample paths of policy $P'$ and policy FUT-NR satisfying Lemma \ref{lemG4}. We first show that there exists a job $w_1$ such that
\begin{align}\label{eq_Condition_3_1}
U_{w_1}(\text{FUT-NR}) \leq C_{(1)}(P').
\end{align}

In policy $P'$, the first job departure occurs at time $t=C_{(1)}(P')$. Suppose that $y_1$ jobs have arrived during $[0,C_{(1)}(P'))$. Then, there are $y_1-1$ unfinished jobs at time $C_{(1)}(P')$ in policy $P'$. Hence, the system state of policy $P'$ satisfies 
\begin{align}\label{eq_proof_0}
\sum_{h=y_1}^\infty\beta_h(C_{(1)}(P'))=0.
\end{align}
This and Lemma \ref{lemG4} imply
%Hence, there are $y-1$ unfinished jobs at time $C_{(1)}(P')$ such that
%Invoking Lemma \ref{lemG4}, we can obtain
\begin{align}\label{eq_proof_1}
\sum_{h=y_1}^\infty \alpha_h(C_{(1)}(P'))\leq \sum_{h=y_1}^\infty  \delta_h(C_{(1)}(P')).
\end{align}
In policy FUT-NR, there are at most $y_1$ jobs at time $C_{(1)}(P')$. Hence, the system state of policy FUT-NR must satisfy
\begin{align}\label{eq_proof_2}
\!\!\alpha_h(C_{(1)}(P'))= \delta_h(C_{(1)}(P'))=0,\forall~h=y_1\!+\!1,y_1\!+\!2,\ldots \!\!
\end{align}
Combining \eqref{eq_proof_1}, \eqref{eq_proof_2}, and the fact that $\alpha_h(t)\geq\delta_h(t)$ for all $h$ and $t$, we can obtain
%Combining \eqref{eq_proof_0}, \eqref{eq_proof_1}, and the fact that $\alpha_h(t)\geq\delta_h(t)$ for all $i,t$, yields
\begin{align}\label{eq_proof_3}
\alpha_{y_1}(C_{(1)}(P'))=\delta_{y_1}(C_{(1)}(P')).
\end{align}
Let $w_1$ be the index of the job associated to the $y_1$-th coordinate of $\bm{\alpha}(t)$ at time $t= C_{(1)}(P')$. Then, \eqref{eq_proof_3} tells us that in FUT-NR, all tasks of job $w_1$ are either completed or under service at time $C_{(1)}(P')$. Hence, \eqref{eq_Condition_3_1} is proven.
%\begin{align}%\label{eq_proof_9}
%U_{w_1}(\text{FUT-NR}) \leq C_{(1)}(P'),\nonumber
%\end{align}
%which implies \eqref{eq_Condition_3_1}.

Next, we prove the induction step. Suppose that there exist $j$ jobs indexed by $w_1,w_2,\ldots,w_j$ such that
\begin{align}
U_{w_i}(\text{FUT-NR}) \leq C_{(i)}(P'),~i=1,\ldots,j,\nonumber
\end{align}
we will show that there exist another job $w_{j+1}$ such that
\begin{align}\label{eq_proof_9}
U_{w_{j+1}}(\text{FUT-NR}) \leq C_{(j+1)}(P').
\end{align}
%Since preemption is not allowed, these $\delta_y(C_{(1)}(P'))$ tasks will be under service in policy FUT-NR until completion. Let $w_1$ be the index of the job associated to the coordinate $y$ at time $C_{(1)}(P')$. According to \eqref{eq_def_state}, we can obtain $\delta_y(C_{(1)}(P'))\leq \min[k_{w_1},M].$ Therefore, the time duration between $C_{(1)}(P')$ and $c_{w_1,\text{FUT-NR}}$ is no more than the time to complete $\min[k_{w_1},M]$ tasks of job $w_1$.
Assume that $y_{j+1}$ jobs have arrived during $[0,C_{(j+1)}(P'))$, which must satisfy $y_{j+1}\geq j+1$. Then, 
there are $(y_{j+1}-j-1)$ unfinished jobs at time $C_{(j+1)}(P')$ in policy $P'$. According to \emph{Definition \ref{def_state_P}}, the system state of policy $P'$ satisfies 
\begin{align}
\sum_{h=y_{j+1}-j}^\infty\beta_h(C_{(j+1)}(P'))=0.\nonumber
\end{align}
Then, by following the arguments of \eqref{eq_proof_1}-\eqref{eq_proof_3}, we can obtain that at time $t=C_{(j+1)}(P')$ the system state of policy FUT-NR satisfies
\begin{align}\label{eq_proof_4}
\alpha_{h}(C_{(j+1)}(P'))=\delta_{h}(C_{(j+1)}(P')),~h=y_{j+1}-j,\ldots,y_{j+1}.
\end{align}
There are $j+1$ jobs satisfying \eqref{eq_proof_4}. At least one of these $j+1$ jobs is different from the jobs $w_1,w_2,\ldots,w_j$. Let $w_{j+1}$ be the index of this job. Then, \eqref{eq_proof_4} tells us that in FUT-NR, all tasks of job $w_{j+1}$ are either completed or under service at time $t=C_{(j+1)}(P')$. Hence, \eqref{eq_proof_9} is proven.

By induction, we can obtain
\begin{align}\label{eq_proof_10}
U_{w_{j}}(\text{FUT-NR}) \leq C_{(j)}(P'),~j=1,\ldots,n.
\end{align}
Because $U_{(j)}(\pi)$ is the $j$-th smallest components of $\bm{U}(\pi)$, it follows that
\begin{align}\label{eq_proof_11}
U_{(j)}(\text{FUT-NR})\! \leq \!\max_{i=1,\ldots,j}U_{w_{j}}(\text{FUT-NR}),~j=1,\ldots,n.\!\!
\end{align}
Combining \eqref{eq_proof_10} and \eqref{eq_proof_11}, we obtain that for each sample path of policy $P'$, there is a sample path of policy FUT-NR with the same probability density such that 
\begin{align}
\bm{U}_{\uparrow}(\text{FUT-NR}) \leq  \bm{C}_{\uparrow}(P').
\end{align}
Considering all possible sample paths of these two policies, the stochastic ordering result in \eqref{eq_condition3} follows.
%Suppose that for some $j\in\{1,\ldots,N-1\}$, the time duration between $c_{i:N}(P')$ and $c_{w_i,\text{FUT-NR}}$ is no more than the time for the system to complete $\min[k_{w_i},M]$ tasks of job $w_i$ for all $h=1,\ldots, j$, and the job indices $w_1,w_2,\ldots,w_j$ are distinct. We will prove that there is a job $w_{j+1}$ different from $w_1,w_2,\ldots,w_j$ such that the time duration between $C_{(j+1)}(P')$ and $c_{w_{j+1},\text{FUT-NR}}$ is no more than the time to complete $\min[k_{w_{j+1}},M]$ tasks of a job $w_{j+1}$.
%Let $z$ be the number of job arrivals during $[0,C_{(j+1)}(P'))$, which must satsify $z\geq j+1$. By following the arguments of \eqref{eq_proof_1}-\eqref{eq_proof_9}, we can obtain
%\begin{align}\label{eq_proof_4}
%\alpha_{i}(C_{(j+1)}(P'))=\delta_{i}(C_{(j+1)}(P')),~h=z-j,\ldots,z.
%\end{align}
%Since preemption is not allowed, in policy FUT-NR, the remaining tasks of the $(j+1)$ jobs associated to the coordinates $z-j,z-j+1,\ldots,z$ will be under service after time $C_{(j+1)}(P')$ until completion (or are already completed before time $C_{(j+1)}(P')$). Moreover, at least one of these $(j+1)$ jobs must be different from the jobs $w_1,w_2,\ldots,w_j$. Let $w_{j+1}$ be the index of this job. 
%Using \eqref{eq_def_state} and \eqref{eq_proof_4}, one can show that the time difference between $c_{(j+1)}(P')$ and $c_{w_{j+1},\text{FUT-NR}}$ is no more than the time duration to complete $\min[k_{w_{j+1}},M]$ tasks of job $w_{j+1}$.
%
%By induction, for all $h=1,\ldots,N$ and all $\omega\in\Omega$, the time difference between $c_{i:N}(P')$ and $c_{w_{i},\text{FUT-NR}}$ is no more than the time duration to complete $\min[k_{w_i},M]$ tasks of job $w_i$. Further, the job indices $w_1,w_2,\ldots,w_N$ are distinct, such that $(w_1,w_2,\ldots,w_N)$ is a permute of $(1,2,\ldots,N)$.
% This tells us that 
%\begin{align}
%\mathbb{E}\left[c_{w_i,\text{FUT-NR}} - c_{i:N}(P')| \mathcal{I}\right] \leq \max_{\substack{S: |S|\leq k_i\\
%S\subseteq\{1,\ldots,m\}}}\!\!\mathbb{E}\left[\max_{l\in S} X_l\right].\nonumber
%\end{align}
%Hence, we have
%\begin{align}\label{eq_proof_5}
%&\mathbb{E}[{D}_{\text{avg,FUT-NR}}-{D}_{\text{avg}}(P')| \mathcal{I}]\nonumber\\
%=&\frac{1}{N}\sum_{h=1}^N\mathbb{E} \left[c_{i,\text{FUT-NR}} - c_{i}(P')| \mathcal{I}\right]\nonumber\\
%=&\frac{1}{N} \sum_{h=1}^N\mathbb{E} \left[c_{w_i,\text{FUT-NR}} - c_{i:N}(P')| \mathcal{I}\right]\nonumber\\
%\leq &\frac{1}{N}\sum_{h=1}^N\max_{\substack{S: |S|\leq k_i\\
%S\subseteq\{1,\ldots,m\}}}\!\!\mathbb{E}\left[\max_{l\in S} X_l\right].
%\end{align}
%By this, condition 3 is proven.
\end{proof}
After establishing conditions 1-3 of Lemma \ref{lem1} for policy FUT-NR,  we can use Lemma \ref{lem1} and Corollary \ref{coro1} to obtain \eqref{eq_delaygap1}. This completes the proof.

\subsection{Proof of {\large \eqref{eq_delaygap2}} in Theorem \ref{thm1}} 
The proof of \eqref{eq_delaygap2} is  similar with that of \eqref{eq_delaygap1} in Appendix \ref{sec_app_thm1_1}, except for the following two differences: 

First, policy FUT-NR in Appendix \ref{sec_app_thm1_1} should be replaced by policy FUT-NIR. 


Second, task replications are allowed in policy FUT-NIR, which will introduce some extra delay to cancel the redundant task copies. %It is important to keep the cancellation overhead small. Otherwise, 
If the cancellation overhead is large, the servers might be busy cancelling the redundant task copies, instead of serving new tasks. In this case, Lemma \ref{lemG4} does not hold. Hence, we should keep the cancellation overhead small. In the design of policy FUT-NIR, a task replica is cancelled if the time to cancel the replica is stochastically shorter than the time to complete the replica; otherwise, the replica will not be cancelled. Using this and the extra conditions {$\bm{O}_{\mathcal{S}}\leq_{\text{st}}[\bm{X}_{\mathcal{S}}-\bm{\tau}_{\mathcal{S}}| \bm{X}>\bm{\tau}]$} and  {$\bm{O}_{\mathcal{S}^c}\geq_{\text{st}}[\bm{X}_{\mathcal{S}^c}-\bm{\tau}_{\mathcal{S}^c}| \bm{X}>\bm{\tau}]$}, we can obtain that in policy FUT-NIR the redundant task copies are completed stochastically earlier than processing these task copies until completion. Using this, the proof arguments of Lemma \ref{lemG4} also work for policy FUT-NIR.

\subsection{Proof of Corollary 3}  
Under the conditions of Corollary \ref{coro3}, policy FUT-NR satisfies the following three properties: (i) all $m$ servers are busy at all time $t\in[0,\infty)$, (ii) there is no task replications, and (iii) any completed task is from a job with the fewest remaining task. Therefore, policy FUT-NR is identical with policy $P'$ constructed in Appendix \ref{sec_app_thm1_1}. In addition, because there are at least $m$ remaining tasks at all time $t\in[0,\infty)$, policy FUT-NIR is identical with policy FUT-NR. Then, \eqref{eq_coro3} follows from Lemma \ref{lem1} and Corollary \ref{coro1}. 

%The details are provided in Appendix \ref{app2}.



%\textbf{Condition 4:} $P\in\Pi$. This condition is trivial. Hence, \eqref{eq_delaygap1} follows from Lemma \ref{thm2}.
%
%The remaining task is to prove \eqref{eq_delaygap2}. Since the $X_l$'s are independent NBU random variables with mean $\mathbb{E}[X_l]=1/\mu_l$, by Theorem 3.A.55 of \cite{StochasticOrderBook}, we can obtain
%\begin{align}
%X_l \leq_{\text{icx}} Z_l,~l=1,\ldots,m,\nonumber
%\end{align}
%where $\leq_{\text{icx}}$ is the increasing convex order defined in \cite[Chapter 4]{StochasticOrderBook} and the $Z_l$'s are independent exponential random variables with mean $\mu_l$. By Corollary 4.A.16 of \cite{StochasticOrderBook}, we have 
%\begin{align}
%\max_{l\in S} X_l \leq_{\text{icx}} \max_{l\in S} Z_l,~\forall~S\subseteq\{1,\ldots,m\}.\nonumber
%\end{align}
%Then, Eq. (4.A.1) of \cite{StochasticOrderBook} and $\mu_1\leq \ldots\leq \mu_M$ tell us that  
%\begin{align}
%\!\!\max_{\substack{S: |S|\leq k_i\\
%S\subseteq\{1,\ldots,m\}}}\!\!\mathbb{E}\!\left[\max_{l\in S} X_l\right]\!\leq\!\mathbb{E}\!\left[\max_{l=1,\ldots,k_i \wedge M} Z_l\right]\!\leq\!\sum_{l=1}^{k_i \wedge M} \frac{1}{\sum_{m=1}^l \mu_l}.\nonumber
%\end{align}
%This and \eqref{eq_proof_5} imply \eqref{eq_delaygap2}. This completes the proof.




==> appendices_3.tex <==
% !TEX root = ./replication.tex

\section{Proof of Thoerem~\ref{thm2}} \label{app2}
%\subsection{Proof of Thoerem~2} \label{sec_app_thm2_1}
%\subsection{Proof of Theorem \ref{thm2}}  
Define $\bm{s}=(s_{1},\ldots,$ $ s_{k_{\text{sum}}})$ as the sequence of task arrival times where $s_1\leq \ldots\leq s_{k_{\text{sum}}}$. Hence, $\bm{s}$ is determined by the job arrival times $a_1,\ldots,a_n$ and job sizes $k_1,\ldots,k_n$.
Recall that $\bm{T}_\pi=(T_{1,\pi},\ldots,$ $ T_{k_{\text{sum}},\pi})$ is the sequence of task completion times in policy $\pi$ where $T_{1,\pi}\leq \ldots\leq T_{k_{\text{sum}},\pi}$. 
We  first show that for all $\pi\in\Pi$
\begin{align}\label{eq_thm2_proof1}
[\bm{T}_{\text{FUT-R}}|\mathcal{I}] \leq_{\text{st}} [\bm{T}_\pi|\mathcal{I}].
\end{align}
We prove \eqref{eq_thm2_proof1} by induction. Consider the first task completion time $T_{1,\pi}$. Job 1 arrives at time $a_1=0$. All policy $\pi\in\Pi$ are non-preemptive. If policy $\pi$ is  work-conserving, then
\begin{align}
[T_{1,\pi}|\mathcal{I}]=\min_{l=1,\ldots,m} X_l,\nonumber
\end{align} 
otherwise, if policy $\pi$ is non-work-conserving, then
\begin{align}
[T_{1,\pi}|\mathcal{I}]\geq\min_{l=1,\ldots,m} X_l,\nonumber
\end{align} 
because of the possibility of server idleness. Since policy FUT-R$\in\Pi$ is work-conserving, we can obtain that for all $\pi\in\Pi$
\begin{align}\label{eq_thm2_condition1_2}
[T_{1,\text{FUT-R}}|\mathcal{I}]=\min_{l=1,\ldots,m} X_l\leq[T_{1,\pi}|\mathcal{I}].
\end{align} 

Next, consider the system evolution from $T_{j,\pi}$ to $T_{j+1,\pi}$. For any work-conserving policy $\pi\in\Pi$, we can obtain
\begin{eqnarray}\label{eq_thm2_2}
T_{j+1,\pi}\!=\max\{s_{j+1},T_{j,\pi}\} + \!\min_{l=1,\ldots,m} R_{j,l,\pi},
\end{eqnarray}
where $R_{j,l,\pi}$ is the time duration for server $l$ to complete a task since time $\max\{s_{j+1},T_{j,\pi}\}$. Suppose that server $l$ has spent $\tau_{l,\pi}$ ($\tau_{l,\pi}\geq0$) seconds on a task by time $\max\{s_{j+1},T_{j,\pi}\}$. 

Because the task service times are independent across the servers and the complementary CDF $\bar{F}$  is absolutely continuous, the probability for any two servers to complete their tasks at the same time is zero. Hence, $\Pr[R_{j,l,\pi} > 0] = 1$.\footnote{If $\bar{F}$  is not absolutely continuous, then it may happen that $\Pr[R_{j,l,\pi} > 0] < 1$ and two servers complete task executions at the same time. In this case, it is better to assign two distinct tasks than two replicated copies of the same task on these two servers.}
Therefore, in policy FUT-R, when a task copy is completed on a server, the remaining $m-1$ replicated copies of this task are still being processed on the other servers. Then, these replicated task copies are cancelled immediately and the servers are assigned to process $m$ replicated copies of a new task. 
Hence, $\tau_{l,\text{FUT-R}}=0$ for $l=1,\ldots,m$. The complementary CDF for the servers to complete a task after time $\max\{s_{j+1},T_{j,\text{FUT-R}})\}$ is 
\begin{align}\label{eq_thm2_7}
&\Pr\Big[\min_{l=1,\ldots,m} R_{j,l,\text{FUT-R}}>t\Big]\nonumber\\
=& \Pr\Big[\min_{l=1,\ldots,m}X_l>t \Big].
\end{align}
If $\pi$ is a work-conserving policy, then we have $\tau_l\geq0$ for $l=1,\ldots,m$. Hence, the tail probability for the servers to complete a task after time $\max\{s_{j+1},T_{j,\pi}\}$ is 
\begin{align}\label{eq_thm2_8}
&\Pr\Big[\min_{l=1,\ldots,m} R_{j,l,\pi}>t\Big]\nonumber\\
=& \Pr\Big[\min_{l=1,\ldots,m}(X_l-\tau_l)>t\Big|X_l> \tau_l, l=1,\ldots,m \Big].
\end{align} 
By \eqref{eq_thm2_7}, \eqref{eq_thm2_8}, and the task service times are independent NWU, yields 
\begin{align}\label{eq_min_thm2}
\min_{l=1,\ldots,m} R_{j,l,\text{FUT-R}}\leq_{\text{st}} \min_{l=1,\ldots,m} R_{j,l,\pi}.
\end{align}
Using \eqref{eq_thm2_2}, \eqref{eq_min_thm2}, and the fact that $s_j$ is uniquely determined by $\mathcal{I}$, it follows that for all work-conserving policy $\pi\in\Pi$
\begin{align}\label{eq_thm2_4}
[T_{j+1,\text{FUT-R}} | \mathcal{I},  T_{j,\text{FUT-R}}= t_j] \leq_{\text{st}} [T_{j+1,\pi} | \mathcal{I},  T_{j,\pi} = t_j'] \nonumber\\
\text{whenever}~ t_j \leq t_j',j=1,2,\ldots
\end{align}
If policy $\pi$ is non-work-conserving, \eqref{eq_thm2_2} becomes
\begin{eqnarray}\label{eq_thm2_2_1}
T_{j+1,\pi}\!\geq\max\{s_{j+1},T_{j,\pi}\} + \!\min_{l=1,\ldots,m} R_{j,l,\pi},\nonumber
\end{eqnarray}
because of the possibility of server idleness. In this case, \eqref{eq_thm2_4} still holds. Hence, \eqref{eq_thm2_4} holds for all $\pi\in\Pi_{\text{non-prmp}}$.
Then, combining \eqref{eq_thm2_condition1_2}, \eqref{eq_thm2_4}, and Theorem 6.B.3 of \cite{StochasticOrderBook}, yields
\begin{align}%\label{eq_thm1_5}
[(T_{1,\text{FUT-R}},\ldots,T_{j,\text{FUT-R}})|\mathcal{I}] \leq_{\text{st}} [(T_{1,\pi},\ldots,T_{j,\pi})|\mathcal{I}],~\forall~\pi\in\Pi.\nonumber
\end{align}
Hence, \eqref{eq_thm2_proof1} is proven.

According to Theorem 6.B.1 of \cite{StochasticOrderBook}, for any policy $\pi\in\Pi$, there exist that FUT-R$_1$ and policy $\pi_1$ which satisfy the same queueing disciplines and stochastic laws with policy FUT-R and policy $\pi$, and policy FUT-R$_1$ is more work-efficient than policy $\pi_1$ with probability one. Because each task is replicated on all $m$ servers and $k_1\leq \ldots\leq k_n$, each task completing service is from the job with the fewest remaining tasks among all unfinished jobs.
By Proposition \ref{lem1_0}, for all $f\in\mathcal{D}_{\text{sym}}$
\begin{align}
\Pr[f(\bm{C}(\text{FUT-R}_1)) \leq f(\bm{C}(\pi_1)) |\mathcal{I}]=1. \nonumber
\end{align}
Then, by Theorem 1.A.1 of \cite{StochasticOrderBook}, we can obtain \eqref{eq_delaygap3}, which completes the proof.

%\section{Proofs of Thoerem~\ref{thm2_exp}} \label{app2_exp}

%We first show that policy FUT-R is more work-efficient than any policy $\pi\in\Pi$.  
%\begin{lemma}\label{lem_work_efficient_FUT_R}
%If the conditions of Theorem \ref{thm2} are satisfied, then policy FUT-R is more work-efficient than any policy $\pi\in\Pi$.  
%\end{lemma}
%\begin{proof}
%Consider any sample path of an arbitrarily chosen policy $\pi\in\Pi$ and an arbitrarily chosen task $j$. Suppose that 
%%on the sample path of policy $\pi$, server $l_w$ starts to process task $j$ at time $\tau$ and completes task $j$ at time $\nu$ ($\tau\leq\nu$). More specifically, suppose that 
%on the sample path of policy $\pi$, $u$ copies of task $j$ are replicated on the servers $l_1,l_2,\dots,l_u$ at the time instants $\tau_1,\tau_2,\ldots, \tau_u$, respectively, where $\tau=\tau_1\leq \tau_2\leq \ldots \leq\tau_u$; server $l_w$ ($w\in\{1,2,\ldots,u\}$) completes one copy of task $j$ at time $\nu$, which is earlier than the other $u-1$ servers; after time $\nu$, the other $u-1$ copies of task $j$ are cancelled. Hence, the service duration of task $j$ is $[\tau,\nu]$ on the sample path of policy $\pi$. One example of this is illustrated in Fig. \ref{fig_theorem_proof_2}, where $u=2$ and $w=2$. We need to prove that \emph{there exists one sample path of policy FUT-R such that these two sample paths of policy FUT-R and policy $\pi$ have the same probability density; and  on the sample path of policy FUT-R, if there exist unassigned tasks in the queue during $[\tau,\nu]$, then there exists one task $j'$ which starts execution during $[\tau,\nu]$ on server $l_w$}.
%
%
%\begin{figure}
%\centering 
%\includegraphics[width=0.5\textwidth]{Figures/theorem_proof_2} \caption{Illustration of the proof of Lemma \ref{lem_work_efficient_FUT_R}. On the sample path of policy $\pi$, two copies of task $j$ are replicated on the server $l_1$ and server $l_2$ at time $\tau_1$ and $\tau_2$, respectively, where $\tau=\tau_1\leq\tau_2$. Server $l_2$ completes one copy of task $j$ at time $\nu$, server $l_1$ cancels one redundant copy of task $j$ after time $\nu$. Hence, the service duration of task $j$ is $[\tau,\nu]$ on the sample path of policy $\pi$. On the sample path of policy FUT-R, server $l_2$ cancels a task at time $\tau_2'\in[\tau_2,\nu]$, and then a new task is assigned to server $l_2$. Server $l_2$ completes this task at time $t\in[\tau_2,\nu]\subseteq[\tau,\nu]$ and a new task $j'$ starts execution at time $t$. This task $j'$ is the task corresponding to task $j$ in the definition of work-efficiency ordering.}
%\label{fig_theorem_proof_2} 
%\end{figure} 
%
%Because policy FUT-R is work-conserving, if there exist unassigned tasks in the queue during $[\tau,\nu]$, then all servers are busy during $[\tau,\nu]$. In particular,  server $l_w$ is busy during $[\tau,\nu]$. 
%Suppose that in policy FUT-R, server $l_w$ has spent $\chi_w$ ($\chi_w\geq0$) seconds on a task by time $\tau_w\in[\tau,\nu]$. We construct the sample path of policy FUT-R by considering the following cases:
%
%\emph{Case 1: No task is completed on the servers $1,\ldots,l_w-1,l_w+1,\ldots,n$, until server $l_w$ completes a task}. Because server $l_w$ starts to process a task earlier in policy FUT-R, one can construct a sample path of policy FUT-R, such that that these two sample paths of policy FUT-R and policy $\pi$ have the same probability density, and server $l_w$ will complete a task before time $\nu$ on the sample path of policy FUT-R. Since in policy FUT-R, all servers are busy during $[\tau,\nu]$, a new task $j'$ will start execution on all servers at time $t$. Let task $j'$ be the task corresponding to task $j$ in the definition of work-efficiency ordering. 
%
%\emph{Case 2: Some of the servers $1,\ldots,l_w-1,l_w+1,\ldots,n$ complete a task at time $\tau_w'>\tau_w$ before server $l_w$ completes a task}. In this case, server $l_w$ will cancel its redundant task copy at time $\tau_w'$, then a new task will start execution on all $m$ servers at time $\tau_w'$. The probability for server $l_w$ to complete a task after time $\tau_w'+s$ is 
%\begin{align}
%\Pr[X_{l_w}>s].\nonumber
%\end{align}
%On the other hand, in policy $\pi$, the probability for server $l_w$ to complete task $j$ after time $\tau_w'+s$ is 
%\begin{align}
%\Pr[X_{l_w}-(\tau_w'-\tau_w)>s  |X_{l_w}> \tau_w'-\tau_w].\nonumber
%\end{align}
%Because $X_{l_w}$ is NWU, we can obtain that 
%\begin{align}
%\Pr[X_{l_w}>s]\leq \Pr[X_{l_w}-(\tau_w'-\tau_w)>s  |X_{l_w}> \tau_w'-\tau_w],\nonumber
%\end{align}
%which can be equivalently expressed as 
%\begin{align}
%X_{l_w} \leq_{\text{st}} [X_{l_w}-(\tau_w'-\tau_w) |X_{l_w}> \tau_w'-\tau_w].\nonumber
%\end{align}
%In other words, the task service time becomes stochastically shorter after task cancellation.
%According to the property of stochastic ordering \cite[Theorem 6.B.1]{StochasticOrderBook}, if on the sample path of policy $\pi$ server $l_w$ completes task $j$ at time $\nu$, one can construct a sample path of policy FUT-R, such that these two sample paths of policy FUT-R and policy $\pi$ have the same probability density, and server $l_w$ completes a task at some time $t$ earlier than $\nu$ on the sample path of policy FUT-R. Since in policy FUT-R, all servers are busy during $[\tau,\nu]$, a new task $j'$ will start execution on all servers at time $t$. Let task $j'$ be the task corresponding to task $j$ in the definition of work-efficiency ordering. This completes the proof.
%
%
%%We need to prove that on the sample path of policy FUT-R, there exists a time $t\in[\tau_w,\nu]$ such that one of the following three cases holds:  (i) server $l_w$ starts to process a task (which is corresponding to task $j$) at time $t$, (ii) all the remaining tasks are under service at time $t$, or (iii) the queue is empty at time $t$. 
%%Hence, we only need to prove that case (i) holds, whenever case (ii) and case (iii) do not hold. 
%%If case (ii) or case (iii) holds, then Lemma \ref{lem_work_efficient_FUT_R} is proven. Hence, we need to prove that case (i) holds, whenever case (ii) and case (iii) do not hold. More specifically, we need to prove that  \emph{on the  sample path of policy FUT-R, if there are one or more unassigned tasks during $[\tau_w,\nu]$, then server $l_w$ starts to process one task corresponding to task $j$ at some time $t\in[\tau_w,\nu]$}.
%
%%Because policy FUT-R is work-conserving, if there are one or more unassigned tasks during $[\tau_w,\nu]$, then all servers are busy during $[\tau_w,\nu]$.  
%%Suppose that in policy FUT-R, server $l_w$ has spent $\chi_w$ ($\chi_w\geq0$) seconds on a task by time $\tau_w$. If no task is cancelled on server $l_w$, then the task service time of server $l_w$ will be the same in both policies. Hence, on the sample path of policy FUT-R,  server $l_w$ will completes a task at time $t=\nu-\chi_w\in[\tau_w,\nu]$. If server $l_w$ cancels a task at time $\tau_w'>\tau_w$, then a new task will be assigned to server $l_w$ at time $\tau_w'$. 
%%
%%We compare the task completion time of server $l_w$ in these two cases: If no task is cancelled on server $l_w$, the probability for server $l_w$ to complete a task after time $\tau_w'+s$ is $\Pr[X_{l_w}-\chi_w-(\tau_w'-\tau_w)>s|X_{l_w}> \chi_w + (\tau_w'-\tau_w)]$ where $\chi_w + (\tau_w'-\tau_w)>0$. On the other hand, if server $l_w$ cancels a task at time $\tau_w'$, the probability for server $l_w$ to complete a task after time $\tau_w'+s$ is $\Pr[X_{l_w}>s]$. Because $X_{l_w}$ is NWU, we can obtain that 
%%\begin{align}
%%\Pr[X_{l_w}-\chi_w-(\tau_w'-\tau_w)>s|X_{l_w}> \chi_w + (\tau_w'-\tau_w)] \leq \Pr[X_{l_w}>s].\nonumber
%%\end{align}
%%By the property of stochastic ordering \cite[Theorem 6.B.1]{StochasticOrderBook}, if server $l_w$ cancels a task at time $\tau_w'$, server $l_w$ will completes a task at a time $t$ earlier than $\nu-\chi_w$. Because policy FUT-R is work-conserving and there are one or more unassigned tasks at time $t$, an unassigned task $j'$ will be allocated to server $l_w$ at time $t$. Let task $j'$ be the task corresponding to task $j$  in the definition of work-efficiency ordering. This completes the proof. 
%\end{proof}

%\ifreport
%\begin{proof}[Proof of Theorem \ref{thm2}]
%\else
%\begin{proof}[of Theorem \ref{thm2}]
%\fi
%In Lemma \ref{lem_work_efficient_FUT_R}, we have shown that policy FUT-R is more work-efficient than any policy $\pi\in\Pi$. Then, Theorem \ref{thm2} follows from Corollary \ref{coro1}. This completes the proof.
%\end{proof}
\section{Proof of Lemma \ref{lem7_NWU}}\label{app_lem7_NWU}  
Consider the time difference ${C}_i(\text{FUT-R})-{U}_i(\text{FUT-R})$.
%\textbf{Condition 4:} $P\in\Pi$. This condition is trivial. Hence, \eqref{eq_delaygap1} follows from Lemma \ref{thm2}.
In policy FUT-R, all servers are allocated to process $m$ replicated copies of a task from the job with the fewest unassigned tasks. Hence, at time ${U}_i(\text{FUT-R})$, one task of job $i$ are being processed by all $m$ servers. 
%Then, $\mathcal{S}_i$ is a random set with cardinality $|\mathcal{S}_i|\leq k_i\wedge m$.
%The remaining task is to prove \eqref{eq_delaygap2}. 
Because the $X_l$'s are independent exponential random variables with mean $\mathbb{E}[X_l]=1/\mu_l$, 
by Theorem 3.A.55 of \cite{StochasticOrderBook}, we can obtain
%\begin{align}
%X_l \leq_{\text{icv}} Z_l,~l=1,\ldots,m,\nonumber
%\end{align}
%where $\leq_{\text{icv}}$ is the increasing concave order defined in \cite[Chapter 4]{StochasticOrderBook} and the $Z_l$'s are independent exponential random variables with mean $\mathbb{E}[Z_l]=\mu_l$. By Corollary 4.A.16 of \cite{StochasticOrderBook}, we have 
%\begin{align}\label{eq_exp_orderNWU}
%\min_{l=1,\ldots,m} X_l \leq_{\text{icv}} \min_{l=1,\ldots,m} Z_l.
%\end{align}
%Note that the set $\mathcal{S}_i$ is determined by the evolution of policy FUT-R up to time ${U}_i(\text{FUT-R})$.Because the task service times are determined by an external process which is not affected by the scheduling policy FUT-R, $X_l$ and $Z_l$ are independent of $\mathcal{S}_i$ for each $l\in \mathcal{S}_i$.
%Then,   
\begin{align}
&\mathbb{E}[{C}_i(\text{FUT-R})-{U}_i(\text{FUT-R})|\mathcal{I}]\nonumber\\
\leq &\mathbb{E}\!\left[\min_{l=1,\ldots,m} X_l\bigg|\mathcal{I}\right]\label{eq_gap_NWU_condition1}\\
=&\mathbb{E}\!\left[ \min_{l=1,\ldots,m} X_l\right]\label{eq_gap_NWU_condition2}\\
%\leq&\mathbb{E}\!\left[ \min_{l=1,\ldots,m} Z_l\right]\label{eq_gap_NWU_condition3}\\
\leq &\frac{1}{\sum_{l=1}^m \mu_l}.\label{eq_gap_NWU_condition5}
\end{align}
where \eqref{eq_gap_NWU_condition1} is because one task of job $i$ are being processed by all $m$ servers at time ${U}_i(\text{FUT-R})$, \eqref{eq_gap_NWU_condition2} is because $X_l$ is independent of $\mathcal{I}$, 
%\eqref{eq_gap_NWU_condition3} is due to\eqref{eq_exp_orderNWU} and Eq. (4.A.1) of \cite{StochasticOrderBook}, 
and \eqref{eq_gap_NWU_condition5} is due to the property of exponential distributions. By this, Lemma \ref{lem7_NWU} is proven.


%\subsection{Proof of Corollary \ref{coro4}}  
%%Similar with Corollary \ref{coro3}, 
%Let $t_i(\pi)$ denote the $i$-th task completion time on the sample path of policy $\pi$. We first show that for all $\pi\in\Pi$ 
%\begin{align}\label{eq_coro4_1}
%t_{i}(\text{FUT-R})\leq t_{i}(\pi), ~i=1,2,\ldots 
%\end{align}  
%
%According  the proof of Lemma \ref{lem_work_efficient_FUT_R}, for each sample path of policy $\pi\in\Pi$ there exists a sample path of policy FUT-R, such that if (i) a task $j$ starts execution at time $\tau$ and completes execution at time $\nu$ ($\tau\leq\nu$) on the sample path of policy $\pi$, and (ii) all servers are busy in policy FUT-R, then on the sample path of policy FUT-R, a task completes execution during $[\tau,\nu]$ before a new task $j'$ starts execution. On the other hand, if (ii') some servers are idle in policy FUT-R, then the queue is empty. 
%%According to 
%%we can obtained from the proof of Lemma \ref{lem_work_efficient_FUT_R} that
%Using this, we can show that for all $t\geq0$, if $b$ tasks are completed during $[0,t]$ on the sample path of policy $\pi$, then at least $b$ tasks are completed during $[0,t]$ on the sample path of policy FUT-R. By this, \eqref{eq_coro4_1}
%follows.
%%Because each job has $k$ tasks, if the servers start to process the tasks of job $i$, job $i$ will have fewer unassigned tasks than any other job in the queue which has $k$ unassigned tasks. No incoming job can have a higher priority than job $i$. Therefore, the servers will keep processing the tasks of job $i$ until job $i$ is completed. Further, 
%
%Next, we use \eqref{eq_coro4_1} to prove Corollary \ref{coro4}.
%Because each job has $k$ tasks,  for any $\pi\in\Pi$ no job can be completed before time $t_{k}(\pi)$, i.e.,
%\begin{align}
%c_{(1)}(\pi)\geq t_{k}(\pi).\nonumber
%\end{align}  
%In general, we have
%\begin{align}
%c_{(i)}(\pi)\geq t_{ik}(\pi), ~i=1,2,\ldots,n. \nonumber
%\end{align}  
%In addition, policy FUT-R satisfies that
%\begin{align}
%c_{(i)}(\text{FUT-R})= t_{ik}(\text{FUT-R}), ~i=1,2,\ldots,n. \nonumber
%\end{align} 
%Hence, for $i=1,2,\ldots,n$
%\begin{align}
%c_{(i)}(\text{FUT-R})= t_{ik}(\text{FUT-R})\leq   t_{ik}(\pi) \leq c_{(i)}(\pi)\nonumber
%\end{align} 
%holds in stochastic ordering. Therefore, for all $f\in\mathcal{D}_{\text{sym}}$ and $\pi\in\Pi$
%\begin{align}
%&[f(\bm{c} (\text{FUT-R}))|\mathcal{I}]=[f(\bm{c}_{\uparrow} (\text{FUT-R}))|\mathcal{I}] \nonumber\\
%\leq_{}&[f(\bm{c}_{\uparrow} (\pi))|\mathcal{I}] = [f(\bm{c}_{} (\pi))|\mathcal{I}] \nonumber
%\end{align} 
%holds in stochastic ordering. By considering all possible sample paths, the stochastic ordering result in Corollary \ref{coro4} is proven.



==> appendices_3version2.tex <==
% !TEX root = ./replication.tex

\section{Proofs of Proposition~\ref{coro3_1}} \label{app0_2}
%\ifreport
%\begin{proof}[Proof of Thoerem \ref{lem3}]
%\else
%\begin{proof}[of Thoerem \ref{lem3}]
%\fi
%Thoerem \ref{lem3} follows from Thoerem \ref{lem2} by letting $d_i=a_i$ for all $i$.
%\end{proof}
%\ifreport
%\begin{proof}[Proof of Corollary~\ref{coro3_1}]
%\else
%\begin{proof}[of Corollary~\ref{coro3_1}]
%\fi
%Proposition~\ref{coro3_1} follows from Corollary \ref{coro2} by letting $d_i=a_i$ for all $i$.
%As in the proof of Corollary \ref{coro2}, let $w_i$ denote the index of the job associated with $v_{(i)}(P)$.
%
%We assume that the arrival times $a_1,\ldots, a_n$ of the $n$ jobs are distinct from each other. This does not lose any generality, because if $a_i=a_j$ for two jobs $i$ and $j$, Proposition~\ref{coro3_1} can be proven by first proving for the case $a_i=a_j+\epsilon$ and then taking the limit $\epsilon\rightarrow 0$. 
We take 3 steps to prove Proposition~\ref{coro3_1}:

\emph{Step 1: We show that}  
%Thoerem \ref{lem3} holds if \emph{$D_{\max}(\cdot)$} is replaced by any $f\in\mathcal{D}_{\text{sym}}$.}
\begin{align}\label{eq_coro2_2_2}
v_{(i)}(P) \leq c_{(i)}(\pi),~i=1,\ldots,n.
\end{align}

In policy $P$, each unassigned task entering the servers is from the job with the earliest arrival time among all jobs with unassigned tasks. Because each job has $k$ tasks, in policy $P$ only the job with the earliest arrival time may have fewer than $k$ unassigned tasks, the other jobs arrived later have exactly $k$ unassigned tasks. Therefore, among all jobs with unassigned tasks, the job with the earliest arrival time is also the job with the fewest unassigned tasks.
Then, \eqref{eq_coro2_2_2} follows from Proposition~\ref{lem1}. 
In addition, we can use Proposition \ref{lem1} to prove that \eqref{eq_coro3_1_1} holds for all $f\in\mathcal{D}_{\text{sym}}$.

The remaining proof is almost identical with \emph{Step 2} and \emph{Step 3} in the proof of Proposition \ref{coro2}, except that $d_i$ should be replaced by $a_i$. 
By this, Proposition~\ref{coro3_1} is proven.
%Because each job has $k$ tasks, a job can have fewer than $k$ unassigned tasks if and only if some of its tasks are under service, which 
%Because each job has $k$ tasks, only the job under service has fewer than $k$ tasks, , 
%at any time in policy $P$, the job with the earliest arrival time is also the job with the fewest unassigned tasks.
%We can utilize Lemma \ref{lem_sample_path_ordering} to show that $v_{w_j}(P) = v_{(j)}(P) \leq c_{(j)}(\pi)$ for all $j=1,\ldots,n$. In addition, 
%According to Corollary \ref{coro1}, the result of Thoerem \ref{lem3} holds if \emph{$D_{\max}(\cdot)$} is replaced by any $f\in\mathcal{D}_{\text{sym}}$.
%\emph{Step 2: We show that}
%\begin{align}\label{eq_coro3_3}
%\bm{u}(P)-\bm{d}\prec_{\text{w}} \bm{c} (\pi)-\bm{d}.
%\end{align} 
%
%
%
%We construct a policy $\pi'$ based on policy $\pi$: The sequence of job completion times of policy $\pi'$ is a reordering (rearrangement) of that of policy $\pi$. And in policy $\pi'$, each completed job has the earliest arrival time among all jobs in the queue. We note that because each job has $k$ tasks, it is feasible to reordering the job completion times such that the job arrives earlier is completed earlier.
%% this reordering operation leads to a feasible policy $\pi'$. %In particular, suppose that job $i$ has an earlier arrival time than job $j$. Because both job $i$ and job $j$ have $k$ tasks, the system can switch to process job $i$
%%and more unassigned tasks than the other jobs in the queue, then it is infeasible to reorder the sequence of job completion times such that job $i$ is the next completed job.
%Hence, for the constructed policy $\pi'$, one can use the proof argument of Lemma \ref{lemG4_thm3} to show that
%\begin{eqnarray}\label{eq_pi'_3}
%\sum_{i:a_i\leq\tau} \gamma_{i,P}(t)\leq \sum_{i:a_i\leq\tau} \xi_{i,\pi'}(t), ~\forall~\tau\in[0,\infty)
%\end{eqnarray}
%holds for all $t\in[0,\infty)$. The remaining proof is the same with \emph{Step 2} and \emph{Step 3} in the proof of Corollary \ref{coro2}, where $d_i$ is replaced by $a_i$. 
%By this, Corollary~\ref{coro3_1} is proven.
%\end{proof}

%\subsection{Proof of Corollary \ref{coro2}}
%
%
%In the proof of Corollary \ref{coro2}, we need to use the following rearrangement inequality: 
%\begin{lemma} \cite[Theorem 6.F.14]{Marshall2011}\label{lem_rearrangement}
%Consider two $n$-vectors $(x_1,\dots,x_n)$ and $(y_1,\ldots,y_n)$. If $(x_i- x_j)(y_i-y_j)<0$ for some indices $i$ and $j$ where $1\leq i<j\leq n$, then 
%\begin{align}
%&(x_1\!-\!y_1,\ldots,x_j\!-\!y_i,\ldots,x_i\!-\!y_j,\ldots,x_n\!-\!y_n)\nonumber\\
%\prec& (x_1\!-\!y_1,\ldots,x_i\!-\!y_i,\ldots,x_j\!-\!y_j,\ldots,x_n\!-\!y_n).\nonumber
%\end{align}
%\end{lemma}
%\ifreport
%\begin{proof}[Proof of Corollary \ref{coro2}]
%\else
%\begin{proof}[of Corollary \ref{coro2}]
%\fi
%As in the proof of Lemma \ref{lem_sample_path_ordering_thm3}, let $w_i$ denote the index of the job associated with $v_{(i)}(P)$. 
%
%\emph{Step 1: We show that  
%Thoerem \ref{lem2} holds if \emph{$L_{\max}(\cdot)$} is replaced by any $f\in\mathcal{D}_{\text{sym}}$.}
%%\begin{align}\label{eq_coro2_2}
%%v_{w_i}(P) \leq c_{(i)}(\pi),~i=1,\ldots,n.
%%\end{align}
%
%Because each job has only one task, it holds in policy $P$ that each task allocated to the servers belongs to the job with the fewest unassigned tasks, whenever there exist unassigned tasks in the system. 
%Hence, 
%%we can utilize Lemma \ref{lem_sample_path_ordering} to show that $v_{w_i}(P) = v_{(i)}(P) \leq c_{(i)}(\pi)$ for all $i=1,\ldots,n$. On the other hand, 
%Corollary \ref{coro1} implies that Thoerem \ref{lem2} holds if \emph{$L_{\max}(\cdot)$} is replaced by any {$f\in\mathcal{D}_{\text{sym}}$}.

%Suppose that $b_j$ tasks have been assigned to the servers in policy $P$ by time $c_{(j)}(\pi)$. Since each job has only one task, $j$ tasks are completed by time $c_{(j)}(\pi)$ in policy $\pi$. Because policy $P$ is more work-efficient than policy $\pi$, it must hold that at least $j$ tasks are completed during $[0,c_{(j)}(\pi)]$  in policy $P$. Hence, at least $j$ tasks are assigned to the servers during $[0,c_{(j)}(\pi)]$ in policy $P$. Because each job has only one task, it follows that $v_{w_j}(P) \leq c_{(j)}(\pi)$  for all $j=1,\ldots,n$.

%We prove Corollary \ref{coro2} by induction. 

%\emph{Step 2: We show that}
%\begin{align}\label{eq_coro2_3}
%\bm{u}(P)-\bm{d}\prec_{\text{w}} \bm{c} (\pi)-\bm{d}.
%\end{align} 
%
%
%%We show that Thoerem \ref{lem2} holds if \emph{$L_{\max}(\cdot)$} is replaced by any $f\in\mathcal{D}_{\text{Sch-1}}$.} 
%
%We construct two policies $\pi'$ and $\pi''$ based on policy $\pi$: The sequence of job completion times of policy $\pi'$ is a rearrangement (reordering) of that of policy $\pi$, such that for each job $i$ there exists a job $j$ such that $c_i(\pi') = c_j(\pi)$.
%%, i.e., the completion time of any job $i'$ in policy $\pi'$ must be the completion time of some job $i$ in policy $\pi$.
%Furthermore, in policy $\pi'$, each completed job has the earliest due time among all jobs presenting in the queue, such that $c_1(\pi')\leq c_2(\pi') \leq \ldots \leq c_n(\pi')$. Hence, 
%\begin{align}\label{coro2_1}
%c_i(\pi') = c_{(i)}(\pi).
%\end{align}
%On the other hand, the task completion times of policy $\pi''$ is a rearrangement (reordering) of the task completion times of policy $\pi$, and in policy $\pi''$, each completed task belongs to the jobs with the earliest due time among all jobs presenting in the queue. 
%Let $t_i(\pi)$ be the $i$-th smallest task completion time of policy $\pi$, then 
%\begin{align}\label{coro2_2}
%c_i(\pi'') = t_{ik}(\pi).
%\end{align} 
%%i.e., if job $i$ arrives before the completion time of job $j$ and $d_i<d_j$, then job $i$ is completed before job $j$ in policy $\pi'$. 
%%Let $t_i(\pi)$ be the $i$-th smallest task completion time of policy $\pi$. 
%In policy $\pi$, because each job has $k$ tasks, the system must complete at least $k$ tasks before one job is completed, i.e.,
%$c_{(1)}(\pi)\geq t_{k}(\pi)$. In general, the system must complete at least $ik$ tasks before $i$ jobs are completed, i.e., 
%\begin{align}\label{coro2_3}
%c_{(i)}(\pi)\geq t_{ki}(\pi).
%\end{align} 
%By combining \eqref{coro2_1}-\eqref{coro2_3}, we have
%\begin{align}
%c_i(\pi') = c_{(i)}(\pi)\geq t_{ik}(\pi)=c_i(\pi'').
%\end{align}
%We note that policy $\pi''$ is feasible, but policy $\pi'$ is not because 
%
%
%
%
%
%
%
%
%In policy $\pi''$, the task completion times 
%
%
%For this constructed policy $\pi'$, one can use the proof argument of Lemma \ref{lemG4_thm3} to show that
%\begin{eqnarray}\label{eq_pi'}
%\sum_{i:a_i\leq\tau} \gamma_{i,P}(t)\leq \sum_{i:a_i\leq\tau} \xi_{i,\pi'}(t), ~\forall~\tau\in[0,\infty)
%\end{eqnarray}
%holds for all $t\in[0,\infty)$. That is, Lemma \ref{lemG4_thm3}  holds even if policy $\pi$ is replaced by this constructed policy $\pi'$. %Note that if the jobs have more than one tasks, \eqref{eq_pi'} may not hold for the constructed policy $\pi'$.
%%We rearrange the job completion times of policy $\pi$ as follows: Consider any two jobs $i$ and $j$ which simultaneously exist in the queue at some time, i.e., there exists a time $t$ such that $a_i\leq t\leq c_i(\pi)$ and  $a_j\leq t\leq c_j(\pi)$. If $(c_i(\pi)-c_j(\pi))(d_i- d_j)<0$, we interchange the completion times of job $i$ and job $j$. Repeat this procedure until $(c_i(\pi)-c_j(\pi))(d_i- d_j)\geq 0$ is satisfied for any pair of jobs $i$ and $j$ which simultaneously exist in the queue at some time. Hence, after the rearrangement, each completed job has the earliest due time among all jobs in the queue. Let $c_i'(\pi)$ denote the completion time of job $i$ after the rearrangement. 
%
%In the sequel, we will use \eqref{eq_pi'}, Lemma \ref{lem_rearrangement}, and the property of policy $\pi'$ to prove the following two claims:
%\begin{itemize}
%\item[1.] $\bm{c}(\pi')-\bm{d}\prec \bm{c} (\pi)-\bm{d}$;
%\item[2.] $v_i(P)\leq c_i(\pi')$ for $i=1,\ldots,n$.
%\end{itemize}
%
%
%%Hence, the $i$-th smallest job completion time $c_{(i)}(\pi')$ of policy $\pi'$ is equal to $i$-th smallest job completion time $c_{(i)}(\pi)$ of policy $\pi$, i.e., $c_{(i)}(\pi')=c_{(i)}(\pi)$.
%
%First, we prove claim 1. An alternative construction procedure of policy $\pi'$ is provided as follows: Suppose that in policy $\pi$, two jobs $i$ and $j$ co-exist in the queue at some time $t$, i.e., $a_i\leq t\leq c_i(\pi)$ and  $a_j\leq t\leq c_j(\pi)$. If $(c_i(\pi)-c_j(\pi))(d_i- d_j)<0$, the completion times of job $i$ and job $j$ are interchanged. 
%Repeat this pair-wise interchange operation until $(c_i(\pi)-c_j(\pi))(d_i- d_j)\geq 0$ is satisfied for any pair of jobs $i$ and $j$ which co-exist in the queue at some time. Then, the job completion times of policy $\pi'$ are obtained.
%By using Lemma \ref{lem_rearrangement} for each pair-wise interchange operation during this construction procedure of policy $\pi'$, we can obtain $\bm{c}(\pi')-\bm{d}\prec \bm{c} (\pi)-\bm{d}$. By this, claim 1 is proven.
%
%
%Next, we prove claim 2 by contradiction. Suppose that
%\begin{align}\label{eq_contradiction_coro2}
%v_{w_j}(P) > c_{w_j}(\pi')
%\end{align} 
%holds for some $j\in\{1,\ldots,n\}$.
%In policy $\pi'$, if job $i$ arrives before time $c_{w_j}(\pi')$ and $d_i<d_{w_j}$, then job $i$ is completed before time $c_{w_j}(\pi')$. Hence, the system state of policy $\pi'$ satisfies 
%\begin{align}
%\sum_{i:d_i\leq d_{w_j}}\xi_{i,\pi'}(c_{w_j}(\pi')) =0,\nonumber
%\end{align}
%where we have used the fact that $d_i\neq d_j$ if $i\neq j$. Combining this with \eqref{eq_pi'}, we can obtain
%%Hence, there are $y-1$ unfinished jobs at time $C_{w_1}(\pi)$ such that
%%Invoking Lemma \ref{lemG4}, we can obtain
%\begin{align}\label{eq_proof_1_coro2}
%\sum_{i:d_i\leq d_{w_j}} \gamma_{i,P}(c_{w_j}(\pi'))\leq 0.
%\end{align}
%By the definition of the system state, we have $\gamma_{i,P}(t)\geq0$ for all $i$ and $t$. This and \eqref{eq_proof_1_coro2} tells us that at time $c_{w_j}(\pi')$, the system state of policy $P$ satisfies
%\begin{align}
%\gamma_{w_j,P}(c_{w_j}(\pi'))= 0.\nonumber
%\end{align}
%That is, all tasks of job $w_j$ are either completed or under service by time $c_{w_j}(\pi')$ in policy $P$. Hence, $v_{w_j}(P)\leq c_{w_j}(\pi')$, which contradicts with \eqref{eq_contradiction_coro2}. Therefore, $v_{w_j}(P)\leq c_{w_j}(\pi')$ holds for all $j=1,\ldots,n$. By this, claim 2 is proven.
%
%Now, we use claim 1 and claim 2 to prove \eqref{eq_coro2_3}. In particular,  claim 1 and claim 2 suggest that
%\begin{align}
%\bm{u}(P)-\bm{d}\leq \bm{c}(\pi')-\bm{d}\prec \bm{c} (\pi)-\bm{d}.
%\end{align}
%By this and Theorem 5.A.9 of \cite{Marshall2011}, \eqref{eq_coro2_3} follows.
%
%
%\emph{Step 3: We use \eqref{eq_coro2_3} to prove Corollary \ref{coro2}.}
%For any $f\in\mathcal{D}_{\text{Sch-1}}$, $f(\bm{x}+\bm{d})$ is Schur convex. 
%According to Theorem 3.A.8 of \cite{Marshall2011}, for all $f\in\mathcal{D}_{\text{Sch-1}}$, 
%\begin{align}
%&f(\bm{u}(P)) \nonumber\\
%= &f[(\bm{u}(P)-\bm{d})+\bm{d}] \nonumber\\
%\leq& f[(\bm{c}(\pi)-\bm{d})+\bm{d}] \nonumber\\
%=& f(\bm{c} (\pi)).\nonumber
%\end{align} 
%By considering all possible sample paths of these two policies, the stochastic ordering result in Corollary \ref{coro2} follows.
%This completes the proof.
%%\end{proof}
%
%\end{proof}
%
%
%%We develop a {sample-path ordering} technique to prove Thoerem \ref{lem3}. The system state of policy $P$ is the same as that in \emph{Definition \ref{def_state_thm3}}, and the system state of policy $\pi$ are the same as that in \emph{Definition \ref{def_state_P_thm3}}. 
%%
%%
%%We assume that the priorities $p_1,\ldots, p_n$ of the $n$ jobs are distinct from each other. This does not lose any generality, because if $p_i=p_j$ for two jobs $i$ and $j$, Thoerem \ref{lem3} can be proven by taking the limit $p_i\rightarrow p_j$.  The first part of the sample-path ordering result is as follows:
%% 
%% 
%%\begin{lemma}\label{lemG4_lem3}
%%Suppose that $\bm{\gamma}(0^-)=\bm{\zeta}(0^-)=\bm{\xi}(0^-)=\bm{0}$ and the conditions of Thoerem \ref{lem3} are satisfied. Then, the following relationship holds on sample path:
%%\begin{eqnarray}\label{eq_lemG4_lem3}
%%\sum_{i: p_i\geq p} [\gamma_i(t) - \zeta_i(t)]\leq \sum_{i: p_i\geq p} \xi_i(t), ~\forall~p\geq 0.
%%\end{eqnarray}
%%holds for all $t\geq0$.
%%\end{lemma}
%%
%%The following two lemmas are needed to prove Lemma \ref{lemG4_lem3}:
%%
%%
%%\begin{lemma}\label{lem_non_prmp1_lem3}
%%Suppose that, under policy $P$, $\{\bm{\gamma}',\bm{\zeta}'\}$ is obtained by allocating $b$ unassigned tasks to the servers in the system whose state is $\{\bm{\gamma},\bm{\zeta}\}$. Further, suppose that, under policy $\pi$, $\bm{\xi}'$ is obtained by completing $b'$ tasks in the system whose state is $\bm{\beta}$.
%%If $b\geq b'$ and
%%\begin{eqnarray}
%%\sum_{i: p_i\geq p} [\gamma_i - \zeta_i]\leq \sum_{i: p_i\geq p} \xi_i, ~\forall~p\geq 0,\nonumber
%%\end{eqnarray}
%%then
%%\begin{eqnarray}\label{eq_non_prmp_40_lem3}
%%\sum_{i: p_i\geq p} [\gamma_i'- \zeta_i']\leq \sum_{i: p_i\geq p} \xi_i', ~\forall~p\geq 0.\end{eqnarray}
%%\end{lemma}
%%
%%\begin{proof}
%%If $\sum_{i: p_i\geq p} [\gamma_i' - \zeta_i']=0$, then the inequality \eqref{eq_non_prmp_40_lem3} follows naturally. 
%%If $\sum_{i: p_i\geq p} [\gamma_i' - \zeta_i']>0$, then there exist some tasks that have not been assigned to any server. 
%%In policy $P$, each idle server will be allocated to process an unassigned task from the job with the highest priority. Hence,
%%$\sum_{i: p_i\geq p} [\gamma_i' - \zeta_i']=\sum_{i: p_i\geq p} [\gamma_i - \zeta_i] - b \leq \sum_{i: p_i\geq p} \xi_i -b' \leq \sum_{i: p_i\geq p} \xi_i'$.
%%\end{proof}
%%
%%
%%\begin{lemma}\label{lem_non_prmp2_lem3}
%%Suppose that under policy $P$, $\{\bm{\gamma}',\bm{\zeta}'\}$ is obtained by adding a job with $b$ tasks and arrival time $a$ to the system whose state is $\{\bm{\gamma},\bm{\zeta}\}$. Further, suppose that under policy $\pi$, $\bm{\xi}'$ is obtained by adding a job with $b$ tasks and arrival time $a$ to the system whose state is $\bm{\xi}$.
%%If
%%\begin{eqnarray}
%%\sum_{i: p_i\geq p} [\gamma_i- \zeta_i]\leq \sum_{i: p_i\geq p} \xi_i, ~\forall~p\geq 0,\nonumber
%%\end{eqnarray}
%%then
%%\begin{eqnarray}
%%\sum_{i: p_i\geq p} [\gamma_i' - \zeta_i']\leq \sum_{i: p_i\geq p} \xi_i', ~\forall~p\geq 0.\nonumber\end{eqnarray}
%%\end{lemma}
%%
%%\begin{proof}
%%If $a\leq a_j$, then
%%$\sum_{i: p_i\geq p} [\gamma_i' - \zeta_i']\leq \sum_{i: p_i\geq p} [\gamma_i - \zeta_i] + b\leq \sum_{i: p_i\geq p} \xi_i+b \leq \sum_{i: p_i\geq p} \xi_i'$.
%%
%%If $a>a_j$, then
%%$\sum_{i: p_i\geq p} [\gamma_i' - \zeta_i']\leq \sum_{i: p_i\geq p} [\gamma_i - \zeta_i] \leq \sum_{i: p_i\geq p} \xi_i \leq \sum_{i: p_i\geq p} \xi_i'$.
%%\end{proof}
%%
%%The proof of Lemma \ref{lemG4_lem3} is quite similar with that of Lemma \ref{lemG4}, and hence is omitted. The only differences are (i) Lemma \ref{lem_non_prmp1} and Lemma \ref{lem_non_prmp2} in the proof of Lemma \ref{lemG4} should be replaced by Lemma \ref{lem_non_prmp1_lem3} and Lemma \ref{lem_non_prmp2_lem3}, respectively, and (ii) $\bm{\alpha}(t)$, $\bm{\delta}(t)$, and $\bm{\beta}(t)$ in the proof of Lemma \ref{lemG4} should be replaced by $\bm{\gamma}(t)$, $\bm{\zeta}(t)$, and $\bm{\xi}(t)$, respectively.
%%
%%
%%
%%
%%
%%
%%The second part of the sample-path ordering result is as follows:
%%
%%\begin{lemma}\label{lem_sample_path_ordering_lem3}
%%If Lemma \ref{lemG4_lem3} holds, then $\bm{u}_{\uparrow}(P)\leq \bm{c}_{\uparrow}(\pi)$ holds on sample path for all $\pi\in\Pi_{PL}$. 
%%\end{lemma}
%%
%%\begin{proof}
%%Let $w_i$ be the index of the job associated with $v_{(i)}(P)$, then job $w_j$ is the $j$-th job whose tasks are completed or under service in policy $P$. Similar with \eqref{eq_proof_3_thm3} in the proof of Lemma \ref{lem_sample_path_ordering_thm3}, we can obtain
%%\begin{align}
%%v_{w_j}(P) \leq \max_{i:a_i\leq v_{w_j}(P),p_i\geq p_{w_j} }c_{i}(\pi).
%%\end{align}
%%
%%Because job $w_j$ is the $j$-th job whose tasks are completed or under service, only the jobs $w_1,\ldots, w_{j-1}$ can be completed during $[0,v_{w_j}(P))$ in policy $P$.
%%In addition, each idle server is assigned to process a task from the job with the highest priority in  policy $P$. This tells us that job $w_j$ has the highest priority among all jobs in the queue at time $v_{w_j}(P)$ in policy $P$.
%%Therefore, if job $i$ satisfies $a_i\leq v_{w_j}(P)$ and $p_i\leq p_{w_j}$, then $i\in\{w_1,\ldots, w_j\}$. 
%%
%%
%%%We  prove Lemma \ref{lem_sample_path_ordering_lem3} by induction. 
%%Consider the sample paths of policy $P$ and policy $\pi$ in Lemma \ref{lemG4_lem3}. 
%%Recall that $U_i(P)$ is the earliest time that all tasks of job $i$ are either completed or under service in policy $P$, $v_i(P)$ is the realization of $U_i(P)$ on the sample path of policy $P$, and $v_{(i)}(P)$ is the $i$-th smallest component of $(v_{1}(P),\ldots,v_{n}(P))$. Let $w_i$ be the index of the job associated with $v_{(i)}(P)$.
%%
%%%\emph{Step 1: We first show that} 
%%%\begin{align}\label{eq_Condition_3_1_lem3}
%%%v_{w_1}(P) - d_{w_1} \leq c_{w_1}(\pi) - d_{w_1}.
%%%\end{align}
%%%%Let $y_1$ be the number of jobs that have arrived by time $v_{w_1}(P)$. 
%%%
%%%
%%%We prove \eqref{eq_Condition_3_1_lem3} by contradiction. Suppose that 
%%%\begin{align}\label{eq_Condition_3_11_lem3}
%%%v_{w_1}(P) > c_{w_1}(\pi),
%%%\end{align} 
%%%i.e., job $w_1$ is completed earlier than $v_{w_1}(P)$ in policy $\pi$. 
%%%
%%%Because job $w_1$ is the first job whose tasks are either completed or under service, no job is completed during $[0,v_{w_1}(P))$ in policy $P$. Because policy $P$ satisfies condition 2 of Thoerem \ref{lem3}, job $w_1$ has the earliest due time among all jobs in the queue at time $v_{w_1}(P)$ in policy $P$.  This tells us that job $w_1$ has the earliest due time among all jobs that have arrived during $[0,v_{w_1}(P))$.
%%%Hence, when job $w_1$ departs at time $c_{w_1}(\pi)$ in policy $\pi$, $d_i> d_{w_1}$ holds for all jobs in the queue. Therefore, the system state of policy $\pi$ satisfies  
%%%\begin{align}\label{eq_proof_0_lem3}
%%%\sum_{i:d_i\leq d_{w_1}}\xi_i(c_{w_1}(\pi)) =0.
%%%\end{align}
%%%Combining \eqref{eq_proof_0_lem3} and Lemma \ref{lemG4_lem3}, we can obtain
%%%%Hence, there are $y-1$ unfinished jobs at time $C_{w_1}(\pi)$ such that
%%%%Invoking Lemma \ref{lemG4}, we can obtain
%%%\begin{align}\label{eq_proof_1_lem3}
%%%\sum_{i:d_i\leq d_{w_1}} \gamma_i(c_{w_1}(\pi))\leq \sum_{i:d_i\leq d_{w_1}}  \zeta_i(c_{w_1}(\pi)).
%%%\end{align}
%%%By the definition of the system state of policy $P$, we have $\gamma_i(t)\geq \zeta_i(t)$ for all $i$ and $t$. This and \eqref{eq_proof_1_lem3} tells us that at time $c_{w_1}(\pi)$, the system state of policy $P$ satisfies
%%%\begin{align}\label{eq_proof_2_lem3}
%%%\!\!\gamma_{w_1}(c_{w_1}(\pi))= \zeta_{w_1}(c_{w_1}(\pi)).
%%%\end{align}
%%%Hence, in policy $P$ all tasks of job $w_1$ are either completed or under service at time $c_{w_1}(\pi)$. Combine this and \eqref{eq_Condition_3_11_lem3}, yields $$v_{w_1}(P)\leq c_{w_1}(\pi)<v_{w_1}(P),$$ which is a contradiction. Hence, $v_{w_1}(P) \leq c_{w_1}(\pi)$. By this, \eqref{eq_Condition_3_1_lem3} is proven.
%%
%%It is sufficient to show that for each $j=1,2,\ldots,n$,
%%\begin{align}\label{eq_Condition_3_12_lem3}
%%v_{w_j}(P)-d_{w_j} \leq \max_{i=1,2,\ldots,n }[c_{i}(\pi)-d_i].
%%\end{align}
%%We prove \eqref{eq_Condition_3_12_lem3} by contradiction. Suppose that 
%%\begin{align}\label{eq_proof_9_lem3}
%%v_{w_j}(P) > c_{i}(\pi)
%%\end{align}
%%holds for all $i$ satisfying $a_i\leq v_{w_j}(P)$ and $d_i\leq d_{w_j}$. That is, if job $i$ satisfies $d_i\leq d_{w_j}$ and $a_i\leq v_{w_j}(P)$, then job $i$ departs before time $v_{w_j}(P)$.
%%Hence, at time 
%%\begin{align}
%%\tau=\max_{i:a_i\leq v_{w_j}(P),d_i\leq d_{w_j}} c_{i}(\pi),\nonumber
%%\end{align} $d_i> d_{w_j}$ holds for all jobs in the queue in policy $\pi$. Therefore, the system state of policy $\pi$ satisfies  
%%\begin{align}
%%\sum_{i:d_i\leq d_{w_j}}\xi_i(\tau) =0.\nonumber
%%\end{align}
%%Combining this with Lemma \ref{lemG4_lem3}, we can obtain
%%%Hence, there are $y-1$ unfinished jobs at time $C_{w_1}(\pi)$ such that
%%%Invoking Lemma \ref{lemG4}, we can obtain
%%\begin{align}\label{eq_proof_1_lem3}
%%\sum_{i:d_i\leq d_{w_j}} [\gamma_i(\tau)-\zeta_i(\tau)]\leq 0.
%%\end{align}
%%By the definition of the system state of policy $P$, we have $\gamma_i(t)\geq \zeta_i(t)$ for all $i$ and $t$. This and \eqref{eq_proof_1_lem3} tells us that at time $t$, job $w_j$ in policy $P$ satisfies
%%\begin{align}
%%\gamma_{w_j}(\tau)= \zeta_{w_j}(\tau).\nonumber
%%\end{align}
%%That is, in policy $P$ all tasks of job $w_j$ are either completed or under service at time $\tau$. Hence, $v_{w_j}(P)\leq \tau$, which contradicts with  \eqref{eq_proof_9_lem3}. Therefore, $v_{w_j}(P) \leq \max_{i:a_i\leq v_{w_j}(P),d_i\leq d_{w_j} }c_{i}(\pi)$ and
%%\begin{align}
%%v_{w_j}(P)-d_{w_j} &\leq \max_{i:a_i\leq v_{w_j}(P),d_i\leq d_{w_j} }c_{i}(\pi)-d_{w_j} \nonumber\\
%%& \leq \max_{i:a_i\leq v_{w_j}(P),d_i\leq d_{w_j} }[c_{i}(\pi)-d_{i}]\nonumber\\
%%&\leq \max_{i=1,2,\ldots,n }[c_{i}(\pi)-d_i].\nonumber
%%\end{align}
%%Hence, \eqref{eq_Condition_3_12_lem3} is obtained. This completes the proof.
%%\end{proof}
%%By considering all possible sample paths of these two policies, the stochastic ordering result in Thoerem \ref{lem3} follows.
%%\subsection{Proof of Corollary \ref{coro2}}
%%
%%In the proof of Corollary \ref{coro2}, we will need the following rearrangement inequality  : 
%%\begin{lemma} \cite[Theorem 6.F.14]{Marshall2011}\label{lem_rearrangement}
%%Consider two $n$-vectors $(x_1,\dots,x_n)$ and $(y_1,\ldots,y_n)$. If $x_i> x_j$ and $y_i<y_j$ for some indices $i$ and $j$ where $1\leq i<j\leq n$, then 
%%\begin{align}
%%&(x_1\!-\!y_1,\ldots,x_j\!-\!y_i,\ldots,x_i\!-\!y_j,\ldots,x_n\!-\!y_n)\nonumber\\
%%\prec& (x_1\!-\!y_1,\ldots,x_i\!-\!y_i,\ldots,x_j\!-\!y_j,\ldots,x_n\!-\!y_n).\nonumber
%%\end{align}
%%\end{lemma}
%%\ifreport
%%\begin{proof}[Proof of Corollary \ref{coro2}]
%%\else
%%\begin{proof}[of Corollary \ref{coro2}]
%%\fi
%%As in the proof of Lemma \ref{lem_sample_path_ordering_lem3}, let $w_i$ denote the index of the job associated with $v_{(i)}(P)$. 
%%
%%\emph{Step 1: We first show that  for all $j=1,\ldots,n$}
%%\begin{align}\label{eq_coro2_2}
%%v_{w_j}(P) \leq c_{(j)}(\pi).
%%\end{align}
%%
%%Suppose that $b_j$ tasks have been assigned to the servers in policy $P$ by time $c_{(j)}(\pi)$. Since each job has only one task, $j$ tasks are completed by time $c_{(j)}(\pi)$ in policy $\pi$.
%%Because policy $P$ is more work-efficient than policy $\pi$, it must hold that (i) at least $j$ unassigned task are allocated to the servers during $[0,c_{(j)}(\pi)]$  in policy $P$, i.e., $b_j\geq j$, or (ii) all the remaining tasks are under service at time $c_{(j)}(\pi)$  in policy $P$. Obviously, case (ii) belongs to case (i). Because each job has only one task, it follows that $v_{w_j}(P) \leq c_{(j)}(\pi)$  for all $j=1,\ldots,n$.
%%
%%%We prove Corollary \ref{coro2} by induction. 
%%
%%\emph{Step 2: We show that one of the following two cases is true:
%%\begin{itemize}
%%\item[1.] $v_{w_1}(P)\leq c_{w_1}(\pi)$, and $v_{w_{2}}(P)\leq c_{w_{2}}(\pi)$;
%%%\item[2.] $d_{w_j}\leq d_{w_{j+1}}$, $v_{w_j}(P)\leq c_{w_j}(\pi)$, and $v_{w_{j+1}}(P)\leq c_{w_{j+1}}(\pi)$.
%%\item[2.] $v_{w_1}(P)\leq c_{w_{2}}(\pi)$, $v_{w_{2}}(P)\leq c_{w_{1}}(\pi)$, $d_{w_1}\leq d_{w_{2}}$, and $c_{w_{1}}(\pi)>c_{w_{2}}(\pi)$.
%%\end{itemize}}
%%
%%In the proof of Lemma \ref{lem_sample_path_ordering_lem3}, it was shown that 
%%\begin{align}\label{eq_coro2_1}
%%v_{w_j}(P) \leq \max_{i:a_i\leq v_{w_j}(P),d_i\leq d_{w_j} }c_{i}(\pi).
%%\end{align}
%%
%%We first consider $j=1$. Because job $w_1$ is the first job whose tasks are either completed or under service, no job is completed during $[0,v_{w_1}(P))$ in policy $P$. Because policy $P$ satisfies condition 2 of Thoerem \ref{lem3}, job $w_1$ has the earliest due time among all jobs in the queue at time $v_{w_1}(P)$ in policy $P$. This tells us that if job $i$ satisfies $a_i\leq v_{w_1}(P)$ and $d_i\leq d_{w_1}$, then $i=w_1$. Hence,  \eqref{eq_coro2_1} implies 
%%$v_{w_1}(P) \leq c_{w_1}(\pi)$. 
%%
%%For $j=2$, because job $w_2$ is the second job whose tasks are either completed or under service, only  job $w_1$ can be completed during $[0,v_{w_2}(P))$ in policy $P$. Because policy $P$ satisfies condition 2 of Thoerem \ref{lem3}, job $w_2$ has the earliest due time among all jobs in the queue at time $v_{w_2}(P)$ in policy $P$. This tells us that if job $i$ satisfies $a_i\leq v_{w_2}(P)$ and $d_i\leq d_{w_2}$, then $i=w_1$ or $i=w_2$. 
%%
%%If $d_{w_1}> d_{w_2}$, then \eqref{eq_coro2_1} implies $v_{w_2}(P) \leq c_{w_2}(\pi)$. 
%%
%%If $d_{w_1}\leq d_{w_2}$, then \eqref{eq_coro2_1} implies $v_{w_2}(P) \leq \max[c_{w_1}(\pi), c_{w_2}(\pi)]$. We first consider two sub-cases: If $c_{w_1}(\pi)\leq c_{w_2}(\pi)$, then $v_{w_2}(P) \leq c_{w_2}(\pi)$. 
%%If $c_{w_1}(\pi)> c_{w_2}(\pi)$, by \eqref{eq_coro2_2}, we can obtain $v_{w_1}(P) \leq c_{w_2}(\pi)$ and $v_{w_2}(P)\leq c_{w_1}(\pi)$.
%%
%%By summarizing these cases, the claim of \emph{Step 2} follows. 
%%
%%\emph{Step 3: We show that}
%%\begin{align}\label{eq_coro2_3}
%%\bm{u}(P)-\bm{d}\prec_{\text{w}} \bm{c} (\pi)-\bm{d}.
%%\end{align} 
%%
%%We carry out the following operation: 
%%If case 2 of \emph{Step 2} holds, we interchange the completion times of job $w_1$ and job $w_2$. 
%%%By Lemma \ref{lem_rearrangement}, we can obtain
%%%\begin{align}
%%%&(c_{w_2}(\pi)\!-\!d_{w_1},c_{w_1}(\pi)\!-\!d_{w_2},c_{w_3}(\pi)\!-\!d_{w_3},\ldots,c_{w_n}(\pi)\!-\!d_{w_n})\nonumber\\
%%%\prec& (c_{w_1}(\pi)\!-\!d_{w_1},c_{w_2}(\pi)\!-\!d_{w_2},c_{w_3}(\pi)\!-\!d_{w_3},\ldots,c_{w_n}(\pi)\!-\!d_{w_n}).\nonumber
%%%\end{align}
%%If case 1 of \emph{Step 2} holds, there is no interchange. 
%%Let $\bm{c}^{0} (\pi)=\bm{c}(\pi)$ and $\bm{c}^{1} (\pi)$, respectively, denote the completion time vectors of the $n$ jobs before and after this operation. By Lemma \ref{lem_rearrangement}, we can get 
%%\begin{align}
%%\bm{c}^{1} (\pi)-\bm{d}\prec \bm{c}^{0} (\pi)-\bm{d}.\nonumber
%%\end{align}
%%In addition, it holds that $v_{w_1}(P)\leq c^{1}_{w_1}(\pi)$, and $v_{w_{2}}(P)\leq c^{1}_{w_{2}}(\pi)$.	
%%We repeating this operation $n-1$ times. More specifically, in the $l$-th operation, for each $i=1,\ldots,l$ if $d_{w_i}\leq d_{w_{l+1}}$ and $c^{l-1}_{w_{i}}(\pi)>c^{l-1}_{w_{l+1}}(\pi)$, we interchange job $w_i$ and job $w_{l+1}$. Let $\bm{c}^{l} (\pi)$ denote the completion time vectors of the $n$ jobs after the $l$-th operation.
%%Using \eqref{eq_coro2_2}, \eqref{eq_coro2_1}, and condition 2 of Thoerem \ref{lem3}, we can obtain 
%%\begin{align}
%%&\bm{c}^{n-1} (\pi)-\bm{d} \prec \ldots \prec \bm{c}^{1} (\pi)-\bm{d} \prec \bm{c}^{0} (\pi)-\bm{d}, \nonumber\\
%%&\bm{u}(P)\leq \bm{c}^{n-1}(\pi).\nonumber
%%\end{align}
%%Hence,
%%\begin{align}
%%\bm{u}(P)-\bm{d}\leq \bm{c}^{n-1}(\pi)-\bm{d}\prec \bm{c} (\pi)-\bm{d}.\nonumber
%%\end{align} 
%%By this, \eqref{eq_coro2_3} follows. According to Theorem 3.A.8 of \cite{Marshall2011}, $f(\bm{u}(P)-\bm{d}) \leq f(\bm{c} (\pi)-\bm{d})$ holds for all $f\in\mathcal{D}_{\text{Sch}}$. This completes the proof.
%%\end{proof}

==> appendices_5.tex <==
% !TEX root = ./replication.tex

\section{Proofs of Thoerem~4 and Corollary 6} \label{app4}
\subsection{Proof of Thoerem~\ref{thm4}} \label{sec_app_4_1}
We prove Thoerem~\ref{thm4} by using Lemma \ref{lem2}, where the policy space $\Pi$ is replaced by $\Pi_{\text{non-prmp}}$ because preemption is not allowed. The proof steps are as follows:

{\bf Construction of Policy $P'$:}
We construct an {infeasible} policy $P'$. Similar with policy EDD-R, when all servers are idle in policy $P'$, a task from the job with the earliest due time is replicated on all $m$ servers. When a copy of this task is completed, the remaining $m-1$ replicated copies of this task are cancelled. The difference between policy EDD-R and policy $P'$ is that \emph{the completed tasks of policy $P'$ are relabelled such that each completed task is from the job with the earliest due time}. (This relabeling operation might be infeasible in the following scenario: If a job with an earlier due time arrives, the servers cannot be reassigned to this incoming job because preemption is not allowed. However, the next completed task is relabelled to be from this incoming job which has the earliest due time.) By this, policy $P'$ is constructed.

Next, we prove the conditions of Lemma \ref{lem2} one by one.

\textbf{Condition 1:} \emph{Policy $P'$ is more {work-efficient} than any policy $\pi\in\Pi_{\text{non-prmp}}$}. Condition 1 can be proven by using the same proof arguments in Appendix \ref{sec_app_thm2_1}.

\textbf{Condition 2:} \emph{Each completed task of policy $P'$ belongs to the job with the earliest due time}. Condition 2 directly follows from the construction of policy $P'$.

\textbf{Condition 3:} \emph{It holds that} 
\begin{align}\label{eq_condition3_thm4}
[\bm{U}_{}(\text{EDD-R})|\mathcal{I}] \leq_{\text{st}} [\bm{C}_{}(P')|\mathcal{I}].
\end{align}

We prove condition 3 by using the \emph{sample-path ordering} technique. The system state $\bm{\xi}$ of policy $P'$ is the same as that in \emph{Definition \ref{def_state_P_thm3}}. The system state $(\bm{\gamma},\bm{\zeta})$ of policy EDD-R is the same as that in \emph{Definition \ref{def_state_thm3}}. 
In policy EDD-R, all servers are simultaneously assigned to process $m$ replicated copies of the same task. Hence, $\bm{\zeta}$ satisfies
\begin{align}
\zeta_i\in\{0,1\},~\sum_{i=1}^n \zeta_i\leq1.
\end{align}
We can prove that Lemmas \ref{lemG4_thm3}-\ref{lem_non_prmp2_thm3} hold for policy EDD-R. 
Using Lemma \ref{lemG4_thm3}, condition 3 can be proven by using the same proof arguments in Appendix \ref{sec_app_3_1}, where policy EDD-NR should be replaced by policy EDD-R.

After establishing conditions 1-3 of Lemma \ref{lem2} for policy EDD-R,  we can use Lemma \ref{lem2} to prove Theorem \ref{thm4}. This completes the proof.

\subsection{Proof of Corollary~\ref{coro4_2}}  
If $d_1\leq\ldots\leq d_n$, then each completed task of policy EDD-R belongs to the job with the earliest due time. Therefore, policy EDD-R is identical with policy $P'$ constructed in Appendix \ref{sec_app_4_1}. Then, Corollary \ref{coro4_2} follows from Lemma \ref{lem2}. 

\subsection{Proof of Corollary~\ref{coro4_1}} \label{sec_app_4_2} 
Because conditions 1-3 of Lemma \ref{lem2} have been established in Appendix \ref{sec_app_4_1},  Corollary~\ref{coro4_1} directly follows from Corollary \ref{coro2}.

==> appendices_6.tex <==
% !TEX root = ./replication.tex

\section{Proof of Thoerem~5} \label{app5}

\subsection{Proof of \eqref{eq_delaygap1_thm5} in Thoerem~5}
We prove \eqref{eq_delaygap1_thm5} in Thoerem~\ref{thm5} by using Lemma \ref{lem3}. In particular, we will use the \emph{sample-path ordering} technique to prove condition \eqref{eq_lem3_1} of Lemma \ref{lem3}.
We first define the system states of policy PL-NR and any policy $\pi\in\Pi_{PL}$, where $PL=(p_1,\ldots,p_n)$ denote a static priority list.

\begin{definition}\label{def_state_P_thm5}
The system state of policy $\pi\in\Pi_{PL}$ is specified by a pair of $n$-dimensional vectors $\bm{\xi}=(\xi_1,\ldots,\xi_n)$ and $\bm{\kappa}=(\kappa_1,\ldots,\kappa_n)$ with non-negative components. At any time, if job $i$ exists in the system, $\xi_i$ is the number of remaining tasks of job $i$ and $\kappa_i$ out of these $\xi_i$ tasks are under service on some servers; if job $i$ has not arrived at the system or has departed from the system, $\xi_i=\kappa_i=0$. Hence, 
\begin{align}%\label{eq_def_state_P_thm5}
\kappa_i  \leq \xi_i \leq k_{i},~\sum_{i=1}^n \kappa_i \leq m. \nonumber
\end{align}
\end{definition}

\begin{definition}\label{def_state_thm5}
The system state of policy PL-NR is specified by a pair of $n$-dimensional vectors $\bm{\gamma}=(\gamma_1,\ldots,\gamma_n)$ and $\bm{\zeta}=(\zeta_1,\ldots,\zeta_n)$ with non-negative components. 
At any time, if job $i$ exists in the system, then $\gamma_i$ is the number of remaining tasks of job $i$ and $\zeta_i$ out of these $\gamma_i$ tasks are under service on some servers; if job $i$ has not arrived at the system or has departed from the system, then $\gamma_i=\zeta_i=0$.
Hence, 
\begin{align}%\label{eq_def_state_thm5}
\zeta_i  \leq \gamma_i \leq k_{i},~\sum_{i=1}^n \zeta_i \leq m. \nonumber
\end{align}
\end{definition}

Let $\{\bm{\xi}(t),\bm{\kappa}(t),t\geq0\}$ be the state process of policy $\pi$, and $\{\bm{\gamma}(t),\bm{\zeta}(t),t\geq0\}$ be the state process of PL-NR, which are assumed to be right-continuous. 
The sample-path ordering result is stated in the following lemma:
 
 
\begin{lemma}\label{lemG4_thm5}
Suppose that $\bm{\xi}(0^-)=\bm{\kappa}(0^-)=\bm{\gamma}(0^-)=\bm{\zeta}(0^-)=\bm{0}$ and the job parameters $\mathcal{I}$ are given. For any sample path of policy PL-NR, there exists a sample path of policy $\pi$ with the same probability density such that
\begin{eqnarray}\label{eq_lemG4_thm5}
\sum_{i:p_i\geq p} [\gamma_i(t) - \zeta_i(t)]\leq \sum_{i:p_i\geq p} [\xi_i(t)-\kappa_i(t)], 
\end{eqnarray}
holds for all $t\geq0$ and $p = 1,2,\ldots,n$.
\end{lemma}

The following two lemmas are needed to prove Lemma \ref{lemG4_thm5}:


\begin{lemma}\label{lem_non_prmp1_thm5}
Suppose that, under policy PL-NR, $\{\bm{\gamma}',\bm{\zeta}'\}$ is obtained by completing a task on one server in the system whose state is $\{\bm{\gamma},\bm{\zeta}\}$. Further, suppose that, under policy $\pi$, $\{\bm{\xi}',\bm{\kappa}'\}$ is obtained by completing a task on one server in the system whose state is $\{\bm{\xi},\bm{\kappa}\}$. If
\begin{eqnarray}
\sum_{i:p_i\geq p} [\gamma_i - \zeta_i]\leq \sum_{i:p_i\geq p} [\xi_i-\kappa_i], ~\forall~p = 1,2,\ldots,n,\nonumber
\end{eqnarray}
then
\begin{eqnarray}\label{eq_non_prmp_40_thm5}
\sum_{i:p_i\geq p} [\gamma_i'- \zeta_i']\leq \sum_{i:p_i\geq p} [\xi_i'-\kappa_i'], ~\forall~p = 1,2,\ldots,n.\end{eqnarray}
\end{lemma}

\begin{proof}
If $\sum_{i:p_i\geq p} [\gamma_i' - \zeta_i']=0$, then the inequality \eqref{eq_non_prmp_40_thm5} follows naturally. 
If $\sum_{i:p_i\geq p} [\gamma_i' - \zeta_i']>0$, then there exist some tasks that have not been assigned to any server. 
In both policy PL-NR and policy $\pi$, a server that has just completed a task will be allocated to process an unassigned task from the job with the highest priority among all jobs in the queue. Hence,
$\sum_{i:p_i\geq p} [\gamma_i' - \zeta_i']=\sum_{i:p_i\geq p} [\gamma_i - \zeta_i] - 1 \leq \sum_{i:p_i\geq p} [\xi_i-\kappa_i] -1 \leq \sum_{i:p_i\geq p} [\xi_i'-\kappa_i']$.
\end{proof}


\begin{lemma}\label{lem_non_prmp2_thm5}
Suppose that, under policy PL-NR, $\{\bm{\gamma}',\bm{\zeta}'\}$ is obtained by adding a job with $b$ tasks and priority $d$ to the system whose state is $\{\bm{\gamma},\bm{\zeta}\}$. Further, suppose that, under policy $\pi$, $\{\bm{\xi}',\bm{\kappa}'\}$ is obtained by adding a job with $b$ tasks and priority $d$ to the system whose state is $\{\bm{\xi},\bm{\kappa}\}$.
If
\begin{eqnarray}
\sum_{i:p_i\geq p} [\gamma_i- \zeta_i]\leq \sum_{i:p_i\geq p} [\xi_i-\kappa_i], ~\forall~p = 1,2,\ldots,n,\nonumber
\end{eqnarray}
then
\begin{eqnarray}
\sum_{i:p_i\geq p} [\gamma_i' - \zeta_i']\leq \sum_{i:p_i\geq p} [\xi_i'-\kappa_i'], ~\forall~p = 1,2,\ldots,n.\nonumber\end{eqnarray}
\end{lemma}

\begin{proof}
If $d\geq p$, then
$\sum_{i:p_i\geq p} [\gamma_i' - \zeta_i']\leq \sum_{i:p_i\geq p} [\gamma_i - \zeta_i] + b\leq \sum_{i:p_i\geq p} [\xi_i-\kappa_i]+b \leq \sum_{i:p_i\geq p} [\xi_i'-\kappa_i']$.

If $d<p$, then
$\sum_{i:p_i\geq p} [\gamma_i' - \zeta_i']\leq \sum_{i:p_i\geq p} [\gamma_i - \zeta_i] \leq \sum_{i:p_i\geq p} [\xi_i-\kappa_i] \leq \sum_{i:p_i\geq p} [\xi_i'-\kappa_i']$.
\end{proof}

Now we are ready to prove Lemma \ref{lemG4_thm5}.
\ifreport
\begin{proof}[Proof of Lemma \ref{lemG4_thm5}]
\else
\begin{proof}[of Lemma \ref{lemG4_thm5}]
\fi
Consider any period $[\tau,\nu)$ of policy PL-NR, during which there are at least $m$ tasks such that all $m$ servers are busy. We prove \eqref{eq_lemG4_thm5} for $t\in[\tau,\nu)$ by considering two cases:

\emph{Case 1: At time $t=\tau$, policy PL-NR has $m$ tasks and the service of these tasks has just started.} Consider the system states of both policies at time $\tau$. The system state of policy PL-NR satisfies 
\begin{align}\label{proof_lemG4_1_thm5}
\sum_{i=1}^n \gamma_i(\tau)= m, ~\bm{\gamma}(\tau)=\bm{\zeta}(\tau).
\end{align}
In policy $P'$, there is no task in the system at time $\tau^-$ such that 
\begin{align}\label{proof_lemG4_5_thm5}
\bm{\xi}(\tau^-)=\bm{0}. 
\end{align}
Consider the evolutions of both policies during $[\tau,\nu)$. 
In policy $P'$, all servers are busy if there is at least one task. On the other hand, in policy EDD-NR, there is no task replication and all servers are busy if there are no less than $m$ tasks. 
By \eqref{proof_lemG4_1_thm5} and \eqref{proof_lemG4_5_thm5}, it holds that for $t=\tau$
\begin{align}\label{proof_lemG4_4_thm5}
\sum_{i=1}^n \gamma_i(t)= \sum_{i=1}^n\xi_i(t) +m\geq m+1.
\end{align}
Therefore, the servers are all busy in policies $P'$ and policy EDD-NR at time $\tau$. By induction over time, we can show that for any sample path of policy $P'$, there is a sample path of policy EDD-NR with the same probability density such that \eqref{proof_lemG4_4_thm5} holds for all $t\in[\tau,\nu)$ and the task arrival times and task completion times of the two policies are exactly the same  during $[\tau,\nu)$. Using Lemma \ref{lem_non_prmp1_thm5}, Lemma \ref{lem_non_prmp2_thm5}, and the initial states at time $\tau^-$, we can prove that \eqref{eq_lemG4_thm5} holds for all $t\in[\tau,\nu)$ on these two sample paths.

\emph{Case 2: At time $t=\tau^-$, policy EDD-NR has less than $m$ tasks or the service of these tasks started before time $\tau^-$}. In both \emph{Case 1} and \emph{Case 2}, the sample path evolutions of policy $P'$ are the same. On the other hand, in policy EDD-NR, the tasks are completed earlier in \emph{Case 2} than in \emph{Case 1}. Therefore, \eqref{eq_lemG4_thm5}  also holds in \emph{Case 2} for $t\in[\tau,\nu)$.

%Note that the case that policy EDD-NR has more than $m$ tasks at time $\tau^-$ will not happen. This will be clear 
Let $[\tau_1,\nu_1)$ be the next busy period of policy $P'$ with $\nu<\tau_1$. Then, $[\nu,\tau_1)$ is an idle period of policy $P'$. We now prove \eqref{eq_lemG4_thm5} during the idle period $[\nu,\tau_1)$. 
Because all servers are idle during $[\nu,\tau_1)$ in policy $P'$, it follows that 
\begin{align}\label{proof_lemG4_2_thm5}
\bm{\xi}(t)=\bm{0},~t\in[\nu,\tau_1).
\end{align}
Hence, there is no task arrival during $[\nu,\tau_1)$; otherwise, \eqref{proof_lemG4_2_thm5} cannot be true.
On the other hand, at time $\nu$ there are no more than $m$ tasks in policy EDD-NR such that 
\begin{align}
\bm{\gamma}(\nu)=\bm{\zeta}(\nu).\nonumber
\end{align}
Because there is no task arrival during $[\nu,\tau_1)$, policy EDD-NR satisfies
\begin{align}\label{proof_lemG4_3_thm5}
\bm{\gamma}(t)=\bm{\zeta}(t),~t\in[\nu,\tau_1).
\end{align}
By \eqref{proof_lemG4_2_thm5} and \eqref{proof_lemG4_3_thm5}, \eqref{eq_lemG4_thm5} holds during $[\nu,\tau_1)$.
Further, from \eqref{proof_lemG4_3_thm5}, we can obtain
\begin{align}
\sum_{i=1}^n \gamma_i(\tau_1^-)=\sum_{i=1}^n \zeta_i(\tau_1^-)\leq m,
\end{align}
such that there are no more than $m$ tasks at time $t=\tau_1^-$ in policy EDD-NR. Hence, either \emph{Case 1} or \emph{Case 2} is satisfied at time $t=\tau_1^-$. Then, we can use the above arguments to prove that  \eqref{eq_lemG4_thm5} holds during the next busy period $[\tau_1,\nu_1)$ of policy $P'$.


Finally, by taking an induction over the busy and idle periods of policy $P'$,  Lemma \ref{lemG4_thm5} is proven.
\end{proof}



After establishing conditions 1-3 of Lemma \ref{lem2} for policy EDD-R,  we can use Lemma \ref{lem2} to prove Theorem \ref{thm4}. This completes the proof.

\subsection{Proof of Corollary~\ref{coro4_2}}  
If $d_1\leq\ldots\leq d_n$, then each completed task of policy EDD-R belongs to the job with the earliest due time. Therefore, policy EDD-R is identical with policy $\pi$ constructed in Appendix \ref{sec_app_4_1}. Then, Corollary \ref{coro4_2} follows from Lemma \ref{lem2}. 

\subsection{Proof of Corollary~\ref{coro4_1}} \label{sec_app_4_2} 
Because conditions 1-3 of Lemma \ref{lem2} have been established in Appendix \ref{sec_app_4_1},  Corollary~\ref{coro4_1} directly follows from Corollary \ref{coro2}.

==> appendices_lem1_0.tex <==
\section{Proof of Proposition \ref{lem1_0}} \label{app_lem1_0}

The following two lemmas are needed to prove Proposition \ref{lem1_0}:  

\begin{lemma}\cite[Lemmas 1-2]{Smith78}\label{lem_non_prmp1_0}
Suppose that under policy $P$, $\{\bm{\xi}_{P}',\bm{\gamma}_{P}'\}$ is obtained by completing $b_P$ tasks in the system whose state is $\{\bm{\xi}_{P},\bm{\gamma}_{P}\}$. Further, suppose that under policy $\pi$, $\{\bm{\xi}_{\pi}',\bm{\gamma}_{\pi}'\}$ is obtained by completing $b_\pi$ tasks in the system whose state is $\{\bm{\xi}_{\pi},\bm{\gamma}_{\pi}\}$.
If $b_P\geq b_\pi$, policy $P$ satisfies condition 3 of Proposition \ref{lem1_0}, and 
\begin{eqnarray}\label{eq_non_prmp_41_0}
\sum_{i=j}^n {\xi}_{[i],P}\leq \sum_{i=j}^n {\xi}_{[i],\pi}, ~j = 1,2,\ldots,n,\nonumber
\end{eqnarray}
then
\begin{eqnarray}\label{eq_non_prmp_40_0}
\sum_{i=j}^n {\xi}_{[i],P}'\leq \sum_{i=j}^n {\xi}_{[i],\pi}', ~j = 1,2,\ldots,n.
\end{eqnarray}
\end{lemma}




\begin{lemma}\cite[Lemma 3]{Smith78}\label{lem_non_prmp2_0}
Suppose that, under policy $P$, $\{\bm{\xi}_{P}',\bm{\gamma}_{P}'\}$ is obtained by adding a job with $b$ tasks to the system whose state is $\{\bm{\xi}_{P},\bm{\gamma}_{P}\}$. Further, suppose that, under policy $\pi$, $\{\bm{\xi}_{\pi}',\bm{\gamma}_{\pi}'\}$ is obtained by adding a job with $b$ tasks to the system whose state is $\{\bm{\xi}_{\pi},\bm{\gamma}_{\pi}\}$.
If
\begin{eqnarray}
\sum_{i=j}^n {\xi}_{[i],P}\leq \sum_{i=j}^n {\xi}_{[i],\pi}, ~j = 1,2,\ldots,n,\nonumber
\end{eqnarray}
then
\begin{eqnarray}
\sum_{i=j}^n {\xi}_{[i],P}'\leq \sum_{i=j}^n {\xi}_{[i],\pi}', ~j = 1,2,\ldots,n.\nonumber
\end{eqnarray}
\end{lemma}


We now use Lemma \ref{lem_non_prmp1_0} and Lemma \ref{lem_non_prmp2_0} to prove Proposition \ref{lem1_0}.
\ifreport
\begin{proof}[Proof of Proposition \ref{lem1_0}]
\else
\begin{proof}[of Proposition \ref{lem1_0}]
\fi

Because policy $P$ is more work-efficient than policy $\pi$, the sequence of task completion times in policy $P$ are  smaller  than those in policy $\pi$, i.e., 
\begin{align}
(t_{1,P},\ldots, t_{k_{\text{sum}},P}) \leq(t_{1,\pi},\ldots, t_{k_{\text{sum}},\pi}). \nonumber
\end{align} 

We modify the sample-path of policy $P$ as follows:  Suppose that for each $i=1,\ldots, k_{\text{sum}}$  a task of job $j_i$ is completed at time $t_{i,P}$ on the original sample-path of policy $P$, then on the modified sample-path of policy $P$ a task of job $j_i$ is completed at time $t_{i,\pi}$. By this modification, the task completion times of policy $P$ are postponed, but the order of completed tasks remain the same. 
Let $\hat{\bm{\xi}}_{P}(t) =(\hat{\xi}_{1,P}(t),\ldots,\hat{\xi}_{n,P}(t))$ and $\hat{\bm{\gamma}}_{P}(t) =(\hat{\gamma}_{1,P}(t),\ldots,\hat{\gamma}_{n,P}(t))$ denote the system state on the modified sample-path of policy $P$. Because the task completion times are postponed,  we can get ${\xi}_{i,P}(t)  \leq \hat{\xi}_{i,P}(t) $ for all $t\geq 0$ and $i=1,\ldots,n$. Hence, for all $t\in[0,\infty)$
\begin{align}\label{eq_lem1_0_proof_1}
\sum_{i=j}^n {\xi}_{[i],P}(t)\leq \sum_{i=j}^n \hat{\xi}_{[i],P}(t), ~i=1,2,\ldots,n.
\end{align}

Next, we compare policy $\pi$ with the modified sample-path of policy $P$. By the foregoing modification, \emph{the task completion times are identical on the sample-path of policy $\pi$ and on the modified sample-path of policy $P$.} 
 
On the original sample-path of policy $P$, each task completing service  is from the job with the fewest remaining tasks among all jobs in the queue. On the modified sample-path of policy $P$, there are more jobs in the queue at the postponed   task completion times due to additional job arrivals. Because $k_1\leq k_2\leq \ldots\leq k_n$, later arrived jobs have more tasks. Hence, on the modified sample-path of policy $P$, each task completing service  is still from the job with the fewest remaining tasks among all jobs in the queue. In other words, \emph{condition 3 of Proposition \ref{lem1_0} is satisfied on the modified sample-path of policy $P$}. 

Because $\hat{\bm{\xi}}_{P}(0) = {\bm{\xi}}_{\pi}(0) =\bm{0}$, by using Lemma \ref{lem_non_prmp1_0} and Lemma \ref{lem_non_prmp2_0}, and taking an induction on the job arrival events and task completion events over time, we can obtain for all $t\in[0,\infty)$
% Then, by using the arguments in \cite{Smith78} we can show 
\begin{align}\label{eq_lem1_0_proof_2}
\sum_{i=j}^n \hat{\xi}_{[i],P}(t)\leq \sum_{i=j}^n {\xi}_{[i],\pi}(t), ~i=1,2,\ldots,n.
\end{align}
Combining \eqref{eq_lem1_0_proof_1} and \eqref{eq_lem1_0_proof_2}, yields \eqref{eq_ordering_1_1}. Then, \eqref{eq_ordering_1_1_2} and \eqref{eq_ordering_1_2} follow from Lemma \ref{ordering_1}, which completes the proof. \end{proof}

%Assume that no task is completed at the job arrival time $a_i$ for $i=1,\ldots,n$. This does not lose any generality, because if a task is completed at time $t_j=a_i$, Proposition \ref{lem1} can be proven by first proving for the case $t_j=a_i+\epsilon$ and then taking the limit $\epsilon\rightarrow 0$. 
%We prove \eqref{eq_ordering_2_1} by induction. 
%
%\emph{Step 1: We will show that \eqref{eq_ordering_2_1} holds during $[0,a_2)$.} 
%
%Because $\bm{\xi}_{P}(0^-) = \bm{\gamma}_{P}(0^-) =\bm{\xi}_{\pi}(0^-) = \bm{\gamma}_{\pi}(0^-)=\bm{0}$, \eqref{eq_ordering_2_1} holds at time $0^-$. Job 1 arrives at time $a_1=0$. By Lemma \ref{lem_non_prmp2}, \eqref{eq_ordering_2_1} holds at time $0$. Let $t$ be an arbitrarily chosen time during $(0,a_{2})$. Suppose that  $b_\pi$ tasks start execution and complete execution during $[0,t]$ in policy $\pi$. We need to consider two cases: 
%
%Case 1: There exist unassigned tasks which are not under service during $[0,t]$ in policy $P$. By the weak work-efficiency ordering, no fewer than $b_\pi$ tasks start execution during $[0,t]$ in policy $P$. Because \eqref{eq_ordering_2_1} holds at time $0$, by Lemma \ref{lem_non_prmp1}, \eqref{eq_ordering_2_1} also holds at time $t$. 
%
%Case 2: All tasks in the system are under service by time $t'\in[0,t]$ in policy $P$. Because $t\in(0,a_{2})$ and there is no task arrival during $(0,a_2)$, there is no task arrival during $(t',t]$. Hence, it must holds that all tasks in the system are under service at time $t$. Then, the system state of policy $P$ satisfies $\sum_{i=j}^n {\gamma}_{[i],P}(t)=0$ for all $j=1,2,\ldots,n$ at time $t$. Hence, \eqref{eq_ordering_2_1} holds at time $t$. 
%
%
%
%
%In summary of these two cases, \eqref{eq_ordering_2_1} holds for all $t\in[0,a_2)$.  
%
%
%
% 
%
%
%\emph{Step 2: Assume that for some integer $i\in\{2,\ldots, n\}$, the conditions of Proposition \ref{lem1} imply that \eqref{eq_ordering_2_1} holds for all $t\in[0,a_i)$. We will prove that the conditions of Proposition \ref{lem1} imply that  \eqref{eq_ordering_2_1} holds for all $t\in[0,a_{i+1})$.}
%
%
%Let $t$ be an arbitrarily chosen time during $(a_i,a_{i+1})$. We modify the task completion times in policy $\pi$ as follows: For each pair of corresponding task $j$ and task $j'$ mentioned in the definition of the weak work-efficiency ordering, if 
%%After this modification, the following three properties are true:
%\begin{itemize}
%\item in policy $\pi$, task $j$ starts execution at time $\tau\in[0,a_i]$ and completes execution at time $\nu\in(a_i,t]$,
%\item in policy $P$, there exist unassigned tasks in the queue during $[\tau,\nu]$,
%\item in policy $P$, the corresponding task $j'$ starts execution at time $t'\in[0,a_i]$,
%\end{itemize}
%then the completion time of task $j$ is modified from $\nu$ to $a_i^-$ in policy $\pi$, as illustrated in Fig. \ref{fig_modification}.
%
%This modification satisfies the following three claims:
%\begin{itemize}
%\item[1.] The system state of policy $\pi$ at time $t$ remains the same before and after this modification;
%\item[2.] Policy $P$ is still weakly more work-efficient than policy $\pi$ after this modification;
%\item[3.] If $b_\pi$ tasks complete execution during $[a_i,t]$ on the modified sample path of policy $\pi$, and there exist unassigned tasks in the queue during $[a_i,t]$ in policy $P$, then no fewer than $b_\pi$ tasks start execution during $[a_i,t]$ in policy $P$.
%\end{itemize}
%We now prove these three claims. Claim 1 follows from the fact that the tasks completed during $[0,t]$ are the same before and after this modification. It is easy to prove claim 2 by the definition of work-efficiency ordering. For claim 3, notice that if a task $j$ completes execution during $[a_i,t]$ on the modified sample path of policy $\pi$, then its corresponding task $j$ must start execution during $[a_i,t]$ in policy $P$. By this, claim 3 follows.
%
%
%
%\ifreport
%\begin{figure}
%\centering 
%\includegraphics[width=0.7\textwidth]{Figures/modification} \caption{Illustration of the modification of task completion times in policy $\pi$: If in policy $\pi$, task $j$ starts execution at time $\tau\in[0,a_i]$ and completes execution at time $\nu\in(a_i,t]$, and in policy $P$, task $j'$ starts execution at time $t'\in[0,a_i]$, then the completion time of task $j$ is changed from $\nu$ to $a_i^-$ in policy $\pi$.}
%\label{fig_modification} 
%\end{figure} 
%\fi
%
%
%
%
%
%We use these three claims to prove the  statement of \emph{Step 2}. According to claim 2, policy $P$ is still weakly more work-efficient than policy $\pi$ after the modification. By the assumption of \emph{Step 2}, \eqref{eq_ordering_2_1} holds during $[0,a_i)$ for the modified sample path of policy $\pi$. Job $j$ arrives at time $a_i$. By Lemma \ref{lem_non_prmp2}, \eqref{eq_ordering_2_1} holds at time $a_i$ for the modified sample path of policy $\pi$. Suppose that $b_\pi$ tasks complete execution during $[a_i,t]$ on the modified sample path of policy $\pi$.
%We need to consider two cases: 
%
%Case 1: There exist unassigned tasks which are not under service during $[a_i,t]$ in policy $P$. By claim 3, no fewer than $b_\pi$ tasks start execution during $[a_i,t]$ in policy $P$. Because \eqref{eq_ordering_2_1} holds at time $a_i$, by Lemma \ref{lem_non_prmp1}, \eqref{eq_ordering_2_1} also holds at time $t$ for the modified sample path of policy $\pi$. 
%
%Case 2: All tasks in the system are under service at some time $t'\in[a_i,t]$ in policy $P$. Because $t\in(a_i,a_{i+1})$ and $t'\in[a_i,t]$, there is no task arrival during $(t',t]$. Hence, it must holds that all tasks in the system are under service at time $t$. Then, the system state of policy $P$ satisfies $\sum_{i=j}^n {\gamma}_{[i],P}(t)=0$ for all $j=1,2,\ldots,n$  at time $t$. Hence, \eqref{eq_ordering_2_1} holds at time $t$ for the modified sample path of policy $\pi$. 
%
%
%
%
%
%
%In summary of these two cases, \eqref{eq_ordering_2_1} holds at time $t$ for the modified sample path of policy $\pi$. By claim 1, the system state of policy $\pi$ at time $t$ remains the same before and after this modification. Hence, \eqref{eq_ordering_2_1} holds at time $t$ for the original sample path of policy $\pi$. Therefore, if  the assumption of \emph{Step 2} is true, then \eqref{eq_ordering_2_1} holds for all $t\in[0,a_{i+1})$. 
%
%% each task (index by $j$) completed during $[0,t]$ in policy $\pi$, we modify the completion time of task $j$ as follows
%%
%%
%%Suppose that $g$ tasks are assigned to the servers during $[a_i,t]$ in policy $P$, and $h$ tasks are completed during $[a_i,t]$ in policy $\pi$. 
%%
%%If $g\geq h$, then by Lemma \ref{lem_non_prmp1} tells us that \eqref{eq_ordering_2_1} holds for all $t\in(a_i,a_{i+1})$. 
%%
%%If $g< h$, suppose that $h'$ tasks ($h'\leq h$) are assigned to the servers during $[a_i,t]$ and are  completed during $[a_i,t]$ in policy $\pi$. Hence, $h-h'$ tasks are assigned to the servers during $[0,a_i)$ and are completed during $[a_i,t]$ in policy $\pi$. Because policy $P$ is more work-efficient than policy $\pi$,  in policy $P$ one of the following cases holds: (i) no fewer than $h'$ unassigned tasks are allocated to the servers during $[a_i,t]$, i.e., $h'\leq g$, (ii) all the remaining tasks are under service at time $t'\in[a_i,t]$, or (iii) the queue is empty at time $t'\in[a_i,t]$.
%%
%%
%%If case (i) happens, %we can obtain that $h-h'$ tasks are assigned to the servers during $[0,a_i)$ and are completed during $[a_i,t]$ in policy $\pi$. 
%% We modify the completion times of these $h-h'$ tasks such that these $h-h'$ tasks are completed at time $a_i^-$ on the modified sample path of policy $\pi$. After this modification, the conditions of Proposition \ref{lem1} still hold and the system state $\bm{\beta}(t)$ of policy $\pi$ at time $t$ remains the same. Hence, we only need to prove \eqref{eq_ordering_2_1} at time $t$ on this modified sample path of policy $\pi$. In particular, by the assumption of \emph{Step 2}, \eqref{eq_ordering_2_1} holds during $[0,a_i)$ on this modified sample path of policy $\pi$. Job $j$ arrives at time $a_i$. By Lemma \ref{lem_non_prmp2}, \eqref{eq_ordering_2_1} holds at time $a_i$ on this modified sample path of policy $\pi$. By Lemma \ref{lem_non_prmp1} and $h'\leq g$, we can obtain that \eqref{eq_ordering_2_1} holds at time $t$ on the modified sample path of policy $\pi$. Hence, \eqref{eq_ordering_2_1} also holds at time $t$ on the original sample path of policy $\pi$.
%%
%%
%%If case (ii) happens, because there is no task arrival during $(t',t]$, it must holds that all the remaining tasks are under service at time $t$. Then, the system state of policy $P$ at time $t$ satisfies $\sum_{i=j}^n [\alpha_h(t)- \delta_h(t)]=0$ for all $h=1,2,\ldots$ Hence, \eqref{eq_ordering_2_1} holds at time $t$. If case (iii) happens, because there is no task arrival during $(t',t]$, it must holds that the queue is empty at time $t$. Similar with case (ii), we can show that \eqref{eq_ordering_2_1} holds at time $t$. In summary, if  the assumption of \emph{Step 2} is true, then \eqref{eq_ordering_2_1} holds for all $t\in[0,a_{i+1})$. 
%By induction, \eqref{eq_ordering_2_1} holds at time $t\in[0,\infty)$. Then, \eqref{eq_ordering_2_2} and \eqref{eq_ordering_2_3} follow from Lemma \ref{ordering_1}.
%This completes the proof.


==> appendices_lem2_0.tex <==
\section{Proof  of Proposition \ref{lem2_0}} \label{app_lem2_0}

The proof of Proposition \ref{lem2_0} requires the following two lemmas:

\begin{lemma}\label{lem_non_prmp1_thm3_0}
Suppose that, in policy $P$, $\{\bm{\xi}_P',\bm{\gamma}_P'\}$ is obtained by completing $b_P$ tasks in the system whose state is $\{\bm{\xi}_P,\bm{\gamma}_P\}$. Further, suppose that, in policy $\pi$, $\{\bm{\xi}_\pi',\bm{\gamma}_\pi'\}$ is obtained by completing $b_\pi$ tasks in the system whose state is $\{\bm{\xi}_\pi,\bm{\gamma}_\pi\}$.
If $b_P\geq b_\pi$, condition 3 of Proposition \ref{lem2_0} is satisfied in policy $P$, and
\begin{eqnarray}
\sum_{i:d_i\leq\tau} \xi_{i,P}\leq \sum_{i:d_i\leq\tau} \xi_{i,\pi}, ~\tau\in[0,\infty),\nonumber
\end{eqnarray}
then
\begin{eqnarray}\label{eq_non_prmp_40_thm3_0}
\sum_{i:d_i\leq\tau} \xi_{i,P}'\leq \sum_{i:d_i\leq\tau} \xi_{i,\pi}', ~\tau\in[0,\infty).\end{eqnarray}
\end{lemma}

\begin{proof}
If $\sum_{i:d_i\leq\tau} \xi_{i,P}'=0$, then the inequality \eqref{eq_non_prmp_40_thm3} follows naturally. 
If $\sum_{i:d_i\leq\tau} \xi_{i,P}'>0$, then there exist some remaining tasks. 
In policy $P$, each task completing service is from the job with the earliest due time. Hence,
$\sum_{i:d_i\leq\tau} \xi_{i,P}'=\sum_{i:d_i\leq\tau} \xi_{i,P} - b_P \leq \sum_{i:d_i\leq\tau} \xi_{i,\pi} -b_\pi \leq \sum_{i:d_i\leq\tau} \xi_{i,\pi}'$.
\end{proof}


\begin{lemma}\label{lem_non_prmp2_thm3_0}
Suppose that under policy $P$, $\{\bm{\xi}_P',\bm{\gamma}_P'\}$ is obtained by adding a job with $b$ tasks and due time $d$ to the system whose state is $\{\bm{\xi}_P,\bm{\gamma}_P\}$. Further, suppose that under policy $\pi$, $\{\bm{\xi}_\pi',\bm{\gamma}_\pi'\}$ is obtained by adding a job with $b$ tasks and due time $d$ to the system whose state is $\{\bm{\xi}_\pi,\bm{\gamma}_\pi\}$.
If
\begin{eqnarray}
\sum_{i:d_i\leq\tau} \xi_{i,P}\leq \sum_{i:d_i\leq\tau} \xi_{i,\pi}, ~\tau\in[0,\infty),\nonumber
\end{eqnarray}
then
\begin{eqnarray}
\sum_{i:d_i\leq\tau} \xi_{i,P}'\leq \sum_{i:d_i\leq\tau} \xi_{i,\pi}', ~\tau\in[0,\infty).\nonumber\end{eqnarray}
\end{lemma}

\begin{proof}
If $d\leq\tau$, then
$\sum_{i:d_i\leq\tau} \xi_{i,P}'\leq \sum_{i:d_i\leq\tau} \xi_{i,P} + b\leq \sum_{i:d_i\leq\tau} \xi_{i,\pi}+b \leq \sum_{i:d_i\leq\tau} \xi_{i,\pi}'$.

If $d>\tau$, then
$\sum_{i:d_i\leq\tau} \xi_{i,P}'\leq \sum_{i:d_i\leq\tau} \xi_{i,P} \leq \sum_{i:d_i\leq\tau} \xi_{i,\pi} \leq \sum_{i:d_i\leq\tau} \xi_{i,\pi}'$.
\end{proof}


\begin{proof}[Proof of Proposition \ref{lem2_0}]

Because policy $P$ is more work-efficient than policy $\pi$, the task completion times in policy $P$ are smaller  than those in policy $\pi$, i.e., 
\begin{align}
(t_{1,P},\ldots, t_{k_{\text{sum}},P}) \leq(t_{1,\pi},\ldots, t_{k_{\text{sum}},\pi}). \nonumber
\end{align} 

We modify the sample-path of policy $P$ as follows:  Suppose that for each $i=1,\ldots, k_{\text{sum}}$  a task of job $j_i$ is completed at time $t_{i,P}$ on the original sample-path of policy $P$, then on the modified sample-path of policy $P$ a task of job $j_i$ is completed at time $t_{i,\pi}$. Hence, the task completion times of policy $P$ are postponed after the modification, but the order of completed tasks remain the same. 
Let $\hat{\bm{\xi}}_{P}(t) =(\hat{\xi}_{1,P}(t),\ldots,\hat{\xi}_{n,P}(t))$ and $\hat{\bm{\gamma}}_{P}(t) =(\hat{\gamma}_{1,P}(t),\ldots,\hat{\gamma}_{n,P}(t))$ denote the system state on the modified sample-path of policy $P$. Then, at any time $t$ we can get ${\xi}_{i,P}(t)  \leq \hat{\xi}_{i,P}(t) $ for $i=1,\ldots,n$ and hence
\begin{align}\label{eq_lem2_0_proof_1}
\sum_{i:d_i\leq\tau} {\xi}_{i,P}(t)\leq \sum_{i:d_i\leq\tau} \hat{\xi}_{i,P}(t), ~\tau\in[0,\infty).
\end{align}

Next, we compare policy $\pi$ with the modified sample-path of policy $P$. By the foregoing construction, \emph{the task completion times are identical on the sample-path of policy $\pi$ and on the modified sample-path of policy $P$.}
 
On the original sample-path of policy $P$, each task completing service  is from the job with the earliest due time among all jobs in the queue. Furthermore, because $k_1\leq k_2\leq \ldots\leq k_n$, later arrived jobs have more tasks. Hence, on the modified sample-path of policy $P$, each task completing service  is also from the job with the earliest due time among all jobs in the queue. In other words, \emph{condition 3 of Proposition \ref{lem2_0} is satisfied on the modified sample-path of policy $P$}. 

Because $\hat{\bm{\xi}}_{P}(0) = {\bm{\xi}}_{\pi}(0) =\bm{0}$, by using Lemma \ref{lem_non_prmp1_thm3_0} and Lemma \ref{lem_non_prmp2_thm3_0}, and taking an induction on the job arrival events and task completion events over time, we can obtain for all $t\in[0,\infty)$
% Then, by using the arguments in \cite{Smith78} we can show 
\begin{align}\label{eq_lem2_0_proof_2}
\sum_{i:d_i\leq\tau} \hat{\xi}_{i,P}(t)\leq \sum_{i:d_i\leq\tau} {\xi}_{i,\pi}(t), ~i=1,2,\ldots,n.
\end{align}
Combining \eqref{eq_lem2_0_proof_1} and \eqref{eq_lem2_0_proof_2}, yields \eqref{eq_ordering_3_1}. Then, \eqref{eq_ordering_3_2} follow from Lemma \ref{ordering_3}, which completes the proof. \end{proof}



==> distributed.tex <==
% !TEX root = ./replication.tex

\section{Replications in Distributed Queueing Systems}\label{sec_distributed}
In this section, we propose replication policies for distributed queueing systems with data-locality constraints,\footnote{Note that if there is no data-locality constraints, each task can be replicated on all servers. In this case, a distributed queueing system can be equivalently viewed as a centralized queueing system and all results in Section \ref{sec_analysis} apply.} and prove that these policies are near delay-optimal for minimizing several classes of delay metrics. To the extent of our knowledge, these are the first results on delay-optimal replications in distributed queueing systems with data-locality constraints.

%, and more general  delay metrics. 


%We will not use study the FUT scheduling principle 

%\subsection{Equivalent System Model}
%First 


\subsection{An Equivalent Hierarchical Distributed Queueing Model}
%The sufficient conditions obtained in Section \ref{sec_sufficient} cannot be directly applied to distributed queueing systems with  data-locality constraints, because these sufficient conditions require policy $P$ to be work-conserving. However, due to data-locality constraints, some groups of servers may be idle while the other groups of servers are busy, and hence policy $P$ cannot be work-conserving. 

%In order to resolve this problem, we propose a hierarchical distributed queueing model of the system, as illustrated in Fig. \ref{fig1model_distri_eq}, which is equivalent with the distributed queueing model in Section \ref{sec:model}. 
There are two types of data locality constraints: per-task constraints and per-job constraints \cite{Sparrow:2013}. In per-task  constraints, the tasks of one job may have a different group of servers on which it can run; while in per-job constraints, all tasks of one job must be executed on the same group of servers. Per-task constraints are more general than per-job constraints, and are also more difficult to handle. Both types of constraints play an important role in cloud computing clusters \cite{taskplacement2011}. We will consider both types of data locality constraints in our study.


For the convenience of analysis, we consider a hierarchical distributed queueing model depicted in Fig. \ref{fig1model_distri_eq}. In this model, there are two levels of job queues: the job queues at the schedulers, and the sub-job queues at the server groups. At the scheduler side, each incoming job is split into $g$ sub-jobs, where the $h$-th sub-job consists of the tasks to be executed by server group $h$ and $h=1,\ldots,g$. Each sub-job is routed its corresponding server group, and stored in a sub-job queue. Then, a local scheduler assigns tasks to the servers within the group. 
In this hierarchical distributed queueing model, each sub-job queue for a group of servers can be considered as a centralized queueing system in Fig. \ref{fig1model_central}. 
It is important to note that this hierarchical distributed queueing model is equivalent with the original distributed queueing model in Fig. \ref{fig1model_distri}. In particular, according to the discussions in Section \ref{sec:model}, each task assignment policy of the local scheduler in the hierarchical distributed queueing model can be equivalently implemented in the original distributed queueing model, and vice versa.


% the task assignments by the local scheduler can be  
% each sub-job queue in Fig. \ref{fig1model_distri_eq}, and further utilize \eqref{eq_sub_job_relation} to obtain near delay optimality results for .

Let $k_{ih}$ denote the number of tasks in sub-job $h$ of job $i$, where $\sum_{h=1}^g k_{ih} = k_i>0$. If no task of job $i$ should be executed by $h$-th group of the servers, then $k_{ih}=0$. 
The arrival time and due time of each sub-job of job $i$ are $a_i$ and $d_i$, respectively. Define $\mathcal{I}_h = \{n,(a_i,d_i,k_{ih})_{i=1}^n\}$ as the parameters of the sub-jobs of server group $h$.
For sub-job $h$ of job $i$, $V_{ih}$ is the earliest time that all tasks of the sub-job have entered the servers, $C_{ih}$ is the completion time, $D_{ih}= C_{ih}-a_i$ is the delay, and $L_{ih} = C_{ih}-d_i$ is the {lateness} after the due time $d_i$. If $k_{ih}=0$, then $V_{ih}=C_{ih}=0$. Then, we have $V_{ih}\leq C_{ih}$.
A job is completed when all of its sub-jobs are completed. Hence, 
\begin{align}\label{eq_sub_job_relation}
C_i = \max_{h=1,\ldots,g}C_{ih}, V_i=\max_{h=1,\ldots,g}V_{ih}, D_i = \max_{h=1,\ldots,g} D_{ih},  L_i = \max_{h=1,\ldots,g}L_{ih},
\end{align}
where $V_i$ and $C_i$  depend only on the sub-jobs with positive sizes $k_{ih}>0$. Define $\bm{V}_h = (V_{1h},\ldots,V_{nh})$ and $\bm{C}_h = (C_{1h},\ldots,C_{nh})$. Let  $V_{(i),h}$ and $C_{(i),h}$ denote the $i$-th smallest components of $\bm{V}_h$ and $\bm{C}_h$, respectively. 
%, and Let $v_{ih}$ and $c_{ih}$ denote the realizations of $V_{ih}$ and $C_{ih}$.
%Let $u_{ih}$ and $c_{ih}$ denote the realization of $U_{ih}$ and $C_{ih}$, respectively. 
All these quantities are functions of the adopted scheduling policy $\pi$. 



Next, we will use the results obtained in Section \ref{sec_analysis} to study the delay performance of replications in distributed queueing systems.

%In this model, each sub-job queue for a group of servers can be considered as a centralized queue system in Fig. \ref{fig1model_central}. 


\begin{figure}
\centering
%\captionsetup{justification=centering}
\includegraphics[width=0.9\textwidth]{Figures/equivalent_distributed_queue}  
\caption{A hierarchical distributed queueing model, which is equivalent with the distributed queueing model in Fig. \ref{fig1model_distri}. } \label{fig1model_distri_eq} 
\end{figure} 

\subsection{Per-Task Data Locality Constraints}
We first consider delay minimization with per-task data locality constraints.
%, which is known to be a difficult scheduling problem \cite{Sparrow:2013}. 
For minimizing the maximum lateness $L_{\max}(\cdot)$, we propose one policy called \textbf{Earliest Due Date first with Group-based Replication (EDD-GR)}: For each local scheduler in the hierarchical distributed queueing model, if the task service times are NBU (but not exponential), the tasks are assigned to this group of servers by following policy EDD-FR; if the task service times are NWU, the tasks are assigned to the this group of servers by following policy EDD-R. The local schedulers of different server group operates independently. Note that in the original distributed queueing systems, policy EDD-FR and policy EDD-R can be implemented by first placing multiple copies of a task to all the servers in one group, and then letting the servers to communicate with each other to cancel the redundant task copies; on each server, the priority of a task is determined by the due time of the job it belongs to. Hence, policy EDD-GR is a fully distributed scheduling policy. The delay performance of policy EDD-GR is provided as follows. 
\begin{theorem}\label{thm_dis4}
If (i) the task service times are independent across the servers, (ii) each server group $h$ and its sub-job parameters $\mathcal{I}_h$ satisfy the conditions of Theorem \ref{thm3}, Theorem \ref{thm4}, or Theorem \ref{thm4_exp}, and (iii) the task assignment is subject to per-task data locality constraints, then for all \emph{$\pi\in\Pi$} and $\mathcal{I}$
\emph{
\begin{align}\label{eq_delaygap3_thm4_dis}
[L_{\max}(\bm{V}(\text{EDD-GR}))|\mathcal{I}] \leq_{\text{st}} [L_{\max}(\bm{C}(\pi))|\mathcal{I}].
\end{align}}
\end{theorem}
\begin{proof}
%See Appendix \ref{app_dis_EDD}.
%Consider the $h$-th group of servers in the distributed queue system. If the task service times of these servers are independent NBU, then EDD-NIR policy and  EDD-NR policy are more work-efficient than any policy $\pi\in\Pi$ for this group of servers. If the task service times of these servers are independent NWU, then EDD-R policy is more work-efficient than any policy $\pi\in\Pi$ for this group of servers. 
By using Theorem \ref{thm3}, Theorem \ref{thm4}, Theorem \ref{thm4_exp}, and the fact that $V_{ih}(\text{EDD-GR})\leq C_{ih}(\text{EDD-GR})$, we obtain that for all $h=1,\ldots,g$, $\pi\in\Pi$
and $\mathcal{I}$
\begin{align}
\Big[\max_{i=1,\ldots,n}[V_{ih}(\text{EDD-GR})-d_i]\Big|\mathcal{I}\Big] \leq_{\text{st}} \Big[\max_{i=1,\ldots,n}[C_{ih}(\pi)-d_i]\Big|\mathcal{I}\Big]. \nonumber
\end{align}
In addition, according to \eqref{eq_sub_job_relation}, we can get  
\begin{align}
&L_{\max}(\bm{V}(\text{EDD-GR})) = \max_{i=1,\ldots,n}[V_{i}(\text{EDD-GR})-d_i] = \max_{h=1,\ldots, g} \max_{i=1,\ldots,n}[V_{ih}(\text{EDD-GR})-d_i], \nonumber\\
&L_{\max}(\bm{C}(\pi)) = \max_{i=1,\ldots,n}[C_{i}(\pi)-d_i] = \max_{h=1,\ldots, g} \max_{i=1,\ldots,n}[C_{ih}(\pi)-d_i].\nonumber
\end{align}
Then, by using Theorem 6.B.16.(b) of \cite{StochasticOrderBook} and the independence of the task service times across the servers, it follows that
\begin{align}
\Big[\max_{i=1,\ldots,n}[V_{i}(\text{EDD-GR})-d_i]\Big|\mathcal{I}\Big] \leq_{\text{st}} \Big[\max_{i=1,\ldots,n}[C_{i}(\pi)-d_i]\Big|\mathcal{I}\Big]. \nonumber
\end{align}
By this, Theorem \ref{thm_dis4} is proven.
\end{proof}


For minimizing the maximum delay $D_{\max}(\cdot)$, we propose one policy called  \textbf{First-Come, First-Served with Group-based Replication (FCFS-GR)}: 
For each local scheduler in the hierarchical distributed queueing model, if task service times are NBU (but not exponential), the tasks are assigned to this group of servers by following policy FCFS-FR; if task service times are NWU, the tasks are assigned to this group of servers by following policy FCFS-R. Similar with policy EDD-GR, policy FCFS-GR can also be implemented distributedly in the original distributed queueing systems.
By choosing $d_i=a_i$ for all $i$, it follows from Theorem \ref{thm_dis4} that



\begin{theorem}\label{thm_dis5}
If (i) the task service times are independent across the servers, (ii) each server group $h$ and its sub-job parameters $\mathcal{I}_h$ satisfy the conditions of Theorem \ref{thm5} or Theorem \ref{thm6}, and (iii) the task assignment is subject to per-task data locality constraints, then for all \emph{$\pi\in\Pi$} and $\mathcal{I}$
\emph{
\begin{align}\label{eq_delaygap3_thm5_dis}
[D_{\max}(\bm{V}(\text{FCFS-GR}))|\mathcal{I}] \leq_{\text{st}} [D_{\max}(\bm{C}(\pi))|\mathcal{I}].
\end{align}}
\end{theorem}




%In policy EDD-GR and policy FCFS-GR, the arrival time and due time are used to determine the priority of a sub-job. However, it is difficult to use the number of unassigned tasks to determine the priority of a job, because the number of unassigned tasks decreases over time and is difficult to track in a distributed queueing system. One important open question is whether policy EDD-GR and policy FCFS-GR are optimal for minimizing more general delay metrics. 

\subsection{Per-Job Data Locality Constraints}
It appears that under per-task constraints it is difficult to generalize Theorem \ref{thm_dis4} and Theorem \ref{thm_dis5} for minimizing other delay metrics. However, under per-job constraints such generalizations are possible, which are discussed in the sequel.

For minimizing the average delay $D_{\text{avg}}(\cdot)$ and the delay metrics in $\mathcal{D}_{\text{sym}}$, we propose one policy called \textbf{Fewest Unassigned Tasks first with Group-based Replication (FUT-GR)}: For each local scheduler, if task service times are NBU (but not exponential), the tasks are assigned to this group of servers by following policy FUT-FR; if task service times are NWU, the tasks are assigned to this group of servers by following policy FUT-R. Hence, the priority of a sub-job is determined by the number of unassigned tasks in this sub-job. If $\max_{i,h} k_{ih}>1$, the local scheduler needs to track the number of unassigned tasks of each sub-job by communicating with each server in the group. If $\max_{i,h} k_{ih}=1$, policy FUT-GR can be implemented distributedly in the original distributed queueing systems. 
%For each server group, if the task service times are NBU (but not exponential) and independent across the servers in this group, the tasks of the sub-jobs are assigned to the servers by following policy FUT-FR; if the task service times are NWU and independent across the servers in this group, the tasks are assigned to the servers by following policy FUT-R. Therefore, each group of servers is treated as an independent centralized queueing system in policy FUT-GR. 
The delay performance of policy FUT-GR is provided as follows. 


\begin{theorem}\label{thm2_dist}
If (i) the task service times are independent across the servers, (ii) each server group $h$ and its sub-job parameters $\mathcal{I}_h$ satisfy the conditions of Theorem \ref{thm1}, %Theorem \ref{coro3}, 
Theorem \ref{thm2}, or Theorem \ref{thm2_exp}, and (iii) the task assignment is subject to per-job data locality constraints, then for all \emph{$f\in\mathcal{D}_{\text{sym}}$},  \emph{$\pi\in\Pi$}, and $\mathcal{I}$
\emph{
\begin{align}\label{eq_delaygap2_dist}
[f(\bm{V}(\text{FUT-GR}))|\mathcal{I}] \leq_{\text{st}} [f(\bm{C}(\pi))|\mathcal{I}].
\end{align}}
\end{theorem}
\begin{proof}
For any policy $\pi\in\Pi$, suppose that policy FUT-GR$_1$  (policy $\pi_1$) satisfies the same queueing discipline and stochastic law with policy FUT-GR (policy $\pi$).
By using the proof arguments of  Theorems \ref{thm1}-\ref{thm2_exp} and the fact that $V_{ih}(\text{FUT-GR}_1)\leq C_{ih}(\text{FUT-GR}_1)$, we can couple policy FUT-GR$_1$ and policy $\pi_1$ to show that 
\begin{align}\label{eq_thm2_dist}
V_{(i),h}(\text{FUT-GR}_1)\leq C_{(i),h}(\pi_1) 
\end{align}
holds with probability one for $h=1,\ldots,g$ and $i=1,\ldots,n$. Under per-job data locality constraints, each job can be only executed by one group of the servers. In addition, if $k_{ih}=0$, $V_{ih}(\text{FUT-GR}_1)=C_{ih}(\pi_1)=0$. By sorting the non-zero elements $V_{ih}(\text{FUT-GR}_1)$ and $C_{ih}(\pi_1)$ with $h=1,\ldots,g$ and $i=1,\ldots,n$, we can obtain  that
\begin{align}%\label{eq_thm2_dist1}
V_{(i)}(\text{FUT-GR}_1)\leq C_{(i)}(\pi_1)\nonumber
\end{align}
holds with probability one for $i=1,\ldots,n$.
Then, by using the proof arguements of Proposition \ref{lem1_1}, we get that for all $f\in\mathcal{D}_{\text{sym}}$
\begin{align}%\label{eq_thm2_dist1}
f(\bm{V}(\text{FUT-GR}_1))\leq f(\bm{C}(\pi_1))\nonumber
\end{align}
holds with probability one.
Then, by the property of stochastic ordering \cite[Theorem 1.A.1]{StochasticOrderBook}, we can obtain \eqref{eq_delaygap2_dist}. This completes the proof.
\end{proof}


Let us further consider the delay metrics in the set $\mathcal{D}_{\text{sym}}\cup\mathcal{D}_{\text{Sch-1}}$, for which we can obtain the following result.

\begin{theorem}\label{thm3_dist}
If (i) the task service times are independent across the servers, (ii) each server group $h$ and its sub-job parameters $\mathcal{I}_h$ satisfy the conditions of Theorem \ref{coro_thm3_1}, Theorem \ref{coro4_1}, or Theorem \ref{coro_thm3_1_exp}, and (iii) the task assignment is subject to per-job data locality constraints, then for all \emph{$f\in\mathcal{D}_{\text{sym}}\cup\mathcal{D}_{\text{Sch-1}}$},  \emph{$\pi\in\Pi$}, and $\mathcal{I}$
\emph{
\begin{align}\label{eq_delaygap3_dist}
[f(\bm{V}(\text{EDD-GR}))|\mathcal{I}] \leq_{\text{st}} [f(\bm{C}(\pi))|\mathcal{I}].
\end{align}}
\end{theorem}
\begin{proof}
If each server group $h$ and its sub-job parameters $\mathcal{I}_h$ satisfy the conditions of Theorem \ref{coro_thm3_1}, Theorem \ref{coro4_1}, or Theorem \ref{coro_thm3_1_exp}, then we can obtain
\begin{itemize}
\item[1.] The job with the earliest due time among all jobs with unassigned tasks is also the jobs with fewest unassigned tasks,

\item[2.] Each server group $h$ and its sub-job parameters $\mathcal{I}_h$  satisfy the conditions of Theorem \ref{thm1}, Theorem \ref{thm2}, or Theorem \ref{thm2_exp}.
\end{itemize}
Then, by using Theorem \ref{thm2_dist}, yields that \eqref{eq_delaygap3_dist} holds for all $f\in\mathcal{D}_{\text{sym}}$. 

Next, we consider the delay metrics in $\mathcal{D}_{\text{Sch-1}}$.
For any policy $\pi\in\Pi$, suppose that policy EDD-GR$_1$  (policy $\pi_1$) satisfies the same queueing discipline and stochastic law with policy EDD-GR (policy $\pi$).
By using the proof arguments of Proposition \ref{coro2_0} and Proposition \ref{coro2} (which are used in the proofs of Theorem \ref{coro_thm3_1}, Theorem \ref{coro4_1}, or Theorem \ref{coro_thm3_1_exp})  and the fact that $V_{ih}(\text{EDD-GR}_1)\leq C_{ih}(\text{EDD-GR}_1)$, we can couple policy EDD-GR$_1$ and policy $\pi_1$ to show that 
\begin{align}%\label{eq_thm3_dist}
\bm{V}_h(\text{EDD-GR}_1)-\bm{d}\prec_{\text{w}} \bm{C}_h (\pi_1)-\bm{d}\nonumber
\end{align}
holds with probability one for $h=1,\ldots,g$. Then, Theorem 5.A.7 of \cite{Marshall2011} tells us that
\begin{align}\label{eq_thm3_dist}
(\bm{V}_1(\text{EDD-GR}_1)-\bm{d}, \ldots,\bm{V}_g(\text{EDD-GR}_1)-\bm{d})\prec_{\text{w}} (\bm{C}_1 (\pi_1)-\bm{d},\ldots,\bm{C}_g (\pi_1)-\bm{d})
\end{align}
holds with probability one. Under per-job data locality constraints, each job can be only executed by one group of the servers. 
In addition, if $k_{ih}=0$, $V_{ih}(\text{EDD-GR}_1)=C_{ih}(\pi_1)=0$. If the elements satisfying $V_{ih}(\text{EDD-GR}_1)=0$  on LHS of \eqref{eq_thm3_dist} and the elements satisfying $C_{ih}(\pi_1)=0$ on RHS of \eqref{eq_thm3_dist} are removed, the obtained inequality still holds with probability one. By this, we get that
%Hence, 
%\begin{align}
%&\bm{V}(\text{EDD-GR}_1) = \sum_{h=1}^g\bm{V}_h(\text{EDD-GR}_1),\nonumber\\
%&\bm{C}(\pi_1) = \sum_{h=1}^g\bm{C}_h(\pi_1).\nonumber
%\end{align}
%By taking the summation over $h$ in \eqref{eq_thm3_dist} and use Theorem \ref{} of \cite{Marshall2011}, we get that
\begin{align}
\bm{V}(\text{EDD-GR}_1)-\bm{d}\prec_{\text{w}} \bm{C} (\pi_1)-\bm{d}\nonumber
\end{align}
holds with probability one.
In addition, by Theorem 3.A.8 of \cite{Marshall2011},
\begin{align}%\label{eq_thm2_dist1}
f(\bm{V}(\text{EDD-GR}_1))\leq f(\bm{C}(\pi_1)) \nonumber
\end{align}
holds with probability one for all $f\in\mathcal{D}_{\text{Sch-1}}$.
Then, by the property of stochastic ordering \cite[Theorem 1.A.1]{StochasticOrderBook}, we can obtain \eqref{eq_delaygap3_dist}. This completes the proof.
\end{proof}

Finally, if $d_i=a_i$ for all job $i$, it follows from Theorem 
\ref{thm3_dist} that 
\begin{theorem}\label{thm4_dist}
If (i) the task service times are independent across the servers, (ii) each server group $h$ and its sub-job parameters $\mathcal{I}_h$ satisfy the conditions of Theorem \ref{coro5_1} or Theorem \ref{coro6_1}, and (iii) the task assignment is subject to per-job data locality constraints, then for all \emph{$f\in\mathcal{D}_{\text{sym}}\cup\mathcal{D}_{\text{Sch-2}}$},  \emph{$\pi\in\Pi$}, and $\mathcal{I}$
\emph{
\begin{align}\label{eq_delaygap4_dist}
[f(\bm{V}(\text{FCFS-GR}))|\mathcal{I}] \leq_{\text{st}} [f(\bm{C}(\pi))|\mathcal{I}].
\end{align}}
\end{theorem}

% \textbf{Earliest Due Date first with Group-based Replication (EDD-GR)}: 
%Each group of servers is treated as an independent centralized queueing system. Consider one particular group of servers. If the task service times of this group of servers are independent NBU, the tasks of the sub-jobs in the sub-job queue are assigned to the servers by following EDD-NIR or EDD-NR policy; if the task service times of this group of the servers are independent NWU, the tasks are assigned to the servers by following EDD-R policy. The delay performance of policy EDD-GR is provided as follows. 

%\begin{theorem}\label{thm_dis4_1}
%If (i) the task service times in each group of servers are either NBU or NWU and independent across the servers, and (ii) ${O}_l={0}$ for each NWU server $l$, then for all \emph{$\pi\in\Pi$} and $\mathcal{I}$
%\emph{
%\begin{align}\label{eq_delaygap3_thm4_dis}
%[L_{\max}(\bm{U}(\text{EDD-GR}))|\mathcal{I}] \leq_{\text{st}} [L_{\max}(\bm{C}(\pi))|\mathcal{I}].
%\end{align}}
%\end{theorem}
%\begin{proof}
%%See Appendix \ref{app_dis_EDD}.
%Consider the $h$-th group of servers in the distributed queue system. If the task service times of these servers are independent NBU, then EDD-NIR policy and  EDD-NR policy are more work-efficient than any policy $\pi\in\Pi$ for this group of servers. If the task service times of these servers are independent NWU, then EDD-R policy is more work-efficient than any policy $\pi\in\Pi$ for this group of servers. 
%By applying Theorem \ref{lem2} for the $h$-th group of servers, we can obtain that for all $\mathcal{I}$ and all $\pi\in\Pi$
%\begin{align}
%\big[\max_{i=1,\ldots,n}[U_{ih}(\text{EDD-GR})-d_i]\big|\text{EDD-GR},\mathcal{I}\big] \leq_{\text{st}} \big[\max_{i=1,\ldots,n}[C_{ih}(\pi)-d_i]\big|\pi,\mathcal{I}\big]. \nonumber
%\end{align}
%Because the task service times are independent across the servers, by \eqref{eq_sub_job_relation} and Theorem 6.B.16.(b) of \cite{StochasticOrderBook}, it follows that
%\begin{align}
%\big[\max_{i=1,\ldots,n}[U_{i}(\text{EDD-GR})-d_i]\big|\mathcal{I}\big] \leq_{\text{st}} \big[\max_{i=1,\ldots,n}[C_{i}(\pi)-d_i]\big|\mathcal{I}\big]. \nonumber
%\end{align}
%By this, Theorem \ref{thm_dis4} is proven.
%\end{proof}


%For minimizing the maximum delay $D_{\max}(\cdot)$, we propose one policy called  \textbf{First-Come, First Served with Group-based Replication (FCFS-GR)}: 
%Consider one particular group of servers, if task service times of this group of servers are independent NBU, the tasks of the sub-jobs in the sub-job queue are assigned to the servers by following FCFS-NIR or FCFS-NR policy; if task service times of this group of servers are independent NWU, the tasks are assigned to the servers by following FCFS-R policy. By choosing $d_i=a_i$ for all $i$, it directly follows from Theorem \ref{thm_dis4} that
%
%\begin{theorem}\label{thm_dis5_1}
%If (i) the task service times of each group of servers are either independent NBU or independent NWU, and (ii) ${O}_l=\bm{0}$ for each NWU server $l$, then for all \emph{$\pi\in\Pi$} and $\mathcal{I}$
%\emph{
%\begin{align}\label{eq_delaygap3_thm5_dis}
%[D_{\max}(\bm{U}(\text{FCFS-GR}))|\mathcal{I}] \leq_{\text{st}} [D_{\max}(\bm{C}(\pi))|\mathcal{I}].
%\end{align}}
%\end{theorem}
%
%In policy EDD-GR and policy FCFS-GR, we have use the arrival time and due time to determine the priority of a job. However, it is difficult to use the number of unassigned tasks to determine the priority of a job, because the number of unassigned tasks decreases over time and is difficult to track in a distributed queueing system. One important open question is whether policy EDD-GR and policy FCFS-GR are optimal for minimizing more general delay metrics. 

%The sub-jobs are allocated to sub-job queues, each for a server group.  

% in Fig. \ref{fig1model_distri}, 



==> numerical.tex <==
% !TEX root = ./replication.tex

\section{Numerical Results}\label{sec_numerical}
In this section, we present some numerical results to illustrate the delay
performance of different scheduling policies and validate our
theoretical results.
\subsection{Centralized Queueing Systems}
Consider a centralized queueing system consisting of 3 servers with heterogeneous service time distributions, 
%50\% jobs are of the size $k_i=1$ and the other 50\% jobs are of the size $k_i = 10$. 
The inter-arrival time of the jobs $T_i=a_{i+1}-a_i$ is exponentially distributed for even $i$; and is zero for odd $i$. 
\ifreport
\begin{figure}
\centering \includegraphics[width=0.6\textwidth]{Figures/figure1_shifted_exp} \caption{Expected average delay $\mathbb{E}[D_{\text{avg}} (\bm{C}(\pi))|\mathcal{I}]$ versus traffic intensity $\rho$ in a centralized queueing system with heterogeneous NBU service time distributions.}
\label{fig1} \vspace{-0.cm}
\end{figure}
\else
\begin{figure}
\centering \includegraphics[width=0.4\textwidth]{Figures/figure1_shifted_exp} \caption{Expected average delay $\mathbb{E}[D_{\text{avg}} (\bm{C}(\pi))|\mathcal{I}]$ versus traffic intensity $\rho$ in a centralized queueing system with heterogeneous NBU service time distributions.}
\label{fig1} \vspace{-0.cm}
\end{figure}
\fi
\subsubsection{Average Delay}
Figure \ref{fig1} plots the expected average delay $\mathbb{E}[D_{\text{avg}} (\bm{C}(\pi))|\mathcal{I}]$ versus traffic intensity $\rho$ in a centralized queueing system with heterogeneous NWU service time distributions. The number of incoming jobs is $n=3000$, the job size $k_i$ is chosen to be either $1$ or $10$ with equal probability.
The task service time $X_l$ follows a shifted exponential distribution:
\begin{align}
\Pr[X_l>x] = \left\{\begin{array}{l l}1,&\text{if}~x<\frac{1}{3\mu_l};\\
\exp[-\frac{3\mu_l}{2}(x-\frac{1}{3\mu_l})],&\text{if}~x\geq \frac{1}{3\mu_l},
\end{array}\right.
\end{align}
and the service rate of the 3 servers are $\mu_1=1.4$, $\mu_2=1$, and $\mu_3=0.6$, respectively. 
%Hence, the total task service rate is $\mu_1+\mu_2+\mu_3=3$, and 
The traffic intensity can be computed as $\rho = 
2\mathbb{E}[T_2] \frac{1+10}{2} (\mu_1+\mu_2+\mu_3) =33 \mathbb{E}[T_2]$. The cancellation overhead $O_l$ of server $l$ is exponentially distributed with rate $3\mu_l/2$. %The numerical results are averaged over 100 random samples for the downloading times of data chunks.
The ``Low bound'' curve is generated by using $\mathbb{E}[D_{\text{avg}}(\bm{V}(\text{FUT-NR}))|\mathcal{I}]$ which, according to Theorem \ref{thm1}, is a lower bound of the optimum expected average delay.
We can observe from Fig. \ref{fig1} that the policies FCFS-NR, FUT-NR, and FUT-NIR are throughput-optimal, while the policies FCFS-R and  FUT-R have a smaller throughput region.  The average delays of policies FUT-NR and FUT-NIR are quite close to the lower bound, while the other policies are far from the lower bound.
%Hence, when the queue length is large, no task should be replicated for NBU service time distributions. In addition, the job with the fewest unassigned tasks should be executed first to reduce the average delay.


  %These results are in accordance with Theorem \ref{thm1}.

\ifreport
\begin{figure}
\centering \includegraphics[width=0.6\textwidth]{Figures/figure2_Pareto} \caption{Expected average delay $\mathbb{E}[D_{\text{avg}} (\bm{C}(\pi))|\mathcal{I}]$ versus traffic intensity $\rho$ in a centralized queueing system with heterogeneous NWU service time distributions.}
\label{fig2} \vspace{-0.cm}
\end{figure}
\else
\begin{figure}
\centering \includegraphics[width=0.4\textwidth]{Figures/figure2_Pareto} \caption{Expected average delay $\mathbb{E}[D_{\text{avg}} (\bm{C}(\pi))|\mathcal{I}]$ versus traffic intensity $\rho$ in a centralized queueing system with heterogeneous NWU service time distributions.}
\label{fig2} \vspace{-0.cm}
\end{figure}
\fi


Figure \ref{fig2} illustrates the expected average delay $\mathbb{E}[D_{\text{avg}} (\bm{C}(\pi))|\mathcal{I}]$ versus traffic intensity $\rho$ in a centralized queueing system with heterogeneous NWU service time distributions. The number of incoming jobs is $n=3000$, the job sizes are $k_i=10$ for all $i$. The task service time $X_l$ follows a Pareto type II (Lomax) distribution \cite{ParetoDis}:
\begin{align}
\Pr[X_l>x] = \left[1+\frac{x}{\sigma}\right]^{-\alpha_l},
\end{align}
where $\sigma = 14/3$, $\alpha_1 = 7$, $\alpha_2 = 5$, and $\alpha_3 = 3$. The cancellation overhead $O_l$ is zero for all servers. According to the property of Pareto type II (Lomax) distribution \cite{ParetoDis}, the maximum task service rate is $1/\mathbb{E}[\min_{l=1,2,3}X_l] = (\alpha_1+\alpha_2+\alpha_3-1)/\sigma=3$, which is achieved when each task is replicated on all 3 servers. Hence, the traffic intensity can be computed as $\rho = 2\mathbb{E}[T_2] \times\frac{1+10}{2}\frac{1}{\mathbb{E}[\min_{l=1,2,3}X_l]} =33 \mathbb{E}[T_2]$. Because all jobs are of the same size, the FUT discipline is identical with the FCFS discipline. %i FCFS-R (policy FCFS-NR, or policy FCFS-NIR)
We can observe that policy FUT-R, which is identical with policy FCFS-R, is throughput-optimal, while  policy FUT-NR and policy FUT-NIR have a smaller throughput region. 
In addition, policy FUT-R achieves better delay performance than the other policies, which is in accordance with Theorem \ref{thm2}. 

%According to Theorem \ref{thm2}, policy FUT-R achieves the optimum delay performance. 

\begin{figure}
\centering \includegraphics[width=0.6\textwidth]{Figures/figure2_exp} \caption{Expected average delay $\mathbb{E}[D_{\text{avg}} (\bm{C}(\pi))|\mathcal{I}]$ versus traffic intensity $\rho$ in a centralized queueing system with heterogeneous exponential service time distributions.}
\label{fig2_exp} \vspace{-0.cm}
\end{figure}

Figure \ref{fig2_exp} depicts the expected average delay $\mathbb{E}[D_{\text{avg}} (\bm{C}(\pi))|\mathcal{I}]$ versus traffic intensity $\rho$ in a centralized queueing system with heterogeneous exponential service time distributions. The number of incoming jobs is $n=3000$, the job size $k_i$ is chosen to be either $1$ or $10$ with equal probability. The service rate of the 3 servers are $\mu_1=1.4$, $\mu_2=1$, and $\mu_3=0.6$, respectively. The cancellation overhead $O_l$ is zero for all servers. The maximum task service rate is $1/\mathbb{E}[\min_{l=1,2,3}X_l] = \mu_1+\mu_2+\mu_3=3$. Hence, the traffic intensity can be computed as $\rho = 2\mathbb{E}[T_2] \times\frac{1+10}{2}\frac{1}{\mathbb{E}[\min_{l=1,2,3}X_l]} =33 \mathbb{E}[T_2]$. The ``Low bound'' curve is generated by using $\mathbb{E}[D_{\text{avg}}(\bm{V}(\text{FUT-R}))|\mathcal{I}]$ which, according to Theorem \ref{thm1}, is a lower bound of the optimum expected average delay. We can observe that the delay performance of policy FUT-R is close to the lower bound, compared with the other policies.


% quite close to the delay lower bound. Hence, for any queue length, each task should be replicated on all servers for NWU service time distributions. 

%These results are in accordance with Theorem \ref{thm1}.

\ifreport
\begin{figure}
\centering \includegraphics[width=0.6\textwidth]{Figures/figure3_lateness_shifted_exp} \caption{Complementary CDF of the maximum lateness $\Pr[L_{\max} (\bm{C}(\pi))>t|\mathcal{I}]$ versus $t$ in a centralized queueing system with heterogeneous NBU service time distributions.}
\label{fig3} \vspace{-0.cm}
\end{figure}
\else
\begin{figure}
\centering \includegraphics[width=0.4\textwidth]{Figures/figure3_lateness_shifted_exp} \caption{Complementary CDF of the maximum lateness $\Pr[L_{\max} (\bm{C}(\pi))>t|\mathcal{I}]$ versus $t$ for different policy $\pi$ in a centralized queueing system  with heterogeneous NBU service time distributions.}
\label{fig3} \vspace{-0.cm}
\end{figure}
\fi

\subsubsection{Maximum Lateness}


Figure \ref{fig3} evaluates the complementary CDF of maximum lateness $\Pr[L_{\max} (\bm{C}(\pi))$ $>t|\mathcal{I}]$ versus $t$ in a centralized queueing system with heterogeneous NBU service time distributions. The number of incoming jobs is $n=100$, the job size $k_i$ is chosen to be either $1$ or $10$ with equal probability, and the due time $d_i$ is chosen to be either $a_i$ or $a_i+50$ with equal probability. 
The distributions of task service times and cancellation overheads are the same with those in Fig. \ref{fig1}. The traffic intensity is set as $\rho = 0.8$.  
The ``Low bound'' curve is generated by using $\Pr[L_{\max}(\bm{V}(\text{EDD-NR}))>t|\mathcal{I}]$, which, according to Theorem \ref{thm3}, is a lower bound of the optimum delay performance.
We can observe that the complementary CDF of the maximum lateness of policies EDD-NR and EDD-NIR are close to the lower bound curve. In addition, the delay performance of policy FCFS-NR is better than that of FCFS-R and EDD-R. This is because policy FCFS-NR  has a larger throughput region than policy  FCFS-R and policy EDD-R. 
%In addition, the job with the earliest due time should be executed first to reduce the maximum lateness.

%Hence, when the queue length is large, no task should be replicated for NBU service time distributions.


\ifreport
\begin{figure}
\centering \includegraphics[width=0.6\textwidth]{Figures/figure4_lateness_Pareto} \caption{Complementary CDF of the maximum lateness $\Pr[L_{\max} (\bm{C}(\pi))>t|\mathcal{I}]$ versus $t$ in a centralized queueing system with heterogeneous service time NWU distributions.}
\label{fig4} \vspace{-0.cm}
\end{figure}
\else
\begin{figure}
\centering \includegraphics[width=0.4\textwidth]{Figures/figure4_lateness_Pareto} \caption{Complementary CDF of the maximum lateness $\Pr[L_{\max} (\bm{C}(\pi))>t|\mathcal{I}]$ versus $t$ for different policy $\pi$ in a centralized queueing system with heterogeneous service time NWU distributions.}
\label{fig4} \vspace{-0.cm}
\end{figure}
\fi

Figure \ref{fig4} shows the complementary CDF of maximum lateness $\Pr[L_{\max} (\bm{C}(\pi))>t|\mathcal{I}]$ versus $t$ for a centralized queueing system with heterogeneous NWU service time distributions. The number of incoming jobs is $n=100$, the job size $k_i$ is chosen to be either $1$ or $10$ with equal probability, and the due time $d_i$ is $a_i+5$. 
The distributions of task service times and cancellation overheads are the same with those in Fig. \ref{fig2}. The traffic intensity is set as $\rho = 0.8$. 
Because $d_1\leq d_2\leq\ldots\leq d_n$, the EDD discipline is identical with the FCFS discipline. %i FCFS-R (policy FCFS-NR, or policy FCFS-NIR)
We can observe that policy EDD-R, which is identical with policy FCFS-R, achieves better  performance than the other policies, which is in accordance with Theorem \ref{thm4}. 

%We can observe that the complementary CDF of the maximum lateness of policy EDD-R is close to the lower bound curve. In addition, the delay performance of policy FCFS-R is better than those of policies EDD-NR, EDD-NIR, and FCFS-NR, which have a smaller throughput region.

\ifreport
\begin{figure}
\centering \includegraphics[width=0.6\textwidth]{Figures/figure4_lateness_exp} \caption{Complementary CDF of the maximum lateness $\Pr[L_{\max} (\bm{C}(\pi))>t|\mathcal{I}]$ versus $t$ in a centralized queueing system with heterogeneous exponential service time distributions.}
\label{fig4_exp} \vspace{-0.cm}
\end{figure}
\else
\begin{figure}
\centering \includegraphics[width=0.4\textwidth]{Figures/figure4_lateness_exp} \caption{Complementary CDF of the maximum lateness $\Pr[L_{\max} (\bm{C}(\pi))>t|\mathcal{I}]$ versus $t$ for different policy $\pi$ in a centralized queueing system with heterogeneous exponential service time  distributions.}
\label{fig4_exp} \vspace{-0.cm}
\end{figure}
\fi

Figure \ref{fig4_exp} provides the complementary CDF of maximum lateness $\Pr[L_{\max} (\bm{C}(\pi))>t|\mathcal{I}]$ versus $t$ for a centralized queueing system with heterogeneous exponential service time distributions. The number of incoming jobs is $n=100$, the job size $k_i$ is chosen to be either $1$ or $10$ with equal probability, and the  due time $d_i$ is chosen to be either $a_i$ or $a_i+50$ with equal probability. 
The distributions of task service times and cancellation overheads are the same with those in Fig. \ref{fig2_exp}. The traffic intensity is set as $\rho = 0.8$. The ``Low bound'' curve is generated by using $\Pr[L_{\max}(\bm{V}(\text{EDD-R}))>t|\mathcal{I}]$.
We can observe that the delay performance of policy EDD-R is quite close to the lower bound curve. The delay performance of policy EDD-NR and policy EDD-NIR is a bit farther than from the lower bound curve. 
Policy FCFS-R and policy FCFS-NR have the worse performance. 
These results are in accordance with  Theorem \ref{thm3} and Theorem \ref{thm4_exp}.

%In addition, the delay performance of policy FCFS-R is better than those of policies EDD-NR, EDD-NIR, and FCFS-NR, which have a smaller throughput region.

%\begin{figure}
%\centering \includegraphics[width=0.6\textwidth]{Figures/figure1_square_lateness_shifted_exp} \caption{Root mean square of tardiness $\mathbb{E}[T_{\text{ms}} (\bm{C}(\pi))|\mathcal{I}]^{1/2}$ versus traffic intensity $\rho$ for different policy $\pi$ in a centralized queueing system, where the task service times of the servers follow {independent} NBU distributions.}
%\label{fig1_1} \vspace{-0.cm}
%\end{figure}

\ifreport
\begin{figure}
\centering \includegraphics[width=0.6\textwidth]{Figures/figure5_maximum_delay_shifted_exp} \caption{Complementary CDF of the maximum delay $\Pr[D_{\max} (\bm{C}(\pi))>t|\mathcal{I}]$ versus $t$  in a centralized queueing system with heterogeneous NBU service time distributions.}
\label{fig5} \vspace{-0.cm}
\end{figure}
\else
\begin{figure}
\centering \includegraphics[width=0.4\textwidth]{Figures/figure5_maximum_delay_shifted_exp} \caption{Complementary CDF of the maximum delay $\Pr[D_{\max} (\bm{C}(\pi))>t|\mathcal{I}]$ versus $t$  in a centralized queueing system with heterogeneous NBU  service time distributions.}
\label{fig5} \vspace{-0.cm}
\end{figure}
\fi
\ifreport
\begin{figure}
\centering \includegraphics[width=0.6\textwidth]{Figures/figure6_maximum_delay_Pareto} \caption{Complementary CDF of the maximum delay $\Pr[D_{\max} (\bm{C}(\pi))>t|\mathcal{I}]$ versus $t$  in a centralized queueing system with heterogeneous NWU service time distributions.}
\label{fig6} \vspace{-0.cm}
\end{figure}
\else
\begin{figure}
\centering \includegraphics[width=0.4\textwidth]{Figures/figure6_maximum_delay_Pareto} \caption{Complementary CDF of the maximum delay $\Pr[D_{\max} (\bm{C}(\pi))>t|\mathcal{I}]$ versus $t$  in a centralized queueing system with heterogeneous NWU service time distributions.}
\label{fig6} \vspace{-0.cm}
\end{figure}
\fi

\subsubsection{Maximum Delay}
Figure \ref{fig5} plots the complementary CDF of maximum delay $\Pr[D_{\max} (\bm{C}(\pi))>t|\mathcal{I}]$ versus $t$ in a centralized queueing system with heterogeneous NBU service time distributions. The system model is the same with that of Fig. \ref{fig3}.
%number of incoming jobs is $n=100$, the job size $k_i$ is chosen to be either $1$ or $10$ with equal probability, and the  due time $d_i$ is chosen to be either $a_i$ or $a_i+50$ with equal probability.  The distributions of task service times and cancellation overheads are the same with those in Fig. \ref{fig1}. The traffic intensity is set as $\rho = 0.8$.  
The ``Low bound'' curve is generated by using $\Pr[D_{\max}(\bm{V}(\text{FCFS-NR}))$ $>t|\mathcal{I}]$,  which, according to Theorem \ref{thm5}, is a lower bound of the optimum delay performance.
We can observe that the delay performance of policy FCFS-NR and policy FCFS-NIR is close to the lower bound curve. In addition, the delay performance of policy EDD-NR is better than that of FCFS-R and EDD-R because policy EDD-NR has a larger throughput region than policy  FCFS-R and policy EDD-R. 
%In addition, the job with the earliest arrival time should be executed first to reduce the maximum delay.



Figure \ref{fig6} illustrates the complementary CDF of maximum delay $\Pr[D_{\max} (\bm{C}(\pi))>t|\mathcal{I}]$ versus $t$ in a centralized queueing system with heterogeneous NWU service time distributions. The system model is almost the same with that of Fig. \ref{fig4}, except that the  due time $d_i$ is chosen to be either $a_i$ or $a_i+50$ with equal probability. 
We can observe that the delay performance of policy FCFS-R is much better than that of the other policies, which validates Theorem \ref{thm6}. 

\ifreport
\begin{figure}
\centering \includegraphics[width=0.6\textwidth]{Figures/figure_3root_mean_square_lateness_shifted_exp} \caption{Root mean square of tardiness $\mathbb{E}[T_{\text{ms}} (\bm{C}(\pi))|\mathcal{I}]^{0.5}$ versus traffic intensity $\rho$ in a centralized queueing system with heterogeneous NBU service time distributions.}
\label{fig5_RMS_tardiness} \vspace{-0.cm}
\end{figure}
\else
\begin{figure}
\centering \includegraphics[width=0.4\textwidth]{Figures/figure_3root_mean_square_lateness_shifted_exp} \caption{Root mean square of tardiness $\mathbb{E}[T_{\text{ms}} (\bm{C}(\pi))|\mathcal{I}]^{0.5}$ versus traffic intensity $\rho$ in a centralized queueing system with heterogeneous NBU  service time distributions.}
\label{fig5_RMS_tardiness} \vspace{-0.cm}
\end{figure}
\fi

\ifreport
\begin{figure}
\centering \includegraphics[width=0.6\textwidth]{Figures/figure_4root_mean_square_lateness_exp} \caption{Root mean square of tardiness $\mathbb{E}[T_{\text{ms}} (\bm{C}(\pi))|\mathcal{I}]^{0.5}$ versus traffic intensity $\rho$ in a centralized queueing system with heterogeneous exponential service time distributions.}
\label{fig6_RMS_tardiness} \vspace{-0.cm}
\end{figure}
\else
\begin{figure}
\centering \includegraphics[width=0.4\textwidth]{Figures/figure_4root_mean_square_lateness_exp} \caption{Root mean square of tardiness $\mathbb{E}[T_{\text{ms}} (\bm{C}(\pi))|\mathcal{I}]^{0.5}$ versus traffic intensity $\rho$ in a centralized queueing system with heterogeneous exponential  service time distributions.}
\label{fig6_RMS_tardiness} \vspace{-0.cm}
\end{figure}
\fi

\subsection{Some Other Delay Metrics}
Figure \ref{fig5_RMS_tardiness} shows the root mean square of tardiness $\mathbb{E}[T_{\text{ms}} (\bm{C}(\pi))|\mathcal{I}]^{0.5}$ versus traffic intensity $\rho$ in a centralized queueing system with heterogeneous NBU service time distributions, where 
\begin{align}
T_{\text{ms}}(\bm{C}(\pi)) \!= \frac{1}{n}\sum_{i=1}^{n} \max[L_i(\pi),0]^2=\frac{1}{n}\sum_{i=1}^{n} \max\left[C_i(\pi)-d_i,0\right]^2.\nonumber
\end{align}
The system model is similar with that of Fig. \ref{fig5}, except that $k_i=1$ for all job $i$ and the due time $d_i$ is either $a_i$ or $a_i+10$ with equal probability.
%number of incoming jobs is $n=100$, the job size $k_i$ is chosen to be either $1$ or $10$ with equal probability, and the  due time $d_i$ is chosen to be either $a_i$ or $a_i+50$ with equal probability.  The distributions of task service times and cancellation overheads are the same with those in Fig. \ref{fig1}. The traffic intensity is set as $\rho = 0.8$.  
The ``Low bound'' curve is generated by using $\mathbb{E}[T_{\text{ms}} (\bm{V}(\text{EDD-NR}))|\mathcal{I}]^{0.5}$, which, according to Theorem \ref{coro_thm3_1}, is a lower bound of the optimum delay performance.
We can observe that the delay performance of policy EDD-NR and policy EDD-NIR is close to the lower bound curve, and is better than that of the other policies. Notice that as  $\rho\rightarrow 0$, policy EDD-R and policy EDD-NIR tends become the same policy, and hence has the same delay performance.

%can achieve a smaller delay than policy EDD-NR and policy EDD-NIR, because replication is beneficial when  low system load. 
% performance 
%In addition, the job with the earliest arrival time should be executed first to reduce the maximum delay.



Figure \ref{fig6_RMS_tardiness} presents the root mean square of tardiness $\mathbb{E}[T_{\text{ms}} (\bm{C}(\pi))|\mathcal{I}]^{0.5}$ versus traffic intensity $\rho$ in a centralized queueing system with heterogeneous exponential service time distributions. The system model is similar with that of Fig. \ref{fig6}, except that $k_i=1$ for all job $i$ and the due time $d_i$ is either $a_i$ or $a_i+10$ with equal probability. 
The ``Low bound'' curve is generated by using $\mathbb{E}[T_{\text{ms}} (\bm{V}(\text{EDD-R}))|\mathcal{I}]^{0.5}$, which, according to Theorem \ref{coro_thm3_1_exp}, is a lower bound of the optimum delay performance.
We can observe that the delay performance of policy EDD-R is close to the lower bound curve, and is better than that of the other policies.


\ifreport
\begin{figure}
\centering \includegraphics[width=0.6\textwidth]{Figures/figure_1root_mean_square_delay_shifted_exp} \caption{Root mean square of delay $\mathbb{E}[D_{\text{ms}} (\bm{C}(\pi))|\mathcal{I}]^{0.5}$ versus traffic intensity $\rho$ in a centralized queueing system with heterogeneous NBU service time distributions.}
\label{fig5_RMS} \vspace{-0.cm}
\end{figure}
\else
\begin{figure}
\centering \includegraphics[width=0.4\textwidth]{Figures/figure_1root_mean_square_delay_shifted_exp} \caption{Root mean square of delay $\mathbb{E}[D_{\text{ms}} (\bm{C}(\pi))|\mathcal{I}]^{0.5}$ versus traffic intensity $\rho$ in a centralized queueing system with heterogeneous NBU  service time distributions.}
\label{fig5_RMS} \vspace{-0.cm}
\end{figure}
\fi

\ifreport
\begin{figure}
\centering \includegraphics[width=0.6\textwidth]{Figures/figure_2root_mean_square_delay_Pareto} \caption{Root mean square of delay $\mathbb{E}[D_{\text{ms}} (\bm{C}(\pi))|\mathcal{I}]^{0.5}$ versus traffic intensity $\rho$ in a centralized queueing system with heterogeneous NWU service time distributions.}
\label{fig6_RMS} \vspace{-0.cm}
\end{figure}
\else
\begin{figure}
\centering \includegraphics[width=0.4\textwidth]{Figures/figure_2root_mean_square_delay_Pareto} \caption{Root mean square of delay $\mathbb{E}[D_{\text{ms}} (\bm{C}(\pi))|\mathcal{I}]^{0.5}$ versus traffic intensity $\rho$ in a centralized queueing system with heterogeneous NWU  service time distributions.}
\label{fig6_RMS} \vspace{-0.cm}
\end{figure}
\fi


Figure \ref{fig5_RMS} illustrates the root mean square of delay $\mathbb{E}[D_{\text{ms}} (\bm{C}(\pi))|\mathcal{I}]^{0.5}$ versus traffic intensity $\rho$ in a centralized queueing system with heterogeneous NBU service time distributions, where 
\begin{align}
D_{\text{ms}}(\bm{C}(\pi)) \!= \frac{1}{n}\sum_{i=1}^{n} D_i^2(\pi)=\frac{1}{n}\sum_{i=1}^{n} \left[C_i(\pi)-a_i\right]^2.\nonumber
\end{align}
The system model is almost the same with that of Fig. \ref{fig5}, except that $k_i=10$ for all job $i$.
%number of incoming jobs is $n=100$, the job size $k_i$ is chosen to be either $1$ or $10$ with equal probability, and the  due time $d_i$ is chosen to be either $a_i$ or $a_i+50$ with equal probability.  The distributions of task service times and cancellation overheads are the same with those in Fig. \ref{fig1}. The traffic intensity is set as $\rho = 0.8$.  
The ``Low bound'' curve is generated by using $\mathbb{E}[D_{\text{ms}} (\bm{V}(\text{FCFS-NR}))|\mathcal{I}]^{0.5}$, which, according to Theorem \ref{coro5_1}, is a lower bound of the optimum delay performance.
We can observe that the delay performance of policy FCFS-NR and policy FCFS-NIR is close to the lower bound curve, and is much better than the other policies. 

%In addition, the job with the earliest arrival time should be executed first to reduce the maximum delay.



Figure \ref{fig6_RMS} presents the root mean square of delay $\mathbb{E}[D_{\text{ms}} (\bm{C}(\pi))|\mathcal{I}]^{0.5}$ versus traffic intensity $\rho$ in a centralized queueing system with heterogeneous NWU service time distributions. The system model is almost the same with that of Fig. \ref{fig6}, except that $k_i=10$ for all job $i$. 
We can observe that the delay performance of policy FCFS-R is much better than that of the other policies, which validates Theorem \ref{coro6_1}. 

\ifreport
\begin{figure}
\centering \includegraphics[width=0.6\textwidth]{Figures/figure7_maximum_lateness_distributed} \caption{Complementary CDF of the maximum lateness $\Pr[L_{\max} (\bm{C}(\pi))>t|\mathcal{I}]$ versus $t$ in a distributed queueing system with per-task data locality constraints.}
\label{fig7} \vspace{-0.cm}
\end{figure}
\else
\begin{figure}
\centering \includegraphics[width=0.4\textwidth]{Figures/figure7_maximum_lateness_distributed} \caption{Complementary CDF of the maximum lateness $\Pr[L_{\max} (\bm{C}(\pi))>t|\mathcal{I}]$ versus $t$ in a distributed queueing system with per-task data locality constraints.}
\label{fig7} \vspace{-0.cm}
\end{figure}
\fi
\subsection{Distributed Queueing Systems}

%The distributions of task service times and cancellation overheads are the same with those in Fig. \ref{fig1}. 


Next, we provide some numerical results for the delay performance of replications in distributed queueing systems with data locality constraints. The inter-arrival time of the jobs $T_i=a_{i+1}-a_i$ is exponentially distributed for even $i$; and is zero for odd $i$. The number of incoming jobs is $n=100$. The due time $d_i$ of job $i$ is $a_i$ or $a_i+50$ with equal probability. The traffic intensity is set as $\rho = 0.8$.  
%\subsubsection{Per-Task Data Locality Constraints}

Figure \ref{fig7} evaluates the complementary CDF of maximum lateness $\Pr[L_{\max} (\bm{C}(\pi))$ $>t|\mathcal{I}]$ versus $t$ in a distributed queueing system with per-task data locality constraints. The system has $g=2$ groups of servers, each consisting of 3 servers. The size of each sub-job $k_{ih}$ is  $1$ or $10$ with equal probability. The distributions of task service times and cancellation overheads of one group of servers are the same with those in Fig. \ref{fig1}, and the distributions of task service times and cancellation overheads of the other  group of servers are the same with those in Fig. \ref{fig2_exp}. 
The ``Low bound'' curve is generated by using $\Pr[L_{\max}(\bm{V}(\text{EDD-GR}))>t|\mathcal{I}]$, which, according to Theorem \ref{thm_dis4}, is a lower bound of the optimum delay performance. We can observe that The delay performance of  policy EDD-GR is close to the lower bound curve. In addition, policy EDD-NR and EDD-GR have similar performance. This is because exponential distribution is also NBU. Hence, both groups of servers have NBU service time distributions.
% and is much better than that of the other policies. 

\ifreport
\begin{figure}
\centering \includegraphics[width=0.6\textwidth]{Figures/figure8_maximum_delay_distributed} \caption{Complementary CDF of the maximum delay $\Pr[D_{\max} (\bm{C}(\pi))>t|\mathcal{I}]$ versus $t$ in a distributed queueing system with per-task data locality constraints.}
\label{fig8} \vspace{-0.cm}
\end{figure}
\else
\begin{figure}
\centering \includegraphics[width=0.4\textwidth]{Figures/figure8_maximum_delay_distributed} \caption{Complementary CDF of the maximum delay $\Pr[D_{\max} (\bm{C}(\pi))>t|\mathcal{I}]$ versus $t$ in a distributed queueing system with per-task data locality constraints.}
\label{fig8} \vspace{-0.cm}
\end{figure}
\fi
Figure \ref{fig8} depicts the complementary CDF of maximum delay $\Pr[D_{\max} (\bm{C}(\pi))$ $>t|\mathcal{I}]$ versus $t$ in a distributed queueing system with per-task data locality constraints. This system has $g=3$ groups of servers, each consisting of 3 servers. The size of each sub-job $k_{ih}$ is  $1$ or $10$ with equal probability. The distributions of task service times and cancellation overheads of two groups of servers are the same with those in Fig. \ref{fig7}, and the distributions of task service times and cancellation overheads of the third group of servers are the same with those in Fig. \ref{fig2}. 
The ``Low bound'' curve is generated by using $\Pr[D_{\max}(\bm{V}(\text{FCFS-GR}))>t|\mathcal{I}]$, which, according to Theorem \ref{thm_dis5}, is a lower bound of the optimum delay performance. We can see that the delay performance of  policy FCFS-GR is quite close to the lower bound curve and is much better than that of the other policies. 
%\subsubsection{Per-Job Data Locality Constraints}
%Figure \ref{fig8_RMS_tardiness_locality} plots the root mean square of tardiness $\mathbb{E}[T_{\text{ms}} (\bm{C}(\pi))|\mathcal{I}]^{0.5}$ versus traffic intensity $\rho$ in a distributed queueing system with per-job data locality constraints. The system model is similar with that of Fig. \ref{fig8}, except that each job has only one task and the due time $d_i$ is either $a_i$ or $a_i+10$ with equal probability.
%%number of incoming jobs is $n=100$, the job size $k_i$ is chosen to be either $1$ or $10$ with equal probability, and the  due time $d_i$ is chosen to be either $a_i$ or $a_i+50$ with equal probability.  The distributions of task service times and cancellation overheads are the same with those in Fig. \ref{fig1}. The traffic intensity is set as $\rho = 0.8$.  
%The ``Low bound'' curve is generated by using $\mathbb{E}[T_{\text{ms}} (\bm{V}(\text{EDD-GR}))|\mathcal{I}]^{0.5}$, which, according to Theorem \ref{thm3_dist}, is a lower bound of the optimum delay performance.
%We can observe that the delay performance of policy EDD-GR is close to the lower bound curve, and is better than that of the other policies. 
%%Notice that as  $\rho\rightarrow 0$, policy EDD-R and policy EDD-NIR tends become the same policy, and hence has the same delay performance.
%
%
%
% The distributions of task service times and cancellation overheads of two groups of servers are the same with those in Fig. \ref{fig7}, and the distributions of task service times and cancellation overheads of the third group of servers are the same with those in Fig. \ref{fig2}. 
%The ``Low bound'' curve is generated by using $\Pr[D_{\max}(\bm{V}(\text{FCFS-GR}))>t|\mathcal{I}]$, which, according to Theorem \ref{thm_dis5}, is a lower bound of the optimum delay performance. We can see that the delay performance of  policy FCFS-GR is quite close to the lower bound curve and is much better than that of the other policies. 
%


==> sufficient_conditions.tex <==
% !TEX root = ./replication.tex

%\section{Sufficient Conditions for Delay Optimality and Near-Optimality}


\section{Sufficient Conditions for Near Delay Optimality}\label{sec_sufficient}
%\section{Proof Structure}
%The existing proof techniques for the delay optimality or near optimality of task replication policies are combinatorial and  difficult to understand. There is a lack of unify framework to unify different proof techniques.  As an attempt to alleviate this difficulty, 

%Existing delay optimality and near delay optimality analyses of task replications \cite{Borst2003,Righter2008,Kim2010,shah-Allerton-2013,ShengboInfocom,Sun2015} focused on the average delay ${D}_{\text{avg}}(\cdot)$, and their proof techniques vary from case to case. 
%There is a lack of unified treatment for minimizing different delay metrics in various system settings. 
In this section, we establish a unified framework for minimizing several classes of delay metrics in various system settings. In particular, sufficient conditions are proposed for proving that a scheduling policy is near delay-optimal, %These sufficient conditions do not need to specify the queueing model or service time distribution, and hence provide a unified treatment for various system settings. 
%In addition, 
%These sufficient conditions can handle not only the average delay ${D}_{\text{avg}}(\cdot)$, but also more general delay metric functions in $\mathcal{D}_{\text{sym}}$, $\mathcal{D}_{\text{Sch-1}}$, and $\mathcal{D}_{\text{Sch-2}}$. 
% for various system settings.
%These sufficient conditions
which will be used to establish our main results in later sections. These sufficient conditions are proven by using stochastic ordering and majorization.
%A \textbf{sample-path ordering} technique is developed to prove 
 %Note that the bounds that we will describe are by no means the tightest that are available from the sample-path ordering technique. In particular, different bounds can be obtained from different forms of sample-path ordering, which will be studied in our future work.
%for centralized queue systems in Section \ref{sec_analysis}, and for distributed queue systems in Section \ref{sec_distributed}.
% for distribued delay metrics and system settings.

%which provide a unified framework in minimizing a number of delay metrics. These sufficient conditions do not depend on a specific system setting, independent, The existing proof techniques for the delay optimality or near optimality results of task replication policies  
%are combinatorial and 
%vary from case to case, 
%which makes them difficult to understand, 
%which do not provide a unified treatment for different system settings.
% and do not provide a unified treatment. 
% combinatorial and  difficult to understand. There is a lack of unify framework to unify different proof techniques.  
%As an attempt to alleviate this difficulty, 


%These sufficient conditions will be used in later sections to %outline the key proof steps of 
%which will be used later sections to prove near delay optimality results in various system settings. 


%We will see that the sufficient conditions for different delay metrics can be expressed in similar forms to provide a unified treatment for different delay metrics, but their proof techniques are different. 
%

%Moreover, in order to compare the task completion times among different scheduling policies, we develop a \emph{sample-path ordering} technique, which enables us to  prove near delay optimality results in the form of \eqref{eq_nearoptimal}. 
%The results of this section are proven in Appendix \ref{app0}.

%When using these sufficient conditions, one key difficulty is to prove that a scheduling policy is near-optimal in terms of \eqref{eq_nearoptimal}. To that end, we develop a novel technique called \emph{sample-path ordering}, which can effectively characterize the delay gap from the optimum. 
%\subsection{} 


%In this section, we propose novel sufficient conditions for proving that a scheduling policy is  delay-optimal or near-optimal. These sufficient conditions reveal the key ideas in delay optimality analysis of task replications and can greatly simplify the corresponding proof arguments.  The proofs of these sufficient conditions are provided in Appendix \ref{app0}.

% showing the existence of a low-complexity policy that is within a finite gap from the optimum delay.
%There is a lack of uniform methodology for bounding the sub-optimality gap from the optimum delay performance.

%Their usage will be illustrated in later sections when studying task replications across heterogeneous servers.

%In this section, we present a general analysis framework of
%redundant executions which serves two purposes: (i) to provide
%sufficient conditions for identifying scheduling policies that
%are delay-optimal or near-optimal, and (ii) to simplify and
%unify the proof techniques for establishing delay optimalityalleviate
%and near-optimality. These analysis tools will be used later tocumbersome
%study redundancy scheduling across heterogeneous servers.

 
%Define $\bm{s}=(s_{1},\ldots, s_{k_{\text{sum}}})$ as the sequence of task arrival times of the system, and $\bm{T}(\pi)=(T_{1}(\pi),\ldots, T_{k_{\text{sum}}}(\pi))$ as the sequence of task completion times of the system. The components of $\bm{s}$ and $\bm{T}(\pi)$ are arranged in the increasing order such that $\bm{s} =\bm{s}_{\uparrow}$ and $\bm{T}(\pi)=\bm{T}_{\uparrow}(\pi)$.~Then, $\bm{s}$ is uniquely determined by $\mathcal{I}$, while $\bm{T}(\pi)$ is determined by $\mathcal{I}$, the scheduling policy $\pi$, and random task service times.
\subsection{Work-Efficiency Ordering}

In traditional queueing systems without task replications, the service delay is largely governed by the following work conservation law (or its generalizations): At any time, the expected total amount of time for completing the jobs in the queue is invariant among all work-conserving policies \cite{Leonard_Kleinrock_book,Gittins:11}. However, this work conservation law does not hold in queueing system with task replications.
%, because each task has multiple replication modes. 
In particular, each task has multiple replication modes (i.e., it can be replicated on different numbers of servers and at different time instants), which require different amounts of service time. In order to minimize delay, the scheduler needs to choose efficient replication modes to execute the tasks. Motivated by this, we define a work-efficiency ordering to compare the efficiency of task executions in different task replication policies, where the job indices of the tasks are not concerned. 
%One illustration of this is provided in Fig. \ref{Work_Efficiency_Ordering}.



% Consider two non-preemptive feasible policies $\pi_1,\pi_2\in\Pi$. Suppose that the 


% in policy $\pi_1$ the tasks are executed in a more efficient replication mode than in policy $\pi_2$, then one would expect the . If , then in policy $\pi_1$ no fewer than $b$ tasks start execution during $[\tau,\nu]$, which may complete execution after time $\nu$ because 







%Define $\bm{s}=(s_{1},\ldots, s_{k_{\text{sum}}})$ as the sequence of task arrival times of the system, and $\bm{T}(\pi)=(T_{1}(\pi),\ldots,$ $ T_{k_{\text{sum}}}(\pi))$ as the sequence of task completion times of the system. The components of $\bm{s}$ and $\bm{T}(\pi)$ are arranged in the increasing order such that $\bm{s} =\bm{s}_{\uparrow}$ and $\bm{T}(\pi)=\bm{T}_{\uparrow}(\pi)$.~Then, $\bm{s}$ is uniquely determined by $\mathcal{I}$, while $\bm{T}(\pi)$ is determined by $\mathcal{I}$, the scheduling policy $\pi$, and random task service times.

%Let $k_{\text{sum}}=\sum_{i=1}^nk_i$ denote the total number of tasks, $\bm{t}(\pi)=(t_{1}(\pi),\ldots, t_{k_{\text{sum}}}(\pi))$ denote the realizations of task completion times on a sample path of policy $\pi$. The components of $\bm{t}(\pi)$ are arranged in the increasing order such that $\bm{t} (\pi)=\bm{t}_{\uparrow}(\pi)$.

%A relationship between two policies $\pi_1$ and $\pi_2$ is said to \textbf{hold on sample path}, if there is a measure preserving one-to-one correspondence between the sample paths of policies $\pi_1$ and $\pi_2$, such that  the relationship holds between each pair of corresponding sample paths of policies $\pi_1$ and $\pi_2$.

%We define a \emph{work efficiency order}:

%For any time interval $[\tau,\nu]$ and policy $\pi$, let $n_{{s}}^{\pi}(\tau,\nu)$ denote the number of tasks that start execution during $[\tau,\nu]$, and $n_{sc}^{\pi}(\tau,\nu)$ denote the number of tasks that start and complete execution during $[\tau,\nu]$. 

A relationship between policy $\pi_1$ and policy $\pi_2$ is said to \textbf{hold in stochastic ordering}, if for each sample path of policy $\pi_1$ there is a corresponding sample path of policy $\pi_2$, such that (i) these two sample paths of policy $\pi_1$ and policy $\pi_2$ have the same probability density, and (ii) the relationship holds between these two sample paths of policy $\pi_1$ and policy $\pi_2$.

\begin{definition} \label{def_order} \textbf{Work-Efficiency Ordering:}
A work-conserving policy $\pi_1\in\Pi$ is said to be \textbf{more work-efficient} than policy $\pi_2\in\Pi$, if 
the following relationship between policy $\pi_1$ and policy $\pi_2$ holds in stochastic ordering: For each task $j$ executed in  policy $\pi_2$, if 
\begin{itemize}
\item[1.] Task $j$ starts execution at time $\tau$ and completes execution at time $\nu$ on the sample path of policy $\pi_2$ where $\nu\geq\tau$, 
\item[2.] There exist unassigned tasks in the queue during $[\tau,\nu]$ on the corresponding sample path of policy $\pi_1$, 
\end{itemize}
then  on the sample path of policy $\pi_1$ there exists one corresponding task $j'$ which starts execution during $[\tau,\nu]$. 
\end{definition}

An illustration of the work-efficiency ordering is provided in Fig. \ref{Work_Efficiency_Ordering}. Informally speaking, policy $\pi_1$ is said to be more work-efficient than policy $\pi_2$, if the tasks are executed faster in policy $\pi_1$ than in policy $\pi_2$. In particular, if the service duration of task $j$ is $[\tau,\nu]$ on the sample path of policy $\pi_2$, then there  exists one task $j'$ whose service time is shorter than $\nu-\tau$ on the corresponding sample path of policy $\pi_1$. Because the task service of policy $\pi_1$ and policy $\pi_2$ is asynchronized, the executions of task $j$ and task $j'$ may start at different time instants. Hence, task $j'$ may start execution during $[\tau,\nu]$, and complete execution either before or after time $\nu$. We note that work-efficiency ordering is defined on task-level, which is not related to the service priority of different jobs. For this reason, the job indices of task $j$ and task $j'$ are not specified in the definition.

% speed  determined by the job indices of task $j$ and task $j'$ are not specified because they do not affect the efficiency of policy $\pi_1$ and policy $\pi_2$.


% the task service of policy $\pi_1$ and policy $\pi_2$ is asynchronized

%If on the sample path of policy $\pi_2$, one server starts to process a task at time $\tau$ and completes this task at time $\nu$ ($\tau\leq\nu$), then  on the sample path of policy $\pi_1$ there exists a time $t\in[\tau,\nu]$ such that one of the following three cases holds:  (i) the same server starts to process a corresponding task at time $t$ (as illustrated in Fig. \ref{Work_Efficiency_Ordering}), (ii) all the remaining tasks are under service at time $t$, or (iii) the queue is empty at time $t$.


%for any time interval $[\tau,\nu]$ if $b$ tasks start execution and also complete execution during $[\tau,\nu]$ in policy $\pi_2$, then one would expect that in policy $\pi_1$ no fewer than $b$ tasks start execution during $[\tau,\nu]$ (unless there are not enough tasks to execute in policy $\pi_1$); however, these tasks may complete execution after time $\nu$ in policy $\pi_1$, because the task service of policy $\pi_1$ and policy $\pi_2$ is asynchronized. 
%By this, the work-efficiency ordering can be defined as follows:


%This definition can be understood as follows: If each task is executed in a more efficient mode in policy $\pi_1$ than policy $\pi_2$, then the service duration of the task is shorter in policy $\pi_1$ than policy $\pi_2$. Because policy $\pi_1$ and policy $\pi_2$ are asynchronized, if $b$ tasks start and complete execution during $[\tau,\nu]$ on the sample path of policy $\pi_2$, than at least $b$ 


% $\pi_1\in\Pi$ is said to be \textbf{more work-efficient} than policy $\pi_2\in\Pi$


% $[\tau,\nu]$ and all servers are busy execution during $[\tau,\nu]$
%
%
%, if all servers are busy during $[\tau,\nu]$  on the sample path of policy $\pi_1$, then
%\begin{align}
%n_{{s}}^{\pi_1}(\tau,\nu)\geq_{\text{st}}  n_{sc}^{\pi_2}(\tau,\nu),
%\end{align}
%where $n_{{s}}^{\pi_1}(\tau,\nu)$ is the number of tasks that start execution during $[\tau,\nu]$  on the sample path of policy $\pi_1$, and $n_{sc}^{\pi_2}(\tau,\nu)$ is the number of tasks that start and complete execution during $[\tau,\nu]$  on the corresponding sample path of policy $\pi_2$.
% all servers are busy and $b$ tasks start execution in a time interval on the sample path of policy $\pi_1$, then no more than $b$ tasks start and complete execution in the same time interval on the sample path of policy $\pi_2$.
%$b$ tasks start and complete execution during $[\tau,\nu]$ on the sample path of policy $\pi_2$, then on the sample path of policy $\pi_1$, it holds that either $b$ tasks start execution during $[\tau,\nu]$ or all the remaining tasks are under service at some time $t\in[\tau,\nu]$.

%for all time interval $[\tau,\nu]\subseteq[0,\infty)$ and job parameters $\mathcal{I}$
%\begin{align}
%[N_{{a}}^{\pi_1}(\tau,\nu)| \mathcal{I}]\geq_{\text{st}}  [N_{ac}^{\pi_2}(\tau,\nu)| \mathcal{I}].
%\end{align}
%the following relationship holds on sample path: 
%\begin{itemize}
%\item[1.] $\bm{t}(\pi_1)\leq\bm{t}(\pi_2)$ holds on sample path.
%
%\item[2.] 
%For all $j=1,\ldots,n$ and $t\in[a_j,a_{j+1})$, 

%If on the sample path of policy $\pi_2$, one server starts to process a task at time $\tau$ and completes this task at time $\nu$ ($\tau\leq\nu$), then  on the sample path of policy $\pi_1$ there exists a time $t\in[\tau,\nu]$ such that one of the following three cases holds:  (i) the same server starts to process a corresponding task at time $t$ (as illustrated in Fig. \ref{Work_Efficiency_Ordering}), (ii) all the remaining tasks are under service at time $t$, or (iii) the queue is empty at time $t$.

\begin{figure}
\centering 
\includegraphics[width=0.4\textwidth]{Figures/work_efficiency_ordering} \caption{Illustration of work-efficiency ordering, where the service duration of a task is indicated by a rectangle. If on the sample path of policy $\pi_2$, task $j$ starts execution at time $\tau$ and completes execution at time $\nu$, then on the sample path of policy $\pi_1$ one corresponding task $j'$ starts execution at some time $t\in[\tau,\nu]$. The job indices of task $j$ and task $j'$ are not specified because they do not affect the efficiency of policy $\pi_1$ and policy $\pi_2$.}
% work--efficiency ordering holds for any priorities of the jobs.
\label{Work_Efficiency_Ordering} 
\end{figure} 
%or (ii') {one server is idle at time $\tau$}.\footnote{Note that the difference between these two definitions are in condition (ii) and condition (ii').}


%$b$ unassigned tasks are allocated to the servers and completed by the servers during $[a_j,t]$ on the sample path of policy $\pi_2$, then on the corresponding sample path of policy $\pi_1$ one of the following cases holds: (i) no fewer than $b$ unassigned tasks are allocated to the servers  during $[a_j,t]$, (ii) all the remaining tasks are under service at time $t$, or (iii) the queue is empty at time $t$.
%\end{itemize}
%in policy $\pi_2$ the system starts to process a task at time $\tau$ and completes the task at time $\nu$ ($\tau\leq\nu$), then in policy $\pi_1$ it holds that (i) a task is completed at some time during $[\tau,\nu]$, or (ii) {the queue is empty at time $\tau$}.
%for any sample path of policy $\pi_2$, there exists a sample path of policy $\pi_1$ with the same probability density such that $\bm{t}(\pi_1)\leq\bm{t}(\pi_2)$.
%Policy $\pi_1$ is said to be \emph{weakly more work-efficient} than policy $\pi_2$, if the following relationship holds on sample path: If in policy $\pi_2$ the system starts to process a task at time $\tau$ and completes the task at time $\nu$ ($\tau\leq\nu$), then in policy $\pi_1$ it holds that (i) a task is completed at some time during $[\tau,\nu]$, or (ii') {one server is idle at time $\tau$}.\footnote{Note that the difference between these two definitions are in condition (ii) and condition (ii').}


%The proof of the following lemma is straightforward and thus omitted: 
%\begin{theorem}\label{lemma_work_efficiency}
%If policy $\pi_1$ is {more work-efficient} than policy $\pi_2$, then
%\begin{itemize}
%\itemsep0em 
%\item[1.] policy $\pi_1$ is {weakly more work-efficient} than policy $\pi_2$;
%\item[2.] $\bm{t}(\pi_1)\leq\bm{t}(\pi_2)$ holds on sample path.
%\end{itemize} 
%\end{lemma}


%
\subsection{Sample-Path Ordering and Sufficient Conditions for Near Optimality}
In the special case that each job has one task, sufficient conditions are provided in \cite{Borst2003,Righter2008,Kim2010,shah-Allerton-2013} for minimizing 
%if policy $P\in\Pi$ is more {work-efficient} than all $\pi\in\Pi$, then policy $P$ minimizes 
the average delay ${D}_{\text{avg}}(\cdot)$% in distribution (or on sample path) 
. However, %as one can imagine, 
it is extremely difficult to establish delay optimality or near delay optimality results when the job sizes are arbitrarily given. 
By using work-efficiency ordering, we obtain the following sufficient condition for near delay optimality in minimizing ${D}_{\text{avg}}(\cdot)$ for general job sizes.

%In Sec. \ref{sec_analysis}, we will use this sufficient condition to study near delay-optimal scheduling of task replications for arbitrary job sizes.  


\begin{theorem}\label{lem1}
If there exists a work-conserving policy $P\in\Pi$ such that for all $\mathcal{I}$
\begin{itemize}
\itemsep0em 
\item[1.] Policy $P$ is {more work-efficient} than any policy $\pi\in\Pi$,
\item[2.] In policy $P$, each task allocated to the servers belongs to the job with the fewest unassigned tasks, whenever there exist unassigned tasks in the queue,
\end{itemize} 
then \emph{$[{D}_{\text{avg}}(\bm{V}_{}(P))|\mathcal{I}]\leq_{\text{st}} [{D}_{\text{avg}}(\bm{C}_{}(\pi))|\mathcal{I}]$} holds for all $\pi\in\Pi$ and $\mathcal{I}$.
\end{theorem}

%The sufficient condition of Theorem \ref{lem1} provides a unified treatment for minimizing ${D}_{\text{avg}}(\cdot)$ in various system settings. 


We note that, in Theorem \ref{lem1} and other sufficient conditions of this section, model-specific information (such as the number of servers and service time distribution) and policy-specific information (such as when to replicate a task and replicate on which servers) is summarized in the work-efficiency ordering. 
%In Section \ref{sec_analysis} and Section \ref{sec_distributed}, 
When applying these sufficient conditions, one needs to first prove the work-efficiency ordering between policy $P$ and any policy $\pi\in\Pi$ for the specified system setting, and then uses these sufficient conditions to show that policy $P$ is near delay-optimal. 

%When using this sufficient condition i
%does not specify one particular queueing model or service time distribution, because such 

%This sufficient condition not depend on the specific queueing model or service time distribution. For each specific system setting, this  as long as a work-efficiency ordering can be established between 



The difficulties in proving Theorem \ref{lem1} are as follows: First, policy $P$ is a dynamic priority policy where the job with the fewest unassigned tasks has the highest priority. Hence, the priority of a job increases as more tasks of this job are assigned to the servers. On the other hand, policy $\pi$ could be any policy in $\Pi$, which may follow a  different priority rule. Therefore,  the servers might be processing completely different jobs in policy $P$ and policy $\pi$, which makes it difficult to compare these two policies. Second, policy $P$ is an online policy, where the scheduling decisions are made without using any information about the future job arrivals. However, policy $\pi$ is allowed to have access to the parameters $(a_i,{k}_i,d_i)$ of future arriving jobs. Hence, the comparison between these two policies is unfair for policy $P$. Third, all policies in $\Pi$ are non-preemptive and server-idleness is allowed for some policies in $\Pi$. These conditions are adversary for finding a delay-optimal or near-optimal policy in $\Pi$ \cite{michael2012book,Gittins:11}. 

%Even if Lemma \ref{thm1} switches to seek for near-delay optimality result, it is unclear 

%suggests that in such adverse scenarios, it is still possible to establish near-delay optimality results.  
%The difficulties in Theorem \ref{lem1} are as follows: 

%



%we consider preemption is not allowed and server-idleness is allowed for the policies in $\Pi$, which makes it extremely difficult to find a delay-optimal policy in $\Pi$ \cite{michael2012book,Gittins:11}. Lemma \ref{thm1} suggests that it is still possible to seek for near delay optimality in such adverse scenario.  of delay optimality, it is still possible to prove Lemma \ref{thm1}. 


%Second,  Second, while policy $P$ is an online policy, policy $\pi$ may have access to the parameters $(a_i,{k}_i,d_i)$ of future arriving jobs. Hence, the comparison between these two policies is unfair for policy $P$. Third, in $\Pi$ are , which is usually 

In order to prove Theorem \ref{lem1}, we need to first define the system state for any policy $\pi\in\Pi$. 

\begin{definition}\label{def_state_thm3}
At any time $t$, the system state of policy $\pi$ is specified by a pair of $n$-vectors $\bm{\xi}_{\pi}(t)=(\xi_{1,\pi}(t),\ldots,\xi_{n,\pi}(t))$ and $\bm{\gamma}_{\pi}(t)=(\gamma_{1,\pi}(t),\ldots,\gamma_{n,\pi}(t))$ %and $\bm{\zeta}=(\zeta_1,\ldots,\zeta_n)$ 
with non-negative components, where $n$ is the number of arriving jobs which can be either finite or infinite. The components of $\bm{\xi}_{\pi}(t)$ and $\bm{\gamma}_{\pi}(t)$ are interpreted as follows:
if job $i$ is present in the system at time $t$, then $\xi_{i,\pi}(t)$ is the number of remaining tasks (which are stored in the queue or being executed  by the servers) of job $i$, and $\gamma_{i,\pi}(t)$ is the number of unassigned tasks (which are stored in the queue and not being executed  by the servers) of job $i$; if job $i$ is not present in the system at time $t$ (i.e., job $i$ has not arrived at the system or has departed from the system), then $\xi_{i,\pi}(t)=\gamma_{i,\pi}(t)=0$. Hence, for all $i=1,\ldots,n$, $\pi\in\Pi$, and $t\in[0,\infty)$
\begin{align}%\label{eq_def_state_thm3}
0\leq \gamma_{i,\pi}(t)\leq \xi_{i,\pi}(t)\leq k_i.
\end{align}
Let $\{\bm{\xi}_{\pi}(t),\bm{\gamma}_{\pi}(t),t\geq0\}$ be the state process of policy $\pi$, which is assumed to be right-continuous. 
\end{definition}





A proof sketch of Theorem \ref{lem1} is provided as follows.
\begin{proof}[Proof sketch of Theorem \ref{lem1}]
%Here is a proof sketch of Theorem \ref{lem1}.
The proof contains two parts: In the first part, we use the conditions of Theorem \ref{lem1} to establish the following stochastic ordering result:
\begin{lemma}[Stochastic Ordering]\label{lemG4}
Suppose that $\bm{\xi}_{P}(0^-) = \bm{\gamma}_{P}(0^-) =\bm{\xi}_{\pi}(0^-) = \bm{\gamma}_{\pi}(0^-)=\bm{0}$ and the conditions of Theorem \ref{lem1} are satisfied. Then, the following relationship holds in stochastic ordering:
\begin{eqnarray}\label{eq_lemG4}
\sum_{i=j}^n {\gamma}_{[i],P}(t)\leq \sum_{i=j}^n {\xi}_{[i],\pi}(t),~j = 1,2,\ldots,n
\end{eqnarray}
for all $t\geq0$, where ${\xi}_{[i],\pi}(t)$ is the $i$-th largest component of vector $\bm{\xi}_{\pi}(t)$, and ${\gamma}_{[i],\pi}(t)$ is the $i$-th largest component of vector $\bm{\gamma}_{\pi}(t)$. 
\end{lemma}
From the perspective of majorization, \eqref{eq_lemG4} can be equivalent expressed as: $\bm{\xi}_{\pi}(t)$ is weakly majorized by $\bm{\gamma}_{P}(t)$ from above, i.e., $\bm{\xi}_{\pi}(t)\prec^{\text{w}}\bm{\gamma}_{P}(t)$ \cite{Marshall2011}. Note that Lemma \ref{lemG4} is a strong statement, because it holds for all $j = 1,2,\ldots,n$, time $t\in[0,\infty)$, job parameters $\mathcal{I}$, and policy $\pi\in\Pi$. In addition, Lemma \ref{lemG4} holds even if  the scheduling decisions of policy $\pi$ are made by using the parameters $(a_i,{k}_i,d_i)$ of future arriving jobs. In the second part of the proof, we use Lemma \ref{lemG4} to show that 
\begin{align}\label{eq_sketch1}
v_{(i)}(P) \leq c_{(i)}(\pi), ~i=1,\ldots,n
\end{align}
holds in stochastic ordering (Lemma \ref{lem_sample_path_ordering}).\footnote{Recall that $c_{(i)}(\pi)$ is the $i$-th smallest job completion time on the sample path of policy $\pi$, $v_{(i)}(P)$ is the $i$-th smallest component of the vector $(v_1(P),\ldots,v_n(P))$, and  $v_{i}(P)$ is the earliest time that all tasks of job $i$ are either completed or under service on the sample path of policy $P$.} Hence, Lemma \ref{lemG4} characterizes the timeline of job
executions on the sample paths of policy $P$ and policy $\pi$. Finally, Theorem \ref{lem1} follows from \eqref{eq_sketch1}. 
The proof details are provided in Appendix \ref{app0}. 
\end{proof}

%In Appendix \ref{app0}, we develop a  {sample-path ordering} technique to prove Theorem \ref{lem1}. 

%The first part of this {sample-path ordering} technique, i.e., 
The stochastic ordering result in Lemma \ref{lemG4} is motivated by \cite{Smith78}, which provided a proof of the optimality of Shortest-Remaining-Processing-Time (SRPT) first policy for single-server queueing systems. The generalization from \cite{Smith78} to Lemma \ref{lemG4} for multiple-server queueing systems with parallel processing and task replications is highly non-trivial. A preliminary version of this {sample-path ordering} technique was proposed in \cite{Sun2015}.  


%Nonetheless, this technique is able to establish a dominance between $v_{(i)}(P)$ and $c_{(i)}(\pi)$ on sample-path, hence the name. 




% but the generalization from \cite{Smith78} to this {sample-path ordering} technique is non-trivial. % and unexpected when this research started. 


%While existing delay optimality analyses of task replications \cite{Borst2003,Righter2008,Kim2010,shah-Allerton-2013,ShengboInfocom,Sun2015} focused on the average delay ${D}_{\text{avg}}(\cdot)$, 
First, Theorem \ref{lem1} can be generalized to all delay metrics in $\mathcal{D}_{\text{sym}}$.
\begin{corollary}\label{coro1}
If \emph{${D}_{\text{avg}}(\cdot)$} is replaced by any \emph{$f\in\mathcal{D}_{\text{sym}}$}, Theorem \ref{lem1} still holds.
\end{corollary}

\begin{proof}
See Appendix \ref{app0}.
\end{proof}

\ifreport
\else
Due to space limitation, the proofs of the remaining results are relegated to our technical report \cite{report2015}.
\fi
In addition, a sufficient condition can be obtained for near optimality in minimizing the maximum lateness $L_{\max}(\cdot)$.
\begin{theorem}\label{lem2}
If there exists a work-conserving policy $P\in\Pi$ such that for all $\mathcal{I}$
\begin{itemize}
\itemsep0em 
\item[1.] Policy $P$ is {more work-efficient} than any policy $\pi\in\Pi$,
\item[2.] In policy $P$, each task allocated to the servers belongs to the job  with the earliest due time, whenever there exist unassigned tasks in the queue,
\end{itemize} 
then \emph{$[L_{\max}(\bm{V}_{}(P))|\mathcal{I}]\leq_{\text{st}} [L_{\max}(\bm{C}_{}(\pi))|\mathcal{I}]$} holds for all $\pi\in\Pi$ and $\mathcal{I}$.
\end{theorem}
%For the ease of understanding, Theorem \ref{lem1} and Theorem \ref{lem2} are expressed in similar forms. However, some parts of their proofs are quite different. In particular, because the delay metric is changed from average delay ${D}_{\text{avg}}(\cdot)$ to maximum lateness $L_{\max}(\cdot)$, a different form of sample-path ordering is required to prove Theorem \ref{lem2}. 
\ifreport
\begin{proof}[Proof sketch of Theorem \ref{lem2}]
The proof contains two parts: In the first part, we use the conditions of Theorem \ref{lem2} to establish a second form of  stochastic ordering:

\begin{lemma}[Stochastic Ordering --- The Second Form]\label{lemG4_thm3}
Suppose that $\bm{\xi}_P(0^-)=\bm{\gamma}_P(0^-)=\bm{\xi}_{\pi}(0^-)=\bm{\gamma}_{\pi}(0^-)=\bm{0}$ and the conditions of Thoerem \ref{lem2} are satisfied. Then, the following relationship holds in stochastic ordering:
\begin{eqnarray}\label{eq_lemG4_thm3}
\sum_{i:d_i\leq\tau} \gamma_{i,P}(t)\leq \sum_{i:d_i\leq\tau} \xi_{i,\pi}(t), ~\forall~\tau\in[0,\infty)
\end{eqnarray}
holds for all $t\geq0$.
\end{lemma}
In the second part of the proof, we use Lemma \ref{lemG4_thm3} to show that 
\begin{align}
v_{i}(P)-d_i \leq \max_{j=1,\ldots,n}[c_{j}(\pi)-d_j],~i=1,\ldots,n
\end{align}
holds in stochastic ordering (Lemma \ref{lem_sample_path_ordering_thm3}). By this, Theorem \ref{lem2} follows. The details are provided in Appendix \ref{app0_1}.
\end{proof}
\fi




If each job has one task, Theorem \ref{lem2} can be generalized to all delay metrics in $\mathcal{D}_{\text{sym}}\cup\mathcal{D}_{\text{Sch-1}}$ by using the rearrangement inequality in \cite[Theorem 6.F.14]{Marshall2011} and\cite{Chang93rearrangement_majorization}. 
%This result is motivated by .
%, but the proof technique is different.
\begin{corollary}\label{coro2}
If $k_1=\ldots=k_n=1$ and \emph{$L_{\max}(\cdot)$} is replaced by any \emph{$f\in\mathcal{D}_{\text{sym}}\cup\mathcal{D}_{\text{Sch-1}}$}, Theorem \ref{lem2} still holds.
\end{corollary}
\ifreport
\begin{proof}[Proof sketch of Corollary \ref{coro2}]
For all $f\in\mathcal{D}_{\text{sym}}$, we use Corollary \ref{coro1} to prove that the statement of Theorem \ref{lem2} holds if \emph{$L_{\max}(\cdot)$} is replaced by any $f\in\mathcal{D}_{\text{sym}}$. For all $f\in\mathcal{D}_{\text{Sch-1}}$, we show that there exists an $n$-vector $\bm{u}'$ satisfying 
%In order to prove \eqref{eq_coro2_3}, 
%it is sufficient to show that there exists an  such that 
\begin{align}\label{eq_coro2_6}
\bm{u}(P)-\bm{d}\prec \bm{u}'- \bm{d} \leq \bm{c} (\pi)-\bm{d},
\end{align}
which further implies 
\begin{align}\label{eq_coro2_3}
\bm{u}(P)-\bm{d}\prec_{\text{w}} \bm{c} (\pi)-\bm{d}. 
\end{align} 
Using this, we can show that the statement of Theorem \ref{lem2} holds if \emph{$L_{\max}(\cdot)$} is replaced by any $f\in\mathcal{D}_{\text{Sch-1}}$.
The details are provided Appendix \ref{app0_1}.
\end{proof}
\fi

If $d_i=a_i$ for all job $i$, $L_{\max}(\cdot)$ reduces to the {maximum delay} $D_{\max}(\cdot)$. In this case, we can obtain
\begin{theorem}\label{lem3}
If there exists a work-conserving policy $P\in\Pi$ such that for all $\mathcal{I}$
\begin{itemize}
\itemsep0em 
\item[1.] Policy $P$ is {more work-efficient} than any policy $\pi\in\Pi$,
\item[2.] In policy $P$, each task allocated to the servers belongs to the job  with the earliest arrival time, whenever there exist unassigned tasks in the queue,
\end{itemize} 
then \emph{$[D_{\max}(\bm{V}_{}(P))|\mathcal{I}]\leq_{\text{st}} [D_{\max}(\bm{C}_{}(\pi))|\mathcal{I}]$} holds for all $\pi\in\Pi$ and $\mathcal{I}$.
\end{theorem}
\ifreport
\begin{proof}
%Because $D_{\max}(\cdot)$ is a special case of $L_{\max}(\cdot)$. 
See Appendix \ref{app0_2}.
\end{proof}
\fi

If each job has $k$ tasks, Theorem \ref{lem3} can be generalized to all delay metrics in $\mathcal{D}_{\text{sym}}\cup\mathcal{D}_{\text{Sch-2}}$.
\begin{corollary}\label{coro3_1}
If $k_1=\ldots=k_n=k$ and \emph{$D_{\max}(\cdot)$} is replaced by any \emph{$f\in\mathcal{D}_{\text{sym}}\cup\mathcal{D}_{\text{Sch-2}}$}, Theorem \ref{lem3} still holds.
\end{corollary}
\ifreport
\begin{proof}
See Appendix \ref{app0_2}.
\end{proof}
\fi


==> v3/abstract.tex <==
\begin{abstract}
We study a class of  scheduling problems, %in multi-server queueing systems, 
where each job is divided into a batch of unit-size tasks and these tasks can be executed in parallel on multiple servers with New-Better-than-Used (NBU) service time distributions. While many delay optimality results are available for single-server queueing systems, generalizing these results to the multi-server case has been challenging. 
%This motivated us to seek for near delay-optimal scheduling. 
% because it is difficult to efficiently utilize the full service capacity of parallel servers. 
This motivated us to investigate near delay-optimal scheduling of batch jobs in multi-server queueing systems. 
%whether there exist scheduling policies that can come close to delay optimality. 
We consider three low-complexity scheduling policies: the Fewest Unassigned Tasks first (FUT) policy, the Earliest Due Date first (EDD) policy, and the First-Come, First-Served  (FCFS) policy. 
We prove that for arbitrary number, batch sizes, arrival times, and due times of the jobs, these scheduling policies are near delay-optimal in stochastic ordering for minimizing three classes of delay metrics among all causal and non-preemptive policies.
%We also characterize the sub-optimal delay gap for minimizing several important delay metrics. 
In particular, the FUT policy is within a constant additive delay gap from the optimum  for minimizing the mean average delay, and  
the FCFS policy within twice of the optimum for minimizing the mean maximum delay and the mean $p$-norm of delay. 
%For instance, the FUT policy is shown to be within a constant additive delay gap from the optimum delay for minimizing the mean average delay, and the FCFS policy is within twice of the optimum for minimizing the mean maximum delay and the mean $p$-norm of delay. 
The key proof tools are several novel sample-path orderings, which can be used to compare the sample-path delay of different policies in a near-optimal sense. 
%The key tools for showing these results are some novel sample-path tools for comparing the delay performance of different policies.
% in a near-optimal sense. 

%tools for showing these results are some novel sample-path sufficient conditions for delay comparison.  
% for minimizing several classes of  delay metrics

% , 

%, no matter with or without task replications
%
%
%In interactive Web services, task service time is highly variable and service latency is bottlenecked by
%the slowest straggling tasks. However, delay-optimal scheduling in  is  and task replications make it more complicated.  In this research, we designed low-complexity task replication policies and proposed a
%novel sample-path ordering technique to prove that these policies are delay-optimal or within a constant gap from the optimum delay among all causal policies. The arrival process is arbitrary, and
%the service time distributions are quite general (New-Better-than-Used or New-Worse-than Used).
%We are generalizing our results to distributed queueing systems, and arbitrary service time distributions. Our study can be applied to many Web services, such as email, Web searching, advertisement,
%E-commerce, gaming, etc.
%
% is the root of 
%
%One critical requirement for such systems is low service delay.
%
%
%In data centers, a job is de 
%
%We first propose a variety of sufficient conditions for 
%
%developed low complexity task replication policies. By using a sample-path and stochastic ordering approach, these policies are proven to be near delay-optimal among all causally feasible policies. 
%
%Task replication is crucial in cloud computing and machine  systems to reduce service delay, which have motivated a lot of recent research interests. 
%
%
%
% 
% 




\end{abstract}

==> v3/analysis.tex <==
% !TEX root = ./parallel_servers.tex

\begin{algorithm}[h]
\SetKwData{NULL}{NULL}
\SetCommentSty{small}
$Q:=\emptyset$\tcp*[r]{$Q$ is the set of  jobs in the queue}
\While{the system is ON} {
\If{job $i$ arrives}{
$\xi_i:=k_i$\tcp*[r]{job $i$ has $\xi_i$ remaining tasks~~~~~~~}
$\gamma_i:=k_i$\tcp*[r]{job $i$ has $\gamma_i$ unassigned tasks~~~~~~}
$Q:=Q \cup \{i\}$\;
}

\While{$\sum_{i\in Q} \gamma_i> 0$ and there are idle servers}{
Pick any idle server $l$\;
$j :=\arg\min\{\gamma_i : i\in Q, \gamma_i>0\}$\;
Allocate a task of job $j$ on server $l$\;
$\gamma_j:=\gamma_j - 1$\;

}

\If{a task of job $i$ is completed}{

%replicated copies of this task\;
$\xi_{i} := \xi_{i} -1$\;
\textbf{if} $\xi_{i}=0$ \textbf{then} {$Q:=Q/ \{i\}$\;   }
}


}
\caption{ Fewest Unassigned Tasks first (FUT).}\label{alg1}
\end{algorithm}
\section{Main Results}\label{sec_analysis}
%In this section, we will develop replication-control policies and prove that
%, for some general classes of processing time distributions,
%these policies are either delay-optimal among all online policies or within a \emph{constant gap} from the optimum delay performance, even compared with the policies with prior knowledge of $(a_1,a_2,\ldots, a_N)$. By ``constant gap'', we mean that the sub-optimality gap is upper bounded by a constant that is independent of the job arrival process, which holds for both Poisson and bursty job arrival processes, and for both low and high system load. Further, the delay sub-optimality gap obtained in this paper is additive. When the system load is high, i.e., the scenario of the greatest practical interests, the obtained delay sub-optimality gap is much tighter than the multiplicative delay gap provided by a competitive ratio result (if any).

%In this section, we study task replications across heterogeneous servers. We develop a heterogeneous replication policy and prove that it is near delay-optimal by using the sufficient conditions.


%  consider several low-complexity scheduling policies and prove that these policies are near delay-optimal in distribution for minimizing the delay metrics in $\mathcal{D}_{\text{sym}}$, $\mathcal{D}_{\text{Sch-1}}$, and $\mathcal{D}_{\text{Sch-2}}$. 
%The proof techniques include the sample-path results developed in Section \ref{sec_sufficient} and coupling arguments.
%The sample-path results developed in Section \ref{sec_sufficient} are used to .
%Delay optimality results are also established when possible.
% for a number of delay metrics.

%In the sequel, we will establish delay optimality and near optimality results for several classes of delay metrics, assuming that the task service times are NBU or NWU.

In this section, we provide some near delay optimality results in the form of \eqref{eq_nearoptimal} and \eqref{eq_nearoptimal1}. 
These results will be proven in Section \ref{sec_proofmain} by using a unified sample-path method.

\subsection{Average Delay $D_{\text{avg}}$ and the Delay Metrics in $\mathcal{D}_{\text{sym}}$}\label{sec_average_delay}


%This  queueing discipline is termed \textbf{Fewest Unassigned Task (FUT)} first, which is a dynamic priority, work-conserving queueing discipline.



%If $O_l\leq_{\text{st}}[X_l-\tau|X_l>\tau]$, i.e., the time to cancel the redundant task  is stochastically shorter than the time to complete this redundant task, server $l$ will cancel this redundant task copy; otherwise, server $l$ will keep processing this task copy until completion (steps 20-24). 
%Note that task cancellation is \emph{optional} in policy FUT-NIR: we can still show that policy FUT-NIR is near delay-optimal, even if no redundant task is cancelled in policy FUT-NIR.



% suppose that a task is completed and server $l$ is still processing a redundant copy of this task: If $[O_l-\tau|O_l>\tau]\leq_{\text{st}}X_l$ for all $\tau\geq0$,\footnote{Recall that $O_l$ is the delay overhead for server $l$ to cancel a redundant task copy.} server $l$ will cancel this redundant task copy; otherwise, server $l$ will keep process this redundant task copy until completion
%is cancelled if the time to cancel the task copy is stochastically shorter than the time to complete the task copy; otherwise, the task copy will be processed until completion
%(steps 20-24).





%The  second policy is called  \textbf{Fewest Unassigned Tasks first with No Replication (FUT-NR)}.
%In this policy, the tasks are assigned to the servers by following the FUT discipline and no task is replicated on more than one servers. %Hence, if all tasks are in service on some servers, the remaining servers can be idle.
%The description of policy FUT-NR can be obtained from Algorithm \ref{alg1} by removing the steps 15-16, 20-24.

%In general, we suggest the following principles for task replication and cancellation with NBU service time distributions:
%\begin{definition}\textbf{Principles for Task Replication and Cancellation with NBU Service Time Distributions:}
%A queueing discipline is termed \textbf{Flexible Replication (FR)} if it satisfies the following two principles:
%\begin{itemize}
%\item[1.] {Task Replication:} {It can either replicate a task to an idle server when there is no unassigned tasks, or not replicate this task at all. 
%%In other words, it cannot replicate a task where there exist unassigned tasks.
%}
%%If there exist unassigned tasks in the queue, then no task should be replicated on multiple servers; if all tasks are in service and some servers are still idle, any task can be replicated on these servers.
%
%\item[2.] {Task Cancellation:} {It can either cancel a redundant task copy when the time to cancel the task is stochastically shorter than the remaining service time to complete the task, or not cancel this task at all. 
%%In other words, it cannot cancel a task if the time to cancel the task is not stochastically shorter than the time to complete the task.
%}
%%Specifically, a redundant task copy should be cancelled only when the time to cancel the redundant task copy is shorter than the remaining processing time of this redundant task copy in probability.
%\end{itemize}
%\end{definition}

Let us first consider the following \textbf{Fewest Unassigned Tasks first (FUT)} policy, which is also described in Algorithm \ref{alg1}: 
Each idle server is allocated to process a task from the job with the earliest due time among all jobs with unassigned tasks. The delay performance of policy FUT is characterized in the following theorem.




%Theorem \ref{thm1} suggests the following principles on task replications for NBU service time distributions with task cancellation costs:
%\begin{itemize}
%\item \emph{Either replicate a task when no task is waiting to be executed, or never replicate a task.}
%%If there exist unassigned tasks in the queue, then no task should be replicated on multiple servers; if all tasks are in service and some servers are still idle, any task can be replicated on these servers.
%
%\item \emph{Either cancel a redundant task when the time to cancel the task is shorter than the time to complete the task in stochastic ordering, or never cancel a redundant task}.
%%Specifically, a redundant task copy should be cancelled only when the time to cancel the redundant task copy is shorter than the remaining processing time of this redundant task copy in probability.
%\end{itemize}

%In FUT-NIR, each idle server is assigned to process a fresh task of the job with the fewest unassigned tasks (i.e.,the job with the smallest $\gamma_i-\zeta_i$ with $\gamma_i>\zeta_i$).  the smallest




%Let $Q$ represent the set of unfinished jobs. For each job $i$ in the queue $Q$, suppose that job $i$ has $\gamma_i$ remaining tasks and $\zeta_i$ out of these $\gamma_i$ tasks are in service. Then, $\gamma_i-\zeta_i$ is the number of unassigned tasks of job $i$. In FUT-NIR, each idle server is


%and Fewest Positive Unassigned Tasks first with No Replication (FPUT-NR). FPUT-NIR is , where $Q$ is the set of unfinished jobs, $\gamma_i$ is the number of remaining tasks of job $i$, and $\zeta_i$ out of these $\gamma_i$ tasks are currently in service on some servers. Then, $\gamma_i-\zeta_i\geq0$ is the number of unassigned tasks of job $i$.

%We also  FPUT-NR can be obtained from Algorithm \ref{alg1} by removing step \ref{step}.

%In both FPUT-NIR and FPUT-NR, the job with the smallest positive $\gamma_i-\zeta_i$ has the highest priority. When $\sum_{i\in Q} \gamma_i> \sum_{i\in Q} \zeta_i$, the operations of FPUT-NIR and FPUT-NR are the same: each idle server is scheduled to process an unassigned task from the job with the smallest positive $\gamma_i-\zeta_i$. When $\sum_{i\in Q} \gamma_i= \sum_{i\in Q} \zeta_i$, FPUT-NIR and FPUT-NR have different operations: In FPUT-NIR, each idle server is assigned to process a replica of any remaining task; In FPUT-NR, no task is replicated such that the unassigned servers are kept idle.




%FPUT-NIR is designed based on the following intuitions: (i) \emph{It is better not to replicate over NBU servers.}
%% and not replicate over NWU servers}. %For NBU servers, task replications  $\sum_i\gamma_i\geq V+1$, tasks should not be replicated over NBU (healthy) servers and should be replicated on as many (unhealthy) servers as possible; when the number of remaining tasks is larger than the number of groups ($\sum_i\gamma_i\leq V$), tasks are replicated on the remaining server groups such that all servers are busy.
%(ii) \emph{When queue length is small, tasks can also be replicated over NBU servers.}
%(iii) \emph{To reduce average delay, small jobs should have higher priority as in the Shortest Remaining Processing Time (SRPT)   discipline \cite{Schrage68,Smith78}}.
%%Preemptive SRPT minimizes the average delay in single-server systems. However, when there are multiple servers, SRPT is no longer optimal and no policy is known to achieve a constant competitive ratio \cite{Leonardi2007}. We use the number of remaining tasks $\gamma_i$ to approximate the remaining processing time of job $i$. If preemption is allowed, the job with the smallest positive $\gamma_i$ has the highest priority.
%(iv) \emph{Since preemption is not allowed, we use the number of unassigned tasks $\gamma_i-\zeta_i$ to determine the priority of unfinished job $i$.} %This is because $\zeta_i$ tasks of job $i$ have been already assigned out and will be in service without interruption in any  policy. Hence, these $\zeta_i$ tasks can be excluded when determining the priority of job $i$. 

%{\red We can provide an example to explain the difficulty on approximating SRPT.}

%These principles enables FPUT-NIR to achieve a short average delay. We now show that no policy can be significantly better than FPUT-NIR.

%\subsubsection{Analysis}



%\DecMargin{1em}

%The first key result of this paper is stated as follows:

%The following theorem tells us that both policy FUT-NR and policy FUT-NIR are near-optimal.
\begin{theorem}\label{thm1}
If the task service times are NBU, independent across the servers, and {i.i.d.} across the tasks assigned to the same server, then for all \emph{$f\in\mathcal{D}_{\text{sym}}$},  ${\pi\in\Pi}$, and $\mathcal{I}$ %FPUT-NR satisfies
\emph{
\begin{align}\label{eq_delaygap1}
&[f(\bm{V}(\text{FUT}))|\mathcal{I}] \leq_{\text{st}} \left[f(\bm{C}(\pi))|\mathcal{I}\right].%\\
\end{align}}
\end{theorem}
%\begin{proof}
%The proof of Theorem \ref{thm1} is relegated to Section \ref{sec_sufficient}.
%\end{proof}
If there are multiple idle servers, the choices of the idle server in Step 9 of Algorithm \ref{alg1} are non-unique. 
The result of Theorem \ref{thm1} holds for any server selection method in Step 9. In practice, one can pick the idle server with the fastest service rate. 





%Theorem \ref{thm1} suggests the following principles on task replications for NBU service time distributions with task cancellation costs:
%\begin{itemize}
%\item \emph{Either replicate a task when no task is waiting to be executed, or never replicate a task.}
%%If there exist unassigned tasks in the queue, then no task should be replicated on multiple servers; if all tasks are in service and some servers are still idle, any task can be replicated on these servers.
%
%\item \emph{Either cancel a redundant task when the time to cancel the task is shorter than the time to complete the task in stochastic ordering, or never cancel a redundant task}.
%%Specifically, a redundant task copy should be cancelled only when the time to cancel the redundant task copy is shorter than the remaining processing time of this redundant task copy in probability.
%\end{itemize}



%Recently, threshold-based replication policies were developed in \cite{addShengboOriginal,Lee-Allerton-2015}, which switch between replication and no-replication based on a threshold on the queue-length.  In certain system settings, the optimal threshold was obtained for minimizing the mean average delay within a specific family of policies. 
%On the other hand, if near delay optimality within is sufficient, Theorem \ref{thm1} suggests to employ the FR discipline for  replications, which is flexible to use and does not need to compute the switching threshold. In addition, the near delay optimality result in Theorem \ref{thm1} holds in quite general system settings, which allow for arbitrary arrival processes, arbitrary job sizes, arbitrary cancellation cost $\bm{O}$, arbitrary number of servers, general NBU service time distributions, and the policy space $\Pi$ contains all non-preemptive and causal policies, as well as the anticipative policies that can predict future job arrivals.

%These policies require to compute the optimal switching threshold for given arrival process, which are difficult to implement when the statistics of the arrival process is unknown. 

%depend on the distributions of $O_l$ and $X_l$.

%when the cancellation delay overhead $O_l$ is negligible,

%åThis intuivtion is true for
%A near delay-optimal policy can be obtained by combining this task replication operation with the FUT discipline.




%In Theorem \ref{thm1}, the extra conditions {$[O_l-\tau|O_l>\tau]\leq_{\text{st}}X_l$} or \emph{$[O_l-\tau|O_l>\tau]\geq_{\text{st}}X_l$} are introduced to ensure that in policy FUT-NIR, the redundant task copies are completed or cancelled stochastically earlier than to keep processing these task copies until completion.


Let us characterize the sub-optimality delay gap of policy FUT. For mean average delay, i.e., $f(\cdot)=D_{\text{avg}}(\cdot)$, it follows from \eqref{eq_delaygap1} that %and \eqref{eq_delaygap2} that
\begin{align}%\label{eq_delaygap1_1}
%\mathbb{E}[D_{\text{avg}}(\bm{V}(\text{FUT-NR}))|\mathcal{I}] \leq&
%\min_{\pi\in\Pi}\mathbb{E}\left[D_{\text{avg}}(\bm{C}(\pi))\left.\right|\mathcal{I}\right]\leq \mathbb{E}[D_{\text{avg}}(\bm{C}(\text{FUT-NR}))|\mathcal{I}] ,\\
\mathbb{E}[D_{\text{avg}}(\bm{V}(\text{FUT}))|\mathcal{I}] \leq 
\min_{\pi\in\Pi}\mathbb{E}\left[D_{\text{avg}}(\bm{C}(\pi))\left.\right|\mathcal{I}\right] \leq \mathbb{E}[D_{\text{avg}}(\bm{C}(\text{FUT}))|\mathcal{I}]. \label{eq_delaygap1_2}
\end{align}
%such that policies FUT-NR and FUT-NIR are near-optimal for minimizing the mean average delay $\mathbb{E}\left[D_{\text{avg}}(\bm{C}(\pi))\left.\right|\mathcal{I}\right]$.
%Denote $\overline{D}_{\text{gap}} $ %and $\overline{D}_{\text{gap},2} $ 
%as the difference 
The delay gap between the LHS and RHS of \eqref{eq_delaygap1_2} is given by 
%. According to \eqref{eq_2},
\begin{align}\label{eq_delaygap1_1_1}
& \mathbb{E}[D_{\text{avg}}(\bm{C}(\text{FUT}))-D_{\text{avg}}(\bm{V}(\text{FUT}))|\mathcal{I}]\nonumber\\
=& \mathbb{E}\bigg[\frac{1}{n}\sum_{i=1}^n\big({C}_i(\text{FUT})-V_i(\text{FUT})\big)\bigg|\mathcal{I}\bigg].\!
\end{align}
Recall that $m$ is the number of servers, and $k_i$ is the number of tasks in job $i$. At time $V_i(\text{FUT})$, all tasks of job $i$ have started service: If $k_i>m$,  then job $i$ has at most $m$ incomplete tasks that are under service at time $V_i(\text{FUT})$; if $k_i\leq m$, then job $i$ has at most $k_i$ incomplete tasks that are under service at time $V_i(\text{FUT})$. Therefore, in policy FUT, at most $k_i\wedge m = \min\{k_i,m\}$ tasks of job $i$ are under service during the time interval $[V_i(\text{FUT}), {C}_i(\text{FUT})]$. Using this and the property of NBU distributions, we can obtain
%after time $V_i(\text{FUT-NR})$ the system only needs to complete $k_i\wedge m$ tasks to accomplish job $i$.

\begin{theorem}\label{lem7_NBU}
Let $\mathbb{E}[X_l]= 1/\mu_l$, and without loss of generality $\mu_1\leq \mu_2\leq \ldots\leq \mu_m$. 
If the task service times are NBU, independent across the servers, {i.i.d.} across the tasks assigned to the same server, then  for all $\mathcal{I}$
\emph{\begin{align}\label{eq_gap}
\mathbb{E}[D_{\text{avg}}(\bm{C}(\text{FUT}))|\mathcal{I}] - \min_{\pi\in\Pi}\mathbb{E}\left[D_{\text{avg}}(\bm{C}(\pi))|\mathcal{I}\right]  \leq&\frac{1}{n}\sum_{i=1}^n\sum_{l=1}^{k_i \wedge m } \frac{1}{\sum_{j=1}^l\mu_j}\\
\leq& \frac{\ln(k_{\max}\wedge m)+1}{\mu_1},\label{eq_gap_2}
\end{align}}
where $k_{\max}$ is the maximum job size in \eqref{eq_0}, and $x\wedge y = \min\{x,y\}$.
\end{theorem}

If $\mathbb{E}[X_l]\leq 1/\mu$ for $l=1,\ldots,m$, then  the sub-optimality delay gap of policy FUT is of the order $O(\ln(k_{\max}\wedge m))/{\mu}$. As the number of servers $m$ increases, this  sub-optimality delay gap is upper bounded by $[\ln(k_{\max})+1]/{\mu}$ which is independent of $m$. 

Theorem \ref{thm1} and Theorem \ref{lem7_NBU} tell us that {for arbitrary number, batch sizes, arrival times, and due times of the jobs, the FUT policy is near delay-optimal for minimizing the average delay $D_{\text{avg}}$ in the mean. 

The FUT policy is a nice approximation of the Shortest Remaining Processing Time (SRPT) first policy  \cite{Schrage68,Smith78}: The FUT policy  utilizes the number of unassigned tasks of a job to approximate the remaining processing time of this job, and is within a small additive sub-optimality gap from the optimum for minimizing the mean average delay in the scheduling problem that we consider.




Due to the difficulty of delay minimization in multi-class multi-server queueing systems, attempts on finding a tight additive sub-optimal delay gap in these systems has met with little success. In \cite{Weiss:1992,Weiss:1995}, closed-form upper bounds on the sub-optimality gaps of the Smith's rule and the Gittin's index rule were established for the cases that all jobs arrive at time zero. In Corollary 2 of \cite{Dacre1999}, the authors studied the optimal control in multi-server queueing systems with stationary arrivals of multiple classes of jobs, and used the achievable region method to obtain an additive sub-optimality delay gap, which is of the order $O(m k_{\max})$. The model and methodology in these studies are significantly different from those in this paper. 




%In , characterizing the sub-optimality gap of scheduling policies is usually  note that it is difficult to obtain bounded gap from delay optimality is difficult to obtain even . A few successful results were obtained in   where it was shown that the delay performance of  has a bounded  in . The obtained delay bounds are of the order $O(m)$. 


% sub-optimality gaps were upper bounded for  in certain multi-server queueing systems, where the upper bounds  comes close to optimality, 


%bounded sub-optimality gap were obtained for queueing systems with general service times and without task replications, where the obtained sub-optimality gaps are of the order $O(m)$, 


%which are unbounded as the number of servers $m$ grows.

%Delay-optimal scheduling in multi-server queueing systems with multiple job classes is known to be notoriously difficult. 


% \cite{Weiss:1992,Weiss:1995,Dacre1999}. In such scenario, near delay-optimal results with bounded sub-optimality gap are not easy to obtain either.  


%In some special cases, policy FUT is delay-optimal. In Theorem 2.1 of \cite{Kim2010} and Theorem 4 of \cite{shah-Allerton-2013}, it was show that if each job has a single task and the system load is high,\footnote{``High system load'' means that there exist unassigned tasks in the queue at all time $t\in[0,\infty)$.} no replication is delay-optimal for minimizing the average delay. Similarly,  one can show that  in these cases policy FUT is delay-optimal in distribution  for minimizing all delay metrics in $\mathcal{D}_{\text{sym}}$. %, which utilizes a different proof technique.


%Interestingly, these principles do not require to  for a specific arrival process, and hence is easier to implement in practical than the threshold-based policies proposed in.

%The sample-path dominance technique developed in this paper provides a new approach for tackling these issues.

%





%We now consider the mean expected delay
%$f=D_{\text{avg}}$ and $\phi(x)=x$.
% the delay sub-optimality gap of FPUT-NR and FPUT-NIR.
%It follows from \eqref{eq_delaygap1} that
%\begin{align}\label{eq_delaygap4}
%\!\!\mathbb{E}[{D}_{\text{avg},\text{FPUT-NR}}|\mathcal{I}] \leq_{\text{st}} \min_{\pi\in\Pi} \mathbb{E}\left[{D}_{\text{avg},\pi}\left.\right|\mathcal{I}\right]\!+\!\frac{1}{N}\sum_{i=1}^N\mathbb{E}[G_i],\!\!
%\end{align}
%Similar result can be obtained for FPUT-NIR from \eqref{eq_delaygap2}. Let $\overline{D}_{\text{gap}}$ represent the last term in \eqref{eq_delaygap4}. Then, we can obtain
%
%\begin{lemma}
%It holds that
%\begin{align}
%\overline{D}_{\text{gap}} \leq \frac{1}{N}\sum_{i=1}^N\max_{\substack{S: |S|= k_i\wedge M\\
%S\subseteq\mathcal{M}}}\!\!\mathbb{E}\left[\max_{m\in S} X_m\right].\nonumber
%\end{align}
%\end{lemma}
%
%\begin{proof}
%See Appendix \ref{app1}.
%\end{proof}


%In Theorem \ref{thm1}, the extra conditions {$\bm{O}_{\mathcal{S}}\leq_{\text{st}}[\bm{X}_{\mathcal{S}}-\bm{\tau}_{\mathcal{S}}| \bm{X}>\bm{\tau}]$} and  {$\bm{O}_{\mathcal{S}^c}\geq_{\text{st}}[\bm{X}_{\mathcal{S}^c}-\bm{\tau}_{\mathcal{S}^c}| \bm{X}>\bm{\tau}]$} are introduced to ensure that in policy FUT-NIR, the redundant task copies are completed stochastically earlier than completing these task copies without cancellation.

%In it was shown that 
%
%
%
%\begin{theorem}\label{coro3}
%In addition to the conditions of Theorem \ref{thm1}, if (i) $k_1=\ldots=k_n=1$, and (ii) the system load is high, then for all \emph{$f\in\mathcal{D}_{\text{sym}}$}, $\pi\in\Pi$, and $\mathcal{I}$
%\emph{
%\begin{align}\label{eq_coro3}
%[f(\bm{C}(\text{FUT}))|\mathcal{I}] \leq_{\text{st}} [f(\bm{C}(\pi))|\mathcal{I}].
%\end{align}}
%\end{theorem}
%\ifreport
%\begin{proof}
%%One can use the proof techniques in \cite{Kim2010} and \cite{shah-Allerton-2013} to prove Theorem \ref{coro3}. 
%See Appendix \ref{app_coro3}.
%\end{proof}
%\fi



%\begin{algorithm}[h]
%\SetKwData{NULL}{NULL}
%\SetCommentSty{small}
%$Q:=\emptyset$\tcp*[r]{the set of  jobs in the queue}
%\While{the system is ON} {
%\If{job $i$ arrives}{
%$\gamma_i:=k_i$\tcp*[r]{job $i$ has $\gamma_i$ unassigned tasks~~~~~~~}
%%$\zeta_i:=0$\tcp*[r]{$\zeta_i$ tasks of job $i$ are in service}
%$Q:=Q \cup \{i\}$\;
%}
%
%\While{$Q\neq\emptyset$ and all servers are idle}{
%%Pick any idle server $m$\;
%%\If{$\sum_{i\in Q} \gamma_i> \sum_{i\in Q} \zeta_i$}{
%%~~~~~~~~~~~~~~~~\tcp*[h]{At least one task is unassigned}
%$j :=\arg\min\{\gamma_i: i\in Q\}$\;
%Replicate a remaining task of job $j$ on all servers\;
%%$\zeta_j:=1$\;
%%}
%}
%
%\If{a task of job $i$ is completed}{
%Cancel the remaining $m-1$ replicas of this task\;
%$\gamma_{i} := \gamma_{i} -1$\;% $\zeta_{i} := 0$\;
%\textbf{if} $\gamma_{i}=0$ \textbf{then} {$Q:=Q/ \{i\}$\;   }
%}
%}
%\caption{ Fewest Unassigned Tasks first with Replication (FUT-R).}\label{alg2}
%\end{algorithm}

%When the task service times are NWU and independent across the servers, we propose a policy called  \textbf{Fewest Unassigned Tasks first with Replication (FUT-R)}, which is described in Algorithm \ref{alg2}. In this policy, a task from the job with the fewest unassigned tasks is replicated on all $m$ servers (steps 7-10). When one copy of this task is completed on one server, the remaining $m-1$ replicated copies of this task are cancelled on the other servers (step 12). In this policy, each time a task enters the servers, all $m$ servers are idle and hence {the job with the fewest unassigned  tasks is also the job with the fewest remaining tasks}.
%Therefore, this policy can be also called Fewest Remaining Tasks first with Replication (FRT-R). The delay performance of policy FUT-R is provided in the following theorem, where the cancellation overhead $\bm{O}$ is assumed to be zero.
%% Theorem \ref{thm2} and Corollary \ref{coro4}.
%
%
%
%%Many existing delay optimality results are special cases of Corollary \ref{coro1}: In Theorem 4 and Theorem 6(c) of \cite{shah-Allerton-2013}, the authors  and the policy space is The result in Corollary \ref{coro1} was stated in \cite{} and \cite{}.
%
%
%
%
%
%
%
%\begin{theorem}\label{thm2}
%If (i) $k_1\leq k_2\leq \ldots\leq k_n$, (ii) the task service times are NWU and independent across the servers, (iii) $\bm{O}=\bm{0}$, then for all \emph{$f\in\mathcal{D}_{\text{sym}}$},  \emph{$\pi\in\Pi$}, and $\mathcal{I}$
%\emph{
%\begin{align}\label{eq_delaygap3}
%[f(\bm{C}(\text{FUT-R}))|\mathcal{I}] \leq_{\text{st}} [f(\bm{C}(\pi))|\mathcal{I}].
%\end{align}}
%\end{theorem}
%\ifreport
%\begin{proof}
%See Appendix \ref{app2}.
%\end{proof}
%\fi
%One special case of Theorem \ref{thm2} was  obtained in Theorem 3.2 of  \cite{Righter2008} and Theorem 3 of \cite{shah-Allerton-2013}, where each job has a single task, i.e., $k_1=k_2=\ldots=k_n=1$.
%%Theorem \ref{thm2} suggests that each task should be replicated on all $m$ servers when the task service times of the servers follow independent NWU distributions. %A near delay-optimal policy can be obtained by combining this task replication operation with the FUT discipline.
%We note that compared to the traditional definition of NWU distributions in reliably theory \cite[p. 1]{StochasticOrderBook}, the definition in \eqref{eq_NWU} has one additional condition on the absolutely continuity of $\bar{F}$. This condition is introduced to ensure that the probability for any two servers to complete task executions at the same time is zero. In particular, if two servers complete task executions at the same time, it is better to assign these two servers to process two distinct tasks than to replicate a task on these two servers. Similar phenomena can be observed in the simulations of \cite{BinInfoCom2016}.
%%This point is important in the analysis of task replications, but was missed in prior studies.
%
%If  the job sizes are arbitrarily given and the task service times are  exponential, the delay performance of policy FUT-R is characterized as follows. 
%
%\begin{theorem}\label{thm2_exp}
%If (i) the task service times are exponential and independent across the servers, (ii) $\bm{O}=\bm{0}$, then for all \emph{$f\in\mathcal{D}_{\text{sym}}$},  \emph{$\pi\in\Pi$}, and $\mathcal{I}$
%\emph{
%\begin{align}\label{eq_delaygap3_exp}
%[f(\bm{V}(\text{FUT-R}))|\mathcal{I}] \leq_{\text{st}} [f(\bm{C}(\pi))|\mathcal{I}].
%\end{align}}
%\end{theorem}
%
%\begin{proof}
%For any policy $\pi\in\Pi$, suppose that policy FUT-R$_1$  (policy $\pi_1$) satisfies the same queueing discipline and stochastic law with policy FUT-R (policy $\pi$). Because exponential distribution is also NBU, using the arguments in the proof of Theorem \ref{thm1}, we can couple policy FUT-R$_1$ and policy $\pi_1$ to show that policy FUT-R$_1$ is weakly more work-efficient than policy $\pi_1$ with probability one. 
%Hence, by Proposition \ref{lem1_1}, for all $f\in\mathcal{D}_{\text{sym}}$
%\begin{align}
%\Pr[f(\bm{V}(\text{FUT-R}_1)) \leq f(\bm{C}(\pi_1)) |\mathcal{I}]=1. \nonumber
%\end{align}
%Then, by the property of stochastic ordering \cite[Theorem 1.A.1]{StochasticOrderBook}, we can obtain \eqref{eq_delaygap3_exp}. This completes the proof.
%%See Appendix \ref{app2_exp}.
%\end{proof}
%
%
%Consider the case of mean average delay, i.e., $f(\cdot)=D_{\text{avg}}(\cdot)$. It follows from \eqref{eq_delaygap3_exp} that
%\begin{align}\label{eq_delaygap1_3}
%\mathbb{E}[D_{\text{avg}}(\bm{V}(\text{FUT-R}))|\mathcal{I}] \leq&
%\min_{\pi\in\Pi}\mathbb{E}\left[D_{\text{avg}}(\bm{C}(\pi))\left.\right|\mathcal{I}\right]\leq \mathbb{E}[D_{\text{avg}}(\bm{C}(\text{FUT-R}))|\mathcal{I}].
%\end{align}
%Define $\overline{D}_{\text{gap},1}$ as the difference between the LHS and RHS of \eqref{eq_delaygap1_3}, we can obtain
%
%\begin{lemma}\label{lem7_NWU}
%Suppose that the $X_l$'s are {independent}~exponential, $E[X_l]= 1/\mu_l$, then for all $\mathcal{I}$
%\emph{\begin{align}\label{eq_gap_NWU}
%\overline{D}_{\text{gap},1} \leq\frac{1}{\sum_{j=1}^m\mu_j}.
%\end{align}}
%\end{lemma}
%\ifreport
%\begin{proof}
%See Appendix \ref{app_lem7_NWU}.
%\end{proof}
%\fi
%
%Hence, if $E[X_l]\leq 1/\mu$ for all $l$, the sub-optimality gap of policy FUT-R diminishes to zero at a speed of $O(1/m)$ as $m\rightarrow\infty$. We note that when there are multiple servers and multiple job classes, establishing tight bounds on the gap from the optimal delay performance of stochastic scheduling is extremely difficult, even in traditional queueing systems without  replications. There exist a few studies towards this goal: In \cite{Weiss:1992,Weiss:1995,Dacre1999}, closed-form upper bounds on the sub-optimality gaps of the Smith's rule  and Gittin's index policy were established for multi-server queueing systems. The upper bounds obtained in these studies are of the order $O(m)$, which are looser than the bounds in Lemma \ref{lem7_NBU} and Lemma \ref{lem7_NWU} for large $m$.
%
%%To the best of our knowledge, there exist only a few results on bounding on the gap from delay optimality, even in traditional multi-server queueing systems without task replications. In \cite{Weiss:1992,Weiss:1995,Dacre1999}, the sub-optimality gaps of Smith's rule and Gittin's index were characterized for multi-server queueing systems, where the obtained upper bounds on the sub-optimality gaps are of the order $O(m)$, which are clearly looser than the bounds obtained in Lemma \ref{lem7_NBU} and Lemma \ref{lem7_NWU}.
%
%
%Because exponential distribution is both NBU and NWU, both Theorem \ref{thm1} and Theorem \ref{thm2_exp} hold for exponential service time distributions. If the cancellation overhead $\bm{O}>\bm{0}$, one can use policy FUT to achieve near-optimal delay performance. If the cancellation overhead $\bm{O}=\bm{0}$, Lemma \ref{lem7_NBU} and Lemma \ref{lem7_NWU} tell us that it is better to use policy FUT-R, because policy FUT-R has a smaller sub-optimality gap than policy FUT; however, if policy FUT is employed, the delay performance is not degraded much. 

%By comparing Lemma \ref{lem7_NBU} with Lemma \ref{lem7_NWU}, we can see that for exponential service time distributions, policy FUT-R achieves a smaller sub-optimality gap than policy FUT.


% provide the first bounds on gap from delay optimality with such tightness.






%There is Prior attempts on solving the delay-optimal scheduling problem have met little success, except for some limiting scenarios such as large system limits, and heavy traffic limits.
%
%In \cite[Theorem 3]{Sun2015}, a sub-optimality gap was obtained for task replications in cloud storage systems: if the $X_l$'s are \emph{i.i.d.} exponential and $E[X_l]= 1/\mu$, then there exists a policy which is within a gap ${1}/{\mu}$ from the optimum, which is looser than \eqref{eq_gap_NWU}. In particular, when the number of servers $m\rightarrow\infty$, $\overline{D}_{\text{gap},1}$ and $\overline{D}_{\text{gap},2}$ are bounded by $[\ln(k_{\max})+1]/{\mu}$, while $\overline{D}_{\text{gap}} \rightarrow\infty$.
%If each job has $k$ tasks, we can further show that policy FUT-R is delay-optimal.
%\begin{corollary}\label{coro4}
%In addition to the conditions of Theorem \ref{thm2}, if $k_1=\ldots=k_n=k$, then for all \emph{$\pi\in\Pi$} and $\mathcal{I}$
%\emph{
%\begin{align}
%[f(\bm{C}(\text{FUT-R}))|\mathcal{I}]  \leq_{\text{st}} [f(\bm{C}(\pi))|\mathcal{I}].
%\end{align}}
%\end{corollary}
%\ifreport
%\begin{proof}
%See Appendix \ref{app2}.
%\end{proof}
%\fi


%{\red revised to here}




\subsection{Maximum Lateness $L_{\max}$ and the Delay Metrics in $\mathcal{D}_{\text{sym}}\cup\mathcal{D}_{\text{Sch-1}}$}
Next, we investigate the maximum lateness $L_{\max}$ and the delay metrics in $\mathcal{D}_{\text{sym}}\cup\mathcal{D}_{\text{Sch-1}}$. We consider a   \textbf{Earliest Due Date first (EDD)} policy: Each idle server is allocated to process a task from the job with the earliest due time among all jobs with unassigned tasks. Policy EDD can be obtained from Algorithm \ref{alg1} by revising step 10 as $j :=\arg\min\{d_i : i\in Q, \gamma_i>0\}$.
The delay performance of policy EDD is characterized in the following theorem.
\begin{theorem}\label{thm3}
If the task service times are NBU, independent across the servers, and {i.i.d.} across the tasks assigned to the same server, then for all ${\pi\in\Pi}$, and $\mathcal{I}$ %FPUT-NR satisfies
\emph{
\begin{align}\label{eq_delaygap1_thm3}
&[L_{\max}(\bm{V}(\text{EDD}))|\mathcal{I}] \leq_{\text{st}} \left[L_{\max}(\bm{C}(\pi))\left.\right|\mathcal{I}\right].
%,\\
%\label{eq_delaygap2_thm3}
%&[L_{\max}(\bm{V}(\text{EDD-NIR}))|\mathcal{I}] \leq_{\text{st}} [L_{\max}(\bm{C}(\pi))|\mathcal{I}].
\end{align}}
\end{theorem}



If the job sizes satisfy certain conditions, policy EDD is identical with policy FUT. In this case, policy EDD is near delay-optimal in stochastic ordering for minimizing both the average delay $D_{\text{avg}}(\cdot)$ and the maximum lateness $L_{\max}(\cdot)$. Interestingly, in this case policy EDD is near delay-optimal in stochastic ordering for minimizing all delay metrics in {$\mathcal{D}_{\text{sym}}\cup\mathcal{D}_{\text{Sch-1}}$}, as stated in the following theorem:

%In some scenarios, policy EDD simultaneously satisfy the conditions of Theorems \ref{thm1} and \ref{thm3}. Hence, policy EDD is near delay-optimal in distribution for minimizing the average delay $D_{\text{avg}}(\cdot)$ and the maximum lateness $L_{\max}(\cdot)$. In this case, we can show that policy EDD is also near delay-optimal in distribution for minimizing all delay metrics in {$\mathcal{D}_{\text{sym}}\cup\mathcal{D}_{\text{Sch-1}}$}, as stated in the following theorem:



%If the jobs parameters $\mathcal{I}$ satisfy certain conditions, Theorem \ref{thm3} can be generalized to all delay metrics in {$\mathcal{D}_{\text{sym}}\cup\mathcal{D}_{\text{Sch-1}}$}.

\begin{theorem}\label{coro_thm3_1}
If $k_1=\ldots=k_n=1$ (or $d_1\leq d_2\leq \ldots\leq d_n$ and $k_1\leq k_2 \leq \ldots\leq k_n$) and \emph{$L_{\max}$} is replaced by any \emph{$f\in\mathcal{D}_{\text{sym}}\cup\mathcal{D}_{\text{Sch-1}}$}, Theorem  \ref{thm3} still holds.
\end{theorem}
%\begin{proof}
%By replacing Proposition \ref{lem2} with Proposition \ref{coro2} in the proof of Theorem \ref{thm3},
%Theorem \ref{coro_thm3_1} is proven.
%%See Appendix \ref{app3}.
%\end{proof}



\subsection{Maximum Delay $D_{\max}$ and the Delay Metrics in $\mathcal{D}_{\text{sym}}\cup\mathcal{D}_{\text{Sch-2}}$}
We now study maximum delay $D_{\max}$ and the delay metrics in $\mathcal{D}_{\text{sym}}\cup\mathcal{D}_{\text{Sch-2}}$. We consider a \textbf{First-Come, First-Served  (FCFS)} policy: Each idle server is allocated to process a task from the job with the earliest arrival time among all jobs with unassigned tasks. Policy FCFS can be obtained from Algorithm \ref{alg1} by revising step 10 as $j :=\arg\min\{a_i : i\in Q, \gamma_i>0\}$. The delay performance of FCFS is characterized as follows:

\begin{corollary}\label{thm5}
If the task service times are NBU, independent across the servers, and {i.i.d.} across the tasks assigned to the same server, then for all  $\pi\in\Pi$, and $\mathcal{I}$
\emph{
\begin{align}\label{eq_delaygap1_thm5}
&[D_{\max}(\bm{V}(\text{FCFS}))|\mathcal{I}] \leq_{\text{st}} \left[D_{\max}(\bm{C}(\pi))|\mathcal{I}\right].
\end{align}}
\end{corollary}

In addition, if the job sizes satisfy certain conditions, policy FCFS is identical with policy FUT. Hence, policy FCFS is near delay-optimal in stochastic ordering for minimizing both the average delay $D_{\text{avg}}(\cdot)$ and the maximum delay $D_{\max}(\cdot)$. In this case, we can further show that policy FCFS is  near delay-optimal in distribution for minimizing all delay metrics in {$\mathcal{D}_{\text{sym}}\cup\mathcal{D}_{\text{Sch-2}}$}, as stated in the following:

%If the job sizes satisfy certain conditions, Theorem \ref{thm5} can be generalized to all delay metrics in {$\mathcal{D}_{\text{sym}}\cup\mathcal{D}_{\text{Sch-2}}$}.
\begin{corollary}\label{coro5_1}
If $k_1\leq k_2 \leq \ldots\leq k_n$ and \emph{$D_{\max}$} is replaced by any \emph{$f\in\mathcal{D}_{\text{sym}}\cup\mathcal{D}_{\text{Sch-2}}$}, Theorem  \ref{thm5} still holds.
\end{corollary}
The proofs of Corollaries \ref{thm5} and \ref{coro5_1} are omitted, because they follow directly from Theorems \ref{thm3} and \ref{coro_thm3_1} by
setting $d_i = a_i$ for all job $i$. 

%Next, we consider the sub-optimality delay gap of the FCFS policy for minimizing the mean maximum delay $\mathbb{E}\left[D_{\max}(\bm{C}(\pi))|\mathcal{I}\right]$ and mean $p$-norm of delay $\mathbb{E}\left[|| \bm{D}(\pi) ||_p|\mathcal{I}\right]$ for $p\geq 1$. 
In the sequel, we show that policy FCFS is within twice of the optimum for minimizing the mean maximum delay $\mathbb{E}\left[D_{\max}(\bm{C}(\pi))|\mathcal{I}\right]$ and mean $p$-norm of delay $\mathbb{E}\left[|| \bm{D}(\pi) ||_p|\mathcal{I}\right]$ for $p\geq 1$.\footnote{Because of the maximum operator over all jobs, $\mathbb{E}\left[D_{\max}(\bm{C}(\pi))|\mathcal{I}\right]$ will likely grow to infinite as the number of jobs $n$ increases. Hence, it is difficult to obtain an additive sub-optimality gap for minimizing $\mathbb{E}\left[D_{\max}(\bm{C}(\pi))|\mathcal{I}\right]$ that remains constant for all $n$.} 

\begin{lemma}\label{lem_ratio}
For arbitrarily given job parameters $\mathcal{I}$, if (i) the task service times are NBU and {i.i.d.} across the tasks and  servers, (ii) $f(\bm{x} + \bm{a})$ is sub-additive and increasing in $\bm{x}$, and (iii) two policies $P,\pi\in \Pi$ satisfy
\emph{ 
\begin{align}\label{eq_ratio_0}
 [f(\bm{V}(P))|\mathcal{I}] \leq_{\text{st}} \left[f(\bm{C}(\pi))|\mathcal{I}\right],
\end{align}}
then 
\emph{
\begin{align}\label{eq_ratio_1}
 [f(\bm{C}(P))|\mathcal{I}] \leq_{\text{st}}  \left[ 2 f(\bm{C}(\pi))|\mathcal{I}\right].
\end{align}}
\end{lemma}
\begin{proof}
See Appendix \ref{app_lem_ratio}.
\end{proof}

By applying Lemma \ref{lem_ratio} in Corollaries \ref{thm5} and \ref{coro5_1}, it is easy to obtain
\begin{theorem}\label{thm_max_delay_ratio}
If the task service times are NBU and {i.i.d.} across the tasks and  servers, then for all $\mathcal{I}$
\emph{
\begin{align}\label{}
&[D_{\max}(\bm{C}(\text{FCFS}))|\mathcal{I}] \leq_{\text{st}} [2 D_{\max}(\bm{C}(\pi))|\mathcal{I}],~\forall~\pi\in\Pi. \nonumber\\
&\mathbb{E}[D_{\max}(\bm{C}(\text{FCFS}))|\mathcal{I}] \leq\min_{\pi\in\Pi} 2 \mathbb{E}\left[D_{\max}(\bm{C}(\pi))|\mathcal{I}\right].\nonumber
\end{align}}
\end{theorem}
\begin{theorem}\label{thm_max_delay_ratio_1}
If (i) $k_1\leq k_2 \leq \ldots\leq k_n$, (ii) the task service times are NBU and {i.i.d.} across the tasks and  servers, (iii) $f(\bm{x} + \bm{a})$ is sub-additive and increasing in $\bm{x}$, (iv) \emph{$f\in\mathcal{D}_{\text{sym}}\cup\mathcal{D}_{\text{Sch-2}}$}, then for all $\mathcal{I}$
\emph{
\begin{align}
&[f(\bm{C}(\text{FCFS}))|\mathcal{I}] \leq_{\text{st}} [2 f(\bm{C}(\pi))|\mathcal{I}],~\forall~\pi\in\Pi. \nonumber\\
&\mathbb{E}[f(\bm{C}(\text{FCFS}))|\mathcal{I}] \leq\min_{\pi\in\Pi} 2 \mathbb{E}\left[f(\bm{C}(\pi))|\mathcal{I}\right].\nonumber
\end{align}}
\end{theorem}
There exist a fair large class of delay metrics satisfying the conditions (iii) and (iv) of Theorem \ref{thm_max_delay_ratio_1}. For example, consider the {$p$-norm of delay} $D_p(\bm{C}(\pi))=D_p(\bm{D}(\pi)+\bm{a}) = || \bm{D}(\pi) ||_p$ for $p\geq 1$. 
It is known that any norm is sub-additive, i.e., $|| \bm{x} + \bm{y} || \leq || \bm{x} || + || \bm{y} ||$. In addition, $|| \bm{D}(\pi) ||_p$ is symmetric and convex  in the delay vector $\bm{D}(\pi)$, and hence is Schur-convex in $\bm{D}(\pi)$. Therefore,
 $f = {D}_{p}$ satisfies the conditions (iii) and (iv) of Theorem \ref{thm_max_delay_ratio_1} for all $p\geq 1$.




%\begin{corollary}\label{coro6_1}
%In addition to the conditions of Theorem \ref{thm6}, if $k_1=\ldots=k_n=k$, then for all \emph{$f\in\mathcal{D}_{\text{sym}}\cup\mathcal{D}_{\text{Sch-2}}$}, \emph{$\pi\in\Pi$}, and $\mathcal{I}$
%\emph{
%\begin{align}\label{eq_coro6_1}
%[f(\bm{C}(\text{FCFS-R}))|\mathcal{I}] \leq_{\text{st}} [f(\bm{C}(\pi))|\mathcal{I}].
%\end{align}}
%\end{corollary}
%\begin{proof}
%See Appendix \ref{app6}.
%\end{proof}

%To conclude this section, we note that when task replications are not allowed, policy FUT-NR, policy EDD-NR, and policy FCFS-NR are near optimal for minimizing $D_{\text{avg}}$, $L_{\max}$, and $D_{\max}$, which will be studied in our future work.





==> v3/appendices.tex <==
% !TEX root = ./replication.tex
\ifreport
\appendices
\else
\appendix
\fi
\section{Proofs of Lemmas~1-3 and Corollaries 1-2} \label{app0}
\ifreport
\begin{proof}[Proof of Lemma \ref{lem1}]
\else
\begin{proof}[of Lemma \ref{lem1}]
\fi
First, fix the sequence of task completion times as $\bm{T}(\pi)=\bm{t}$ for all $\pi\in\Pi$. Because a job is completed at the time that the last task of the job is completed, each job completion time $C_i(\pi)$ must be equal to one element of $\bm{t}$. Using condition 2 and the sample-path optimality of the preemptive SRPT discipline \cite{Schrage68,Smith78}, one can obtain that for all $\pi\in\Pi$ and $\bm{t}\geq\bm{0}$
\begin{align}
[\bm{C}_{\uparrow} (P')|\bm{T}(P')=\bm{t}] \leq[\bm{C}_{\uparrow} (\pi)|\bm{T}(\pi)=\bm{t}],\nonumber
\end{align} 
where $\bm{C}_{\uparrow} (\pi)= (C_{(1)}(\pi),\ldots,$ $C_{(n)}(\pi))$ is the increasing time sequence of job completions. In addition, using the proof arguments in \cite{Schrage68,Smith78}, we can show that $[\bm{C}_{\uparrow} (P') | \bm{T}(P')=\bm{t}]$ is an increasing function of $\bm{t}$. This implies
\begin{align}\label{eq_order}
[\bm{C}_{\uparrow} (P')|\bm{T}(P')=\bm{t}] \leq[\bm{C}_{\uparrow} (\pi)|\bm{T}(\pi)=\bm{t}'],
\end{align} 
whenever $\bm{0}\leq\bm{t}\leq \bm{t}'$. On the other hand, condition 1 tells us that for all $\pi\in\Pi$ and $\mathcal{I}$
\begin{align}\label{eq_order_}
[\bm{T}(P')|\mathcal{I}] \leq_{\text{st}}[\bm{T}(\pi)|\mathcal{I}].
\end{align} 
%Therefore, 
%\begin{align}
%[{D}_{\text{avg}}(\bm{C}_{} (P))|\mathcal{I}] \leq_{\text{st}}[{D}_{\text{avg}}(\bm{C}_{} (\pi))|\mathcal{I}].\nonumber
%\end{align} 
According to Theorem 6.B.3 and Theorem 6.B.16(c) of \cite{StochasticOrderBook}, we can obtain from  \eqref{eq_order} and \eqref{eq_order_} that
\begin{align}\label{eq_order_1}
[\bm{C}_{\uparrow} (P')|\mathcal{I}] \leq_{\text{st}}[\bm{C}_{\uparrow} (\pi)|\mathcal{I}].
\end{align} 
Combining this and condition 3, we can get
\begin{align}
[\bm{U}_{\uparrow} (P)|\mathcal{I}] \leq_{\text{st}}[\bm{C}_{\uparrow} (\pi)|\mathcal{I}].\nonumber
\end{align} 
Since ${D}_{\text{avg}}\in \mathcal{D}_{\text{sym}}$ is symmetric and increasing, we can obtain that for all $\pi\in\Pi$ and $\mathcal{I}$
\begin{align}
&[{D}_{\text{avg}}(\bm{U} (P))|\mathcal{I}]=[{D}_{\text{avg}}(\bm{U}_{\uparrow} (P))|\mathcal{I}] \nonumber\\
\leq_{\text{st}}&[{D}_{\text{avg}}(\bm{C}_{\uparrow} (\pi))|\mathcal{I}] = [{D}_{\text{avg}}(\bm{C} (\pi))|\mathcal{I}],\nonumber
\end{align} 
where the inequality follows from Theorem 6.B.16(a) of \cite{StochasticOrderBook}. By this, \eqref{eq_lem1_1} is proven.

If condition 3 is replaced by $P'=P$, then \eqref{eq_lem1_2} follows from \eqref{eq_order_1} and Theorem 6.B.16(a) of \cite{StochasticOrderBook}. This completes the proof.
%In addition, 
%
%Let $[{D}_{\text{avg},\pi} |\mathcal{I}, (t_{1,\pi},\ldots,t_{J,\pi}) = (t_1,$ $\ldots, t_J)]$ denote the average delay of policy $\pi$ for given parameters $\mathcal{I}$ and task completion instants $(t_1,\ldots, t_J)$. According to the sample-path optimality of the preemptive SRPT discipline \cite{Schrage68,Smith78}, $[{D}_{\text{avg},\pi} | \mathcal{I}, (t_{1,\pi},\ldots,t_{J,\pi}) = (t_1,\ldots,$ $ t_J)]$ is minimized among all policies in $\Pi$, if each completed task belongs to a job with the fewest remaining tasks. By condition 2, policy $P$ satisfies this requirement, and hence
%\begin{align}
%&~~~[{D}_{\text{avg},P} | \mathcal{I}, (t_{1,P},\ldots,t_{J,P}) = (t_1,\ldots, t_J)] \nonumber\\
%&\leq [{D}_{\text{avg},\pi} | \mathcal{I}, (t_{1,\pi},\ldots,t_{J,\pi}) = (t_1,\ldots, t_J)],~\forall~\pi\in\Pi.\nonumber
%\end{align}
%Further, $[{D}_{\text{avg},\pi} | \mathcal{I}, (t_{1,\pi},\ldots,t_{J,\pi}) = (t_1,\ldots, t_J)]$ is an increasing function of $(t_1,\ldots, t_J)$, because if task completions are postponed, the job completions are also postponed.
%Therefore, for any $\pi\in\Pi$, we have
%\begin{align}\label{eq_order}
%&~~~[{D}_{\text{avg},P} | \mathcal{I}, (t_{1,P},\ldots,t_{J,P}) = (t_1,\ldots, t_J)] \nonumber\\
%&\leq [{D}_{\text{avg},\pi} | \mathcal{I}, (t_{1,\pi},\ldots,t_{J,\pi}) = (t_1',\ldots,t_J')],\nonumber\\
%&~~~~~~~~~~~~~~~~~~~~\text{whenever}~(t_1,\ldots, t_J)\leq (t_1',\ldots,t_J').
%\end{align}
%By condition 1, we can obtain 
%\begin{align}\label{eq_order_}
%(t_{1,P},\ldots,t_{J,P})\leq_{\text{st}}(t_{1,\pi},\ldots,t_{J,\pi}),~\forall~\pi\in\Pi.
%\end{align}
%With \eqref{eq_order} and \eqref{eq_order_}, we can use the standard construction argument
% in Theorem 6.B.3 of \cite{StochasticOrderBook} to show that for all $\pi\in\Pi$
%\begin{align}\label{eq_order1}
%\!\!\!\![{D}_{\text{avg},P}, (t_{1,P},\ldots,t_{J,P})| \mathcal{I}] \leq_{\text{st}} [{D}_{\text{avg},\pi}, (t_{1,\pi},\ldots,t_{J,\pi}) | \mathcal{I}].\!\!\!\!
%\end{align}
%Then, \eqref{eq_thm1} follows from \eqref{eq_order1} and Theorem 6.B.16 (c) of \cite{StochasticOrderBook}. 
%Finally, \eqref{eq_thm1_1} follows from condition 3, \eqref{eq_thm1}, and Eq (6.B.4) of \cite{StochasticOrderBook}.
%By Theorem \ref{thm1}, for all $\mathcal{I}$, we have
%\begin{align}
%\mathbb{E}[{D}_{\text{avg},P'}| \mathcal{I}]  \leq \mathbb{E}[{D}_{\text{avg},\pi}| \mathcal{I}],~\forall~\pi\in\Pi.\nonumber
%\end{align}
%%Hence,
%%\begin{align}
%%[{D}_{\text{avg},P'}| \mathcal{I}]  \leq_{\text{st}} [{D}_{\text{avg},\pi}| \mathcal{I}],~\forall~\pi\in\Pi.\nonumber
%%\end{align}
%%
%%Because $G$ is independent of $P$, $P'$, and $\mathcal{I}$, by Theorem 1.A.3 (b) of \cite{StochasticOrderBook}, we have
%%\begin{align}
%%[{D}_{\text{avg},P'}| \mathcal{I}] +G  \leq_{\text{st}} [{D}_{\text{avg},\pi}| \mathcal{I}] + G,~\forall~\pi\in\Pi.\nonumber
%%\end{align}
%This, together with condition 3, implies %\eqref{eq_thm2}. Finally, 
%\eqref{eq_thm2_1}. % follows from \eqref{eq_thm2} and Eq (6.B.4) of \cite{StochasticOrderBook}.
\end{proof}
\ifreport
\begin{proof}[Proof of Corollary \ref{coro1}]
\else
\begin{proof}[of Corollary \ref{coro1}]
\fi
Corollary \ref{coro1} is proven by replacing ${D}_{\text{avg}}$ in the proof of Lemma \ref{lem1} with any $f\in\mathcal{D}_{\text{sym}}$.
\end{proof}


\ifreport
\begin{proof}[Proof of Lemma \ref{lem2}]
\else
\begin{proof}[of Lemma \ref{lem2}]
\fi

First, fix the sequence of task completion times such that $\bm{T}(P')=\bm{T}(\pi)=\bm{t}$ for all $\pi\in\Pi$. Using condition 2 and the sample-path optimality of the preemptive earliest due date (EDD) discipline \cite{Jackson55}, one can obtain that for all $\pi\in\Pi$ and $\bm{t}\geq\bm{0}$
\begin{align}
[L_{\max}(\bm{C}(P'))|\bm{T}(P')=\bm{t}] \leq[L_{\max}(\bm{C}(\pi))|\bm{T}(\pi)=\bm{t}].\nonumber
\end{align} 
In addition, one can show that $[L_{\max}(\bm{C}(P')) | \bm{T}(P')=\bm{t}]$ is increasing in $\bm{t}$. Hence,
\begin{align}\label{eq_lem2_order1}
[L_{\max}(\bm{C}(P'))|\bm{T}(P')=\bm{t}] \leq[L_{\max}(\bm{C}(\pi))|\bm{T}(\pi)=\bm{t}'],
\end{align} 
whenever $\bm{0}\leq\bm{t}\leq \bm{t}'$. On the other hand, condition 1 tells us that for all $\pi\in\Pi$ and $\mathcal{I}$
\begin{align}\label{eq_lem2_order2}
[\bm{T}(P')|\mathcal{I}] \leq_{\text{st}}[\bm{T}(\pi)|\mathcal{I}].
\end{align} 
Using \eqref{eq_lem2_order1}, \eqref{eq_lem2_order2}, Theorem 6.B.3, and Theorem 6.B.16(c) of \cite{StochasticOrderBook}, yields that for all $\pi\in\Pi$ and $\mathcal{I}$
\begin{align}\label{eq_lem2_order3}
[L_{\max}(\bm{C}(P'))|\mathcal{I}] \leq_{\text{st}}[L_{\max}(\bm{C}(\pi))|\mathcal{I}].
\end{align} 
Using condition 3, the fact that $L_{\max}$ is increasing, and Theorem 6.B.16(a) of \cite{StochasticOrderBook}, we can obtain 
\begin{align}\label{eq_lem2_order4}
[L_{\max}(\bm{U}(P))|\mathcal{I}]\leq_{\text{st}} [L_{\max}(\bm{C}(P'))|\mathcal{I}].
\end{align} 
Combining \eqref{eq_lem2_order3} and \eqref{eq_lem2_order4}, \eqref{eq_lem2_1} follows. If condition 3 is replaced by $P'=P$, then 
\eqref{eq_lem2_2} follows from \eqref{eq_lem2_order3}. This completes the proof.
\end{proof}
\ifreport
\begin{proof}[Proof of Corollary \ref{coro2}]
\else
\begin{proof}[of Corollary \ref{coro2}]
\fi
We need the rearrangement partial ordering $\leq^{\text{a}}$ defined in \cite[Sec. 6.F]{Marshall2011}: Consider two $n$-vector $\bm{x}$ and $\bm{y}$, $\bm{x}$ is said to \emph{immediately precede} $\bm{y}$ by one pairwise interchange, denote $\bm{x}<^{\text{p}}\bm{y}$, if for some index $i$, $1\leq i\leq n-1$,
\begin{align}
y_i<y_{i+1}, ~x_i= y_{i+1}, ~x_{i+1}=y_i, ~x_l= y_l,~l\neq i,i+1.\nonumber
\end{align}
Let $\leq^{\text{b}}$ denote the ordering of successive interchanges, such that $\bm{x}\leq^{\text{b}}\bm{y}$ if $\bm{x}=\bm{y}$ or if there exists a finite chain $\bm{z}^1,\ldots,\bm{z}^k$ of permutations such that
\begin{align}
\bm{x}<^{\text{p}}\bm{z}^1<^{\text{p}}\ldots<^{\text{p}}\bm{z}^k<^{\text{p}}\bm{y}.\nonumber
\end{align}
Suppose that $\bm{x}$ is a permutation of $\bm{u}$ and $\bm{y}$ is a permutation of $\bm{v}$ such that $\bm{x}_{\uparrow}=\bm{u}_{\uparrow}$ and $\bm{y}_{\uparrow}=\bm{v}_{\uparrow}$. Then, $(\bm{x},\bm{y})\leq^{\text{a}} (\bm{u},\bm{v})$ if there exists permutation matrices $W$ and $U$ such that
\begin{align}
\bm{x}W = \bm{u} U=\bm{x}_{\uparrow},~~~\text{and}~~ \bm{y} W \leq^{\text{b}} \bm{v} U.\nonumber
\end{align}
Hence, one can obtain
\begin{align}
(\bm{x}_{\uparrow},\bm{y}_{\downarrow})\leq^{\text{a}}(\bm{x},\bm{y})\leq^{\text{a}}(\bm{x}_{\uparrow},\bm{y}_{\uparrow}).\nonumber
\end{align}
The following rearrangement inequality is an immediate consequence of Theorem F.14 in Chapter 6 of \cite{Marshall2011}:
\begin{lemma}\label{lem_coro_2}
If \emph{$(\bm{x},\bm{y})\geq^{\text{a}} (\bm{u},\bm{v})$}, then
\begin{align}
\bm{x}-\bm{y}\prec \bm{u}-\bm{v}.\nonumber
\end{align}
\end{lemma}

Now, we are ready to prove Corollary \ref{coro2}. As before, we first fix the sequence of task completion times such that $\bm{T}(P')=\bm{T}(\pi)=\bm{t}$ for all $\pi\in\Pi$. Since $k_1=\ldots=k_n=1$, $\bm{C}(P')$ and $\bm{C}(\pi)$ are permutations of $\bm{t}$. According to condition 2 of Lemma \ref{lem2}, each completed job of policy $P'$ has the smallest due time $d_i$ among all unfinished jobs in the queue. Hence,
\begin{align}
[(\bm{C}(P'), \bm{d}) |\bm{T}(P')=\bm{t}] \geq^{\text{a}} [(\bm{C}(\pi), \bm{d}) |\bm{T}(\pi)=\bm{t}].\nonumber
\end{align}
Then, Lemma \ref{lem_coro_2} tells us that for all $\pi\in\Pi$
\begin{align}\label{eq_coro2_4}
&[\bm{L} (P') |\bm{T}(P')=\bm{t}]\nonumber\\
=&[\bm{C}(P') - \bm{d}|\bm{T}(P')=\bm{t}]\nonumber\\
\prec& [\bm{C}(\pi) - \bm{d}|\bm{T}(\pi)=\bm{t}] \nonumber\\
=&[\bm{L}(\pi)|\bm{T}(\pi)=\bm{t}]. 
\end{align} 
%it is easy to show that $t_{i}\leq {C}_{(i)}(\pi)$ for all $i=1,2,\ldots, n$ and $\pi\in\Pi$. Using condition 2 of Lemma \ref{lem2}, we can obtain that for all $\pi\in\Pi$
%\begin{align}\label{eq_coro2_1}
%[\bm{C}_{\uparrow}(P')|\bm{T}(P')=\bm{t}] = (t_1,t_{2},\ldots,t_{n}) \leq [\bm{C}_{\uparrow}(\pi)|\bm{T}(\pi)=\bm{t}].
%\end{align} 
%On the other hand, the rearrangement inequality \cite[Theorem F.14 of Sec. 6]{Marshall2011} implies that for all $\pi\in\Pi$
%\begin{align}\label{eq_coro2_2}
%\bm{C}_{\uparrow}(\pi) - \bm{d}_{\uparrow} \prec \bm{C}(\pi) - \bm{d}.
%\end{align} 
%In addition, condition 2 of Lemma \ref{lem2} tells us that the jobs are completed in the increasing order of $\bm{d}$. Hence, the job completed at time $C_{(i)}(P')$ has a due time $d_{(i)}$ for all $i=1,\ldots,n$. This implies
%\begin{align}\label{eq_coro2_3}
%\bm{L}_{\uparrow} (P')= \bm{C}_{\uparrow}(P') - \bm{d}_{\uparrow}.
%\end{align} 
%Combining \eqref{eq_coro2_1}-\eqref{eq_coro2_3}, yields for all $\pi\in\Pi$
%\begin{align}\label{eq_coro2_4}
%&[\bm{L}_{\uparrow} (P') |\bm{T}(P')=\bm{t}]\nonumber\\
%=&[\bm{C}_{\uparrow}(P') - \bm{d}_{\uparrow}|\bm{T}(P')=\bm{t}]\nonumber\\
%\leq&[\bm{C}_{\uparrow}(\pi)- \bm{d}_{\uparrow}|\bm{T}(\pi)=\bm{t}]\nonumber\\
%\prec& [\bm{C}(\pi) - \bm{d}|\bm{T}(\pi)=\bm{t}] \nonumber\\
%=&[\bm{L}(\pi)|\bm{T}(\pi)=\bm{t}]. 
%\end{align} 
For any $f\in\mathcal{D}_{\text{Sc}}$, define $g(\bm{x})=f(\bm{x}+\bm{d})$. Then, $g$ is Schur convex. For $\pi\in\Pi$, we can obtain
\begin{align}
&[f(\bm{C} (P')) |\bm{T}(P')=\bm{t}]\nonumber\\
=&[g(\bm{L} (P') ) |\bm{T}(P')=\bm{t}]\nonumber\\
\leq&[g(\bm{L} (\pi)) |\bm{T}(\pi)=\bm{t}]\nonumber\\
=&[f(\bm{C} (\pi)) |\bm{T}(\pi)=\bm{t}],\nonumber
\end{align}
where the inequality is due to \eqref{eq_coro2_4} and the definition of Schur convex functions. The remaining proof is the same as \eqref{eq_lem2_order1}-\eqref{eq_lem2_order4}, where we will need to use the fact that $f$ is increasing.
\end{proof}

%\begin{proof}[of Lemma \ref{thm1}]
%
%\end{proof}
%
%\begin{proof}[of Lemma \ref{thm3}]
%Let $[L_{\max,\pi} | \mathcal{I}, (t_{1,\pi},\ldots,t_{J,\pi}) = (t_1,$ $\ldots, t_J)]$ denote the maximum lateness of policy $\pi$ for given parameters $\mathcal{I}$ and task completion instants $(t_1,\ldots, t_J)$. According to the sample-path optimality of the preemptive Earliest Due Date (EDD) discipline \cite{Jackson55}, $[L_{\max,\pi} | \mathcal{I}, (t_{1,\pi},\ldots,$ $t_{J,\pi}) = (t_1,\ldots, t_J)]$ is minimized among all policies in $\Pi$, if each completed task belongs to the job with the earliest due date. By condition 2, policy $R$ satisfies this requirement, and hence
%\begin{align}
%&~~~[L_{\max,R} | \mathcal{I}, (t_{1,R},\ldots,t_{J,R}) = (t_1,\ldots, t_J)] \nonumber\\
%&\leq [L_{\max,\pi} | \mathcal{I}, (t_{1,\pi},\ldots,t_{J,\pi}) = (t_1,\ldots, t_J)],~\forall~\pi\in\Pi.\nonumber
%\end{align}
%%Further, $[L_{\max,\pi} | \mathcal{I}, (t_{1,\pi},\ldots,t_{J,\pi}) = (t_1,\ldots, t_J)]$ is an increasing function of $(t_1,\ldots, t_J)$, because if task completions are postponed, the job completions are also postponed. 
%The remaining proof steps are the same with Theorem \ref{thm1}.
%%Therefore, for all $\pi\in\Pi$, we have
%%\begin{align}\label{eq_order2}
%%&~~~~[L_{\max,R} | \mathcal{I}, (t_{1,R},\ldots,t_{J,R}) = (t_1,\ldots, t_J)] \nonumber\\
%%&\leq [L_{\max,\pi} | \mathcal{I}, (t_{1,\pi},\ldots,t_{J,\pi}) = (t_1',\ldots,t_J')],\nonumber\\
%%&~~~~~~~~~~~~~~~~~~~~\text{whenever}~(t_1,\ldots, t_J)\leq (t_1',\ldots,t_J').
%%\end{align}
%%Using condition 1, \eqref{eq_order2}, and the proof arguments of Theorem 6.B.3 of \cite{StochasticOrderBook}, we can obtain that  for all $\pi\in\Pi$
%%\begin{align}\label{eq_order3}
%%(L_{\max,R},t_{1,R},t_{2,R},\ldots) \leq_{\text{st}} (L_{\max,\pi}, t_{1,\pi},t_{2,\pi},\ldots).
%%\end{align}
%%Then, \eqref{eq_thm3} follows from \eqref{eq_order3} and Theorem 6.B.16 (c) of \cite{StochasticOrderBook}. Finally, \eqref{eq_thm3_1} follows from \eqref{eq_thm3} and Eq (6.B.4) of \cite{StochasticOrderBook}.
%\end{proof}



%\begin{proof}[of Lemma \ref{thm4}]
%The proof steps are the same with Theorem \ref{thm2}.
%\end{proof}

\ifreport
\begin{proof}[Proof of Lemma \ref{lem3}]
\else
\begin{proof}[of Lemma \ref{lem3}]
\fi
Using \eqref{eq_lem3_1} and $\bm{U}(\pi)\leq\bm{C}(\pi)$, we can obtain $[\bm{U}(P)|\mathcal{I}] \leq_{\text{st}} [\bm{C}(\pi)|\mathcal{I}]$ for all $\pi\in\Pi_{PL}$. By this, Theorem 6.B.4.(a) of \cite{StochasticOrderBook}, and the fact that $f$ is increasing, \eqref{eq_lem3_2} follows. This completes the proof.
\end{proof}

==> v3/appendices_2.tex <==


\section{Proofs of Theorem~1 and Corollary 3} \label{app1}
\subsection{Proof of {\large \eqref{eq_delaygap1}} in Theorem \ref{thm1}} \label{sec_app_thm1_1}
We prove \eqref{eq_delaygap1} by using the sufficient conditions in Lemma \ref{lem1} and Corollary \ref{coro1}. The proof steps are as follows:

{\bf Construction of Policy $P'$:}
We construct an {infeasible} policy $P'$. \emph{First, in policy $P'$, all servers are busy whenever the queue is not empty.} If the number of tasks is less than $m$, some tasks are replicated over multiple servers. 
\emph{Second, the task completion times of policy $P'$ are constructed as if there is no task cancellations.} Suppose that at any time $t$, server $l$ has processed a task for $\tau$ seconds, and another copy of this task is completed at time $t$ on another server. In policy $P'$, server $l$ will cancel this task and process a new task. More specifically, in policy $P'$, server $l$ will not process the new task from scratch; instead, it is assumed that the new task assigned to server $l$ has already been processed for $\tau$ seconds by time $t$ (which is infeasible),~and server $l$ will serve the task from this progress point. If two task copies are completed at the same time on two servers, they are assumed to be distinct tasks, instead of two replicated copy of the same task. 
\emph{Finally, the completed tasks of policy $P'$ are relabelled such that each completed task is from the job with the fewest remaining tasks}. (This relabeling operation might be infeasible, because the tasks from different jobs may be simultaneously processed on parallel servers.) 
By this, policy $P'$ is constructed.


%\emph{In policy $P'$, all servers are working whenever the queue is not empty, and task cancellations do not affect the task completion times in policy $P'$.} More specifically, if the number of remaining tasks is larger than 0 and less than the number of servers $m$, some of the tasks are replicated over multiple servers to make sure that all servers are working. 

%In both policy $P'$ and FUT-NR, all servers are busy whenever the queue is not empty. 
%
%Suppose that at any time $t$, server $l$ has processed a task for $\tau$ seconds, and another copy of this task is completed at time $t$ on another server. In FUT-NR, after canceling the task with some delay overhead, server $l$ will process a new task that have not been served. 
%%In policy $P'$, task cancellations are implemented for two cases: If server $l$ is an NWU server, server $l$ will process a new task that have not been served (the same as FUT-NR). If server $l$ is an NBU server, 
%In policy $P'$, server $l$ will not process a new task from scratch; instead, it is assumed that at time $t$, the next task assigned to server $l$ is already processed for $\tau$ seconds by a genie (which is infeasible!) and server $l$ will serve the task from this progress point. Therefore, in policy $P'$, the task completion times of NBU servers are constructed as if there is no task cancellations. Finally, the completed tasks in policy $P'$ are relabelled such that each completed task is from the job with the fewest remaining tasks (which is also infeasible, because the tasks from different jobs are processed simultaneously). Note that both policy $P'$ and FUT-NR are work-conserving.

Next, we prove the conditions of Lemma \ref{lem1} one by one.

\textbf{Condition 1:} \emph{Policy $P'$ is more {work-efficient} than any policy $\pi\in\Pi$}. 
%Recall that $\bm{T}(\pi)=(T_1(\pi),\ldots, T_{k_{\text{sum}}}(\pi))$ is the sequence of task completion times of the system. 
\ifreport
\begin{proof}[Proof of Condition 1]
\else
\begin{proof}[of Condition 1]
\fi
We prove condition 1 by induction. Consider the first task completion time $T_1(\pi)$. Job 1 arrives at time $a_1=0$. 
If policy $\pi$ is non-preemptive and work-conserving, then
\begin{align}
[T_1(\pi)|\mathcal{I}]=\min_{l=1,\ldots,m} X_l.\nonumber
\end{align} 
If policy $\pi$ is preemptive and work-conserving, then some  servers may cancel the current task and switch to process a new task at time $t\in[0,T_1(\pi))$, then Lemma \ref{lem_property_MNBUMNWU} tells us that
\begin{align}\label{eq_condition1_2_1}
\min_{l=1,\ldots,m} X_l \leq_{\text{st}}[T_1(\pi)|\mathcal{I}].
\end{align}
If policy $\pi$ is non-work-conserving, then \eqref{eq_condition1_2_1} still holds, because of the possibility of server idleness. Since policy $P'$ is non-preemptive and work-conserving, we can obtain that for all $\pi\in\Pi$
\begin{align}\label{eq_condition1_2}
[T_1(P')|\mathcal{I}]=\min_{l=1,\ldots,m} X_l\leq_{\text{st}}[T_1(\pi)|\mathcal{I}].
\end{align} 



Next, consider the update from $T_j(\pi)$ to $T_{j+1}(\pi)$. Recall that $s_j$ is the $j$-th task arrival time of the system. If $s_{j+1}>T_j(\pi)$, the first $j$ tasks are completed before the $(j+1)$-th task arrives, hence all servers are idle during $[T_j(\pi),s_{j+1})$; otherwise, if $s_{j+1}\leq T_j(\pi)$, the servers can keep working after $T_j(\pi)$. For any work-conserving policy $\pi$, we can obtain
\begin{eqnarray}\label{eq_thm1_2}
T_{j+1}(\pi)\!=\max\{s_{j+1},T_j(\pi)\} + \!\min_{l=1,\ldots,m} R_{j,l}(\pi),
\end{eqnarray}
where $R_{j,l}(\pi)$ is the time duration for server $l$ to complete a task after time $\max\{s_{j+1},T_j(\pi)\}$. 



Suppose that $s_{j+1}\leq T_j(\pi)$ and server $l$ has spent $\tau_l$ ($\tau_l\geq0$) seconds on a task by time $T_j(\pi)$. 
In policy $P'$,  the task completion times are constructed as if there is no task cancellations. Hence, the tail probability for the servers to complete a task after time $T_j(P')$ is 
\begin{align}\label{eq_thm1_7}
&\Pr\Big[\min_{l=1,\ldots,m} R_{j,l}(P')>t\Big]\nonumber\\
=& \Pr\Big[\min_{l=1,\ldots,m}(X_l-\tau_l)>t\Big|\bm{X}> \bm{\tau} \Big].
\end{align}
If $\pi$ is a non-preemptive work-conserving policy, some servers may cancel the tasks they are processing  at time $T_j(\pi)$. If the servers in $\mathcal{S}^c$ cancel the current task and switch to process a new task at time $T_j(\pi)$, then the tail probability for the servers to complete a task after time $T_j(\pi)$ is 
\begin{align}\label{eq_thm1_8}
&\Pr\Big[\min_{l=1,\ldots,m} R_{j,l}(\pi)>t\Big]\nonumber\\
=&\Pr\!\Big[\min\Big\{\min_{l\in\mathcal{S}}(X_l-\tau_l),\min_{l\in\mathcal{S}^c}X_l\Big\}\!>t \Big| \bm{X}_{\mathcal{S}}> \bm{\tau}_{\mathcal{S}}\Big].
\end{align} 
Combining \eqref{eq_thm1_7}, \eqref{eq_thm1_8}, and Lemma \ref{lem_property_MNBUMNWU}, yields 
\begin{align}\label{eq_min}
\min_{l=1,\ldots,m} R_{j,l}(P') \leq_{\text{st}} \min_{l=1,\ldots,m} R_{j,l}(\pi).
\end{align}
If $\pi$ is a preemptive work-conserving policy, then some servers may cancel the current task and switch to process a new task at a particular time $t\in[T_j(\pi),T_{j+1}(\pi))$.
In this case, we can use Lemma \ref{lem_property_MNBUMNWU} to show that \eqref{eq_min} holds. Hence, \eqref{eq_min} holds for all work-conserving policy $\pi$. 

Suppose that $s_{j+1}> T_j(\pi)$, then the servers start to process new tasks at time $s_{j+1}$. In this case, we can show that
\eqref{eq_min} also holds for all work-conserving policy $\pi$. 

Using \eqref{eq_thm1_2}, \eqref{eq_min}, and the fact that $s_j$ is uniquely determined by $\mathcal{I}$, it follows that for all work-conserving policy $\pi$
\begin{align}\label{eq_thm1_4}
[T_{j+1}(P') | \mathcal{I},  T_j(P') = t_j] \leq_{\text{st}} [T_{j+1}(\pi) | \mathcal{I},  T_j(\pi) = t_j'] \nonumber\\
\text{whenever}~ t_j \leq t_j',j=1,2,\ldots
\end{align}
If policy $\pi$ is non-work-conserving, \eqref{eq_thm1_2} becomes
\begin{eqnarray}\label{eq_thm1_2_1}
T_{j+1}(\pi)\!\geq\max\{s_{j+1},T_j(\pi)\} + \!\min_{l=1,\ldots,m} R_{j,l}(\pi),\nonumber
\end{eqnarray}
because of the possibility of server idleness. In this case, \eqref{eq_thm1_4} still holds. Hence, \eqref{eq_thm1_4} holds for all $\pi\in\Pi$.
Then, combining \eqref{eq_condition1_2}, \eqref{eq_thm1_4}, and Theorem 6.B.3 of \cite{StochasticOrderBook}, yields
\begin{align}%\label{eq_thm1_5}
[(T_1(P'),\ldots,T_j(P'))|\mathcal{I}] \leq_{\text{st}} [(T_1(\pi),\ldots,T_j(\pi))|\mathcal{I}],~\forall~\pi\in\Pi.\nonumber
\end{align}
Hence, condition 1 is proven.
\end{proof}

\textbf{Condition 2:} \emph{Each completed task of policy $P'$ belongs to the job with the fewest remaining tasks}. Condition 2 directly follows from the construction of policy $P'$.

\textbf{Condition 3:} \emph{It holds that} 
%\begin{align}
%\mathbb{E}\left[{D}_{\text{avg,FUT-NR}}\right]\leq \mathbb{E}\left[{D}_{\text{avg}}(P')| \mathcal{I}\right] \nonumber\\
%+\frac{1}{N}\sum_{h=1}^N \max_{\substack{S: |S|\leq k_i\\
%S\subseteq\{1,\ldots,m\}}}\!\!\mathbb{E}\left[\max_{l\in S} X_l\right].
%\end{align}
\begin{align}\label{eq_condition3}
[\bm{U}_{\uparrow}(\text{FUT-NR})|\mathcal{I}] \leq_{\text{st}} [\bm{C}_{\uparrow}(P')|\mathcal{I}].
\end{align}
We prove condition 3 by a \emph{sample-path ordering} technique, which is motivated by the second proof of the  optimality of SRPT in single-server queueing systems \cite{Smith78}. The generalization from \cite{Smith78} to this {sample-path ordering} technique is non-trivial and unexpected when this research started.


%It is difficult to compare policies $P'$ and FUT-NR directly.~Hence, we will construct an intermediate policy called
%Fewest Positive Unassigned Tasks first with Virtual Tasks (FUT-VT), and prove the following results:
%\begin{align}\label{eq_condition3_1}
%&[{D}_{\text{avg,FUT-NR}}|\mathcal{I}]  \leq_{\text{st}} [{D}_{\text{avg,FUT-VT}}| \mathcal{I}],\\
%&[{D}_{\text{avg,FUT-VT}}|\mathcal{I}]  \leq_{\text{st}} [{D}_{\text{avg}}(P')| \mathcal{I}] + G.\label{eq_condition3_2}
%\end{align}
%Then, \eqref{eq_condition3} follows from \eqref{eq_condition3_1} and \eqref{eq_condition3_2}. 
%
%First, we construct the sample path of policy FUT-VT. In FUT-VT, there are always $m$ virtual tasks in the system, each belongs to a virtual job. Because of these $m$ virtual tasks, the total number of remaining tasks is always no smaller than $m$. Hence, there is no task replications in FUT-VT. In the meanwhile, the task completion times of policy $P'$ are constructed as if there is no task cancellations. Therefore, the task completion sample paths of policies $P'$ and FUT-VT can be aligned (see Fig. \ref{fig_compare} for an illustration): Consider a busy period $[\tau,\nu)$ of policy $P'$. If all $m$ servers start to process new tasks at time $\tau$ in both policies $P'$ and FUT-VT, the task completion times of the two policies are exact the same during the period $[\tau,\nu)$. At time $\nu$, the queue of policy $P'$ is empty, and hence all severs becomes empty.  
%
%An illustration of FUT-NR, FUT-VT, and the lower bound policy $P'$ is provided in .
%
% policy $P'$
%
%On the other hand, there is no virtual task in FUT-NR and hence the servers can spend time to process replicated task copies, instead of wasting time on virtual tasks. By this, \eqref{eq_condition3_1} follows. 
%
%Next, we compare policies $P'$ and FUT-VT. Consider the completion times $(T_1(\pi),\ldots,T_j(\pi))$ of the first $J$ tasks in policies $P'$ and FUT-VT. Note that virtual tasks are completed in FUT-VT, which is not counted in job completion time. We will show that 
%\begin{align}
%[(t_{1,\text{FUT-VT}},\ldots,t_{J,\text{FUT-VT}})|\mathcal{I}] \leq_{\text{st}} [(T_1(P'),\ldots,T_j(P'))|\mathcal{I}].
%\end{align}


First, we define the system states of policies $P'$ and FUT-NR. 
\begin{definition}\label{def_state_P}
The system state of  policy $P'$ is specified by an infinite vector $\bm{\beta}=(\beta_1,\beta_2,\ldots)$ with non-negative, non-increasing components. At any time, the coordinates of $\bm{\beta}$ are interpreted as follows: $\beta_1$ is the maximum number of remaining tasks among all jobs in the queue, $\beta_2$ is the next greatest number of remaining tasks among all jobs in the queue, and so on, with duplications being explicitly repeated. If there are $l$ unfinished jobs in the system, then it holds that
\begin{eqnarray}
\beta_1\geq\beta_2\geq\ldots\geq\beta_l>0 = \beta_{l+1} =\beta_{l+2}=\ldots.\nonumber
\end{eqnarray}
\end{definition}

\begin{definition}\label{def_state}
The system state of FUT-NR is specified by a pair of infinite vectors $\bm{\alpha}=(\alpha_1,\alpha_2,\ldots)$ and $\bm{\delta}=(\delta_1,\delta_2,$ $\ldots)$ with non-negative components. At any time, the coordinates of $\bm{\alpha}$ and $\bm{\delta}$ are interpreted as follows: $\alpha_h$ is the number of unfinished tasks of the job associated to the $h$-th coordinate, and $\delta_h$ out of these $\alpha_h$ tasks are being processed on some servers. Hence, 
\begin{align}\label{eq_def_state}
\delta_h \leq \alpha_h\leq k_{\max},~\sum_{h=1}^\infty \delta_h\leq m. 
\end{align}
The coordinates of $\bm{\alpha}$ and $\bm{\delta}$ are sorted in the non-increasing order of $\alpha_h-\delta_h$, with duplications being explicitly repeated. 
%When $\alpha_h-\delta_h=\alpha_{i+1}-\delta_{i+1}$, the coordinates are sorted such that $\alpha_h\geq \alpha_{i+1}$. 
If there are $l$ unfinished jobs in the system, then there exists an integer $r$ ($0\leq r\leq l$) such that 
\begin{eqnarray}
&&\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\alpha_1-\delta_1\geq\ldots\geq \alpha_{r}-\delta_{r}>0= \alpha_{r+1}-\delta_{r+1}=\ldots,\\
&&\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\!\alpha_h \left\{\begin{array}{l l} >0, &\text{if}~ h\leq l;\\
  =0, &\text{if}~ h\geq l+1,\end{array}\right.~~\delta_h \left\{\begin{array}{l l} \geq0, &\text{if}~ h\leq l;\\
  =0, &\text{if}~ h\geq l+1.\end{array}\right.
  \end{eqnarray}
\end{definition}

Let $\{\bm{\beta}(t),t\geq0\}$ be the state process of policy $P'$ and $\{\bm{\alpha}(t),\bm{\delta}(t),t\geq0\}$ be the state process of FUT-NR, which are assumed to be right-continuous. One key result of the sample-path ordering technique is the following lemma:



\begin{lemma}\label{lemG4}
Suppose that $\bm{\alpha}(0^-) = \bm{\delta}(0^-)=\bm{\beta}(0^-)=\bm{0}$ and the job parameters $\mathcal{I}$ are given. For any sample path of policy $P'$, there exists a sample path of FUT-NR with the same probability density such that
\begin{eqnarray}\label{eq_lemG4}
\sum_{h=j}^\infty [\alpha_h(t)- \delta_h(t)]\leq \sum_{h=j}^\infty \beta_h(t)
\end{eqnarray}
holds for all $t\geq0$ and j = $1,2,\ldots$
\end{lemma}

The following lemmas are needed to prove Lemma \ref{lemG4}:

\begin{lemma}\label{lem_non_prmp1}
Suppose that, under policy FUT-NR, $\{\bm{\alpha}',\bm{\delta}'\}$ is obtained by completing a task on one server in the system whose state is $\{\bm{\alpha},\bm{\delta}\}$. Further, suppose that, under policy $P'$, $\bm{\beta}'$ is obtained by completing a task on one server in the system whose state is $\bm{\beta}$.
If
\begin{eqnarray}\label{eq_non_prmp_41}
\sum_{h=j}^\infty [\alpha_h - \delta_h]\leq \sum_{h=j}^\infty \beta_h, ~\forall~j=1,2,\ldots,\nonumber
\end{eqnarray}
then
\begin{eqnarray}\label{eq_non_prmp_40}
\sum_{h=j}^\infty [\alpha'_h - \delta'_h]\leq \sum_{h=j}^\infty \beta'_h, ~\forall~j=1,2,\ldots
\end{eqnarray}
\end{lemma}

\begin{proof}
The proof is similar to that of Lemma 2 in \cite{Smith78}.
If $\sum_{h=j}^\infty [\alpha'_h - \delta'_h]=0$, then the inequality \eqref{eq_non_prmp_40} follows naturally. 
If $\sum_{h=j}^\infty [\alpha'_h - \delta'_h]>0$, then there exist some tasks that have not been assigned to any server. 
In FUT-NR, a server that has just completed a task will be allocated to process an unassigned task from the job with the minimum positive $\alpha'_h - \delta'_h$. Hence,
$\sum_{h=j}^\infty [\alpha'_h - \delta'_h]=\sum_{h=j}^\infty [\alpha_h - \delta_h] - 1 \leq \sum_{h=j}^\infty \beta_h -1 \leq \sum_{h=j}^\infty \beta'_h$.
\end{proof}


\begin{lemma}\label{lem_non_prmp2}
Suppose that, under policy FUT-NR, $\{\bm{\alpha}',\bm{\delta}'\}$ is obtained by adding a job with $b$ tasks to the system whose state is $\{\bm{\alpha},\bm{\delta}\}$. Further, suppose that, under policy $P'$, $\bm{\beta}'$ is obtained by adding a job with $b$ tasks to the system whose state is $\bm{\beta}$.
If
\begin{eqnarray}
\sum_{h=j}^\infty [\alpha_h - \delta_h]\leq \sum_{h=j}^\infty \beta_h, ~\forall~j=1,2,\ldots,\nonumber
\end{eqnarray}
then
\begin{eqnarray}
\sum_{h=j}^\infty [\alpha'_h - \delta'_h]\leq \sum_{h=j}^\infty \beta'_h, ~\forall~j=1,2,\ldots\nonumber
\end{eqnarray}
\end{lemma}

\begin{proof}
The proof is similar to that of Lemma 3 in \cite{Smith78}.
Without loss of generalization, we suppose that after the job arrival, $b$ is the $l$-th coordinate of $\bm{\alpha}'$ and the $m$-th coordinate of $\bm{\beta}'$. Hence, $\alpha'_l = \beta'_m= b$. Because no server completes a task at this time instant, $\delta'_l =0$. We consider the following four cases:

{Case 1}: $l<j, m<j$. We can obtain $\sum_{h=j}^\infty [\alpha'_h - \delta'_h] = \sum_{h=j-1}^\infty [\alpha_h - \delta_h] \leq \sum_{h=j-1}^\infty \beta_h= \sum_{h=j}^\infty \beta_h'$.

{Case 2}: $l<j, m\geq j$. We have $\sum_{h=j}^\infty [\alpha'_h - \delta'_h] =\sum_{h=j-1}^\infty $ $[\alpha_h - \delta_h] \leq b + \sum_{h=j}^\infty [\alpha_h - \delta_h] \leq b + \sum_{h=j}^\infty \beta_h = \sum_{h=j}^\infty \beta_h'$.

{Case 3}: $l\geq j, m<j$. We have $\sum_{h=j}^\infty [\alpha'_h - \delta'_h] = b + \sum_{h=j}^\infty [\alpha_h - \delta_h] \leq \sum_{h=j-1}^\infty [\alpha_h - \delta_h] \leq \sum_{h=j-1}^\infty \beta_h = \sum_{h=j}^\infty \beta_h'$.

{Case 4}: $l\geq j, m\geq j$. We have $\sum_{h=j}^\infty [\alpha'_h - \delta'_h] = b + \sum_{h=j}^\infty [\alpha_h - \delta_h] \leq b + \sum_{h=j}^\infty \beta_h = \sum_{h=j}^\infty \beta_h'$.
\end{proof}


\ifreport
\begin{proof}[Proof of Lemma \ref{lemG4}]
\else
\begin{proof}[of Lemma \ref{lemG4}]
\fi
Consider any busy period $[\tau,\nu)$ of policy $P'$. Then, in policy $P'$, all servers are busy during $[\tau,\nu)$, and are idle at time $\tau^-$ and time $\nu$. We prove \eqref{eq_lemG4} for $t\in[\tau,\nu)$ by considering two cases:

\emph{Case 1: At time $t=\tau^-$, policy FUT-NR has $m$ tasks and the service of these tasks has just started.} Consider the system states of both policies at time $\tau^-$. The system state of policy FUT-NR satisfies 
\begin{align}\label{proof_lemG4_1}
\sum_{h=1}^\infty \alpha_h(\tau^-)= m, ~\bm{\alpha}(\tau^-)=\bm{\delta}(\tau^-).
\end{align}
In policy $P'$, there is no task in the system at time $\tau^-$ such that 
\begin{align}\label{proof_lemG4_5}
\bm{\beta}(\tau^-)=\bm{0}. 
\end{align}
Consider the evolutions of both policies during $[\tau,\nu)$. 
In policy $P'$, all servers are busy if there is at least one task. On the other hand, in policy FUT-NR, there is no task replication. Hence, all servers are busy if there are no less than $m$ tasks. Because the servers become busy in policy $P'$ at time $\tau$, a job must has arrived. By \eqref{proof_lemG4_1} and \eqref{proof_lemG4_5}, it holds that for $t=\tau$
%^there are no less than $m$ tasks in policy FUT-NR at time $\tau^-$.
\begin{align}\label{proof_lemG4_4}
\sum_{h=1}^\infty \alpha_h(t)= \sum_{h=1}^\infty \beta_h(t) +m\geq m+1.
\end{align}
Therefore,  the servers are all busy in policy $P'$ and policy FUT-NR at time $\tau$. Hence, for any sample path of policy $P'$, there is a sample path of policy FUT-NR such that for sufficiently small $\Delta t$ the task arrival times and task completion times of the two policies are exactly the same during $[\tau,\tau+\Delta t)$, and \eqref{proof_lemG4_4} holds during $[\tau,\tau+\Delta t)$. By induction over time, we can show that for any sample path of policy $P'$, there is a sample path of policy FUT-NR with the same probability density such that the task arrival times and task completion times of the two policies are exactly the same  during $[\tau,\nu)$, and \eqref{proof_lemG4_4} holds for all $t\in[\tau,\nu)$. Using Lemma \ref{lem_non_prmp1}, Lemma \ref{lem_non_prmp2}, and the initial states at time $\tau^-$, we can prove that \eqref{eq_lemG4} holds for all $t\in[\tau,\nu)$ on these two sample paths.

%In general, suppose that at some time $t\in[\tau,\nu)$
%\begin{align}
%\sum_{h=1}^\infty \alpha_h(t)= \sum_{h=1}^\infty \beta_h(t) +m\geq m+1.\nonumber
%\end{align}
%Then, the scheduling decisions of policies $P'$ and policy FUT-NR are the same at time $t$. This further implies that for any sample path of policy $P'$, we can construct a sample path of policy FUT-NR such that 
%\begin{align}
%\sum_{h=1}^\infty \alpha_h(t^+)= \sum_{h=1}^\infty \beta_h(t^+) +m\geq m+1.\nonumber
%\end{align}
%Therefore, 
%
%Using Lemma \ref{lem_non_prmp1} and Lemma \ref{lem_non_prmp2}, and we can prove that 
%\begin{align}
%\sum_{h=1}^\infty \alpha_h(t^+)= \sum_{h=1}^\infty \beta_h(t^+) +m.\nonumber
%\end{align}
%
%For any sample path of policy $P'$ during $[\tau,\nu)$, we can construct a sample path of policy FUT-NR during $[\tau,\nu)$ with the same probability density such that the task arrival times and task completion times of the two policies are exactly the same. In particular, if 
%
%
%if policy $P'$ has $b$ tasks at time $t\in[\tau,\nu)$, policy FUT-NR has $m+b$ tasks at time $t$. Hence, the scheduling decisions of policies $P'$ and policy FUT-NR are the same at time $t$. Therefore, we can obtain
%\begin{align}
%\sum_{h=1}^\infty \alpha_h(t)= \sum_{h=1}^\infty \beta_h(t) +m,~\forall~t\in [\tau,\nu).\nonumber
%\end{align}
%Because the task arrivals and departures of policies $P'$ and FUT-NR are aligned during $[\tau,\nu)$, using Lemma \ref{lem_non_prmp1}, Lemma \ref{lem_non_prmp2}, and the initial states at time $\tau^-$, we can prove by induction that \eqref{eq_lemG4} holds for $t\in[\tau,\nu)$.

\emph{Case 2: At time $t=\tau^-$, policy FUT-NR has less than $m$ tasks or the service of these tasks started before time $\tau^-$}. In both \emph{Case 1} and \emph{Case 2}, the sample path evolutions of policy $P'$ are the same. On the other hand, in policy FUT-NR, the tasks are completed earlier in \emph{Case 2} than in \emph{Case 1}. Therefore, \eqref{eq_lemG4} also holds in \emph{Case 2} for $t\in[\tau,\nu)$.

%Note that the case that policy FUT-NR has more than $m$ tasks at time $\tau^-$ will not happen. This will be clear 
Let $[\tau_1,\nu_1)$ be the next busy period of policy $P'$ with $\nu<\tau_1$. Then, $[\nu,\tau_1)$ is an idle period of policy $P'$. We prove \eqref{eq_lemG4} during the idle period $[\nu,\tau_1)$. 
Because all servers are idle during $[\nu,\tau_1)$ in policy $P'$, it follows that 
\begin{align}\label{proof_lemG4_2}
\bm{\beta}(t)=\bm{0},~t\in[\nu,\tau_1).
\end{align}
Hence, there is no task arrival during $[\nu,\tau_1)$; otherwise, \eqref{proof_lemG4_2} cannot be true.
On the other hand, at time $\nu$ there are no more than $m$ tasks in policy FUT-NR such that 
\begin{align}
\bm{\alpha}(\nu)=\bm{\delta}(\nu).\nonumber
\end{align}
Because there is no task arrival during $[\nu,\tau_1)$, policy FUT-NR satisfies
\begin{align}\label{proof_lemG4_3}
\bm{\alpha}(t)=\bm{\delta}(t),~t\in[\nu,\tau_1).
\end{align}
By \eqref{proof_lemG4_2} and \eqref{proof_lemG4_3}, \eqref{eq_lemG4} holds during $[\nu,\tau_1)$.
Further, from \eqref{proof_lemG4_3}, we can obtain
\begin{align}
\sum_{h=1}^\infty \alpha_h(\tau_1^-)=\sum_{h=1}^\infty \delta(\tau_1^-)\leq m,
\end{align}
such that there are no more than $m$ tasks at time $t=\tau_1^-$ in policy FUT-NR. Hence, either \emph{Case 1} or \emph{Case 2} is satisfied at time $t=\tau_1^-$. Then, we can use the above arguments to prove that  \eqref{eq_lemG4} holds during the next busy period $[\tau_1,\nu_1)$ of policy $P'$.


Finally, by taking an induction over the busy and idle periods of policy $P'$,  Lemma \ref{lemG4} is proven.
%Let $[\nu,\tau_1)$ and $[\tau_1,\nu_1)$ be the next idle and busy periods of policy $P'$, respectively. Because policy $P'$ is work-conserving, all $m$ servers are idle in policy $P'$ during $[\nu,\tau_1)$. Hence, there is no job arrival during $[\nu,\tau_1)$. At time $\nu$, we have
%\begin{align}
%\sum_{h=j}^\infty [\alpha_h(\nu)- \delta_h(\nu)]\leq 0.\nonumber
%\end{align}
%This and $\alpha_h(\nu)\geq\delta_h(\nu)$ imply that $\alpha_h(\nu)=\delta_h(\nu)$ for all $h=1,2,\ldots$ Since no job arrives during $[\nu,\tau_1)$, we can obtain that $\alpha_h(t)=\delta_h(t)$ for all $t\in[\nu,\tau_1)$ and $h=1,2,\ldots$ Hence, \eqref{eq_lemG4} holds during $[\nu,\tau_1)$. 
%
%Because there is no job arrival during $[\nu,\tau_1)$, there are no more than $m$ remaining tasks in FUT-NR at time $\tau_1$ and each remaining task has been processed by a certain amount of time. Similar with the case of $[\tau,\nu)$, we can prove that \eqref{eq_lemG4} holds in the busy period $[\tau_1,\nu_1)$.
%By taking an induction over the busy and idle periods of policy $P'$, Lemma \ref{lemG4} follows.
\end{proof}

\ifreport
\begin{proof}[Proof of Condition 3]
\else
\begin{proof}[of Condition 3]
\fi
%Let the evolution of the system state under some scheduling policy be on a space $(\Omega,\mathcal{F},P)$. Each $\omega\in\Omega$ corresponds to a sample path of policy $P'$ and a sample path of policy FUT-NR. The job arrival parameters $\mathcal{I}$ is fixed for all $\omega\in\Omega$. 
%Let $(C_{(1)}(P'),\ldots,c_{N:N}(P'))$ be a permute of the job completion time sequence $(c_{1}(P'),\ldots,c_{N}(P'))$ in the increasing order, such that $c_{i:N}(P')\leq c_{i+1:N}(P')$. 

%Pick any $\omega\in\Omega$ and consider the first job completion time $C_{(1)}(P')$ of policy $P'$. Suppose that there are $y$ job arrivals during $[0,C_{(1)}(P'))$. 

We will prove Condition 3 by induction. Consider the sample paths of policy $P'$ and policy FUT-NR satisfying Lemma \ref{lemG4}. We first show that there exists a job $w_1$ such that
\begin{align}\label{eq_Condition_3_1}
U_{w_1}(\text{FUT-NR}) \leq C_{(1)}(P').
\end{align}

In policy $P'$, the first job departure occurs at time $t=C_{(1)}(P')$. Suppose that $y_1$ jobs have arrived during $[0,C_{(1)}(P'))$. Then, there are $y_1-1$ unfinished jobs at time $C_{(1)}(P')$ in policy $P'$. Hence, the system state of policy $P'$ satisfies 
\begin{align}\label{eq_proof_0}
\sum_{h=y_1}^\infty\beta_h(C_{(1)}(P'))=0.
\end{align}
This and Lemma \ref{lemG4} imply
%Hence, there are $y-1$ unfinished jobs at time $C_{(1)}(P')$ such that
%Invoking Lemma \ref{lemG4}, we can obtain
\begin{align}\label{eq_proof_1}
\sum_{h=y_1}^\infty \alpha_h(C_{(1)}(P'))\leq \sum_{h=y_1}^\infty  \delta_h(C_{(1)}(P')).
\end{align}
In policy FUT-NR, there are at most $y_1$ jobs at time $C_{(1)}(P')$. Hence, the system state of policy FUT-NR must satisfy
\begin{align}\label{eq_proof_2}
\!\!\alpha_h(C_{(1)}(P'))= \delta_h(C_{(1)}(P'))=0,\forall~h=y_1\!+\!1,y_1\!+\!2,\ldots \!\!
\end{align}
Combining \eqref{eq_proof_1}, \eqref{eq_proof_2}, and the fact that $\alpha_h(t)\geq\delta_h(t)$ for all $h$ and $t$, we can obtain
%Combining \eqref{eq_proof_0}, \eqref{eq_proof_1}, and the fact that $\alpha_h(t)\geq\delta_h(t)$ for all $i,t$, yields
\begin{align}\label{eq_proof_3}
\alpha_{y_1}(C_{(1)}(P'))=\delta_{y_1}(C_{(1)}(P')).
\end{align}
Let $w_1$ be the index of the job associated to the $y_1$-th coordinate of $\bm{\alpha}(t)$ at time $t= C_{(1)}(P')$. Then, \eqref{eq_proof_3} tells us that in FUT-NR, all tasks of job $w_1$ are either completed or under service at time $C_{(1)}(P')$. Hence, \eqref{eq_Condition_3_1} is proven.
%\begin{align}%\label{eq_proof_9}
%U_{w_1}(\text{FUT-NR}) \leq C_{(1)}(P'),\nonumber
%\end{align}
%which implies \eqref{eq_Condition_3_1}.

Next, we prove the induction step. Suppose that there exist $j$ jobs indexed by $w_1,w_2,\ldots,w_j$ such that
\begin{align}
U_{w_i}(\text{FUT-NR}) \leq C_{(i)}(P'),~i=1,\ldots,j,\nonumber
\end{align}
we will show that there exist another job $w_{j+1}$ such that
\begin{align}\label{eq_proof_9}
U_{w_{j+1}}(\text{FUT-NR}) \leq C_{(j+1)}(P').
\end{align}
%Since preemption is not allowed, these $\delta_y(C_{(1)}(P'))$ tasks will be under service in policy FUT-NR until completion. Let $w_1$ be the index of the job associated to the coordinate $y$ at time $C_{(1)}(P')$. According to \eqref{eq_def_state}, we can obtain $\delta_y(C_{(1)}(P'))\leq \min[k_{w_1},M].$ Therefore, the time duration between $C_{(1)}(P')$ and $c_{w_1,\text{FUT-NR}}$ is no more than the time to complete $\min[k_{w_1},M]$ tasks of job $w_1$.
Assume that $y_{j+1}$ jobs have arrived during $[0,C_{(j+1)}(P'))$, which must satisfy $y_{j+1}\geq j+1$. Then, 
there are $(y_{j+1}-j-1)$ unfinished jobs at time $C_{(j+1)}(P')$ in policy $P'$. According to \emph{Definition \ref{def_state_P}}, the system state of policy $P'$ satisfies 
\begin{align}
\sum_{h=y_{j+1}-j}^\infty\beta_h(C_{(j+1)}(P'))=0.\nonumber
\end{align}
Then, by following the arguments of \eqref{eq_proof_1}-\eqref{eq_proof_3}, we can obtain that at time $t=C_{(j+1)}(P')$ the system state of policy FUT-NR satisfies
\begin{align}\label{eq_proof_4}
\alpha_{h}(C_{(j+1)}(P'))=\delta_{h}(C_{(j+1)}(P')),~h=y_{j+1}-j,\ldots,y_{j+1}.
\end{align}
There are $j+1$ jobs satisfying \eqref{eq_proof_4}. At least one of these $j+1$ jobs is different from the jobs $w_1,w_2,\ldots,w_j$. Let $w_{j+1}$ be the index of this job. Then, \eqref{eq_proof_4} tells us that in FUT-NR, all tasks of job $w_{j+1}$ are either completed or under service at time $t=C_{(j+1)}(P')$. Hence, \eqref{eq_proof_9} is proven.

By induction, we can obtain
\begin{align}\label{eq_proof_10}
U_{w_{j}}(\text{FUT-NR}) \leq C_{(j)}(P'),~j=1,\ldots,n.
\end{align}
Because $U_{(j)}(\pi)$ is the $j$-th smallest components of $\bm{U}(\pi)$, it follows that
\begin{align}\label{eq_proof_11}
U_{(j)}(\text{FUT-NR})\! \leq \!\max_{i=1,\ldots,j}U_{w_{j}}(\text{FUT-NR}),~j=1,\ldots,n.\!\!
\end{align}
Combining \eqref{eq_proof_10} and \eqref{eq_proof_11}, we obtain that for each sample path of policy $P'$, there is a sample path of policy FUT-NR with the same probability density such that 
\begin{align}
\bm{U}_{\uparrow}(\text{FUT-NR}) \leq  \bm{C}_{\uparrow}(P').
\end{align}
Considering all possible sample paths of these two policies, the stochastic ordering result in \eqref{eq_condition3} follows.
%Suppose that for some $j\in\{1,\ldots,N-1\}$, the time duration between $c_{i:N}(P')$ and $c_{w_i,\text{FUT-NR}}$ is no more than the time for the system to complete $\min[k_{w_i},M]$ tasks of job $w_i$ for all $h=1,\ldots, j$, and the job indices $w_1,w_2,\ldots,w_j$ are distinct. We will prove that there is a job $w_{j+1}$ different from $w_1,w_2,\ldots,w_j$ such that the time duration between $C_{(j+1)}(P')$ and $c_{w_{j+1},\text{FUT-NR}}$ is no more than the time to complete $\min[k_{w_{j+1}},M]$ tasks of a job $w_{j+1}$.
%Let $z$ be the number of job arrivals during $[0,C_{(j+1)}(P'))$, which must satsify $z\geq j+1$. By following the arguments of \eqref{eq_proof_1}-\eqref{eq_proof_9}, we can obtain
%\begin{align}\label{eq_proof_4}
%\alpha_{i}(C_{(j+1)}(P'))=\delta_{i}(C_{(j+1)}(P')),~h=z-j,\ldots,z.
%\end{align}
%Since preemption is not allowed, in policy FUT-NR, the remaining tasks of the $(j+1)$ jobs associated to the coordinates $z-j,z-j+1,\ldots,z$ will be under service after time $C_{(j+1)}(P')$ until completion (or are already completed before time $C_{(j+1)}(P')$). Moreover, at least one of these $(j+1)$ jobs must be different from the jobs $w_1,w_2,\ldots,w_j$. Let $w_{j+1}$ be the index of this job. 
%Using \eqref{eq_def_state} and \eqref{eq_proof_4}, one can show that the time difference between $c_{(j+1)}(P')$ and $c_{w_{j+1},\text{FUT-NR}}$ is no more than the time duration to complete $\min[k_{w_{j+1}},M]$ tasks of job $w_{j+1}$.
%
%By induction, for all $h=1,\ldots,N$ and all $\omega\in\Omega$, the time difference between $c_{i:N}(P')$ and $c_{w_{i},\text{FUT-NR}}$ is no more than the time duration to complete $\min[k_{w_i},M]$ tasks of job $w_i$. Further, the job indices $w_1,w_2,\ldots,w_N$ are distinct, such that $(w_1,w_2,\ldots,w_N)$ is a permute of $(1,2,\ldots,N)$.
% This tells us that 
%\begin{align}
%\mathbb{E}\left[c_{w_i,\text{FUT-NR}} - c_{i:N}(P')| \mathcal{I}\right] \leq \max_{\substack{S: |S|\leq k_i\\
%S\subseteq\{1,\ldots,m\}}}\!\!\mathbb{E}\left[\max_{l\in S} X_l\right].\nonumber
%\end{align}
%Hence, we have
%\begin{align}\label{eq_proof_5}
%&\mathbb{E}[{D}_{\text{avg,FUT-NR}}-{D}_{\text{avg}}(P')| \mathcal{I}]\nonumber\\
%=&\frac{1}{N}\sum_{h=1}^N\mathbb{E} \left[c_{i,\text{FUT-NR}} - c_{i}(P')| \mathcal{I}\right]\nonumber\\
%=&\frac{1}{N} \sum_{h=1}^N\mathbb{E} \left[c_{w_i,\text{FUT-NR}} - c_{i:N}(P')| \mathcal{I}\right]\nonumber\\
%\leq &\frac{1}{N}\sum_{h=1}^N\max_{\substack{S: |S|\leq k_i\\
%S\subseteq\{1,\ldots,m\}}}\!\!\mathbb{E}\left[\max_{l\in S} X_l\right].
%\end{align}
%By this, condition 3 is proven.
\end{proof}
After establishing conditions 1-3 of Lemma \ref{lem1} for policy FUT-NR,  we can use Lemma \ref{lem1} and Corollary \ref{coro1} to obtain \eqref{eq_delaygap1}. This completes the proof.

\subsection{Proof of {\large \eqref{eq_delaygap2}} in Theorem \ref{thm1}} 
The proof of \eqref{eq_delaygap2} is  similar with that of \eqref{eq_delaygap1} in Appendix \ref{sec_app_thm1_1}, except for the following two differences: 

First, policy FUT-NR in Appendix \ref{sec_app_thm1_1} should be replaced by policy FUT-NIR. 


Second, task replications are allowed in policy FUT-NIR, which will introduce some extra delay to cancel the redundant task copies. %It is important to keep the cancellation overhead small. Otherwise, 
If the cancellation overhead is large, the servers might be busy cancelling the redundant task copies, instead of serving new tasks. In this case, Lemma \ref{lemG4} does not hold. Hence, we should keep the cancellation overhead small. In the design of policy FUT-NIR, a task replica is cancelled if the time to cancel the replica is stochastically shorter than the time to complete the replica; otherwise, the replica will not be cancelled. Using this and the extra conditions {$\bm{O}_{\mathcal{S}}\leq_{\text{st}}[\bm{X}_{\mathcal{S}}-\bm{\tau}_{\mathcal{S}}| \bm{X}>\bm{\tau}]$} and  {$\bm{O}_{\mathcal{S}^c}\geq_{\text{st}}[\bm{X}_{\mathcal{S}^c}-\bm{\tau}_{\mathcal{S}^c}| \bm{X}>\bm{\tau}]$}, we can obtain that in policy FUT-NIR the redundant task copies are completed stochastically earlier than processing these task copies until completion. Using this, the proof arguments of Lemma \ref{lemG4} also work for policy FUT-NIR.

\subsection{Proof of Corollary 3}  
Under the conditions of Corollary \ref{coro3}, policy FUT-NR satisfies the following three properties: (i) all $m$ servers are busy at all time $t\in[0,\infty)$, (ii) there is no task replications, and (iii) any completed task is from a job with the fewest remaining task. Therefore, policy FUT-NR is identical with policy $P'$ constructed in Appendix \ref{sec_app_thm1_1}. In addition, because there are at least $m$ remaining tasks at all time $t\in[0,\infty)$, policy FUT-NIR is identical with policy FUT-NR. Then, \eqref{eq_coro3} follows from Lemma \ref{lem1} and Corollary \ref{coro1}. 

%The details are provided in Appendix \ref{app2}.



%\textbf{Condition 4:} $P\in\Pi$. This condition is trivial. Hence, \eqref{eq_delaygap1} follows from Lemma \ref{thm2}.
%
%The remaining task is to prove \eqref{eq_delaygap2}. Since the $X_l$'s are independent NBU random variables with mean $\mathbb{E}[X_l]=1/\mu_l$, by Theorem 3.A.55 of \cite{StochasticOrderBook}, we can obtain
%\begin{align}
%X_l \leq_{\text{icx}} Z_l,~l=1,\ldots,m,\nonumber
%\end{align}
%where $\leq_{\text{icx}}$ is the increasing convex order defined in \cite[Chapter 4]{StochasticOrderBook} and the $Z_l$'s are independent exponential random variables with mean $\mu_l$. By Corollary 4.A.16 of \cite{StochasticOrderBook}, we have 
%\begin{align}
%\max_{l\in S} X_l \leq_{\text{icx}} \max_{l\in S} Z_l,~\forall~S\subseteq\{1,\ldots,m\}.\nonumber
%\end{align}
%Then, Eq. (4.A.1) of \cite{StochasticOrderBook} and $\mu_1\leq \ldots\leq \mu_M$ tell us that  
%\begin{align}
%\!\!\max_{\substack{S: |S|\leq k_i\\
%S\subseteq\{1,\ldots,m\}}}\!\!\mathbb{E}\!\left[\max_{l\in S} X_l\right]\!\leq\!\mathbb{E}\!\left[\max_{l=1,\ldots,k_i \wedge M} Z_l\right]\!\leq\!\sum_{l=1}^{k_i \wedge M} \frac{1}{\sum_{m=1}^l \mu_l}.\nonumber
%\end{align}
%This and \eqref{eq_proof_5} imply \eqref{eq_delaygap2}. This completes the proof.




==> v3/appendices_2version2.tex <==
% !TEX root = ./replication.tex

\section{Proof  of Proposition \ref{lem2}} \label{app0_1}
%\subsection{Proof of Thoerem \ref{lem2}}
%\begin{definition}\label{def_state_P_thm3}
%The system state of policy $\pi$  is specified by a $n$-dimensional vector $\bm{\xi}=(\xi_1,\ldots,\xi_n)$ with non-negative components. At any time, if job $i$ exists in the system, $\xi_{i,\pi}$ is the number of remaining tasks of job $i$; if job $i$ has not arrived at the system or has departed from the system, $\xi_{i,\pi}=0$.
%\end{definition}


%We assume that the due times $d_1,\ldots, d_n$ of the $n$ jobs are distinct from each other. This does not lose any generality, because if $d_i=d_j$ for two jobs $i$ and $j$, Thoerem \ref{lem2} can be proven by first proving for the case $d_i=d_j+\epsilon$ and then taking the limit $\epsilon\rightarrow 0$. 
%by taking the limit $d_i\rightarrow d_j$. 

%We develop another form of {sample-path dominance} to prove Thoerem \ref{lem2}. 
%The first part of the sample-path dominance result is as follows:
 
 

The proof of Proposition \ref{lem2} requires the following two lemmas:


\begin{lemma}\label{lem_non_prmp1_thm3}
Suppose that, in policy $P$, $\{\bm{\xi}_P',\bm{\gamma}_P'\}$ is obtained by allocating $b_P$ unassigned tasks to the servers in the system whose state is $\{\bm{\xi}_P,\bm{\gamma}_P\}$. Further, suppose that, in policy $\pi$, $\{\bm{\xi}_\pi',\bm{\gamma}_\pi'\}$ is obtained by completing $b_\pi$ tasks in the system whose state is $\{\bm{\xi}_\pi,\bm{\gamma}_\pi\}$.
If $b_P\geq b_\pi$, condition 2 of Proposition \ref{lem2} is satisfied in policy $P$, and
\begin{eqnarray}
\sum_{i:d_i\leq\tau} \gamma_{i,P}\leq \sum_{i:d_i\leq\tau} \xi_{i,\pi},~\forall~\tau\in[0,\infty),\nonumber
\end{eqnarray}
then
\begin{eqnarray}\label{eq_non_prmp_40_thm3}
\sum_{i:d_i\leq\tau} \gamma_{i,P}'\leq \sum_{i:d_i\leq\tau} \xi_{i,\pi}',~\forall~\tau\in[0,\infty).\end{eqnarray}
\end{lemma}

\begin{proof}
If $\sum_{i:d_i\leq\tau} \gamma_{i,P}'=0$, then the inequality \eqref{eq_non_prmp_40_thm3} follows naturally. 
If $\sum_{i:d_i\leq\tau} \gamma_{i,P}'>0$, then there exist some unassigned tasks in the queue. 
In policy $P$, each task allocated to the servers is from the job with the earliest due time. Hence,
$\sum_{i:d_i\leq\tau} \gamma_{i,P}'=\sum_{i:d_i\leq\tau} \gamma_{i,P} - b_P \leq \sum_{i:d_i\leq\tau} \xi_{i,\pi} -b_\pi \leq \sum_{i:d_i\leq\tau} \xi_{i,\pi}'$.
\end{proof}


\begin{lemma}\label{lem_non_prmp2_thm3}
Suppose that under policy $P$, $\{\bm{\xi}_P',\bm{\gamma}_P'\}$ is obtained by adding a job with $b$ tasks and due time $d$ to the system whose state is $\{\bm{\xi}_P,\bm{\gamma}_P\}$. Further, suppose that under policy $\pi$, $\{\bm{\xi}_\pi',\bm{\gamma}_\pi'\}$ is obtained by adding a job with $b$ tasks and due time $d$ to the system whose state is $\{\bm{\xi}_\pi,\bm{\gamma}_\pi\}$.
If
\begin{eqnarray}
\sum_{i:d_i\leq\tau} \gamma_{i,P}\leq \sum_{i:d_i\leq\tau} \xi_{i,\pi}, ~\forall~\tau\in[0,\infty),\nonumber
\end{eqnarray}
then
\begin{eqnarray}
\sum_{i:d_i\leq\tau} \gamma_{i,P}'\leq \sum_{i:d_i\leq\tau} \xi_{i,\pi}', ~\forall~\tau\in[0,\infty).\nonumber\end{eqnarray}
\end{lemma}

\begin{proof}
If $d\leq\tau$, then
$\sum_{i:d_i\leq\tau} \gamma_{i,P}'\leq \sum_{i:d_i\leq\tau} \gamma_{i,P} + b\leq \sum_{i:d_i\leq\tau} \xi_{i,\pi}+b \leq \sum_{i:d_i\leq\tau} \xi_{i,\pi}'$.

If $d>\tau$, then
$\sum_{i:d_i\leq\tau} \gamma_{i,P}'\leq \sum_{i:d_i\leq\tau} \gamma_{i,P} \leq \sum_{i:d_i\leq\tau} \xi_{i,\pi} \leq \sum_{i:d_i\leq\tau} \xi_{i,\pi}'$.
\end{proof}

The proof of Proposition \ref{lem2} is almost identical with that of Proposition \ref{lem1}, and hence is not repeated here. The only difference is that Lemma \ref{lem_non_prmp1} and Lemma \ref{lem_non_prmp2} in the proof of Proposition \ref{lem1} should be replaced by Lemma \ref{lem_non_prmp1_thm3} and Lemma \ref{lem_non_prmp2_thm3}, respectively.


\section{Proof of Proposition \ref{lem1_1}} \label{app_lem1_1}


We have proven that \eqref{eq_ordering_2_2} holds under the conditions of Proposition \ref{lem1_1}.
Note that \eqref{eq_ordering_2_2} can be equivalently expressed in the following vector form:
\begin{align}
\bm{v}_{\uparrow} (P)\leq \bm{c}_{\uparrow} (\pi).\nonumber
\end{align}
Because any $f\in\mathcal{D}_{\text{sym}}$ is a symmetric and increasing function, we can obtain
\begin{align}%\label{eq_lem1_1}
&f(\bm{v} (P))=f(\bm{v}_{\uparrow} (P)) \nonumber\\
\leq_{}&f(\bm{c}_{\uparrow} (\pi))= f(\bm{c} (\pi)).\nonumber
\end{align} 
This completes the proof.




%By considering all possible sample paths of policy $P$ and policy $\pi$, the stochastic ordering result in Theorem \ref{lem2} follows.


==> v3/appendices_3.tex <==
% !TEX root = ./replication.tex

\section{Proof of Thoerem~\ref{thm2}} \label{app2}
%\subsection{Proof of Thoerem~2} \label{sec_app_thm2_1}
%\subsection{Proof of Theorem \ref{thm2}}  
Define $\bm{s}=(s_{1},\ldots,$ $ s_{k_{\text{sum}}})$ as the sequence of task arrival times where $s_1\leq \ldots\leq s_{k_{\text{sum}}}$. Hence, $\bm{s}$ is determined by the job arrival times $a_1,\ldots,a_n$ and job sizes $k_1,\ldots,k_n$.
Recall that $\bm{T}_\pi=(T_{1,\pi},\ldots,$ $ T_{k_{\text{sum}},\pi})$ is the sequence of task completion times in policy $\pi$ where $T_{1,\pi}\leq \ldots\leq T_{k_{\text{sum}},\pi}$. 
We  first show that for all $\pi\in\Pi$
\begin{align}\label{eq_thm2_proof1}
[\bm{T}_{\text{FUT-R}}|\mathcal{I}] \leq_{\text{st}} [\bm{T}_\pi|\mathcal{I}].
\end{align}
We prove \eqref{eq_thm2_proof1} by induction. Consider the first task completion time $T_{1,\pi}$. Job 1 arrives at time $a_1=0$. All policy $\pi\in\Pi$ are non-preemptive. If policy $\pi$ is  work-conserving, then
\begin{align}
[T_{1,\pi}|\mathcal{I}]=\min_{l=1,\ldots,m} X_l,\nonumber
\end{align} 
otherwise, if policy $\pi$ is non-work-conserving, then
\begin{align}
[T_{1,\pi}|\mathcal{I}]\geq\min_{l=1,\ldots,m} X_l,\nonumber
\end{align} 
because of the possibility of server idleness. Since policy FUT-R$\in\Pi$ is work-conserving, we can obtain that for all $\pi\in\Pi$
\begin{align}\label{eq_thm2_condition1_2}
[T_{1,\text{FUT-R}}|\mathcal{I}]=\min_{l=1,\ldots,m} X_l\leq[T_{1,\pi}|\mathcal{I}].
\end{align} 

Next, consider the system evolution from $T_{j,\pi}$ to $T_{j+1,\pi}$. For any work-conserving policy $\pi\in\Pi$, we can obtain
\begin{eqnarray}\label{eq_thm2_2}
T_{j+1,\pi}\!=\max\{s_{j+1},T_{j,\pi}\} + \!\min_{l=1,\ldots,m} R_{j,l,\pi},
\end{eqnarray}
where $R_{j,l,\pi}$ is the time duration for server $l$ to complete a task since time $\max\{s_{j+1},T_{j,\pi}\}$. Suppose that server $l$ has spent $\tau_{l,\pi}$ ($\tau_{l,\pi}\geq0$) seconds on a task by time $\max\{s_{j+1},T_{j,\pi}\}$. 

Because the task service times are independent across the servers and the complementary CDF $\bar{F}$  is absolutely continuous, the probability for any two servers to complete their tasks at the same time is zero. Hence, $\Pr[R_{j,l,\pi} > 0] = 1$.\footnote{If $\bar{F}$  is not absolutely continuous, then it may happen that $\Pr[R_{j,l,\pi} > 0] < 1$ and two servers complete task executions at the same time. In this case, it is better to assign two distinct tasks than two replicated copies of the same task on these two servers.}
Therefore, in policy FUT-R, when a task copy is completed on a server, the remaining $m-1$ replicated copies of this task are still being processed on the other servers. Then, these replicated task copies are cancelled immediately and the servers are assigned to process $m$ replicated copies of a new task. 
Hence, $\tau_{l,\text{FUT-R}}=0$ for $l=1,\ldots,m$. The complementary CDF for the servers to complete a task after time $\max\{s_{j+1},T_{j,\text{FUT-R}})\}$ is 
\begin{align}\label{eq_thm2_7}
&\Pr\Big[\min_{l=1,\ldots,m} R_{j,l,\text{FUT-R}}>t\Big]\nonumber\\
=& \Pr\Big[\min_{l=1,\ldots,m}X_l>t \Big].
\end{align}
If $\pi$ is a work-conserving policy, then we have $\tau_l\geq0$ for $l=1,\ldots,m$. Hence, the tail probability for the servers to complete a task after time $\max\{s_{j+1},T_{j,\pi}\}$ is 
\begin{align}\label{eq_thm2_8}
&\Pr\Big[\min_{l=1,\ldots,m} R_{j,l,\pi}>t\Big]\nonumber\\
=& \Pr\Big[\min_{l=1,\ldots,m}(X_l-\tau_l)>t\Big|X_l> \tau_l, l=1,\ldots,m \Big].
\end{align} 
By \eqref{eq_thm2_7}, \eqref{eq_thm2_8}, and the task service times are independent NWU, yields 
\begin{align}\label{eq_min_thm2}
\min_{l=1,\ldots,m} R_{j,l,\text{FUT-R}}\leq_{\text{st}} \min_{l=1,\ldots,m} R_{j,l,\pi}.
\end{align}
Using \eqref{eq_thm2_2}, \eqref{eq_min_thm2}, and the fact that $s_j$ is uniquely determined by $\mathcal{I}$, it follows that for all work-conserving policy $\pi\in\Pi$
\begin{align}\label{eq_thm2_4}
[T_{j+1,\text{FUT-R}} | \mathcal{I},  T_{j,\text{FUT-R}}= t_j] \leq_{\text{st}} [T_{j+1,\pi} | \mathcal{I},  T_{j,\pi} = t_j'] \nonumber\\
\text{whenever}~ t_j \leq t_j',j=1,2,\ldots
\end{align}
If policy $\pi$ is non-work-conserving, \eqref{eq_thm2_2} becomes
\begin{eqnarray}\label{eq_thm2_2_1}
T_{j+1,\pi}\!\geq\max\{s_{j+1},T_{j,\pi}\} + \!\min_{l=1,\ldots,m} R_{j,l,\pi},\nonumber
\end{eqnarray}
because of the possibility of server idleness. In this case, \eqref{eq_thm2_4} still holds. Hence, \eqref{eq_thm2_4} holds for all $\pi\in\Pi_{\text{non-prmp}}$.
Then, combining \eqref{eq_thm2_condition1_2}, \eqref{eq_thm2_4}, and Theorem 6.B.3 of \cite{StochasticOrderBook}, yields
\begin{align}%\label{eq_thm1_5}
[(T_{1,\text{FUT-R}},\ldots,T_{j,\text{FUT-R}})|\mathcal{I}] \leq_{\text{st}} [(T_{1,\pi},\ldots,T_{j,\pi})|\mathcal{I}],~\forall~\pi\in\Pi.\nonumber
\end{align}
Hence, \eqref{eq_thm2_proof1} is proven.

According to Theorem 6.B.1 of \cite{StochasticOrderBook}, for any policy $\pi\in\Pi$, there exist that FUT-R$_1$ and policy $\pi_1$ which satisfy the same queueing disciplines and stochastic laws with policy FUT-R and policy $\pi$, and policy FUT-R$_1$ is more work-efficient than policy $\pi_1$ with probability one. Because each task is replicated on all $m$ servers and $k_1\leq \ldots\leq k_n$, each task completing service is from the job with the fewest remaining tasks among all unfinished jobs.
By Proposition \ref{lem1_0}, for all $f\in\mathcal{D}_{\text{sym}}$
\begin{align}
\Pr[f(\bm{C}(\text{FUT-R}_1)) \leq f(\bm{C}(\pi_1)) |\mathcal{I}]=1. \nonumber
\end{align}
Then, by Theorem 1.A.1 of \cite{StochasticOrderBook}, we can obtain \eqref{eq_delaygap3}, which completes the proof.

%\section{Proofs of Thoerem~\ref{thm2_exp}} \label{app2_exp}

%We first show that policy FUT-R is more work-efficient than any policy $\pi\in\Pi$.  
%\begin{lemma}\label{lem_work_efficient_FUT_R}
%If the conditions of Theorem \ref{thm2} are satisfied, then policy FUT-R is more work-efficient than any policy $\pi\in\Pi$.  
%\end{lemma}
%\begin{proof}
%Consider any sample path of an arbitrarily chosen policy $\pi\in\Pi$ and an arbitrarily chosen task $j$. Suppose that 
%%on the sample path of policy $\pi$, server $l_w$ starts to process task $j$ at time $\tau$ and completes task $j$ at time $\nu$ ($\tau\leq\nu$). More specifically, suppose that 
%on the sample path of policy $\pi$, $u$ copies of task $j$ are replicated on the servers $l_1,l_2,\dots,l_u$ at the time instants $\tau_1,\tau_2,\ldots, \tau_u$, respectively, where $\tau=\tau_1\leq \tau_2\leq \ldots \leq\tau_u$; server $l_w$ ($w\in\{1,2,\ldots,u\}$) completes one copy of task $j$ at time $\nu$, which is earlier than the other $u-1$ servers; after time $\nu$, the other $u-1$ copies of task $j$ are cancelled. Hence, the service duration of task $j$ is $[\tau,\nu]$ on the sample path of policy $\pi$. One example of this is illustrated in Fig. \ref{fig_theorem_proof_2}, where $u=2$ and $w=2$. We need to prove that \emph{there exists one sample path of policy FUT-R such that these two sample paths of policy FUT-R and policy $\pi$ have the same probability density; and  on the sample path of policy FUT-R, if there exist unassigned tasks in the queue during $[\tau,\nu]$, then there exists one task $j'$ which starts execution during $[\tau,\nu]$ on server $l_w$}.
%
%
%\begin{figure}
%\centering 
%\includegraphics[width=0.5\textwidth]{Figures/theorem_proof_2} \caption{Illustration of the proof of Lemma \ref{lem_work_efficient_FUT_R}. On the sample path of policy $\pi$, two copies of task $j$ are replicated on the server $l_1$ and server $l_2$ at time $\tau_1$ and $\tau_2$, respectively, where $\tau=\tau_1\leq\tau_2$. Server $l_2$ completes one copy of task $j$ at time $\nu$, server $l_1$ cancels one redundant copy of task $j$ after time $\nu$. Hence, the service duration of task $j$ is $[\tau,\nu]$ on the sample path of policy $\pi$. On the sample path of policy FUT-R, server $l_2$ cancels a task at time $\tau_2'\in[\tau_2,\nu]$, and then a new task is assigned to server $l_2$. Server $l_2$ completes this task at time $t\in[\tau_2,\nu]\subseteq[\tau,\nu]$ and a new task $j'$ starts execution at time $t$. This task $j'$ is the task corresponding to task $j$ in the definition of work-efficiency ordering.}
%\label{fig_theorem_proof_2} 
%\end{figure} 
%
%Because policy FUT-R is work-conserving, if there exist unassigned tasks in the queue during $[\tau,\nu]$, then all servers are busy during $[\tau,\nu]$. In particular,  server $l_w$ is busy during $[\tau,\nu]$. 
%Suppose that in policy FUT-R, server $l_w$ has spent $\chi_w$ ($\chi_w\geq0$) seconds on a task by time $\tau_w\in[\tau,\nu]$. We construct the sample path of policy FUT-R by considering the following cases:
%
%\emph{Case 1: No task is completed on the servers $1,\ldots,l_w-1,l_w+1,\ldots,n$, until server $l_w$ completes a task}. Because server $l_w$ starts to process a task earlier in policy FUT-R, one can construct a sample path of policy FUT-R, such that that these two sample paths of policy FUT-R and policy $\pi$ have the same probability density, and server $l_w$ will complete a task before time $\nu$ on the sample path of policy FUT-R. Since in policy FUT-R, all servers are busy during $[\tau,\nu]$, a new task $j'$ will start execution on all servers at time $t$. Let task $j'$ be the task corresponding to task $j$ in the definition of work-efficiency ordering. 
%
%\emph{Case 2: Some of the servers $1,\ldots,l_w-1,l_w+1,\ldots,n$ complete a task at time $\tau_w'>\tau_w$ before server $l_w$ completes a task}. In this case, server $l_w$ will cancel its redundant task copy at time $\tau_w'$, then a new task will start execution on all $m$ servers at time $\tau_w'$. The probability for server $l_w$ to complete a task after time $\tau_w'+s$ is 
%\begin{align}
%\Pr[X_{l_w}>s].\nonumber
%\end{align}
%On the other hand, in policy $\pi$, the probability for server $l_w$ to complete task $j$ after time $\tau_w'+s$ is 
%\begin{align}
%\Pr[X_{l_w}-(\tau_w'-\tau_w)>s  |X_{l_w}> \tau_w'-\tau_w].\nonumber
%\end{align}
%Because $X_{l_w}$ is NWU, we can obtain that 
%\begin{align}
%\Pr[X_{l_w}>s]\leq \Pr[X_{l_w}-(\tau_w'-\tau_w)>s  |X_{l_w}> \tau_w'-\tau_w],\nonumber
%\end{align}
%which can be equivalently expressed as 
%\begin{align}
%X_{l_w} \leq_{\text{st}} [X_{l_w}-(\tau_w'-\tau_w) |X_{l_w}> \tau_w'-\tau_w].\nonumber
%\end{align}
%In other words, the task service time becomes stochastically shorter after task cancellation.
%According to the property of stochastic ordering \cite[Theorem 6.B.1]{StochasticOrderBook}, if on the sample path of policy $\pi$ server $l_w$ completes task $j$ at time $\nu$, one can construct a sample path of policy FUT-R, such that these two sample paths of policy FUT-R and policy $\pi$ have the same probability density, and server $l_w$ completes a task at some time $t$ earlier than $\nu$ on the sample path of policy FUT-R. Since in policy FUT-R, all servers are busy during $[\tau,\nu]$, a new task $j'$ will start execution on all servers at time $t$. Let task $j'$ be the task corresponding to task $j$ in the definition of work-efficiency ordering. This completes the proof.
%
%
%%We need to prove that on the sample path of policy FUT-R, there exists a time $t\in[\tau_w,\nu]$ such that one of the following three cases holds:  (i) server $l_w$ starts to process a task (which is corresponding to task $j$) at time $t$, (ii) all the remaining tasks are under service at time $t$, or (iii) the queue is empty at time $t$. 
%%Hence, we only need to prove that case (i) holds, whenever case (ii) and case (iii) do not hold. 
%%If case (ii) or case (iii) holds, then Lemma \ref{lem_work_efficient_FUT_R} is proven. Hence, we need to prove that case (i) holds, whenever case (ii) and case (iii) do not hold. More specifically, we need to prove that  \emph{on the  sample path of policy FUT-R, if there are one or more unassigned tasks during $[\tau_w,\nu]$, then server $l_w$ starts to process one task corresponding to task $j$ at some time $t\in[\tau_w,\nu]$}.
%
%%Because policy FUT-R is work-conserving, if there are one or more unassigned tasks during $[\tau_w,\nu]$, then all servers are busy during $[\tau_w,\nu]$.  
%%Suppose that in policy FUT-R, server $l_w$ has spent $\chi_w$ ($\chi_w\geq0$) seconds on a task by time $\tau_w$. If no task is cancelled on server $l_w$, then the task service time of server $l_w$ will be the same in both policies. Hence, on the sample path of policy FUT-R,  server $l_w$ will completes a task at time $t=\nu-\chi_w\in[\tau_w,\nu]$. If server $l_w$ cancels a task at time $\tau_w'>\tau_w$, then a new task will be assigned to server $l_w$ at time $\tau_w'$. 
%%
%%We compare the task completion time of server $l_w$ in these two cases: If no task is cancelled on server $l_w$, the probability for server $l_w$ to complete a task after time $\tau_w'+s$ is $\Pr[X_{l_w}-\chi_w-(\tau_w'-\tau_w)>s|X_{l_w}> \chi_w + (\tau_w'-\tau_w)]$ where $\chi_w + (\tau_w'-\tau_w)>0$. On the other hand, if server $l_w$ cancels a task at time $\tau_w'$, the probability for server $l_w$ to complete a task after time $\tau_w'+s$ is $\Pr[X_{l_w}>s]$. Because $X_{l_w}$ is NWU, we can obtain that 
%%\begin{align}
%%\Pr[X_{l_w}-\chi_w-(\tau_w'-\tau_w)>s|X_{l_w}> \chi_w + (\tau_w'-\tau_w)] \leq \Pr[X_{l_w}>s].\nonumber
%%\end{align}
%%By the property of stochastic ordering \cite[Theorem 6.B.1]{StochasticOrderBook}, if server $l_w$ cancels a task at time $\tau_w'$, server $l_w$ will completes a task at a time $t$ earlier than $\nu-\chi_w$. Because policy FUT-R is work-conserving and there are one or more unassigned tasks at time $t$, an unassigned task $j'$ will be allocated to server $l_w$ at time $t$. Let task $j'$ be the task corresponding to task $j$  in the definition of work-efficiency ordering. This completes the proof. 
%\end{proof}

%\ifreport
%\begin{proof}[Proof of Theorem \ref{thm2}]
%\else
%\begin{proof}[of Theorem \ref{thm2}]
%\fi
%In Lemma \ref{lem_work_efficient_FUT_R}, we have shown that policy FUT-R is more work-efficient than any policy $\pi\in\Pi$. Then, Theorem \ref{thm2} follows from Corollary \ref{coro1}. This completes the proof.
%\end{proof}
\section{Proof of Lemma \ref{lem7_NWU}}\label{app_lem7_NWU}  
Consider the time difference ${C}_i(\text{FUT-R})-{U}_i(\text{FUT-R})$.
%\textbf{Condition 4:} $P\in\Pi$. This condition is trivial. Hence, \eqref{eq_delaygap1} follows from Lemma \ref{thm2}.
In policy FUT-R, all servers are allocated to process $m$ replicated copies of a task from the job with the fewest unassigned tasks. Hence, at time ${U}_i(\text{FUT-R})$, one task of job $i$ are being processed by all $m$ servers. 
%Then, $\mathcal{S}_i$ is a random set with cardinality $|\mathcal{S}_i|\leq k_i\wedge m$.
%The remaining task is to prove \eqref{eq_delaygap2}. 
Because the $X_l$'s are independent exponential random variables with mean $\mathbb{E}[X_l]=1/\mu_l$, 
by Theorem 3.A.55 of \cite{StochasticOrderBook}, we can obtain
%\begin{align}
%X_l \leq_{\text{icv}} Z_l,~l=1,\ldots,m,\nonumber
%\end{align}
%where $\leq_{\text{icv}}$ is the increasing concave order defined in \cite[Chapter 4]{StochasticOrderBook} and the $Z_l$'s are independent exponential random variables with mean $\mathbb{E}[Z_l]=\mu_l$. By Corollary 4.A.16 of \cite{StochasticOrderBook}, we have 
%\begin{align}\label{eq_exp_orderNWU}
%\min_{l=1,\ldots,m} X_l \leq_{\text{icv}} \min_{l=1,\ldots,m} Z_l.
%\end{align}
%Note that the set $\mathcal{S}_i$ is determined by the evolution of policy FUT-R up to time ${U}_i(\text{FUT-R})$.Because the task service times are determined by an external process which is not affected by the scheduling policy FUT-R, $X_l$ and $Z_l$ are independent of $\mathcal{S}_i$ for each $l\in \mathcal{S}_i$.
%Then,   
\begin{align}
&\mathbb{E}[{C}_i(\text{FUT-R})-{U}_i(\text{FUT-R})|\mathcal{I}]\nonumber\\
\leq &\mathbb{E}\!\left[\min_{l=1,\ldots,m} X_l\bigg|\mathcal{I}\right]\label{eq_gap_NWU_condition1}\\
=&\mathbb{E}\!\left[ \min_{l=1,\ldots,m} X_l\right]\label{eq_gap_NWU_condition2}\\
%\leq&\mathbb{E}\!\left[ \min_{l=1,\ldots,m} Z_l\right]\label{eq_gap_NWU_condition3}\\
\leq &\frac{1}{\sum_{l=1}^m \mu_l}.\label{eq_gap_NWU_condition5}
\end{align}
where \eqref{eq_gap_NWU_condition1} is because one task of job $i$ are being processed by all $m$ servers at time ${U}_i(\text{FUT-R})$, \eqref{eq_gap_NWU_condition2} is because $X_l$ is independent of $\mathcal{I}$, 
%\eqref{eq_gap_NWU_condition3} is due to\eqref{eq_exp_orderNWU} and Eq. (4.A.1) of \cite{StochasticOrderBook}, 
and \eqref{eq_gap_NWU_condition5} is due to the property of exponential distributions. By this, Lemma \ref{lem7_NWU} is proven.


%\subsection{Proof of Corollary \ref{coro4}}  
%%Similar with Corollary \ref{coro3}, 
%Let $t_i(\pi)$ denote the $i$-th task completion time on the sample path of policy $\pi$. We first show that for all $\pi\in\Pi$ 
%\begin{align}\label{eq_coro4_1}
%t_{i}(\text{FUT-R})\leq t_{i}(\pi), ~i=1,2,\ldots 
%\end{align}  
%
%According  the proof of Lemma \ref{lem_work_efficient_FUT_R}, for each sample path of policy $\pi\in\Pi$ there exists a sample path of policy FUT-R, such that if (i) a task $j$ starts execution at time $\tau$ and completes execution at time $\nu$ ($\tau\leq\nu$) on the sample path of policy $\pi$, and (ii) all servers are busy in policy FUT-R, then on the sample path of policy FUT-R, a task completes execution during $[\tau,\nu]$ before a new task $j'$ starts execution. On the other hand, if (ii') some servers are idle in policy FUT-R, then the queue is empty. 
%%According to 
%%we can obtained from the proof of Lemma \ref{lem_work_efficient_FUT_R} that
%Using this, we can show that for all $t\geq0$, if $b$ tasks are completed during $[0,t]$ on the sample path of policy $\pi$, then at least $b$ tasks are completed during $[0,t]$ on the sample path of policy FUT-R. By this, \eqref{eq_coro4_1}
%follows.
%%Because each job has $k$ tasks, if the servers start to process the tasks of job $i$, job $i$ will have fewer unassigned tasks than any other job in the queue which has $k$ unassigned tasks. No incoming job can have a higher priority than job $i$. Therefore, the servers will keep processing the tasks of job $i$ until job $i$ is completed. Further, 
%
%Next, we use \eqref{eq_coro4_1} to prove Corollary \ref{coro4}.
%Because each job has $k$ tasks,  for any $\pi\in\Pi$ no job can be completed before time $t_{k}(\pi)$, i.e.,
%\begin{align}
%c_{(1)}(\pi)\geq t_{k}(\pi).\nonumber
%\end{align}  
%In general, we have
%\begin{align}
%c_{(i)}(\pi)\geq t_{ik}(\pi), ~i=1,2,\ldots,n. \nonumber
%\end{align}  
%In addition, policy FUT-R satisfies that
%\begin{align}
%c_{(i)}(\text{FUT-R})= t_{ik}(\text{FUT-R}), ~i=1,2,\ldots,n. \nonumber
%\end{align} 
%Hence, for $i=1,2,\ldots,n$
%\begin{align}
%c_{(i)}(\text{FUT-R})= t_{ik}(\text{FUT-R})\leq   t_{ik}(\pi) \leq c_{(i)}(\pi)\nonumber
%\end{align} 
%holds in stochastic ordering. Therefore, for all $f\in\mathcal{D}_{\text{sym}}$ and $\pi\in\Pi$
%\begin{align}
%&[f(\bm{c} (\text{FUT-R}))|\mathcal{I}]=[f(\bm{c}_{\uparrow} (\text{FUT-R}))|\mathcal{I}] \nonumber\\
%\leq_{}&[f(\bm{c}_{\uparrow} (\pi))|\mathcal{I}] = [f(\bm{c}_{} (\pi))|\mathcal{I}] \nonumber
%\end{align} 
%holds in stochastic ordering. By considering all possible sample paths, the stochastic ordering result in Corollary \ref{coro4} is proven.



==> v3/appendices_3version2.tex <==
% !TEX root = ./replication.tex

\section{Proofs of Proposition~\ref{coro3_1}} \label{app0_2}
%\ifreport
%\begin{proof}[Proof of Thoerem \ref{lem3}]
%\else
%\begin{proof}[of Thoerem \ref{lem3}]
%\fi
%Thoerem \ref{lem3} follows from Thoerem \ref{lem2} by letting $d_i=a_i$ for all $i$.
%\end{proof}
%\ifreport
%\begin{proof}[Proof of Corollary~\ref{coro3_1}]
%\else
%\begin{proof}[of Corollary~\ref{coro3_1}]
%\fi
%Proposition~\ref{coro3_1} follows from Corollary \ref{coro2} by letting $d_i=a_i$ for all $i$.
%As in the proof of Corollary \ref{coro2}, let $w_i$ denote the index of the job associated with $v_{(i)}(P)$.
%
%We assume that the arrival times $a_1,\ldots, a_n$ of the $n$ jobs are distinct from each other. This does not lose any generality, because if $a_i=a_j$ for two jobs $i$ and $j$, Proposition~\ref{coro3_1} can be proven by first proving for the case $a_i=a_j+\epsilon$ and then taking the limit $\epsilon\rightarrow 0$. 
We take 3 steps to prove Proposition~\ref{coro3_1}:

\emph{Step 1: We show that}  
%Thoerem \ref{lem3} holds if \emph{$D_{\max}(\cdot)$} is replaced by any $f\in\mathcal{D}_{\text{sym}}$.}
\begin{align}\label{eq_coro2_2_2}
v_{(i)}(P) \leq c_{(i)}(\pi),~i=1,\ldots,n.
\end{align}

In policy $P$, each unassigned task entering the servers is from the job with the earliest arrival time among all jobs with unassigned tasks. Because each job has $k$ tasks, in policy $P$ only the job with the earliest arrival time may have fewer than $k$ unassigned tasks, the other jobs arrived later have exactly $k$ unassigned tasks. Therefore, among all jobs with unassigned tasks, the job with the earliest arrival time is also the job with the fewest unassigned tasks.
Then, \eqref{eq_coro2_2_2} follows from Proposition~\ref{lem1}. 
In addition, we can use Proposition \ref{lem1} to prove that \eqref{eq_coro3_1_1} holds for all $f\in\mathcal{D}_{\text{sym}}$.

The remaining proof is almost identical with \emph{Step 2} and \emph{Step 3} in the proof of Proposition \ref{coro2}, except that $d_i$ should be replaced by $a_i$. 
By this, Proposition~\ref{coro3_1} is proven.
%Because each job has $k$ tasks, a job can have fewer than $k$ unassigned tasks if and only if some of its tasks are under service, which 
%Because each job has $k$ tasks, only the job under service has fewer than $k$ tasks, , 
%at any time in policy $P$, the job with the earliest arrival time is also the job with the fewest unassigned tasks.
%We can utilize Lemma \ref{lem_sample_path_ordering} to show that $v_{w_j}(P) = v_{(j)}(P) \leq c_{(j)}(\pi)$ for all $j=1,\ldots,n$. In addition, 
%According to Corollary \ref{coro1}, the result of Thoerem \ref{lem3} holds if \emph{$D_{\max}(\cdot)$} is replaced by any $f\in\mathcal{D}_{\text{sym}}$.
%\emph{Step 2: We show that}
%\begin{align}\label{eq_coro3_3}
%\bm{u}(P)-\bm{d}\prec_{\text{w}} \bm{c} (\pi)-\bm{d}.
%\end{align} 
%
%
%
%We construct a policy $\pi'$ based on policy $\pi$: The sequence of job completion times of policy $\pi'$ is a reordering (rearrangement) of that of policy $\pi$. And in policy $\pi'$, each completed job has the earliest arrival time among all jobs in the queue. We note that because each job has $k$ tasks, it is feasible to reordering the job completion times such that the job arrives earlier is completed earlier.
%% this reordering operation leads to a feasible policy $\pi'$. %In particular, suppose that job $i$ has an earlier arrival time than job $j$. Because both job $i$ and job $j$ have $k$ tasks, the system can switch to process job $i$
%%and more unassigned tasks than the other jobs in the queue, then it is infeasible to reorder the sequence of job completion times such that job $i$ is the next completed job.
%Hence, for the constructed policy $\pi'$, one can use the proof argument of Lemma \ref{lemG4_thm3} to show that
%\begin{eqnarray}\label{eq_pi'_3}
%\sum_{i:a_i\leq\tau} \gamma_{i,P}(t)\leq \sum_{i:a_i\leq\tau} \xi_{i,\pi'}(t), ~\forall~\tau\in[0,\infty)
%\end{eqnarray}
%holds for all $t\in[0,\infty)$. The remaining proof is the same with \emph{Step 2} and \emph{Step 3} in the proof of Corollary \ref{coro2}, where $d_i$ is replaced by $a_i$. 
%By this, Corollary~\ref{coro3_1} is proven.
%\end{proof}

%\subsection{Proof of Corollary \ref{coro2}}
%
%
%In the proof of Corollary \ref{coro2}, we need to use the following rearrangement inequality: 
%\begin{lemma} \cite[Theorem 6.F.14]{Marshall2011}\label{lem_rearrangement}
%Consider two $n$-vectors $(x_1,\dots,x_n)$ and $(y_1,\ldots,y_n)$. If $(x_i- x_j)(y_i-y_j)<0$ for some indices $i$ and $j$ where $1\leq i<j\leq n$, then 
%\begin{align}
%&(x_1\!-\!y_1,\ldots,x_j\!-\!y_i,\ldots,x_i\!-\!y_j,\ldots,x_n\!-\!y_n)\nonumber\\
%\prec& (x_1\!-\!y_1,\ldots,x_i\!-\!y_i,\ldots,x_j\!-\!y_j,\ldots,x_n\!-\!y_n).\nonumber
%\end{align}
%\end{lemma}
%\ifreport
%\begin{proof}[Proof of Corollary \ref{coro2}]
%\else
%\begin{proof}[of Corollary \ref{coro2}]
%\fi
%As in the proof of Lemma \ref{lem_sample_path_ordering_thm3}, let $w_i$ denote the index of the job associated with $v_{(i)}(P)$. 
%
%\emph{Step 1: We show that  
%Thoerem \ref{lem2} holds if \emph{$L_{\max}(\cdot)$} is replaced by any $f\in\mathcal{D}_{\text{sym}}$.}
%%\begin{align}\label{eq_coro2_2}
%%v_{w_i}(P) \leq c_{(i)}(\pi),~i=1,\ldots,n.
%%\end{align}
%
%Because each job has only one task, it holds in policy $P$ that each task allocated to the servers belongs to the job with the fewest unassigned tasks, whenever there exist unassigned tasks in the system. 
%Hence, 
%%we can utilize Lemma \ref{lem_sample_path_ordering} to show that $v_{w_i}(P) = v_{(i)}(P) \leq c_{(i)}(\pi)$ for all $i=1,\ldots,n$. On the other hand, 
%Corollary \ref{coro1} implies that Thoerem \ref{lem2} holds if \emph{$L_{\max}(\cdot)$} is replaced by any {$f\in\mathcal{D}_{\text{sym}}$}.

%Suppose that $b_j$ tasks have been assigned to the servers in policy $P$ by time $c_{(j)}(\pi)$. Since each job has only one task, $j$ tasks are completed by time $c_{(j)}(\pi)$ in policy $\pi$. Because policy $P$ is more work-efficient than policy $\pi$, it must hold that at least $j$ tasks are completed during $[0,c_{(j)}(\pi)]$  in policy $P$. Hence, at least $j$ tasks are assigned to the servers during $[0,c_{(j)}(\pi)]$ in policy $P$. Because each job has only one task, it follows that $v_{w_j}(P) \leq c_{(j)}(\pi)$  for all $j=1,\ldots,n$.

%We prove Corollary \ref{coro2} by induction. 

%\emph{Step 2: We show that}
%\begin{align}\label{eq_coro2_3}
%\bm{u}(P)-\bm{d}\prec_{\text{w}} \bm{c} (\pi)-\bm{d}.
%\end{align} 
%
%
%%We show that Thoerem \ref{lem2} holds if \emph{$L_{\max}(\cdot)$} is replaced by any $f\in\mathcal{D}_{\text{Sch-1}}$.} 
%
%We construct two policies $\pi'$ and $\pi''$ based on policy $\pi$: The sequence of job completion times of policy $\pi'$ is a rearrangement (reordering) of that of policy $\pi$, such that for each job $i$ there exists a job $j$ such that $c_i(\pi') = c_j(\pi)$.
%%, i.e., the completion time of any job $i'$ in policy $\pi'$ must be the completion time of some job $i$ in policy $\pi$.
%Furthermore, in policy $\pi'$, each completed job has the earliest due time among all jobs presenting in the queue, such that $c_1(\pi')\leq c_2(\pi') \leq \ldots \leq c_n(\pi')$. Hence, 
%\begin{align}\label{coro2_1}
%c_i(\pi') = c_{(i)}(\pi).
%\end{align}
%On the other hand, the task completion times of policy $\pi''$ is a rearrangement (reordering) of the task completion times of policy $\pi$, and in policy $\pi''$, each completed task belongs to the jobs with the earliest due time among all jobs presenting in the queue. 
%Let $t_i(\pi)$ be the $i$-th smallest task completion time of policy $\pi$, then 
%\begin{align}\label{coro2_2}
%c_i(\pi'') = t_{ik}(\pi).
%\end{align} 
%%i.e., if job $i$ arrives before the completion time of job $j$ and $d_i<d_j$, then job $i$ is completed before job $j$ in policy $\pi'$. 
%%Let $t_i(\pi)$ be the $i$-th smallest task completion time of policy $\pi$. 
%In policy $\pi$, because each job has $k$ tasks, the system must complete at least $k$ tasks before one job is completed, i.e.,
%$c_{(1)}(\pi)\geq t_{k}(\pi)$. In general, the system must complete at least $ik$ tasks before $i$ jobs are completed, i.e., 
%\begin{align}\label{coro2_3}
%c_{(i)}(\pi)\geq t_{ki}(\pi).
%\end{align} 
%By combining \eqref{coro2_1}-\eqref{coro2_3}, we have
%\begin{align}
%c_i(\pi') = c_{(i)}(\pi)\geq t_{ik}(\pi)=c_i(\pi'').
%\end{align}
%We note that policy $\pi''$ is feasible, but policy $\pi'$ is not because 
%
%
%
%
%
%
%
%
%In policy $\pi''$, the task completion times 
%
%
%For this constructed policy $\pi'$, one can use the proof argument of Lemma \ref{lemG4_thm3} to show that
%\begin{eqnarray}\label{eq_pi'}
%\sum_{i:a_i\leq\tau} \gamma_{i,P}(t)\leq \sum_{i:a_i\leq\tau} \xi_{i,\pi'}(t), ~\forall~\tau\in[0,\infty)
%\end{eqnarray}
%holds for all $t\in[0,\infty)$. That is, Lemma \ref{lemG4_thm3}  holds even if policy $\pi$ is replaced by this constructed policy $\pi'$. %Note that if the jobs have more than one tasks, \eqref{eq_pi'} may not hold for the constructed policy $\pi'$.
%%We rearrange the job completion times of policy $\pi$ as follows: Consider any two jobs $i$ and $j$ which simultaneously exist in the queue at some time, i.e., there exists a time $t$ such that $a_i\leq t\leq c_i(\pi)$ and  $a_j\leq t\leq c_j(\pi)$. If $(c_i(\pi)-c_j(\pi))(d_i- d_j)<0$, we interchange the completion times of job $i$ and job $j$. Repeat this procedure until $(c_i(\pi)-c_j(\pi))(d_i- d_j)\geq 0$ is satisfied for any pair of jobs $i$ and $j$ which simultaneously exist in the queue at some time. Hence, after the rearrangement, each completed job has the earliest due time among all jobs in the queue. Let $c_i'(\pi)$ denote the completion time of job $i$ after the rearrangement. 
%
%In the sequel, we will use \eqref{eq_pi'}, Lemma \ref{lem_rearrangement}, and the property of policy $\pi'$ to prove the following two claims:
%\begin{itemize}
%\item[1.] $\bm{c}(\pi')-\bm{d}\prec \bm{c} (\pi)-\bm{d}$;
%\item[2.] $v_i(P)\leq c_i(\pi')$ for $i=1,\ldots,n$.
%\end{itemize}
%
%
%%Hence, the $i$-th smallest job completion time $c_{(i)}(\pi')$ of policy $\pi'$ is equal to $i$-th smallest job completion time $c_{(i)}(\pi)$ of policy $\pi$, i.e., $c_{(i)}(\pi')=c_{(i)}(\pi)$.
%
%First, we prove claim 1. An alternative construction procedure of policy $\pi'$ is provided as follows: Suppose that in policy $\pi$, two jobs $i$ and $j$ co-exist in the queue at some time $t$, i.e., $a_i\leq t\leq c_i(\pi)$ and  $a_j\leq t\leq c_j(\pi)$. If $(c_i(\pi)-c_j(\pi))(d_i- d_j)<0$, the completion times of job $i$ and job $j$ are interchanged. 
%Repeat this pair-wise interchange operation until $(c_i(\pi)-c_j(\pi))(d_i- d_j)\geq 0$ is satisfied for any pair of jobs $i$ and $j$ which co-exist in the queue at some time. Then, the job completion times of policy $\pi'$ are obtained.
%By using Lemma \ref{lem_rearrangement} for each pair-wise interchange operation during this construction procedure of policy $\pi'$, we can obtain $\bm{c}(\pi')-\bm{d}\prec \bm{c} (\pi)-\bm{d}$. By this, claim 1 is proven.
%
%
%Next, we prove claim 2 by contradiction. Suppose that
%\begin{align}\label{eq_contradiction_coro2}
%v_{w_j}(P) > c_{w_j}(\pi')
%\end{align} 
%holds for some $j\in\{1,\ldots,n\}$.
%In policy $\pi'$, if job $i$ arrives before time $c_{w_j}(\pi')$ and $d_i<d_{w_j}$, then job $i$ is completed before time $c_{w_j}(\pi')$. Hence, the system state of policy $\pi'$ satisfies 
%\begin{align}
%\sum_{i:d_i\leq d_{w_j}}\xi_{i,\pi'}(c_{w_j}(\pi')) =0,\nonumber
%\end{align}
%where we have used the fact that $d_i\neq d_j$ if $i\neq j$. Combining this with \eqref{eq_pi'}, we can obtain
%%Hence, there are $y-1$ unfinished jobs at time $C_{w_1}(\pi)$ such that
%%Invoking Lemma \ref{lemG4}, we can obtain
%\begin{align}\label{eq_proof_1_coro2}
%\sum_{i:d_i\leq d_{w_j}} \gamma_{i,P}(c_{w_j}(\pi'))\leq 0.
%\end{align}
%By the definition of the system state, we have $\gamma_{i,P}(t)\geq0$ for all $i$ and $t$. This and \eqref{eq_proof_1_coro2} tells us that at time $c_{w_j}(\pi')$, the system state of policy $P$ satisfies
%\begin{align}
%\gamma_{w_j,P}(c_{w_j}(\pi'))= 0.\nonumber
%\end{align}
%That is, all tasks of job $w_j$ are either completed or under service by time $c_{w_j}(\pi')$ in policy $P$. Hence, $v_{w_j}(P)\leq c_{w_j}(\pi')$, which contradicts with \eqref{eq_contradiction_coro2}. Therefore, $v_{w_j}(P)\leq c_{w_j}(\pi')$ holds for all $j=1,\ldots,n$. By this, claim 2 is proven.
%
%Now, we use claim 1 and claim 2 to prove \eqref{eq_coro2_3}. In particular,  claim 1 and claim 2 suggest that
%\begin{align}
%\bm{u}(P)-\bm{d}\leq \bm{c}(\pi')-\bm{d}\prec \bm{c} (\pi)-\bm{d}.
%\end{align}
%By this and Theorem 5.A.9 of \cite{Marshall2011}, \eqref{eq_coro2_3} follows.
%
%
%\emph{Step 3: We use \eqref{eq_coro2_3} to prove Corollary \ref{coro2}.}
%For any $f\in\mathcal{D}_{\text{Sch-1}}$, $f(\bm{x}+\bm{d})$ is Schur convex. 
%According to Theorem 3.A.8 of \cite{Marshall2011}, for all $f\in\mathcal{D}_{\text{Sch-1}}$, 
%\begin{align}
%&f(\bm{u}(P)) \nonumber\\
%= &f[(\bm{u}(P)-\bm{d})+\bm{d}] \nonumber\\
%\leq& f[(\bm{c}(\pi)-\bm{d})+\bm{d}] \nonumber\\
%=& f(\bm{c} (\pi)).\nonumber
%\end{align} 
%By considering all possible sample paths of these two policies, the stochastic ordering result in Corollary \ref{coro2} follows.
%This completes the proof.
%%\end{proof}
%
%\end{proof}
%
%
%%We develop a {sample-path ordering} technique to prove Thoerem \ref{lem3}. The system state of policy $P$ is the same as that in \emph{Definition \ref{def_state_thm3}}, and the system state of policy $\pi$ are the same as that in \emph{Definition \ref{def_state_P_thm3}}. 
%%
%%
%%We assume that the priorities $p_1,\ldots, p_n$ of the $n$ jobs are distinct from each other. This does not lose any generality, because if $p_i=p_j$ for two jobs $i$ and $j$, Thoerem \ref{lem3} can be proven by taking the limit $p_i\rightarrow p_j$.  The first part of the sample-path ordering result is as follows:
%% 
%% 
%%\begin{lemma}\label{lemG4_lem3}
%%Suppose that $\bm{\gamma}(0^-)=\bm{\zeta}(0^-)=\bm{\xi}(0^-)=\bm{0}$ and the conditions of Thoerem \ref{lem3} are satisfied. Then, the following relationship holds on sample path:
%%\begin{eqnarray}\label{eq_lemG4_lem3}
%%\sum_{i: p_i\geq p} [\gamma_i(t) - \zeta_i(t)]\leq \sum_{i: p_i\geq p} \xi_i(t), ~\forall~p\geq 0.
%%\end{eqnarray}
%%holds for all $t\geq0$.
%%\end{lemma}
%%
%%The following two lemmas are needed to prove Lemma \ref{lemG4_lem3}:
%%
%%
%%\begin{lemma}\label{lem_non_prmp1_lem3}
%%Suppose that, under policy $P$, $\{\bm{\gamma}',\bm{\zeta}'\}$ is obtained by allocating $b$ unassigned tasks to the servers in the system whose state is $\{\bm{\gamma},\bm{\zeta}\}$. Further, suppose that, under policy $\pi$, $\bm{\xi}'$ is obtained by completing $b'$ tasks in the system whose state is $\bm{\beta}$.
%%If $b\geq b'$ and
%%\begin{eqnarray}
%%\sum_{i: p_i\geq p} [\gamma_i - \zeta_i]\leq \sum_{i: p_i\geq p} \xi_i, ~\forall~p\geq 0,\nonumber
%%\end{eqnarray}
%%then
%%\begin{eqnarray}\label{eq_non_prmp_40_lem3}
%%\sum_{i: p_i\geq p} [\gamma_i'- \zeta_i']\leq \sum_{i: p_i\geq p} \xi_i', ~\forall~p\geq 0.\end{eqnarray}
%%\end{lemma}
%%
%%\begin{proof}
%%If $\sum_{i: p_i\geq p} [\gamma_i' - \zeta_i']=0$, then the inequality \eqref{eq_non_prmp_40_lem3} follows naturally. 
%%If $\sum_{i: p_i\geq p} [\gamma_i' - \zeta_i']>0$, then there exist some tasks that have not been assigned to any server. 
%%In policy $P$, each idle server will be allocated to process an unassigned task from the job with the highest priority. Hence,
%%$\sum_{i: p_i\geq p} [\gamma_i' - \zeta_i']=\sum_{i: p_i\geq p} [\gamma_i - \zeta_i] - b \leq \sum_{i: p_i\geq p} \xi_i -b' \leq \sum_{i: p_i\geq p} \xi_i'$.
%%\end{proof}
%%
%%
%%\begin{lemma}\label{lem_non_prmp2_lem3}
%%Suppose that under policy $P$, $\{\bm{\gamma}',\bm{\zeta}'\}$ is obtained by adding a job with $b$ tasks and arrival time $a$ to the system whose state is $\{\bm{\gamma},\bm{\zeta}\}$. Further, suppose that under policy $\pi$, $\bm{\xi}'$ is obtained by adding a job with $b$ tasks and arrival time $a$ to the system whose state is $\bm{\xi}$.
%%If
%%\begin{eqnarray}
%%\sum_{i: p_i\geq p} [\gamma_i- \zeta_i]\leq \sum_{i: p_i\geq p} \xi_i, ~\forall~p\geq 0,\nonumber
%%\end{eqnarray}
%%then
%%\begin{eqnarray}
%%\sum_{i: p_i\geq p} [\gamma_i' - \zeta_i']\leq \sum_{i: p_i\geq p} \xi_i', ~\forall~p\geq 0.\nonumber\end{eqnarray}
%%\end{lemma}
%%
%%\begin{proof}
%%If $a\leq a_j$, then
%%$\sum_{i: p_i\geq p} [\gamma_i' - \zeta_i']\leq \sum_{i: p_i\geq p} [\gamma_i - \zeta_i] + b\leq \sum_{i: p_i\geq p} \xi_i+b \leq \sum_{i: p_i\geq p} \xi_i'$.
%%
%%If $a>a_j$, then
%%$\sum_{i: p_i\geq p} [\gamma_i' - \zeta_i']\leq \sum_{i: p_i\geq p} [\gamma_i - \zeta_i] \leq \sum_{i: p_i\geq p} \xi_i \leq \sum_{i: p_i\geq p} \xi_i'$.
%%\end{proof}
%%
%%The proof of Lemma \ref{lemG4_lem3} is quite similar with that of Lemma \ref{lemG4}, and hence is omitted. The only differences are (i) Lemma \ref{lem_non_prmp1} and Lemma \ref{lem_non_prmp2} in the proof of Lemma \ref{lemG4} should be replaced by Lemma \ref{lem_non_prmp1_lem3} and Lemma \ref{lem_non_prmp2_lem3}, respectively, and (ii) $\bm{\alpha}(t)$, $\bm{\delta}(t)$, and $\bm{\beta}(t)$ in the proof of Lemma \ref{lemG4} should be replaced by $\bm{\gamma}(t)$, $\bm{\zeta}(t)$, and $\bm{\xi}(t)$, respectively.
%%
%%
%%
%%
%%
%%
%%The second part of the sample-path ordering result is as follows:
%%
%%\begin{lemma}\label{lem_sample_path_ordering_lem3}
%%If Lemma \ref{lemG4_lem3} holds, then $\bm{u}_{\uparrow}(P)\leq \bm{c}_{\uparrow}(\pi)$ holds on sample path for all $\pi\in\Pi_{PL}$. 
%%\end{lemma}
%%
%%\begin{proof}
%%Let $w_i$ be the index of the job associated with $v_{(i)}(P)$, then job $w_j$ is the $j$-th job whose tasks are completed or under service in policy $P$. Similar with \eqref{eq_proof_3_thm3} in the proof of Lemma \ref{lem_sample_path_ordering_thm3}, we can obtain
%%\begin{align}
%%v_{w_j}(P) \leq \max_{i:a_i\leq v_{w_j}(P),p_i\geq p_{w_j} }c_{i}(\pi).
%%\end{align}
%%
%%Because job $w_j$ is the $j$-th job whose tasks are completed or under service, only the jobs $w_1,\ldots, w_{j-1}$ can be completed during $[0,v_{w_j}(P))$ in policy $P$.
%%In addition, each idle server is assigned to process a task from the job with the highest priority in  policy $P$. This tells us that job $w_j$ has the highest priority among all jobs in the queue at time $v_{w_j}(P)$ in policy $P$.
%%Therefore, if job $i$ satisfies $a_i\leq v_{w_j}(P)$ and $p_i\leq p_{w_j}$, then $i\in\{w_1,\ldots, w_j\}$. 
%%
%%
%%%We  prove Lemma \ref{lem_sample_path_ordering_lem3} by induction. 
%%Consider the sample paths of policy $P$ and policy $\pi$ in Lemma \ref{lemG4_lem3}. 
%%Recall that $U_i(P)$ is the earliest time that all tasks of job $i$ are either completed or under service in policy $P$, $v_i(P)$ is the realization of $U_i(P)$ on the sample path of policy $P$, and $v_{(i)}(P)$ is the $i$-th smallest component of $(v_{1}(P),\ldots,v_{n}(P))$. Let $w_i$ be the index of the job associated with $v_{(i)}(P)$.
%%
%%%\emph{Step 1: We first show that} 
%%%\begin{align}\label{eq_Condition_3_1_lem3}
%%%v_{w_1}(P) - d_{w_1} \leq c_{w_1}(\pi) - d_{w_1}.
%%%\end{align}
%%%%Let $y_1$ be the number of jobs that have arrived by time $v_{w_1}(P)$. 
%%%
%%%
%%%We prove \eqref{eq_Condition_3_1_lem3} by contradiction. Suppose that 
%%%\begin{align}\label{eq_Condition_3_11_lem3}
%%%v_{w_1}(P) > c_{w_1}(\pi),
%%%\end{align} 
%%%i.e., job $w_1$ is completed earlier than $v_{w_1}(P)$ in policy $\pi$. 
%%%
%%%Because job $w_1$ is the first job whose tasks are either completed or under service, no job is completed during $[0,v_{w_1}(P))$ in policy $P$. Because policy $P$ satisfies condition 2 of Thoerem \ref{lem3}, job $w_1$ has the earliest due time among all jobs in the queue at time $v_{w_1}(P)$ in policy $P$.  This tells us that job $w_1$ has the earliest due time among all jobs that have arrived during $[0,v_{w_1}(P))$.
%%%Hence, when job $w_1$ departs at time $c_{w_1}(\pi)$ in policy $\pi$, $d_i> d_{w_1}$ holds for all jobs in the queue. Therefore, the system state of policy $\pi$ satisfies  
%%%\begin{align}\label{eq_proof_0_lem3}
%%%\sum_{i:d_i\leq d_{w_1}}\xi_i(c_{w_1}(\pi)) =0.
%%%\end{align}
%%%Combining \eqref{eq_proof_0_lem3} and Lemma \ref{lemG4_lem3}, we can obtain
%%%%Hence, there are $y-1$ unfinished jobs at time $C_{w_1}(\pi)$ such that
%%%%Invoking Lemma \ref{lemG4}, we can obtain
%%%\begin{align}\label{eq_proof_1_lem3}
%%%\sum_{i:d_i\leq d_{w_1}} \gamma_i(c_{w_1}(\pi))\leq \sum_{i:d_i\leq d_{w_1}}  \zeta_i(c_{w_1}(\pi)).
%%%\end{align}
%%%By the definition of the system state of policy $P$, we have $\gamma_i(t)\geq \zeta_i(t)$ for all $i$ and $t$. This and \eqref{eq_proof_1_lem3} tells us that at time $c_{w_1}(\pi)$, the system state of policy $P$ satisfies
%%%\begin{align}\label{eq_proof_2_lem3}
%%%\!\!\gamma_{w_1}(c_{w_1}(\pi))= \zeta_{w_1}(c_{w_1}(\pi)).
%%%\end{align}
%%%Hence, in policy $P$ all tasks of job $w_1$ are either completed or under service at time $c_{w_1}(\pi)$. Combine this and \eqref{eq_Condition_3_11_lem3}, yields $$v_{w_1}(P)\leq c_{w_1}(\pi)<v_{w_1}(P),$$ which is a contradiction. Hence, $v_{w_1}(P) \leq c_{w_1}(\pi)$. By this, \eqref{eq_Condition_3_1_lem3} is proven.
%%
%%It is sufficient to show that for each $j=1,2,\ldots,n$,
%%\begin{align}\label{eq_Condition_3_12_lem3}
%%v_{w_j}(P)-d_{w_j} \leq \max_{i=1,2,\ldots,n }[c_{i}(\pi)-d_i].
%%\end{align}
%%We prove \eqref{eq_Condition_3_12_lem3} by contradiction. Suppose that 
%%\begin{align}\label{eq_proof_9_lem3}
%%v_{w_j}(P) > c_{i}(\pi)
%%\end{align}
%%holds for all $i$ satisfying $a_i\leq v_{w_j}(P)$ and $d_i\leq d_{w_j}$. That is, if job $i$ satisfies $d_i\leq d_{w_j}$ and $a_i\leq v_{w_j}(P)$, then job $i$ departs before time $v_{w_j}(P)$.
%%Hence, at time 
%%\begin{align}
%%\tau=\max_{i:a_i\leq v_{w_j}(P),d_i\leq d_{w_j}} c_{i}(\pi),\nonumber
%%\end{align} $d_i> d_{w_j}$ holds for all jobs in the queue in policy $\pi$. Therefore, the system state of policy $\pi$ satisfies  
%%\begin{align}
%%\sum_{i:d_i\leq d_{w_j}}\xi_i(\tau) =0.\nonumber
%%\end{align}
%%Combining this with Lemma \ref{lemG4_lem3}, we can obtain
%%%Hence, there are $y-1$ unfinished jobs at time $C_{w_1}(\pi)$ such that
%%%Invoking Lemma \ref{lemG4}, we can obtain
%%\begin{align}\label{eq_proof_1_lem3}
%%\sum_{i:d_i\leq d_{w_j}} [\gamma_i(\tau)-\zeta_i(\tau)]\leq 0.
%%\end{align}
%%By the definition of the system state of policy $P$, we have $\gamma_i(t)\geq \zeta_i(t)$ for all $i$ and $t$. This and \eqref{eq_proof_1_lem3} tells us that at time $t$, job $w_j$ in policy $P$ satisfies
%%\begin{align}
%%\gamma_{w_j}(\tau)= \zeta_{w_j}(\tau).\nonumber
%%\end{align}
%%That is, in policy $P$ all tasks of job $w_j$ are either completed or under service at time $\tau$. Hence, $v_{w_j}(P)\leq \tau$, which contradicts with  \eqref{eq_proof_9_lem3}. Therefore, $v_{w_j}(P) \leq \max_{i:a_i\leq v_{w_j}(P),d_i\leq d_{w_j} }c_{i}(\pi)$ and
%%\begin{align}
%%v_{w_j}(P)-d_{w_j} &\leq \max_{i:a_i\leq v_{w_j}(P),d_i\leq d_{w_j} }c_{i}(\pi)-d_{w_j} \nonumber\\
%%& \leq \max_{i:a_i\leq v_{w_j}(P),d_i\leq d_{w_j} }[c_{i}(\pi)-d_{i}]\nonumber\\
%%&\leq \max_{i=1,2,\ldots,n }[c_{i}(\pi)-d_i].\nonumber
%%\end{align}
%%Hence, \eqref{eq_Condition_3_12_lem3} is obtained. This completes the proof.
%%\end{proof}
%%By considering all possible sample paths of these two policies, the stochastic ordering result in Thoerem \ref{lem3} follows.
%%\subsection{Proof of Corollary \ref{coro2}}
%%
%%In the proof of Corollary \ref{coro2}, we will need the following rearrangement inequality  : 
%%\begin{lemma} \cite[Theorem 6.F.14]{Marshall2011}\label{lem_rearrangement}
%%Consider two $n$-vectors $(x_1,\dots,x_n)$ and $(y_1,\ldots,y_n)$. If $x_i> x_j$ and $y_i<y_j$ for some indices $i$ and $j$ where $1\leq i<j\leq n$, then 
%%\begin{align}
%%&(x_1\!-\!y_1,\ldots,x_j\!-\!y_i,\ldots,x_i\!-\!y_j,\ldots,x_n\!-\!y_n)\nonumber\\
%%\prec& (x_1\!-\!y_1,\ldots,x_i\!-\!y_i,\ldots,x_j\!-\!y_j,\ldots,x_n\!-\!y_n).\nonumber
%%\end{align}
%%\end{lemma}
%%\ifreport
%%\begin{proof}[Proof of Corollary \ref{coro2}]
%%\else
%%\begin{proof}[of Corollary \ref{coro2}]
%%\fi
%%As in the proof of Lemma \ref{lem_sample_path_ordering_lem3}, let $w_i$ denote the index of the job associated with $v_{(i)}(P)$. 
%%
%%\emph{Step 1: We first show that  for all $j=1,\ldots,n$}
%%\begin{align}\label{eq_coro2_2}
%%v_{w_j}(P) \leq c_{(j)}(\pi).
%%\end{align}
%%
%%Suppose that $b_j$ tasks have been assigned to the servers in policy $P$ by time $c_{(j)}(\pi)$. Since each job has only one task, $j$ tasks are completed by time $c_{(j)}(\pi)$ in policy $\pi$.
%%Because policy $P$ is more work-efficient than policy $\pi$, it must hold that (i) at least $j$ unassigned task are allocated to the servers during $[0,c_{(j)}(\pi)]$  in policy $P$, i.e., $b_j\geq j$, or (ii) all the remaining tasks are under service at time $c_{(j)}(\pi)$  in policy $P$. Obviously, case (ii) belongs to case (i). Because each job has only one task, it follows that $v_{w_j}(P) \leq c_{(j)}(\pi)$  for all $j=1,\ldots,n$.
%%
%%%We prove Corollary \ref{coro2} by induction. 
%%
%%\emph{Step 2: We show that one of the following two cases is true:
%%\begin{itemize}
%%\item[1.] $v_{w_1}(P)\leq c_{w_1}(\pi)$, and $v_{w_{2}}(P)\leq c_{w_{2}}(\pi)$;
%%%\item[2.] $d_{w_j}\leq d_{w_{j+1}}$, $v_{w_j}(P)\leq c_{w_j}(\pi)$, and $v_{w_{j+1}}(P)\leq c_{w_{j+1}}(\pi)$.
%%\item[2.] $v_{w_1}(P)\leq c_{w_{2}}(\pi)$, $v_{w_{2}}(P)\leq c_{w_{1}}(\pi)$, $d_{w_1}\leq d_{w_{2}}$, and $c_{w_{1}}(\pi)>c_{w_{2}}(\pi)$.
%%\end{itemize}}
%%
%%In the proof of Lemma \ref{lem_sample_path_ordering_lem3}, it was shown that 
%%\begin{align}\label{eq_coro2_1}
%%v_{w_j}(P) \leq \max_{i:a_i\leq v_{w_j}(P),d_i\leq d_{w_j} }c_{i}(\pi).
%%\end{align}
%%
%%We first consider $j=1$. Because job $w_1$ is the first job whose tasks are either completed or under service, no job is completed during $[0,v_{w_1}(P))$ in policy $P$. Because policy $P$ satisfies condition 2 of Thoerem \ref{lem3}, job $w_1$ has the earliest due time among all jobs in the queue at time $v_{w_1}(P)$ in policy $P$. This tells us that if job $i$ satisfies $a_i\leq v_{w_1}(P)$ and $d_i\leq d_{w_1}$, then $i=w_1$. Hence,  \eqref{eq_coro2_1} implies 
%%$v_{w_1}(P) \leq c_{w_1}(\pi)$. 
%%
%%For $j=2$, because job $w_2$ is the second job whose tasks are either completed or under service, only  job $w_1$ can be completed during $[0,v_{w_2}(P))$ in policy $P$. Because policy $P$ satisfies condition 2 of Thoerem \ref{lem3}, job $w_2$ has the earliest due time among all jobs in the queue at time $v_{w_2}(P)$ in policy $P$. This tells us that if job $i$ satisfies $a_i\leq v_{w_2}(P)$ and $d_i\leq d_{w_2}$, then $i=w_1$ or $i=w_2$. 
%%
%%If $d_{w_1}> d_{w_2}$, then \eqref{eq_coro2_1} implies $v_{w_2}(P) \leq c_{w_2}(\pi)$. 
%%
%%If $d_{w_1}\leq d_{w_2}$, then \eqref{eq_coro2_1} implies $v_{w_2}(P) \leq \max[c_{w_1}(\pi), c_{w_2}(\pi)]$. We first consider two sub-cases: If $c_{w_1}(\pi)\leq c_{w_2}(\pi)$, then $v_{w_2}(P) \leq c_{w_2}(\pi)$. 
%%If $c_{w_1}(\pi)> c_{w_2}(\pi)$, by \eqref{eq_coro2_2}, we can obtain $v_{w_1}(P) \leq c_{w_2}(\pi)$ and $v_{w_2}(P)\leq c_{w_1}(\pi)$.
%%
%%By summarizing these cases, the claim of \emph{Step 2} follows. 
%%
%%\emph{Step 3: We show that}
%%\begin{align}\label{eq_coro2_3}
%%\bm{u}(P)-\bm{d}\prec_{\text{w}} \bm{c} (\pi)-\bm{d}.
%%\end{align} 
%%
%%We carry out the following operation: 
%%If case 2 of \emph{Step 2} holds, we interchange the completion times of job $w_1$ and job $w_2$. 
%%%By Lemma \ref{lem_rearrangement}, we can obtain
%%%\begin{align}
%%%&(c_{w_2}(\pi)\!-\!d_{w_1},c_{w_1}(\pi)\!-\!d_{w_2},c_{w_3}(\pi)\!-\!d_{w_3},\ldots,c_{w_n}(\pi)\!-\!d_{w_n})\nonumber\\
%%%\prec& (c_{w_1}(\pi)\!-\!d_{w_1},c_{w_2}(\pi)\!-\!d_{w_2},c_{w_3}(\pi)\!-\!d_{w_3},\ldots,c_{w_n}(\pi)\!-\!d_{w_n}).\nonumber
%%%\end{align}
%%If case 1 of \emph{Step 2} holds, there is no interchange. 
%%Let $\bm{c}^{0} (\pi)=\bm{c}(\pi)$ and $\bm{c}^{1} (\pi)$, respectively, denote the completion time vectors of the $n$ jobs before and after this operation. By Lemma \ref{lem_rearrangement}, we can get 
%%\begin{align}
%%\bm{c}^{1} (\pi)-\bm{d}\prec \bm{c}^{0} (\pi)-\bm{d}.\nonumber
%%\end{align}
%%In addition, it holds that $v_{w_1}(P)\leq c^{1}_{w_1}(\pi)$, and $v_{w_{2}}(P)\leq c^{1}_{w_{2}}(\pi)$.	
%%We repeating this operation $n-1$ times. More specifically, in the $l$-th operation, for each $i=1,\ldots,l$ if $d_{w_i}\leq d_{w_{l+1}}$ and $c^{l-1}_{w_{i}}(\pi)>c^{l-1}_{w_{l+1}}(\pi)$, we interchange job $w_i$ and job $w_{l+1}$. Let $\bm{c}^{l} (\pi)$ denote the completion time vectors of the $n$ jobs after the $l$-th operation.
%%Using \eqref{eq_coro2_2}, \eqref{eq_coro2_1}, and condition 2 of Thoerem \ref{lem3}, we can obtain 
%%\begin{align}
%%&\bm{c}^{n-1} (\pi)-\bm{d} \prec \ldots \prec \bm{c}^{1} (\pi)-\bm{d} \prec \bm{c}^{0} (\pi)-\bm{d}, \nonumber\\
%%&\bm{u}(P)\leq \bm{c}^{n-1}(\pi).\nonumber
%%\end{align}
%%Hence,
%%\begin{align}
%%\bm{u}(P)-\bm{d}\leq \bm{c}^{n-1}(\pi)-\bm{d}\prec \bm{c} (\pi)-\bm{d}.\nonumber
%%\end{align} 
%%By this, \eqref{eq_coro2_3} follows. According to Theorem 3.A.8 of \cite{Marshall2011}, $f(\bm{u}(P)-\bm{d}) \leq f(\bm{c} (\pi)-\bm{d})$ holds for all $f\in\mathcal{D}_{\text{Sch}}$. This completes the proof.
%%\end{proof}

==> v3/appendices_4.tex <==
% !TEX root = ./replication.tex
%\section{Proofs of Thoerem~6 and Corollary 6} \label{app3}
%Similar with the proof of Theorem \ref{thm1}, we can show that policy EDD-NR and policy EDD-NIR are more work-efficient than any policy $\pi\in\Pi$. Then, Theorem \ref{thm3} follows from Thoerem \ref{lem2}, and Corollary \ref{coro_thm3_1} follows from Corollary \ref{coro2}.

%\section{Proofs of Thoerem~7 and Corollary 7} \label{app4}
%Similar with the proof of Theorem \ref{thm2}, we can show that policy EDD-R is more work-efficient than any policy $\pi\in\Pi$. Then, Theorem \ref{thm4} follows from Thoerem \ref{lem2}, and Corollary \ref{coro4_1} follows from Corollary \ref{coro2}.
%
%\section{Proofs of Thoerem~8 and Corollary 8} \label{app5}
%Similar with the proof of Theorem \ref{thm1}, we can show that policy FCFS-NR and policy FCFS-NIR are more work-efficient than any policy $\pi\in\Pi$. Then, Theorem \ref{thm5} follows from Thoerem \ref{lem3}, and Corollary \ref{coro5_1} follows from Corollary \ref{coro3_1}.
%
%\section{Proofs of Thoerem~9 and Corollary 9} \label{app6}
%Similar with the proof of Theorem \ref{thm2}, we can show that policy FCFS-R is more work-efficient than any policy $\pi\in\Pi$. Then, Theorem \ref{thm6} follows from Thoerem \ref{lem3}, and Corollary \ref{coro6_1} follows from Corollary \ref{coro3_1}.

%\end{proof}

%\subsection{Proof of Thoerem~\ref{thm3}} \label{sec_app_3_1} 
%We prove Thoerem~\ref{thm3} by using the sufficient conditions in Thoerem \ref{lem2}. The details are as follows:
%
%{\bf Construction of Policy $P'$:}
%We construct an {infeasible} policy $P'$. \emph{First, in policy $P'$, all servers are busy whenever the queue is not empty.} If the number of tasks is less than $m$, some tasks are replicated over multiple servers. 
%\emph{Second, the task completion times of policy $P'$ are constructed as if there is no task cancellations.} Suppose that at any time $t$, server $l$ has processed a task for $\tau$ seconds, and another copy of this task is completed at time $t$ on another server. In policy $P'$, server $l$ will cancel this task and process a new task. More specifically, in policy $P'$, server $l$ will not process the new task from scratch; instead, it is assumed that the new task assigned to server $l$ has already been processed for $\tau$ seconds by time $t$ (which is infeasible),~and server $l$ will serve the task from this progress point. If two task copies are completed  at the same time on two servers, these two task copies are assumed to be distinct tasks; that is, they are not replicated copy of each other.  \emph{Finally, the completed tasks of policy $P'$ are relabelled such that each completed task is from the job with the earliest due time}. (This relabeling operation might be infeasible, because the tasks from different jobs may be simultaneously processed on parallel servers.) By this, policy $P'$ is constructed.
%
%
%Next, we prove the conditions of Thoerem \ref{lem2} one by one.
%
%\textbf{Condition 1:} \emph{Policy $P'$ is more {work-efficient} than any policy $\pi\in\Pi$}. Condition 1 can be proven by using the same proof arguments in Appendix \ref{sec_app_thm1_1}.
%
%\textbf{Condition 2:} \emph{Each completed task of policy $P'$ belongs to the job with the earliest due time}. Condition 2 directly follows from the construction of policy $P'$.
%
%\textbf{Condition 3:} \emph{It holds that} 
%\begin{align}\label{eq_condition3_thm3}
%[\bm{U}_{}(\text{EDD-NR})|\mathcal{I}] \leq_{\text{st}} [\bm{C}_{}(P')|\mathcal{I}].
%\end{align}
%
%We prove condition 3 by using the \emph{sample-path ordering} technique. First, we define the system states of policies $P'$ and EDD-NR. 
%\begin{definition}\label{def_state_P_thm3}
%The system state of policy $P'$ is specified by a $n$-dimensional vector $\bm{\xi}=(\xi_1,\ldots,\xi_n)$ with non-negative components. At any time, if job $i$ exists in the system, $\xi_i$ is the number of remaining tasks of job $i$; if job $i$ has not arrived at the system or has departed from the system, $\xi_i=0$.
%\end{definition}
%
%\begin{definition}\label{def_state_thm3}
%The system state of policy EDD-NR is specified by a pair of $n$-dimensional vectors $\bm{\gamma}=(\gamma_1,\ldots,\gamma_n)$ and $\bm{\zeta}=(\zeta_1,\ldots,\zeta_n)$ with non-negative components. 
%At any time, if job $i$ exists in the system, then $\gamma_i$ is the number of remaining tasks of job $i$ and $\zeta_i$ out of these $\gamma_i$ tasks are under service on some servers; if job $i$ has not arrived at the system or has departed from the system, then $\gamma_i=\zeta_i=0$.
%Hence, 
%\begin{align}%\label{eq_def_state_thm3}
%\zeta_i  \leq \gamma_i \leq k_{i},~\sum_{i=1}^n \zeta_i \leq m. \nonumber
%\end{align}
%\end{definition}
%
% Let $\{\bm{\xi}(t),t\geq0\}$ be the state process of policy $P'$, and $\{\bm{\gamma}(t),\bm{\zeta}(t),t\geq0\}$ be the state process of EDD-NR, which are assumed to be right-continuous. During the proof of condition 3, we assume that the due times $d_1,\ldots, d_n$ of the $n$ jobs are distinct from each other. This does not lose any generality, because if $d_i=d_j$ for two jobs $i$ and $j$, condition 3 can be proven by taking the limit $d_i\rightarrow d_j$. 
%
%The sample-path ordering result is stated in the following lemma:
% 
% 
%\begin{lemma}\label{lemG4_thm3}
%Suppose that $\bm{\xi}(0^-)=\bm{\gamma}(0^-)=\bm{\zeta}(0^-)=\bm{0}$ and the job parameters $\mathcal{I}$ are given. For any sample path of policy $P'$, there exists a sample path of EDD-NR with the same probability density such that
%\begin{eqnarray}\label{eq_lemG4_thm3}
%\sum_{i:d_i\leq\tau} [\gamma_i(t) - \zeta_i(t)]\leq \sum_{i:d_i\leq\tau} \xi_i(t), 
%\end{eqnarray}
%holds for all $t,\tau\geq0$.
%\end{lemma}
%
%The following two lemmas are needed to prove Lemma \ref{lemG4_thm3}:
%
%
%\begin{lemma}\label{lem_non_prmp1_thm3}
%Suppose that, under policy EDD-NR, $\{\bm{\gamma}',\bm{\zeta}'\}$ is obtained by completing a task on one server in the system whose state is $\{\bm{\gamma},\bm{\zeta}\}$. Further, suppose that, under policy $P'$, $\bm{\xi}'$ is obtained by completing a task on one server in the system whose state is $\bm{\xi}$. If
%\begin{eqnarray}
%\sum_{i:d_i\leq\tau} [\gamma_i - \zeta_i]\leq \sum_{i:d_i\leq\tau} \xi_i, ~\forall~\tau\in[0,\infty),\nonumber
%\end{eqnarray}
%then
%\begin{eqnarray}\label{eq_non_prmp_40_thm3}
%\sum_{i:d_i\leq\tau} [\gamma_i'- \zeta_i']\leq \sum_{i:d_i\leq\tau} \xi_i', ~\forall~\tau\in[0,\infty).\end{eqnarray}
%\end{lemma}
%
%\begin{proof}
%If $\sum_{i:d_i\leq\tau} [\gamma_i' - \zeta_i']=0$, then the inequality \eqref{eq_non_prmp_40_thm3} follows naturally. 
%If $\sum_{i:d_i\leq\tau} [\gamma_i' - \zeta_i']>0$, then there exist some tasks that have not been assigned to any server. 
%In EDD-NR, a server that has just completed a task will be allocated to an unassigned task from the job with the earliest due time. Hence,
%$\sum_{i:d_i\leq\tau} [\gamma_i' - \zeta_i']=\sum_{i:d_i\leq\tau} [\gamma_i - \zeta_i] - 1 \leq \sum_{i:d_i\leq\tau} \xi_i -1 \leq \sum_{i:d_i\leq\tau} \xi_i'$.
%\end{proof}
%
%
%\begin{lemma}\label{lem_non_prmp2_thm3}
%Suppose that, under policy EDD-NR, $\{\bm{\gamma}',\bm{\zeta}'\}$ is obtained by adding a job with $b$ tasks and due time $d$ to the system whose state is $\{\bm{\gamma},\bm{\zeta}\}$. Further, suppose that, under policy $P'$, $\bm{\xi}'$ is obtained by adding a job with $b$ tasks and due time $d$ to the system whose state is $\bm{\xi}$.
%If
%\begin{eqnarray}
%\sum_{i:d_i\leq\tau} [\gamma_i- \zeta_i]\leq \sum_{i:d_i\leq\tau} \xi_i, ~\forall~\tau\in[0,\infty),\nonumber
%\end{eqnarray}
%then
%\begin{eqnarray}
%\sum_{i:d_i\leq\tau} [\gamma_i' - \zeta_i']\leq \sum_{i:d_i\leq\tau} \xi_i', ~\forall~\tau\in[0,\infty).\nonumber\end{eqnarray}
%\end{lemma}
%
%\begin{proof}
%If $d\leq\tau$, then
%$\sum_{i:d_i\leq\tau} [\gamma_i' - \zeta_i']\leq \sum_{i:d_i\leq\tau} [\gamma_i - \zeta_i] + b\leq \sum_{i:d_i\leq\tau} \xi_i+b \leq \sum_{i:d_i\leq\tau} \xi_i'$.
%
%If $d>\tau$, then
%$\sum_{i:d_i\leq\tau} [\gamma_i' - \zeta_i']\leq \sum_{i:d_i\leq\tau} [\gamma_i - \zeta_i] \leq \sum_{i:d_i\leq\tau} \xi_i \leq \sum_{i:d_i\leq\tau} \xi_i'$.
%\end{proof}
%
%Now we are ready to prove Lemma \ref{lemG4_thm3}.
%\ifreport
%\begin{proof}[Proof of Lemma \ref{lemG4_thm3}]
%\else
%\begin{proof}[of Lemma \ref{lemG4_thm3}]
%\fi
%Consider any busy period $[\tau,\nu)$ of policy $P'$. Then, in policy $P'$, all servers are busy during $[\tau,\nu)$, and are idle at time $\tau^-$ and time $\nu$. We prove \eqref{eq_lemG4_thm3} for $t\in[\tau,\nu)$ by considering two cases:
%
%\emph{Case 1: At time $t=\tau^-$, policy EDD-NR has $m$ tasks and the service of these tasks has just started.} Consider the system states of both policies at time $\tau^-$. The system state of policy EDD-NR satisfies 
%\begin{align}\label{proof_lemG4_1_thm3}
%\sum_{i=1}^n \gamma_i(\tau^-)= m, ~\bm{\gamma}(\tau^-)=\bm{\zeta}(\tau^-).
%\end{align}
%In policy $P'$, there is no task in the system at time $\tau^-$ such that 
%\begin{align}\label{proof_lemG4_5_thm3}
%\bm{\xi}(\tau^-)=\bm{0}. 
%\end{align}
%Consider the evolutions of both policies during $[\tau,\nu)$. 
%In policy $P'$, all servers are busy if there is at least one task. On the other hand, in policy EDD-NR, there is no task replication and all servers are busy if there are no less than $m$ tasks. 
%By \eqref{proof_lemG4_1_thm3} and \eqref{proof_lemG4_5_thm3}, it holds that for $t=\tau$
%\begin{align}\label{proof_lemG4_4_thm3}
%\sum_{i=1}^n \gamma_i(t)= \sum_{i=1}^n\xi_i(t) +m\geq m+1.
%\end{align}
%Therefore, the servers are all busy in policies $P'$ and policy EDD-NR at time $\tau$. By induction over time, we can show that for any sample path of policy $P'$, there is a sample path of policy EDD-NR with the same probability density such that \eqref{proof_lemG4_4_thm3} holds for all $t\in[\tau,\nu)$ and the task arrival times and task completion times of the two policies are exactly the same  during $[\tau,\nu)$. Using Lemma \ref{lem_non_prmp1_thm3}, Lemma \ref{lem_non_prmp2_thm3}, and the initial states at time $\tau^-$, we can prove that \eqref{eq_lemG4_thm3} holds for all $t\in[\tau,\nu)$ on these two sample paths.
%
%\emph{Case 2: At time $t=\tau^-$, policy EDD-NR has less than $m$ tasks or the service of these tasks started before time $\tau^-$}. In both \emph{Case 1} and \emph{Case 2}, the sample path evolutions of policy $P'$ are the same. On the other hand, in policy EDD-NR, the tasks are completed earlier in \emph{Case 2} than in \emph{Case 1}. Therefore, \eqref{eq_lemG4_thm3}  also holds in \emph{Case 2} for $t\in[\tau,\nu)$.
%
%%Note that the case that policy EDD-NR has more than $m$ tasks at time $\tau^-$ will not happen. This will be clear 
%Let $[\tau_1,\nu_1)$ be the next busy period of policy $P'$ with $\nu<\tau_1$. Then, $[\nu,\tau_1)$ is an idle period of policy $P'$. We now prove \eqref{eq_lemG4_thm3} during the idle period $[\nu,\tau_1)$. 
%Because all servers are idle during $[\nu,\tau_1)$ in policy $P'$, it follows that 
%\begin{align}\label{proof_lemG4_2_thm3}
%\bm{\xi}(t)=\bm{0},~t\in[\nu,\tau_1).
%\end{align}
%Hence, there is no task arrival during $[\nu,\tau_1)$; otherwise, \eqref{proof_lemG4_2_thm3} cannot be true.
%On the other hand, at time $\nu$ there are no more than $m$ tasks in policy EDD-NR such that 
%\begin{align}
%\bm{\gamma}(\nu)=\bm{\zeta}(\nu).\nonumber
%\end{align}
%Because there is no task arrival during $[\nu,\tau_1)$, policy EDD-NR satisfies
%\begin{align}\label{proof_lemG4_3_thm3}
%\bm{\gamma}(t)=\bm{\zeta}(t),~t\in[\nu,\tau_1).
%\end{align}
%By \eqref{proof_lemG4_2_thm3} and \eqref{proof_lemG4_3_thm3}, \eqref{eq_lemG4_thm3} holds during $[\nu,\tau_1)$.
%Further, from \eqref{proof_lemG4_3_thm3}, we can obtain
%\begin{align}
%\sum_{i=1}^n \gamma_i(\tau_1^-)=\sum_{i=1}^n \zeta_i(\tau_1^-)\leq m,
%\end{align}
%such that there are no more than $m$ tasks at time $t=\tau_1^-$ in policy EDD-NR. Hence, either \emph{Case 1} or \emph{Case 2} is satisfied at time $t=\tau_1^-$. Then, we can use the above arguments to prove that  \eqref{eq_lemG4_thm3} holds during the next busy period $[\tau_1,\nu_1)$ of policy $P'$.
%
%
%Finally, by taking an induction over the busy and idle periods of policy $P'$,  Lemma \ref{lemG4_thm3} is proven.
%\end{proof}
%
%
%\ifreport
%\begin{proof}[Proof of Condition 3]
%\else
%\begin{proof}[of Condition 3]
%\fi
%%Let the evolution of the system state under some scheduling policy be on a space $(\Omega,\mathcal{F},P)$. Each $\omega\in\Omega$ corresponds to a sample path of policy $P'$ and a sample path of policy EDD-NR. The job arrival parameters $\mathcal{I}$ is fixed for all $\omega\in\Omega$. 
%%Let $(C_{w_1}(P'),\ldots,c_{N:N}(P'))$ be a permute of the job completion time sequence $(c_{1}(P'),\ldots,c_{N}(P'))$ in the increasing order, such that $c_{i:N}(P')\leq c_{i+1:N}(P')$. 
%
%%Pick any $\omega\in\Omega$ and consider the first job completion time $C_{w_1}(P')$ of policy $P'$. Suppose that there are $y$ job arrivals during $[0,C_{w_1}(P'))$. 
%
%We  prove Condition 3 by induction. Consider the sample paths of policy $P'$ and policy EDD-NR satisfying Lemma \ref{lemG4_thm3}. Suppose that job $w_i$ is the $i$-th completed job in the sample path of policy $P'$. We first show that 
%\begin{align}\label{eq_Condition_3_1_thm3}
%U_{w_1}(\text{EDD-NR}) \leq C_{w_1}(P').
%\end{align}
%
%According to the construction of policy $P'$, at time $t=C_{w_1}(P')$, the system state of policy $P'$ must satisfy 
%\begin{align}\label{eq_proof_0_thm3}
%\sum_{i:d_i\leq d_{w_1}}\xi_i(C_{w_1}(P'))=0.
%\end{align}
%That is, when job $w_1$ leaves the system in policy $P'$, no job with a due time earlier than $d_{w_1}$ can exist in the system.
%This and Lemma \ref{lemG4_thm3} imply
%%Hence, there are $y-1$ unfinished jobs at time $C_{w_1}(P')$ such that
%%Invoking Lemma \ref{lemG4}, we can obtain
%\begin{align}\label{eq_proof_1_thm3}
%\sum_{i:d_i\leq d_{w_1}} \gamma_i(C_{w_1}(P'))\leq \sum_{i:d_i\leq d_{w_1}}  \zeta_i(C_{w_1}(P')).
%\end{align}
%
%
%
%By \emph{Definition \ref{def_state_thm3}}, we have $\gamma_i(t)\geq \zeta_i(t)$. Hence, the system state of policy EDD-NR satisfies 
%\begin{align}\label{eq_proof_2_thm3}
%\!\!\gamma_i(C_{w_1}(P'))= \zeta_i(C_{w_1}(P')),
%\end{align}
%for all job $i$ with $d_i\leq d_{w_1}$. In particular, job $w_1$ satisfy
%\begin{align}\label{eq_proof_3_thm3}
%\gamma_{w_1}(C_{w_1}(P'))= \zeta_{w_1}(C_{w_1}(P')).
%\end{align}
%This tells us that in EDD-NR, all tasks of job $w_1$ are either completed or under service at time $C_{w_1}(P')$. Hence, \eqref{eq_Condition_3_1_thm3} is proven.
%%\begin{align}%\label{eq_proof_9}
%%U_{w_1}(\text{EDD-NR}) \leq C_{w_1}(P'),\nonumber
%%\end{align}
%%which implies \eqref{eq_Condition_3_1}.
%
%Next, we prove the induction step. Suppose that 
%\begin{align}
%U_{w_i}(\text{EDD-NR}) \leq C_{w_i}(P'),~i=1,\ldots,j,\nonumber
%\end{align}
%we will show that \begin{align}\label{eq_proof_9_thm3}
%U_{w_{j+1}}(\text{EDD-NR}) \leq C_{w_{j+1}}(P').
%\end{align}
%At time $t=C_{w_{j+1}}(P')$, the system state of policy $P'$ satisfies 
%\begin{align}
%\sum_{i: d_i\leq d_{w_{j+1}}}\xi_i(C_{w_{j+1}}(P'))=0.\nonumber
%\end{align}
%That is, when job $w_{j+1}$ leaves the system in policy $P'$, no job with a due time earlier than $d_{w_{j+1}}$ can exist in the system.
%Then, by following the arguments of \eqref{eq_proof_1_thm3}-\eqref{eq_proof_3_thm3}, we can obtain that job $w_{j+1}$ satisfies
%\begin{align}\label{eq_proof_4_thm3}
%\gamma_{w_{j+1}}(C_{w_{j+1}}(P'))= \zeta_{w_{j+1}}(C_{w_{j+1}}(P')).
%\end{align}
%Then, \eqref{eq_proof_4_thm3} tells us that in EDD-NR, all tasks of job $w_{j+1}$ are either completed or under service at time $t=C_{w_{j+1}}(P')$. Hence, \eqref{eq_proof_9_thm3} is proven.
%
%By induction, we can obtain
%\begin{align}\label{eq_proof_10_thm3}
%U_{i}(\text{EDD-NR}) \leq C_{i}(P'),~i=1,\ldots,n.
%\end{align}
%Consider all possible sample paths of policy $P'$ and policy EDD-NR, the stochastic ordering result in \eqref{eq_condition3_thm3} follows.
%\end{proof}
%After establishing conditions 1-3 of Thoerem \ref{lem2} for policy EDD-NR,  we can prove \eqref{eq_delaygap1_thm3}. 
%
%Similar proof procedure can be used to prove \eqref{eq_delaygap2_thm3}. By this, Theorem \ref{thm3} is proven.
%\subsection{Proof of Corollary~\ref{coro_thm3_1}} \label{sec_app_3_2} 
%Because conditions 1-3 of Thoerem \ref{lem2} have been established in Appendix \ref{sec_app_3_1},  Corollary~\ref{coro_thm3_1} directly follows from Corollary \ref{coro2}.

==> v3/appendices_5.tex <==
% !TEX root = ./replication.tex

\section{Proofs of Thoerem~4 and Corollary 6} \label{app4}
\subsection{Proof of Thoerem~\ref{thm4}} \label{sec_app_4_1}
We prove Thoerem~\ref{thm4} by using Lemma \ref{lem2}, where the policy space $\Pi$ is replaced by $\Pi_{\text{non-prmp}}$ because preemption is not allowed. The proof steps are as follows:

{\bf Construction of Policy $P'$:}
We construct an {infeasible} policy $P'$. Similar with policy EDD-R, when all servers are idle in policy $P'$, a task from the job with the earliest due time is replicated on all $m$ servers. When a copy of this task is completed, the remaining $m-1$ replicated copies of this task are cancelled. The difference between policy EDD-R and policy $P'$ is that \emph{the completed tasks of policy $P'$ are relabelled such that each completed task is from the job with the earliest due time}. (This relabeling operation might be infeasible in the following scenario: If a job with an earlier due time arrives, the servers cannot be reassigned to this incoming job because preemption is not allowed. However, the next completed task is relabelled to be from this incoming job which has the earliest due time.) By this, policy $P'$ is constructed.

Next, we prove the conditions of Lemma \ref{lem2} one by one.

\textbf{Condition 1:} \emph{Policy $P'$ is more {work-efficient} than any policy $\pi\in\Pi_{\text{non-prmp}}$}. Condition 1 can be proven by using the same proof arguments in Appendix \ref{sec_app_thm2_1}.

\textbf{Condition 2:} \emph{Each completed task of policy $P'$ belongs to the job with the earliest due time}. Condition 2 directly follows from the construction of policy $P'$.

\textbf{Condition 3:} \emph{It holds that} 
\begin{align}\label{eq_condition3_thm4}
[\bm{U}_{}(\text{EDD-R})|\mathcal{I}] \leq_{\text{st}} [\bm{C}_{}(P')|\mathcal{I}].
\end{align}

We prove condition 3 by using the \emph{sample-path ordering} technique. The system state $\bm{\xi}$ of policy $P'$ is the same as that in \emph{Definition \ref{def_state_P_thm3}}. The system state $(\bm{\gamma},\bm{\zeta})$ of policy EDD-R is the same as that in \emph{Definition \ref{def_state_thm3}}. 
In policy EDD-R, all servers are simultaneously assigned to process $m$ replicated copies of the same task. Hence, $\bm{\zeta}$ satisfies
\begin{align}
\zeta_i\in\{0,1\},~\sum_{i=1}^n \zeta_i\leq1.
\end{align}
We can prove that Lemmas \ref{lemG4_thm3}-\ref{lem_non_prmp2_thm3} hold for policy EDD-R. 
Using Lemma \ref{lemG4_thm3}, condition 3 can be proven by using the same proof arguments in Appendix \ref{sec_app_3_1}, where policy EDD-NR should be replaced by policy EDD-R.

After establishing conditions 1-3 of Lemma \ref{lem2} for policy EDD-R,  we can use Lemma \ref{lem2} to prove Theorem \ref{thm4}. This completes the proof.

\subsection{Proof of Corollary~\ref{coro4_2}}  
If $d_1\leq\ldots\leq d_n$, then each completed task of policy EDD-R belongs to the job with the earliest due time. Therefore, policy EDD-R is identical with policy $P'$ constructed in Appendix \ref{sec_app_4_1}. Then, Corollary \ref{coro4_2} follows from Lemma \ref{lem2}. 

\subsection{Proof of Corollary~\ref{coro4_1}} \label{sec_app_4_2} 
Because conditions 1-3 of Lemma \ref{lem2} have been established in Appendix \ref{sec_app_4_1},  Corollary~\ref{coro4_1} directly follows from Corollary \ref{coro2}.

==> v3/appendices_6.tex <==
% !TEX root = ./replication.tex

\section{Proof of Thoerem~5} \label{app5}

\subsection{Proof of \eqref{eq_delaygap1_thm5} in Thoerem~5}
We prove \eqref{eq_delaygap1_thm5} in Thoerem~\ref{thm5} by using Lemma \ref{lem3}. In particular, we will use the \emph{sample-path ordering} technique to prove condition \eqref{eq_lem3_1} of Lemma \ref{lem3}.
We first define the system states of policy PL-NR and any policy $\pi\in\Pi_{PL}$, where $PL=(p_1,\ldots,p_n)$ denote a static priority list.

\begin{definition}\label{def_state_P_thm5}
The system state of policy $\pi\in\Pi_{PL}$ is specified by a pair of $n$-dimensional vectors $\bm{\xi}=(\xi_1,\ldots,\xi_n)$ and $\bm{\kappa}=(\kappa_1,\ldots,\kappa_n)$ with non-negative components. At any time, if job $i$ exists in the system, $\xi_i$ is the number of remaining tasks of job $i$ and $\kappa_i$ out of these $\xi_i$ tasks are under service on some servers; if job $i$ has not arrived at the system or has departed from the system, $\xi_i=\kappa_i=0$. Hence, 
\begin{align}%\label{eq_def_state_P_thm5}
\kappa_i  \leq \xi_i \leq k_{i},~\sum_{i=1}^n \kappa_i \leq m. \nonumber
\end{align}
\end{definition}

\begin{definition}\label{def_state_thm5}
The system state of policy PL-NR is specified by a pair of $n$-dimensional vectors $\bm{\gamma}=(\gamma_1,\ldots,\gamma_n)$ and $\bm{\zeta}=(\zeta_1,\ldots,\zeta_n)$ with non-negative components. 
At any time, if job $i$ exists in the system, then $\gamma_i$ is the number of remaining tasks of job $i$ and $\zeta_i$ out of these $\gamma_i$ tasks are under service on some servers; if job $i$ has not arrived at the system or has departed from the system, then $\gamma_i=\zeta_i=0$.
Hence, 
\begin{align}%\label{eq_def_state_thm5}
\zeta_i  \leq \gamma_i \leq k_{i},~\sum_{i=1}^n \zeta_i \leq m. \nonumber
\end{align}
\end{definition}

Let $\{\bm{\xi}(t),\bm{\kappa}(t),t\geq0\}$ be the state process of policy $\pi$, and $\{\bm{\gamma}(t),\bm{\zeta}(t),t\geq0\}$ be the state process of PL-NR, which are assumed to be right-continuous. 
The sample-path ordering result is stated in the following lemma:
 
 
\begin{lemma}\label{lemG4_thm5}
Suppose that $\bm{\xi}(0^-)=\bm{\kappa}(0^-)=\bm{\gamma}(0^-)=\bm{\zeta}(0^-)=\bm{0}$ and the job parameters $\mathcal{I}$ are given. For any sample path of policy PL-NR, there exists a sample path of policy $\pi$ with the same probability density such that
\begin{eqnarray}\label{eq_lemG4_thm5}
\sum_{i:p_i\geq p} [\gamma_i(t) - \zeta_i(t)]\leq \sum_{i:p_i\geq p} [\xi_i(t)-\kappa_i(t)], 
\end{eqnarray}
holds for all $t\geq0$ and $p = 1,2,\ldots,n$.
\end{lemma}

The following two lemmas are needed to prove Lemma \ref{lemG4_thm5}:


\begin{lemma}\label{lem_non_prmp1_thm5}
Suppose that, under policy PL-NR, $\{\bm{\gamma}',\bm{\zeta}'\}$ is obtained by completing a task on one server in the system whose state is $\{\bm{\gamma},\bm{\zeta}\}$. Further, suppose that, under policy $\pi$, $\{\bm{\xi}',\bm{\kappa}'\}$ is obtained by completing a task on one server in the system whose state is $\{\bm{\xi},\bm{\kappa}\}$. If
\begin{eqnarray}
\sum_{i:p_i\geq p} [\gamma_i - \zeta_i]\leq \sum_{i:p_i\geq p} [\xi_i-\kappa_i], ~\forall~p = 1,2,\ldots,n,\nonumber
\end{eqnarray}
then
\begin{eqnarray}\label{eq_non_prmp_40_thm5}
\sum_{i:p_i\geq p} [\gamma_i'- \zeta_i']\leq \sum_{i:p_i\geq p} [\xi_i'-\kappa_i'], ~\forall~p = 1,2,\ldots,n.\end{eqnarray}
\end{lemma}

\begin{proof}
If $\sum_{i:p_i\geq p} [\gamma_i' - \zeta_i']=0$, then the inequality \eqref{eq_non_prmp_40_thm5} follows naturally. 
If $\sum_{i:p_i\geq p} [\gamma_i' - \zeta_i']>0$, then there exist some tasks that have not been assigned to any server. 
In both policy PL-NR and policy $\pi$, a server that has just completed a task will be allocated to process an unassigned task from the job with the highest priority among all jobs in the queue. Hence,
$\sum_{i:p_i\geq p} [\gamma_i' - \zeta_i']=\sum_{i:p_i\geq p} [\gamma_i - \zeta_i] - 1 \leq \sum_{i:p_i\geq p} [\xi_i-\kappa_i] -1 \leq \sum_{i:p_i\geq p} [\xi_i'-\kappa_i']$.
\end{proof}


\begin{lemma}\label{lem_non_prmp2_thm5}
Suppose that, under policy PL-NR, $\{\bm{\gamma}',\bm{\zeta}'\}$ is obtained by adding a job with $b$ tasks and priority $d$ to the system whose state is $\{\bm{\gamma},\bm{\zeta}\}$. Further, suppose that, under policy $\pi$, $\{\bm{\xi}',\bm{\kappa}'\}$ is obtained by adding a job with $b$ tasks and priority $d$ to the system whose state is $\{\bm{\xi},\bm{\kappa}\}$.
If
\begin{eqnarray}
\sum_{i:p_i\geq p} [\gamma_i- \zeta_i]\leq \sum_{i:p_i\geq p} [\xi_i-\kappa_i], ~\forall~p = 1,2,\ldots,n,\nonumber
\end{eqnarray}
then
\begin{eqnarray}
\sum_{i:p_i\geq p} [\gamma_i' - \zeta_i']\leq \sum_{i:p_i\geq p} [\xi_i'-\kappa_i'], ~\forall~p = 1,2,\ldots,n.\nonumber\end{eqnarray}
\end{lemma}

\begin{proof}
If $d\geq p$, then
$\sum_{i:p_i\geq p} [\gamma_i' - \zeta_i']\leq \sum_{i:p_i\geq p} [\gamma_i - \zeta_i] + b\leq \sum_{i:p_i\geq p} [\xi_i-\kappa_i]+b \leq \sum_{i:p_i\geq p} [\xi_i'-\kappa_i']$.

If $d<p$, then
$\sum_{i:p_i\geq p} [\gamma_i' - \zeta_i']\leq \sum_{i:p_i\geq p} [\gamma_i - \zeta_i] \leq \sum_{i:p_i\geq p} [\xi_i-\kappa_i] \leq \sum_{i:p_i\geq p} [\xi_i'-\kappa_i']$.
\end{proof}

Now we are ready to prove Lemma \ref{lemG4_thm5}.
\ifreport
\begin{proof}[Proof of Lemma \ref{lemG4_thm5}]
\else
\begin{proof}[of Lemma \ref{lemG4_thm5}]
\fi
Consider any period $[\tau,\nu)$ of policy PL-NR, during which there are at least $m$ tasks such that all $m$ servers are busy. We prove \eqref{eq_lemG4_thm5} for $t\in[\tau,\nu)$ by considering two cases:

\emph{Case 1: At time $t=\tau$, policy PL-NR has $m$ tasks and the service of these tasks has just started.} Consider the system states of both policies at time $\tau$. The system state of policy PL-NR satisfies 
\begin{align}\label{proof_lemG4_1_thm5}
\sum_{i=1}^n \gamma_i(\tau)= m, ~\bm{\gamma}(\tau)=\bm{\zeta}(\tau).
\end{align}
In policy $P'$, there is no task in the system at time $\tau^-$ such that 
\begin{align}\label{proof_lemG4_5_thm5}
\bm{\xi}(\tau^-)=\bm{0}. 
\end{align}
Consider the evolutions of both policies during $[\tau,\nu)$. 
In policy $P'$, all servers are busy if there is at least one task. On the other hand, in policy EDD-NR, there is no task replication and all servers are busy if there are no less than $m$ tasks. 
By \eqref{proof_lemG4_1_thm5} and \eqref{proof_lemG4_5_thm5}, it holds that for $t=\tau$
\begin{align}\label{proof_lemG4_4_thm5}
\sum_{i=1}^n \gamma_i(t)= \sum_{i=1}^n\xi_i(t) +m\geq m+1.
\end{align}
Therefore, the servers are all busy in policies $P'$ and policy EDD-NR at time $\tau$. By induction over time, we can show that for any sample path of policy $P'$, there is a sample path of policy EDD-NR with the same probability density such that \eqref{proof_lemG4_4_thm5} holds for all $t\in[\tau,\nu)$ and the task arrival times and task completion times of the two policies are exactly the same  during $[\tau,\nu)$. Using Lemma \ref{lem_non_prmp1_thm5}, Lemma \ref{lem_non_prmp2_thm5}, and the initial states at time $\tau^-$, we can prove that \eqref{eq_lemG4_thm5} holds for all $t\in[\tau,\nu)$ on these two sample paths.

\emph{Case 2: At time $t=\tau^-$, policy EDD-NR has less than $m$ tasks or the service of these tasks started before time $\tau^-$}. In both \emph{Case 1} and \emph{Case 2}, the sample path evolutions of policy $P'$ are the same. On the other hand, in policy EDD-NR, the tasks are completed earlier in \emph{Case 2} than in \emph{Case 1}. Therefore, \eqref{eq_lemG4_thm5}  also holds in \emph{Case 2} for $t\in[\tau,\nu)$.

%Note that the case that policy EDD-NR has more than $m$ tasks at time $\tau^-$ will not happen. This will be clear 
Let $[\tau_1,\nu_1)$ be the next busy period of policy $P'$ with $\nu<\tau_1$. Then, $[\nu,\tau_1)$ is an idle period of policy $P'$. We now prove \eqref{eq_lemG4_thm5} during the idle period $[\nu,\tau_1)$. 
Because all servers are idle during $[\nu,\tau_1)$ in policy $P'$, it follows that 
\begin{align}\label{proof_lemG4_2_thm5}
\bm{\xi}(t)=\bm{0},~t\in[\nu,\tau_1).
\end{align}
Hence, there is no task arrival during $[\nu,\tau_1)$; otherwise, \eqref{proof_lemG4_2_thm5} cannot be true.
On the other hand, at time $\nu$ there are no more than $m$ tasks in policy EDD-NR such that 
\begin{align}
\bm{\gamma}(\nu)=\bm{\zeta}(\nu).\nonumber
\end{align}
Because there is no task arrival during $[\nu,\tau_1)$, policy EDD-NR satisfies
\begin{align}\label{proof_lemG4_3_thm5}
\bm{\gamma}(t)=\bm{\zeta}(t),~t\in[\nu,\tau_1).
\end{align}
By \eqref{proof_lemG4_2_thm5} and \eqref{proof_lemG4_3_thm5}, \eqref{eq_lemG4_thm5} holds during $[\nu,\tau_1)$.
Further, from \eqref{proof_lemG4_3_thm5}, we can obtain
\begin{align}
\sum_{i=1}^n \gamma_i(\tau_1^-)=\sum_{i=1}^n \zeta_i(\tau_1^-)\leq m,
\end{align}
such that there are no more than $m$ tasks at time $t=\tau_1^-$ in policy EDD-NR. Hence, either \emph{Case 1} or \emph{Case 2} is satisfied at time $t=\tau_1^-$. Then, we can use the above arguments to prove that  \eqref{eq_lemG4_thm5} holds during the next busy period $[\tau_1,\nu_1)$ of policy $P'$.


Finally, by taking an induction over the busy and idle periods of policy $P'$,  Lemma \ref{lemG4_thm5} is proven.
\end{proof}



After establishing conditions 1-3 of Lemma \ref{lem2} for policy EDD-R,  we can use Lemma \ref{lem2} to prove Theorem \ref{thm4}. This completes the proof.

\subsection{Proof of Corollary~\ref{coro4_2}}  
If $d_1\leq\ldots\leq d_n$, then each completed task of policy EDD-R belongs to the job with the earliest due time. Therefore, policy EDD-R is identical with policy $\pi$ constructed in Appendix \ref{sec_app_4_1}. Then, Corollary \ref{coro4_2} follows from Lemma \ref{lem2}. 

\subsection{Proof of Corollary~\ref{coro4_1}} \label{sec_app_4_2} 
Because conditions 1-3 of Lemma \ref{lem2} have been established in Appendix \ref{sec_app_4_1},  Corollary~\ref{coro4_1} directly follows from Corollary \ref{coro2}.

==> v3/appendices_Theorem1.tex <==
% !TEX root = ./replication.tex


\begin{figure}
\centering
\includegraphics[width=0.45\textwidth]{Figures/theorem_proof_1_2} \caption{Illustration of the weak work-efficiency ordering between policy $\pi_1$ and policy $P_1$.}
\label{fig_theorem_proof_1}
\end{figure}
\section{Proof of Lemma \ref{lem_coupling}}\label{app1}
We use coupling to prove Lemma \ref{lem_coupling}: We construct two policies $P_1$ and $\pi_1$ such that policy $P_1$
satisfies the same queueing discipline with policy $P$, and policy $\pi_1$ satisfies the same queueing discipline with policy $\pi$. Hence, policy $P_1$ is work-conserving.
%It is known that the job parameters $\mathcal{I}$ and random task service times are \emph{mutually independent} and do not change according to the scheduling policy. Therefore, 
The task and job completion times of policy $P_1$ (policy $\pi_1$) have the same distribution as those of policy $P$ (policy $\pi$). Because the state process is determined by the job parameters $\mathcal{I}$ and the task/job completion events, the state process $\{\bm{\xi}_{P_1}(t),\bm{\gamma}_{P_1}(t),t\in[0,\infty)\}$ of policy $P_1$ has the same distribution as the state process $\{\bm{\xi}_{P}(t),\bm{\gamma}_{P}(t),t\in[0,\infty)\}$ of policy $P$, and the state process $\{\bm{\xi}_{\pi_1}(t),\bm{\gamma}_{\pi_1}(t),t\in[0,\infty)\}$ of policy $\pi_1$ has the same distribution as the state process $\{\bm{\xi}_{\pi}(t),\bm{\gamma}_{\pi}(t),t\in[0,\infty)\}$  of policy $\pi$.
 
Next, we show that policy $P_1$ and policy $\pi_1$ can be constructed such that policy $P_1$ is weakly more work-efficient than policy $\pi_1$ with probability one. Let us consider any task $j$ executed in policy $\pi_1$. Suppose that in policy $\pi_1$ task $j$ starts service in server $l$ at time $\tau$ and completes service at time $\nu$, and the queue is not empty during $[\tau,\nu]$ in policy $P_1$. Because policy $P_1$ is work-conserving, all servers are busy in policy $P_1$ during $[\tau,\nu]$. In particular, server $l$ is busy in policy $P_1$ during $[\tau,\nu]$. Suppose that  in policy $P_1$, server $l$ has spent a time duration $\chi$ ($\chi\geq0$) on executing a task $h$ before time $\tau$. Let $R_{l,P_1}$ denote the remaining service time of server $l$ for executing task $h$ after time $\tau$ in policy $P_1$. Let $X_{l,\pi_1}=\nu-\tau$ denote the service time of task $j$ in policy $\pi_1$ and $X_{l,P_1}=\chi+R_{l,P_1}$ denote the service time of task $h$ in policy $P_1$. 
Then, the complementary CDF of $R_{l,P_1}$  is given by
\begin{align}
\Pr[R_{l,P_1}>s] = \Pr[X_{l,P_1}-\chi>s|X_{l,P_1}> \chi ].\nonumber
\end{align}
Because the task service times are NBU, we can obtain that for all $s,\chi\geq 0$ 
\begin{align}
\Pr[X_{l,P_1}-\chi>s|X_{l,P_1}> \chi ] =\Pr[X_{l,\pi_1}-\chi>s|X_{l,\pi_1}> \chi ] \leq \Pr[X_{l,\pi_1}>s],\nonumber
\end{align}
and hence $R_{l,P_1} \leq_{\text{st}} X_{l,\pi_1}$.
By Theorem 1.A.1 of \cite{StochasticOrderBook} (i.e., a constructive definition of stochastic ordering), the random variables $R_{l,P_1}$ and $X_{l,\pi_1}$ can be constructed such that $R_{l,P_1} \leq X_{l,\pi_1}$ with probability one. That is, in policy $P_1$ server $l$ completes executing task $h$ at time $t=\tau + R_{l,P_1}$, which is earlier than time $\nu = \tau + X_{l,\pi_1}$ with probability one. Because in policy $P_1$ server $l$ is kept busy during $[\tau,\nu]$, a new task, say task $j'$, will start execution on server $l$ at time $t\in [\tau,\nu]$ with probability one. 

In the above coupling arguments, conditioned on every possible realization of policy $P_1$ and policy $\pi_1$ before the service of task $j$ starts, we can construct the service of task $j$ in policy $\pi_1$ and the service of the corresponding task $j'$ in policy $P_1$ such that the requirement of weak work-efficiency ordering is satisfied for this pair of tasks. Next, following the proof of \cite[Theorem 6.B.3]{StochasticOrderBook}, one can continue this procedure to progressively construct the service of all tasks in policy $\pi_1$ and policy $P_1$. By this, we obtain that policy $P$$_1$ is weakly more work-efficient than policy $\pi_1$ with probability one, which completes the proof.

\section{Proof of Theorem \ref{lem7_NBU}}\label{app_lem7}


%\begin{proof} [Proof of Theorem \ref{lem7_NBU}]
%\textbf{Condition 4:} $P\in\Pi$. This condition is trivial. Hence, \eqref{eq_delaygap1} follows from Lemma \ref{thm2}.
Consider the time difference ${C}_i(\text{FUT})-V_i(\text{FUT})$.
At time $V_i(\text{FUT})$, all tasks of job $i$ are completed or in service.
if $k_i>m$,  then job $i$ has at most $m$ incomplete tasks that are in service at time $V_i(\text{FUT})$, see Fig. \ref{V_i} for an illustration; if $k_i\leq m$, then job $i$ has at most $k_i$ incomplete tasks that are in service  at time $V_i(\text{FUT})$. Therefore, in policy FUT, no more than $k_i\wedge m = \min\{k_i,m\}$ tasks of job $i$ are completed during the time interval $[V_i(\text{FUT}), {C}_i(\text{FUT})]$. 

Suppose that at time $V_i(\text{FUT})$, the remaining tasks of job $i$ are being executed by the set of servers  $\mathcal{S}_i\subseteq\{1,\ldots,m\}$, which satisfies $|\mathcal{S}_i|\leq k_i \wedge m$. Let $\chi_l$ denote the amount of time that server $l\in \mathcal{S}_i$ has spent on executing a task of job $i$ by time $V_i(\text{FUT})$ in policy FUT. Let $R_{l}$ denote the remaining service time of server $l\in \mathcal{S}_i$ for executing this task after time $V_i(\text{FUT})$. Then, $R_l$ can be expressed as $R_l = [X_l - \chi_l | X_l > \chi_l]$. Because the $X_l$'s are independent NBU random variables with mean $\mathbb{E}[X_l]=1/\mu_l$, for all realizations of $\chi_l$
\begin{align}
[R_l|\chi_l] \leq_{\text{st}} X_l,~\forall~l\in \mathcal{S}_i.\nonumber
\end{align}
In addition, Theorem 3.A.55 of \cite{StochasticOrderBook} tells us that
\begin{align}
X_l \leq_{\text{icx}} Z_l,~\forall~l\in \mathcal{S}_i,\nonumber
\end{align}
where $\leq_{\text{icx}}$ is the increasing convex order defined in \cite[Chapter 4]{StochasticOrderBook} and the $Z_l$'s are independent exponential random variables with mean $\mathbb{E}[Z_l]=\mathbb{E}[X_l] =\mu_l$. Hence, 
\begin{align}
[R_l|\chi_l] \leq_{\text{icx}} Z_l,~\forall~l\in \mathcal{S}_i.\nonumber
\end{align}
Lemma \ref{lem_independent} tells us that 
the $R_l$'s are conditional independent for any given realization of $\{\chi_l,l\in \mathcal{S}_i\}$. Hence, by Corollary 4.A.16 of \cite{StochasticOrderBook}, for all realizations of $\mathcal{S}_i$ and $\{\chi_l,l\in \mathcal{S}_i\}$
\begin{align}\label{eq_exp_order}
\big[\max_{l\in \mathcal{S}_i} R_l \big| \mathcal{S}_i, \{\chi_l, l\in \mathcal{S}_i\}\big] \leq_{\text{icx}} \big[\max_{l\in \mathcal{S}_i} Z_l\big| \mathcal{S}_i\big].
\end{align}
%Because job $i$ only have $k_i$ tasks and the number of servers is $m$, job $i$ may have at most $k_i\wedge m$ remaining tasks at time $V_i(\text{FUT})$. In other words, the servers need to complete at most $k_i\wedge m$ remaining tasks of job $i$  during $[V_i(\text{FUT}), {C}_i(\text{FUT})]$.  %Then, $\mathcal{S}_i$ is a random set with cardinality $|\mathcal{S}_i|\leq k_i\wedge m$.
%The remaining task is to prove \eqref{eq_delaygap2}.
%Because the $X_l$'s are independent NBU random variables with mean $\mathbb{E}[X_l]=1/\mu_l$, Theorem 3.A.55 of \cite{StochasticOrderBook} tells us
%\begin{align}
%X_l \leq_{\text{icx}} Z_l,~l=1,\ldots,m,\nonumber
%\end{align}
%where $\leq_{\text{icx}}$ is the increasing convex order defined in \cite[Chapter 4]{StochasticOrderBook} and the $Z_l$'s are independent exponential random variables with mean $\mathbb{E}[Z_l]=\mathbb{E}[X_l] =\mu_l$. %Note that the set $\mathcal{S}_i$ is determined by the evolution of policy FUT up to time $V_i(\text{FUT})$.Because the task service times are determined by an external process which is not affected by the scheduling policy FUT, $X_l$ and $Z_l$ are independent of $\mathcal{S}_i$ for each $l\in \mathcal{S}_i$.
%Suppose that at time $V_i(\text{FUT})$, the remaining tasks of job $i$ are being executed by the set of servers  $\mathcal{S}_i\subseteq\{1,\ldots,m\}$, which satisfies $|\mathcal{S}_i|\leq k_i \wedge m$. 
Then,
\begin{align}
&\mathbb{E}[{C}_i(\text{FUT})-V_i(\text{FUT})|\mathcal{S}_i ,\{\chi_l, l\in \mathcal{S}_i\}]\nonumber\\
%=&\mathbb{E}\!\left[\max_{l\in \mathcal{S}_i} R_l \bigg|\chi_l, l\in \mathcal{S}_i\right]
%\leq &\mathbb{E}\!\left[\max_{l\in \mathcal{S}_i} X_l \bigg|\mathcal{I}\right]
%\\
=& \mathbb{E}\!\left[ \max_{l\in \mathcal{S}_i} R_l \bigg| \mathcal{S}_i ,\{\chi_l, l\in \mathcal{S}_i\}\right]\nonumber\\%\label{eq_gap_condition2}\\
\leq&\mathbb{E}\!\left[ \max_{l\in \mathcal{S}_i} Z_l \bigg| \mathcal{S}_i \right]\label{eq_gap_condition3}\\
\leq &\mathbb{E}\!\left[\max_{l=1,\ldots,k_i \wedge m} Z_l\right]\label{eq_gap_condition4}\\
\leq &\sum_{l=1}^{k_i \wedge m} \frac{1}{\sum_{j=1}^l \mu_j},\label{eq_gap_condition5}
\end{align}
where %\eqref{eq_gap_condition1} is because the remaining tasks of job $i$ are being processed by the set of servers  $\mathcal{S}_i\subseteq\{1,\ldots,m\}$ at time $V_i(\text{FUT})$, 
%\eqref{eq_gap_condition2} is due to the law of iterated expectations,
\eqref{eq_gap_condition3} is due to
\eqref{eq_exp_order} and Eq. (4.A.1) of \cite{StochasticOrderBook},
\eqref{eq_gap_condition4} is due to $\mu_1\leq \ldots\leq \mu_M$, $|\mathcal{S}_i|\leq k_i \wedge m$, and the fact that $\max_{l=1,\ldots,k_i \wedge m} Z_l$ is independent of $\mathcal{S}_i$, and \eqref{eq_gap_condition5} is due to the property of exponential distributions. Because $\mathcal{S}_{i}$ and $\{\chi_{l}, l\in \mathcal{S}_{i}\}$
 are random variables which are determined by the job parameters $\mathcal{I}$, taking the conditional expectation for given $\mathcal{I}$ in \eqref{eq_gap_condition5}, yields
\begin{align} 
\mathbb{E}\!\left[ {C}_i(\text{FUT})-V_i(\text{FUT}) | \mathcal{I}\right] \leq \sum_{l=1}^{k_i \wedge m} \frac{1}{\sum_{j=1}^l \mu_j}.\nonumber
\end{align} 
By taking the average over all $n$ jobs,  \eqref{eq_gap} is proven.
In addition, it is known that for each $k=1,2,\ldots,$
\begin{align}
\sum_{l=1}^k \frac{1}{l} \leq \ln(k)+1.\nonumber
\end{align}
By this, \eqref{eq_gap_2} holds. This completes the proof.
%\end{proof}





==> v3/appendices_coro2_0.tex <==



\section{Proof of Proposition \ref{lem_general}}\label{app_coro2}

In the proof of Proposition \ref{lem_general}, we need to use the following rearrangement inequality: 
\begin{lemma} \cite[Theorem 6.F.14]{Marshall2011}\label{lem_rearrangement}
Consider two $n$-dimensional vectors $(x_1,\dots,x_n)$ and $(y_1,\ldots,y_n)$. If $(x_i- x_j)(y_i-y_j)\leq0$ for two indices $i$ and $j$ where $1\leq i<j\leq n$, then 
\begin{align}
&(x_1\!-\!y_1,\ldots,x_j\!-\!y_i,\ldots,x_i\!-\!y_j,\ldots,x_n\!-\!y_n)\nonumber\\
\prec& (x_1\!-\!y_1,\ldots,x_i\!-\!y_i,\ldots,x_j\!-\!y_j,\ldots,x_n\!-\!y_n).\nonumber
\end{align}
\end{lemma}
\ifreport
\begin{proof}[Proof of Proposition \ref{lem_general}]
\else
\begin{proof}[of Proposition \ref{lem_general}]
\fi

For  $f\in\mathcal{D}_{\text{sym}}$, \eqref{eq_ordering_2_2} and  \eqref{eq_lem_general} follow from Proposition \ref{lem1} and Proposition \ref{lem1_1}.

For  $f\in\mathcal{D}_{\text{Sch-1}}$, \eqref{eq_lem_general} is proven in 3 steps, which are described as follows:





%Suppose that $b_j$ tasks have been assigned to the servers in policy $P$ by time $c_{(j)}(\pi)$. Since each job has only one task, $j$ tasks are completed by time $c_{(j)}(\pi)$ in policy $\pi$. Because policy $P$ is more work-efficient than policy $\pi$, it must hold that at least $j$ tasks are completed during $[0,c_{(j)}(\pi)]$  in policy $P$. Hence, at least $j$ tasks are assigned to the servers during $[0,c_{(j)}(\pi)]$ in policy $P$. Because each job has only one task, it follows that $v_{w_j}(P) \leq c_{(j)}(\pi)$  for all $j=1,\ldots,n$.

%We prove Proposition \ref{coro2} by induction. 

\emph{Step 1: We will show that}
\begin{align}\label{eq_coro2_3}
\bm{v}(P)-\bm{d}\prec_{\text{w}} \bm{c} (\pi)-\bm{d}.
\end{align} 
According to Eq. (1.A.17) and Theorem 5.A.9 of \cite{Marshall2011},
%In order to prove \eqref{eq_coro2_3}, 
it is sufficient to show that there exists an $n$-dimensional vector $\bm{v}'$ such that 
\begin{align}\label{eq_coro2_6}
\bm{v}(P)-\bm{d}\prec \bm{v}'- \bm{d} \leq \bm{c} (\pi)-\bm{d}.
\end{align}
Vector $\bm{v}'$ is constructed as follows: First, the components of the vector $\bm{v}'$ is a rearrangement (or permutation) of the components of the vector $\bm{v}(P)$, which can be equivalently expressed as
\begin{align}\label{eq_coro2_4}
v_{(i)}'=v_{(i)}(P),~\forall~i=1,\ldots,n.
\end{align}
Second, for each $j=1,\ldots,n$, if the completion time $c_j(\pi)$ of job $j$  is the $i_j$-th smallest component of $\bm{c}(\pi)$, i.e., 
\begin{align}
c_j(\pi)= c_{(i_j)}(\pi),
\end{align}
then $v_j'$ associated with job $j$ is the $i_j$-th smallest component of $\bm{v}'$, i.e., 
\begin{align}\label{eq_coro2_5}
v_j' = v_{(i_j)}'.
\end{align}
%then $c_j(\pi)$ associated with job $j$ is the $i$-th smallest component of $\bm{c}(\pi)$, i.e., 
%\begin{align}\label{eq_coro2_5}
%c_j(\pi)= c_{(i)}(\pi).
%\end{align}
Combining \eqref{eq_ordering_2_2} and \eqref{eq_coro2_4}-\eqref{eq_coro2_5}, yields
\begin{align}
v_j' = v_{(i_j)}'=v_{(i_j)}(P) \leq c_{(i_j)}(\pi) = c_j(\pi)\nonumber
\end{align}
for $j=1,\ldots,n$. This implies $\bm{v}' \leq \bm{c} (\pi)$, and hence the second inequality in \eqref{eq_coro2_6} is proven.

The remaining task is to prove the first inequality in \eqref{eq_coro2_6}. 
First, consider the case that the due times $d_1,\ldots, d_n$ of the $n$ jobs are  different from each other. 
The vector  $\bm{v}(P)$ can be obtained from  $\bm{v}'$ by the following procedure: For each $j=1,\ldots,n$, define a set 
\begin{align}
S_j = \{i: a_i\leq v_{j}(P), d_i < d_{j}\}.
\end{align}
If there exist two jobs $i$ and $j$ which satisfy $i\in S_j$ and $v_i' > v_{j}'$, we interchange the components $v_i'$ and $v_{j}'$ in vector $\bm{v}'$. Repeat this interchange operation, until such two jobs $i$ and $j$ satisfying  $i\in S_j$ and $v_i' > v_{j}'$ cannot be found. Therefore, at the end of this procedure, if job $i$ arrives before $v_{j}(P)$ and job $i$ has an earlier due time than job $j$, then $v_i' < v_{j}'$, which is exactly the priority rule of job service satisfied by policy $P$. Therefore, the vector  $\bm{v}(P)$ is obtained at the end of this procedure.
In each interchange operation of this procedure, $(v_i' - v_{j}')(d_i - d_{j})\leq0$ is satisfied before the interchange of $v_i'$ and $v_{j}'$. By Lemma \ref{lem_rearrangement} and the transitivity of the ordering of majorization, we can obtain $\bm{v}(P)-\bm{d}\prec \bm{v}'- \bm{d}$, which is the first inequality in \eqref{eq_coro2_6}. 

Next, consider the case that two jobs $i$ and $j$ have identical due time $d_i = d_j$. Hence, $(v_i' - v_{j}')(d_i - d_{j})=0$. In this case, the service order of job $i$ and job $j$ are indeterminate in policy $P$. Nonetheless, by Lemma \ref{lem_rearrangement}, the service order of job $i$ and job $j$ does not affect the first inequality in \eqref{eq_coro2_6}. Hence, the first inequality in \eqref{eq_coro2_6} holds even when $d_i = d_j$.
 
Finally, \eqref{eq_coro2_3} follows from \eqref{eq_coro2_6}.




%for each job $i$ there exists a job $j$ such that $v_i(P) = c_j(\pi)$ and vice versa. 
%We show that Thoerem \ref{lem2} holds if \emph{$L_{\max}(\cdot)$} is replaced by any $f\in\mathcal{D}_{\text{Sch-1}}$.} 

%We first construct another policy $\pi'$ based on policy $\pi$: The sequence of job completion times in policy $\pi'$ is a reordering (rearrangement) of that in policy $\pi$. Hence, for each job $i$ there exists a job $j$ such that 
%$c_i(\pi') = c_j(\pi)$. 
%%We note that if $k_i>1$ this rearrangement may not be lead to a feasible policy $\pi'$ because 
%Furthermore, in policy $\pi'$, each completed job has the earliest due time among all jobs in the queue, i.e., if job $i$ arrives before the completion time of job $j$ and $d_i<d_j$, then job $i$ is completed before job $j$ in policy $\pi'$. We note that because $k_i=1$ for all $i$, this reordering operation leads to a feasible policy $\pi'$; otherwise, if $k_i>1$, this reordering operation may not be feasible. In particular, suppose that job $i$ has an earlier due time and more unassigned tasks than the other jobs in the queue, then it is infeasible to reorder the sequence of job completion times such that job $i$ is the next completed job.
%For the constructed policy $\pi'$, one can use the proof argument of Lemma \ref{lemG4_thm3} to show that
%\begin{eqnarray}\label{eq_pi'}
%\sum_{i:d_i\leq\tau_j} \gamma_{i,P}(t)\leq \sum_{i:d_i\leq\tau_j} \xi_{i,\pi'}(t), ~\tau_j\in[0,\infty)
%\end{eqnarray}
%holds for all $t\in[0,\infty)$. That is, Lemma \ref{lemG4_thm3}  holds even if policy $\pi$ is replaced by this constructed policy $\pi'$. %Note that if the jobs have more than one tasks, \eqref{eq_pi'} may not hold for the constructed policy $\pi'$.
%%We rearrange the job completion times of policy $\pi$ as follows: Consider any two jobs $i$ and $j$ which simultaneously exist in the queue at some time, i.e., there exists a time $t$ such that $a_i\leq t\leq c_i(\pi)$ and  $a_j\leq t\leq c_j(\pi)$. If $(c_i(\pi)-c_j(\pi))(d_i- d_j)<0$, we interchange the completion times of job $i$ and job $j$. Repeat this procedure until $(c_i(\pi)-c_j(\pi))(d_i- d_j)\geq 0$ is satisfied for any pair of jobs $i$ and $j$ which simultaneously exist in the queue at some time. Hence, after the rearrangement, each completed job has the earliest due time among all jobs in the queue. Let $c_i'(\pi)$ denote the completion time of job $i$ after the rearrangement. 
%
%In the sequel, we will use \eqref{eq_pi'}, Lemma \ref{lem_rearrangement}, and the property of policy $\pi'$ to prove the following two claims:
%\begin{itemize}
%\item[1.] $\bm{c}(\pi')-\bm{d}\prec \bm{c} (\pi)-\bm{d}$;
%\item[2.] $v_i(P)\leq c_i(\pi')$ for $i=1,\ldots,n$.
%\end{itemize}
%
%
%%Hence, the $i$-th smallest job completion time $c_{(i)}(\pi')$ of policy $\pi'$ is equal to $i$-th smallest job completion time $c_{(i)}(\pi)$ of policy $\pi$, i.e., $c_{(i)}(\pi')=c_{(i)}(\pi)$.
%
%First, we prove claim 1. An alternative construction procedure of policy $\pi'$ is provided as follows: Suppose that in policy $\pi$, two jobs $i$ and $j$ co-exist in the queue at some time $t$, i.e., $a_i\leq t\leq c_i(\pi)$ and  $a_j\leq t\leq c_j(\pi)$. If $(c_i(\pi)-c_j(\pi))(d_i- d_j)<0$, the completion times of job $i$ and job $j$ are interchanged. 
%Repeat this pair-wise interchange operation until $(c_i(\pi)-c_j(\pi))(d_i- d_j)\geq 0$ is satisfied for any pair of jobs $i$ and $j$ which co-exist in the queue at some time. Then, the job completion times of policy $\pi'$ are obtained.
%By using Lemma \ref{lem_rearrangement} for each pair-wise interchange operation during this construction procedure of policy $\pi'$, we can obtain $\bm{c}(\pi')-\bm{d}\prec \bm{c} (\pi)-\bm{d}$. By this, claim 1 is proven.
%
%
%Next, we prove claim 2 by contradiction. Suppose that
%\begin{align}\label{eq_contradiction_coro2}
%v_{w_j}(P) > c_{w_j}(\pi')
%\end{align} 
%holds for some $j\in\{1,\ldots,n\}$.
%In policy $\pi'$, if job $i$ arrives before time $c_{w_j}(\pi')$ and $d_i<d_{w_j}$, then job $i$ is completed before time $c_{w_j}(\pi')$. Hence, the system state of policy $\pi'$ satisfies 
%\begin{align}
%\sum_{i:d_i\leq d_{w_j}}\xi_{i,\pi'}(c_{w_j}(\pi')) =0,\nonumber
%\end{align}
%where we have used the fact that $d_i\neq d_j$ if $i\neq j$. Combining this with \eqref{eq_pi'}, we can obtain
%%Hence, there are $y-1$ unfinished jobs at time $C_{w_1}(\pi)$ such that
%%Invoking Lemma \ref{lemG4}, we can obtain
%\begin{align}\label{eq_proof_1_coro2}
%\sum_{i:d_i\leq d_{w_j}} \gamma_{i,P}(c_{w_j}(\pi'))\leq 0.
%\end{align}
%By the definition of the system state, we have $\gamma_{i,P}(t)\geq0$ for all $i$ and $t$. This and \eqref{eq_proof_1_coro2} tells us that at time $c_{w_j}(\pi')$, the system state of policy $P$ satisfies
%\begin{align}
%\gamma_{w_j,P}(c_{w_j}(\pi'))= 0.\nonumber
%\end{align}
%That is, all tasks of job $w_j$ are either completed or under service by time $c_{w_j}(\pi')$ in policy $P$. Hence, $v_{w_j}(P)\leq c_{w_j}(\pi')$, which contradicts with \eqref{eq_contradiction_coro2}. Therefore, $v_{w_j}(P)\leq c_{w_j}(\pi')$ holds for all $j=1,\ldots,n$. By this, claim 2 is proven.

%Now, we use claim 1 and claim 2 to prove \eqref{eq_coro2_3}. In particular,  claim 1 and claim 2 suggest that
%\begin{align}
%\bm{v}(P)-\bm{d}\leq \bm{c}(\pi')-\bm{d}\prec \bm{c} (\pi)-\bm{d}.
%\end{align}
%By this and Theorem 5.A.9 of \cite{Marshall2011}, \eqref{eq_coro2_3} follows.

%In policy $P$, each task allocated to the servers belongs to the job with the earliest due time, whenever there exist unassigned tasks in the queue. Hence, jobs $w_1,\ldots,w_j$ have the earliest due time among all jobs which arrive during $[0, v_{w_j}(P)]$. In policy $\pi$, let job $v_i$ be the $i$-th completed job after the rearrangement such that $c_{v_i}'(\pi) = c_{(i)}'(\pi)$. After the rearrangement, each completed job has the earliest due time among all jobs in the queue. Hence, jobs $v_1,\ldots,v_j$ have the earliest due time among all jobs which arrive during $[0, c_{(j)}'(\pi)]$.
%
% Towards this goal, we need to show that 
%\begin{align}
%c_{(i)}'(\pi) \leq c_{w_i}'(\pi),~i=1,\ldots,n. 
%\end{align}
%
%
%
%because  this with  \eqref{eq_coro2_2}, we have
%\begin{align}
%v_{w_i}(P) \leq c_{(i)}(\pi) = c_{(i)}'(\pi) = c_{w_i}'(\pi),~i=1,\ldots,n.
%\end{align}
%
%
%,  According to \eqref{eq_coro2_2}, we have
%\begin{align}
%v_{w_j}(P) \leq c_{(i)}(\pi) = c_{(i)}'(\pi) = c_{v_i}'(\pi).
%\end{align}
%Because after this rearrangement each completed job has the earliest due time among all jobs in the queue, 
%$d_i\leq d_{v_i}$ holds for all job $i$ satisfying $a_i\leq c_{v_i}'(\pi)$.
%
% that after the rearrangement, each completed job has the earliest due time among all jobs in the queue.  
%
%
%after the rearrangement, each completed job has the earliest due time among all jobs in the queue.  
%
%
%
%
%show that one of the following two cases is true:
%\begin{itemize}
%\item[1.] $v_{w_1}(P)\leq c_{w_1}(\pi)$, and $v_{w_{2}}(P)\leq c_{w_{2}}(\pi)$;
%%\item[2.] $d_{w_j}\leq d_{w_{j+1}}$, $v_{w_j}(P)\leq c_{w_j}(\pi)$, and $v_{w_{j+1}}(P)\leq c_{w_{j+1}}(\pi)$.
%\item[2.] $v_{w_1}(P)\leq c_{w_{2}}(\pi)$, $v_{w_{2}}(P)\leq c_{w_{1}}(\pi)$, $d_{w_1}\leq d_{w_{2}}$, and $c_{w_{1}}(\pi)>c_{w_{2}}(\pi)$.
%\end{itemize}
%
%In the proof of Lemma \ref{lem_sample_path_ordering_thm3}, it was shown that 
%\begin{align}\label{eq_coro2_1}
%v_{w_j}(P) \leq \max_{i:a_i\leq v_{w_j}(P),d_i\leq d_{w_j} }c_{i}(\pi).
%\end{align}
%We now use \eqref{eq_coro2_2}, \eqref{eq_coro2_1}, and condition 2 of Thoerem \ref{lem2} to prove the claim of \emph{Step 2}.
%
%We first consider $j=1$. Because job $w_1$ is the first job whose tasks are either completed or under service, no job is completed during $[0,v_{w_1}(P))$ in policy $P$. Because policy $P$ satisfies condition 2 of Thoerem \ref{lem2}, job $w_1$ has the earliest due time among all jobs in the queue at time $v_{w_1}(P)$ in policy $P$. This tells us that if job $i$ satisfies $a_i\leq v_{w_1}(P)$ and $d_i\leq d_{w_1}$, then $i=w_1$. Hence,  \eqref{eq_coro2_1} implies 
%$v_{w_1}(P) \leq c_{w_1}(\pi)$. 
%
%For $j=2$, because job $w_2$ is the second job whose tasks are either completed or under service  in policy $P$, only  job $w_1$ can be completed during $[0,v_{w_2}(P))$ in policy $P$. Because policy $P$ satisfies condition 2 of Thoerem \ref{lem2}, job $w_2$ has the earliest due time among all jobs in the queue at time $v_{w_2}(P)$ in policy $P$. This tells us that if job $i$ satisfies $a_i\leq v_{w_2}(P)$ and $d_i\leq d_{w_2}$, then $i=w_1$ or $i=w_2$. 
%
%If $d_{w_1}> d_{w_2}$, then \eqref{eq_coro2_1} implies 
%\begin{align}
%v_{w_2}(P) \leq \max_{i:a_i\leq v_{w_2}(P),d_i\leq d_{w_2} }c_{i}(\pi) = c_{w_2}(\pi).
%\end{align}
%This belongs to case 1 of \emph{Step 2}.
%
%If $d_{w_1}\leq d_{w_2}$, then \eqref{eq_coro2_1} becomes $v_{w_2}(P) \leq \max[c_{w_1}(\pi), c_{w_2}(\pi)]$. We  consider two sub-cases: If $c_{w_1}(\pi)\leq c_{w_2}(\pi)$, then $v_{w_2}(P) \leq c_{w_2}(\pi)$. This also belongs to case 1 of \emph{Step 2}.
%If $c_{w_1}(\pi)> c_{w_2}(\pi)$, by \eqref{eq_coro2_2}, we can obtain $v_{w_1}(P) \leq c_{(1)}(\pi)\leq c_{w_2}(\pi)$. Further,  \eqref{eq_coro2_1} becomes $v_{w_2}(P)\leq c_{w_1}(\pi)$. This belongs to case 2 of \emph{Step 2}.
%
%By summarizing these cases, we obtain the claim of \emph{Step 2}. 
%
%\emph{Step 3: We show that}
%\begin{align}\label{eq_coro2_3}
%\bm{v}(P)-\bm{d}\prec_{\text{w}} \bm{c} (\pi)-\bm{d}.
%\end{align} 
%
%We rearrange the completion times of job $w_1$ and job $w_2$ as follows: If case 2 of \emph{Step 2} occurs, we interchange the completion times of job $w_1$ and job $w_2$. 
%%By Lemma \ref{lem_rearrangement}, we can obtain
%%\begin{align}
%%&(c_{w_2}(\pi)\!-\!d_{w_1},c_{w_1}(\pi)\!-\!d_{w_2},c_{w_3}(\pi)\!-\!d_{w_3},\ldots,c_{w_n}(\pi)\!-\!d_{w_n})\nonumber\\
%%\prec& (c_{w_1}(\pi)\!-\!d_{w_1},c_{w_2}(\pi)\!-\!d_{w_2},c_{w_3}(\pi)\!-\!d_{w_3},\ldots,c_{w_n}(\pi)\!-\!d_{w_n}).\nonumber
%%\end{align}
%If case 1 of \emph{Step 2} occurs, there is no operation. 
%Let $\bm{c}(\pi)$ and $\bm{c}' (\pi)$, respectively, denote the completion time vectors of the $n$ jobs before and after this rearrangement operation. By Lemma \ref{lem_rearrangement}, we can get 
%\begin{align}
%\bm{c}' (\pi)-\bm{d}\prec \bm{c} (\pi)-\bm{d}.\nonumber
%\end{align}
%In addition, it holds that $v_{w_1}(P)\leq c'_{w_1}(\pi)$ and $v_{w_{2}}(P)\leq c'_{w_{2}}(\pi)$ after the rearrangement.	
%
%We repeat this rearrangement operation iteratively by following a two-layer bubble sorting algorithm. In the $l$-th out-layer iteration of the algorithm, we rearrange the completion times of two neighboring jobs $w_i$ and $w_{i+1}$ for $l$ times, where the value of $i$ is chosen in the order of $i=l,l-1,\ldots,1$. For any two neighboring jobs $w_i$ and $w_{i+1}$, if $v_{w_i}(P)\leq c_{w_{i+1}}(\pi)$, $v_{w_{i+1}}(P)\leq c_{w_{i}}(\pi)$, $d_{w_i}\leq d_{w_{i+1}}$, and $c_{w_{i}}(\pi)>c_{w_{i+1}}(\pi)$ hold before the rearrangement operation, we interchange the completion times of job $w_i$ and job $w_{i+1}$; otherwise there is no operation. 
%
%Let $\bm{c}^{l-1} (\pi)$ and $\bm{c}^{l} (\pi)$, respectively, denote the completion time vectors of the $n$ jobs before and after the $l$-th out-layer iteration. Using \eqref{eq_coro2_2}, \eqref{eq_coro2_1}, and condition 2 of Theorem \ref{lem2}, we can obtain 
%\begin{align}
%&\bm{c}^{l} (\pi)-\bm{d} \prec \bm{c}^{l-1} (\pi)-\bm{d}, \nonumber\\
%&v_{w_i}(P)\leq c^{l}_{w_i}(\pi),~i=1,\ldots,l+1.\nonumber
%\end{align}
%After repeating the out-layer iteration for $n-1$ times, we have
%\begin{align}
%&\bm{c}^{n-1} (\pi)-\bm{d} \prec \ldots \prec \bm{c}^{1} (\pi)-\bm{d} \prec \bm{c}^{0} (\pi)-\bm{d}, \nonumber\\
%&\bm{v}(P)\leq \bm{c}^{n-1}(\pi).\nonumber
%\end{align}
%%for each $i=1,\ldots,l$ if $d_{w_i}\leq d_{w_{l+1}}$ and $c^{l-1}_{w_{i}}(\pi)>c^{l-1}_{w_{l+1}}(\pi)$, we interchange the completion times of job $w_i$ and job $w_{l+1}$. 
%Hence,
%\begin{align}
%\bm{v}(P)-\bm{d}\leq \bm{c}^{n-1}(\pi)-\bm{d}\prec \bm{c} (\pi)-\bm{d}.\nonumber
%\end{align} 
%By this, \eqref{eq_coro2_3} follows. 
\emph{Step 3: We use \eqref{eq_coro2_3} to prove Proposition \ref{lem_general}.}
For any $f\in\mathcal{D}_{\text{Sch-1}}$, $f(\bm{x}+\bm{d})$ is increasing and Schur convex. 
According to Theorem 3.A.8 of \cite{Marshall2011}, for all $f\in\mathcal{D}_{\text{Sch-1}}$, we have
\begin{align}
&f(\bm{v}(P)) \nonumber\\
= &f[(\bm{v}(P)-\bm{d})+\bm{d}] \nonumber\\
\leq& f[(\bm{c}(\pi)-\bm{d})+\bm{d}] \nonumber\\
=& f(\bm{c} (\pi)).\nonumber
\end{align} 
%By considering all possible sample paths of policy $P$ and policy $\pi$, the stochastic ordering result in Proposition \ref{coro2} follows.
This completes the proof.
\end{proof}

==> v3/appendices_dis.tex <==
% !TEX root = ./replication.tex
%\section{Proofs of Thoerem~10 and Corollary 10} \label{app_dis_EDD}
%Similar with the proof of Theorem \ref{thm2}, we can show that policy FCFS-R is more work-efficient than any policy $\pi\in\Pi$. Then, Theorem \ref{thm6} follows from Thoerem \ref{lem3}, and Corollary \ref{coro6_1} follows from Corollary \ref{coro3_1}.

==> v3/appendices_lem1_0.tex <==
\section{Proof of Proposition \ref{lem1_0}} \label{app_lem1_0}

The following two lemmas are needed to prove Proposition \ref{lem1_0}:  

\begin{lemma}\cite[Lemmas 1-2]{Smith78}\label{lem_non_prmp1_0}
Suppose that under policy $P$, $\{\bm{\xi}_{P}',\bm{\gamma}_{P}'\}$ is obtained by completing $b_P$ tasks in the system whose state is $\{\bm{\xi}_{P},\bm{\gamma}_{P}\}$. Further, suppose that under policy $\pi$, $\{\bm{\xi}_{\pi}',\bm{\gamma}_{\pi}'\}$ is obtained by completing $b_\pi$ tasks in the system whose state is $\{\bm{\xi}_{\pi},\bm{\gamma}_{\pi}\}$.
If $b_P\geq b_\pi$, policy $P$ satisfies condition 3 of Proposition \ref{lem1_0}, and 
\begin{eqnarray}\label{eq_non_prmp_41_0}
\sum_{i=j}^n {\xi}_{[i],P}\leq \sum_{i=j}^n {\xi}_{[i],\pi}, ~j = 1,2,\ldots,n,\nonumber
\end{eqnarray}
then
\begin{eqnarray}\label{eq_non_prmp_40_0}
\sum_{i=j}^n {\xi}_{[i],P}'\leq \sum_{i=j}^n {\xi}_{[i],\pi}', ~j = 1,2,\ldots,n.
\end{eqnarray}
\end{lemma}




\begin{lemma}\cite[Lemma 3]{Smith78}\label{lem_non_prmp2_0}
Suppose that, under policy $P$, $\{\bm{\xi}_{P}',\bm{\gamma}_{P}'\}$ is obtained by adding a job with $b$ tasks to the system whose state is $\{\bm{\xi}_{P},\bm{\gamma}_{P}\}$. Further, suppose that, under policy $\pi$, $\{\bm{\xi}_{\pi}',\bm{\gamma}_{\pi}'\}$ is obtained by adding a job with $b$ tasks to the system whose state is $\{\bm{\xi}_{\pi},\bm{\gamma}_{\pi}\}$.
If
\begin{eqnarray}
\sum_{i=j}^n {\xi}_{[i],P}\leq \sum_{i=j}^n {\xi}_{[i],\pi}, ~j = 1,2,\ldots,n,\nonumber
\end{eqnarray}
then
\begin{eqnarray}
\sum_{i=j}^n {\xi}_{[i],P}'\leq \sum_{i=j}^n {\xi}_{[i],\pi}', ~j = 1,2,\ldots,n.\nonumber
\end{eqnarray}
\end{lemma}


We now use Lemma \ref{lem_non_prmp1_0} and Lemma \ref{lem_non_prmp2_0} to prove Proposition \ref{lem1_0}.
\ifreport
\begin{proof}[Proof of Proposition \ref{lem1_0}]
\else
\begin{proof}[of Proposition \ref{lem1_0}]
\fi

Because policy $P$ is more work-efficient than policy $\pi$, the sequence of task completion times in policy $P$ are  smaller  than those in policy $\pi$, i.e., 
\begin{align}
(t_{1,P},\ldots, t_{k_{\text{sum}},P}) \leq(t_{1,\pi},\ldots, t_{k_{\text{sum}},\pi}). \nonumber
\end{align} 

We modify the sample-path of policy $P$ as follows:  Suppose that for each $i=1,\ldots, k_{\text{sum}}$  a task of job $j_i$ is completed at time $t_{i,P}$ on the original sample-path of policy $P$, then on the modified sample-path of policy $P$ a task of job $j_i$ is completed at time $t_{i,\pi}$. By this modification, the task completion times of policy $P$ are postponed, but the order of completed tasks remain the same. 
Let $\hat{\bm{\xi}}_{P}(t) =(\hat{\xi}_{1,P}(t),\ldots,\hat{\xi}_{n,P}(t))$ and $\hat{\bm{\gamma}}_{P}(t) =(\hat{\gamma}_{1,P}(t),\ldots,\hat{\gamma}_{n,P}(t))$ denote the system state on the modified sample-path of policy $P$. Because the task completion times are postponed,  we can get ${\xi}_{i,P}(t)  \leq \hat{\xi}_{i,P}(t) $ for all $t\geq 0$ and $i=1,\ldots,n$. Hence, for all $t\in[0,\infty)$
\begin{align}\label{eq_lem1_0_proof_1}
\sum_{i=j}^n {\xi}_{[i],P}(t)\leq \sum_{i=j}^n \hat{\xi}_{[i],P}(t), ~i=1,2,\ldots,n.
\end{align}

Next, we compare policy $\pi$ with the modified sample-path of policy $P$. By the foregoing modification, \emph{the task completion times are identical on the sample-path of policy $\pi$ and on the modified sample-path of policy $P$.} 
 
On the original sample-path of policy $P$, each task completing service  is from the job with the fewest remaining tasks among all jobs in the queue. On the modified sample-path of policy $P$, there are more jobs in the queue at the postponed   task completion times due to additional job arrivals. Because $k_1\leq k_2\leq \ldots\leq k_n$, later arrived jobs have more tasks. Hence, on the modified sample-path of policy $P$, each task completing service  is still from the job with the fewest remaining tasks among all jobs in the queue. In other words, \emph{condition 3 of Proposition \ref{lem1_0} is satisfied on the modified sample-path of policy $P$}. 

Because $\hat{\bm{\xi}}_{P}(0) = {\bm{\xi}}_{\pi}(0) =\bm{0}$, by using Lemma \ref{lem_non_prmp1_0} and Lemma \ref{lem_non_prmp2_0}, and taking an induction on the job arrival events and task completion events over time, we can obtain for all $t\in[0,\infty)$
% Then, by using the arguments in \cite{Smith78} we can show 
\begin{align}\label{eq_lem1_0_proof_2}
\sum_{i=j}^n \hat{\xi}_{[i],P}(t)\leq \sum_{i=j}^n {\xi}_{[i],\pi}(t), ~i=1,2,\ldots,n.
\end{align}
Combining \eqref{eq_lem1_0_proof_1} and \eqref{eq_lem1_0_proof_2}, yields \eqref{eq_ordering_1_1}. Then, \eqref{eq_ordering_1_1_2} and \eqref{eq_ordering_1_2} follow from Lemma \ref{ordering_1}, which completes the proof. \end{proof}

%Assume that no task is completed at the job arrival time $a_i$ for $i=1,\ldots,n$. This does not lose any generality, because if a task is completed at time $t_j=a_i$, Proposition \ref{lem1} can be proven by first proving for the case $t_j=a_i+\epsilon$ and then taking the limit $\epsilon\rightarrow 0$. 
%We prove \eqref{eq_ordering_2_1} by induction. 
%
%\emph{Step 1: We will show that \eqref{eq_ordering_2_1} holds during $[0,a_2)$.} 
%
%Because $\bm{\xi}_{P}(0^-) = \bm{\gamma}_{P}(0^-) =\bm{\xi}_{\pi}(0^-) = \bm{\gamma}_{\pi}(0^-)=\bm{0}$, \eqref{eq_ordering_2_1} holds at time $0^-$. Job 1 arrives at time $a_1=0$. By Lemma \ref{lem_non_prmp2}, \eqref{eq_ordering_2_1} holds at time $0$. Let $t$ be an arbitrarily chosen time during $(0,a_{2})$. Suppose that  $b_\pi$ tasks start execution and complete execution during $[0,t]$ in policy $\pi$. We need to consider two cases: 
%
%Case 1: There exist unassigned tasks which are not under service during $[0,t]$ in policy $P$. By the weak work-efficiency ordering, no fewer than $b_\pi$ tasks start execution during $[0,t]$ in policy $P$. Because \eqref{eq_ordering_2_1} holds at time $0$, by Lemma \ref{lem_non_prmp1}, \eqref{eq_ordering_2_1} also holds at time $t$. 
%
%Case 2: All tasks in the system are under service by time $t'\in[0,t]$ in policy $P$. Because $t\in(0,a_{2})$ and there is no task arrival during $(0,a_2)$, there is no task arrival during $(t',t]$. Hence, it must holds that all tasks in the system are under service at time $t$. Then, the system state of policy $P$ satisfies $\sum_{i=j}^n {\gamma}_{[i],P}(t)=0$ for all $j=1,2,\ldots,n$ at time $t$. Hence, \eqref{eq_ordering_2_1} holds at time $t$. 
%
%
%
%
%In summary of these two cases, \eqref{eq_ordering_2_1} holds for all $t\in[0,a_2)$.  
%
%
%
% 
%
%
%\emph{Step 2: Assume that for some integer $i\in\{2,\ldots, n\}$, the conditions of Proposition \ref{lem1} imply that \eqref{eq_ordering_2_1} holds for all $t\in[0,a_i)$. We will prove that the conditions of Proposition \ref{lem1} imply that  \eqref{eq_ordering_2_1} holds for all $t\in[0,a_{i+1})$.}
%
%
%Let $t$ be an arbitrarily chosen time during $(a_i,a_{i+1})$. We modify the task completion times in policy $\pi$ as follows: For each pair of corresponding task $j$ and task $j'$ mentioned in the definition of the weak work-efficiency ordering, if 
%%After this modification, the following three properties are true:
%\begin{itemize}
%\item in policy $\pi$, task $j$ starts execution at time $\tau\in[0,a_i]$ and completes execution at time $\nu\in(a_i,t]$,
%\item in policy $P$, there exist unassigned tasks in the queue during $[\tau,\nu]$,
%\item in policy $P$, the corresponding task $j'$ starts execution at time $t'\in[0,a_i]$,
%\end{itemize}
%then the completion time of task $j$ is modified from $\nu$ to $a_i^-$ in policy $\pi$, as illustrated in Fig. \ref{fig_modification}.
%
%This modification satisfies the following three claims:
%\begin{itemize}
%\item[1.] The system state of policy $\pi$ at time $t$ remains the same before and after this modification;
%\item[2.] Policy $P$ is still weakly more work-efficient than policy $\pi$ after this modification;
%\item[3.] If $b_\pi$ tasks complete execution during $[a_i,t]$ on the modified sample path of policy $\pi$, and there exist unassigned tasks in the queue during $[a_i,t]$ in policy $P$, then no fewer than $b_\pi$ tasks start execution during $[a_i,t]$ in policy $P$.
%\end{itemize}
%We now prove these three claims. Claim 1 follows from the fact that the tasks completed during $[0,t]$ are the same before and after this modification. It is easy to prove claim 2 by the definition of work-efficiency ordering. For claim 3, notice that if a task $j$ completes execution during $[a_i,t]$ on the modified sample path of policy $\pi$, then its corresponding task $j$ must start execution during $[a_i,t]$ in policy $P$. By this, claim 3 follows.
%
%
%
%\ifreport
%\begin{figure}
%\centering 
%\includegraphics[width=0.7\textwidth]{Figures/modification} \caption{Illustration of the modification of task completion times in policy $\pi$: If in policy $\pi$, task $j$ starts execution at time $\tau\in[0,a_i]$ and completes execution at time $\nu\in(a_i,t]$, and in policy $P$, task $j'$ starts execution at time $t'\in[0,a_i]$, then the completion time of task $j$ is changed from $\nu$ to $a_i^-$ in policy $\pi$.}
%\label{fig_modification} 
%\end{figure} 
%\fi
%
%
%
%
%
%We use these three claims to prove the  statement of \emph{Step 2}. According to claim 2, policy $P$ is still weakly more work-efficient than policy $\pi$ after the modification. By the assumption of \emph{Step 2}, \eqref{eq_ordering_2_1} holds during $[0,a_i)$ for the modified sample path of policy $\pi$. Job $j$ arrives at time $a_i$. By Lemma \ref{lem_non_prmp2}, \eqref{eq_ordering_2_1} holds at time $a_i$ for the modified sample path of policy $\pi$. Suppose that $b_\pi$ tasks complete execution during $[a_i,t]$ on the modified sample path of policy $\pi$.
%We need to consider two cases: 
%
%Case 1: There exist unassigned tasks which are not under service during $[a_i,t]$ in policy $P$. By claim 3, no fewer than $b_\pi$ tasks start execution during $[a_i,t]$ in policy $P$. Because \eqref{eq_ordering_2_1} holds at time $a_i$, by Lemma \ref{lem_non_prmp1}, \eqref{eq_ordering_2_1} also holds at time $t$ for the modified sample path of policy $\pi$. 
%
%Case 2: All tasks in the system are under service at some time $t'\in[a_i,t]$ in policy $P$. Because $t\in(a_i,a_{i+1})$ and $t'\in[a_i,t]$, there is no task arrival during $(t',t]$. Hence, it must holds that all tasks in the system are under service at time $t$. Then, the system state of policy $P$ satisfies $\sum_{i=j}^n {\gamma}_{[i],P}(t)=0$ for all $j=1,2,\ldots,n$  at time $t$. Hence, \eqref{eq_ordering_2_1} holds at time $t$ for the modified sample path of policy $\pi$. 
%
%
%
%
%
%
%In summary of these two cases, \eqref{eq_ordering_2_1} holds at time $t$ for the modified sample path of policy $\pi$. By claim 1, the system state of policy $\pi$ at time $t$ remains the same before and after this modification. Hence, \eqref{eq_ordering_2_1} holds at time $t$ for the original sample path of policy $\pi$. Therefore, if  the assumption of \emph{Step 2} is true, then \eqref{eq_ordering_2_1} holds for all $t\in[0,a_{i+1})$. 
%
%% each task (index by $j$) completed during $[0,t]$ in policy $\pi$, we modify the completion time of task $j$ as follows
%%
%%
%%Suppose that $g$ tasks are assigned to the servers during $[a_i,t]$ in policy $P$, and $h$ tasks are completed during $[a_i,t]$ in policy $\pi$. 
%%
%%If $g\geq h$, then by Lemma \ref{lem_non_prmp1} tells us that \eqref{eq_ordering_2_1} holds for all $t\in(a_i,a_{i+1})$. 
%%
%%If $g< h$, suppose that $h'$ tasks ($h'\leq h$) are assigned to the servers during $[a_i,t]$ and are  completed during $[a_i,t]$ in policy $\pi$. Hence, $h-h'$ tasks are assigned to the servers during $[0,a_i)$ and are completed during $[a_i,t]$ in policy $\pi$. Because policy $P$ is more work-efficient than policy $\pi$,  in policy $P$ one of the following cases holds: (i) no fewer than $h'$ unassigned tasks are allocated to the servers during $[a_i,t]$, i.e., $h'\leq g$, (ii) all the remaining tasks are under service at time $t'\in[a_i,t]$, or (iii) the queue is empty at time $t'\in[a_i,t]$.
%%
%%
%%If case (i) happens, %we can obtain that $h-h'$ tasks are assigned to the servers during $[0,a_i)$ and are completed during $[a_i,t]$ in policy $\pi$. 
%% We modify the completion times of these $h-h'$ tasks such that these $h-h'$ tasks are completed at time $a_i^-$ on the modified sample path of policy $\pi$. After this modification, the conditions of Proposition \ref{lem1} still hold and the system state $\bm{\beta}(t)$ of policy $\pi$ at time $t$ remains the same. Hence, we only need to prove \eqref{eq_ordering_2_1} at time $t$ on this modified sample path of policy $\pi$. In particular, by the assumption of \emph{Step 2}, \eqref{eq_ordering_2_1} holds during $[0,a_i)$ on this modified sample path of policy $\pi$. Job $j$ arrives at time $a_i$. By Lemma \ref{lem_non_prmp2}, \eqref{eq_ordering_2_1} holds at time $a_i$ on this modified sample path of policy $\pi$. By Lemma \ref{lem_non_prmp1} and $h'\leq g$, we can obtain that \eqref{eq_ordering_2_1} holds at time $t$ on the modified sample path of policy $\pi$. Hence, \eqref{eq_ordering_2_1} also holds at time $t$ on the original sample path of policy $\pi$.
%%
%%
%%If case (ii) happens, because there is no task arrival during $(t',t]$, it must holds that all the remaining tasks are under service at time $t$. Then, the system state of policy $P$ at time $t$ satisfies $\sum_{i=j}^n [\alpha_h(t)- \delta_h(t)]=0$ for all $h=1,2,\ldots$ Hence, \eqref{eq_ordering_2_1} holds at time $t$. If case (iii) happens, because there is no task arrival during $(t',t]$, it must holds that the queue is empty at time $t$. Similar with case (ii), we can show that \eqref{eq_ordering_2_1} holds at time $t$. In summary, if  the assumption of \emph{Step 2} is true, then \eqref{eq_ordering_2_1} holds for all $t\in[0,a_{i+1})$. 
%By induction, \eqref{eq_ordering_2_1} holds at time $t\in[0,\infty)$. Then, \eqref{eq_ordering_2_2} and \eqref{eq_ordering_2_3} follow from Lemma \ref{ordering_1}.
%This completes the proof.


==> v3/appendices_lem2.tex <==
\section{Proof of Lemma  \ref{lem_ratio}}\label{app_lem_ratio}
We will need the following lemma:
\begin{lemma}\label{lem_independent}
Suppose that $X_1, \ldots, X_m$ are non-negative independent random variables, $\chi_1, \ldots, \chi_m$ are arbitrarily given non-negative constants, $R_l = [X_l - \chi_l | X_l > \chi_l]$ for  $l=1,\ldots,m$, then $R_1, \ldots, R_m$  are  mutually independent.
\end{lemma}
\begin{proof}
For all constants $t_l \geq 0$, $l=1,\dots m$, we have
\begin{align}
&\Pr[R_l >t_l, l=1,\ldots,m] \nonumber\\
=& \Pr[X_l - \chi_l >t_l, l=1,\ldots,m| X_l > \chi_l, l=1,\ldots,m]\nonumber\\
=&\frac{\Pr[X_l   >t_l + \chi_l, l=1,\ldots,m]}{\Pr[X_l > \chi_l, l=1,\ldots,m]}\nonumber\\
=& \frac{\prod_{l=1}^m \Pr[X_l   >t_l + \chi_l]}{\prod_{l=1}^m \Pr[X_l   > \chi_l]}\nonumber\\
=& \prod_{l=1}^m \Pr[X_l - \chi_l >t_l| X_l > \chi_l]\nonumber\\
=&\prod_{l=1}^m \Pr[R_l >t_l].
\end{align}
Hence, $R_1, \ldots, R_m$  are mutually independent.
\end{proof}

\begin{proof}[Proof of lemma \ref{lem_ratio}]
Define a function $g_2(\bm{x})=f(\bm{x}+\bm{a})$.
Because $g_2(\bm{x})=f(\bm{x} + \bm{a})$ is sub-additive in $\bm{x}$, i.e., $g_2(\bm{x} + \bm{y}) \leq g_2(\bm{x} ) + g_2(\bm{y} )$, we can obtain
\begin{align}
& f(\bm{C}(P)) \nonumber\\
=& g_2(\left[\bm{V}(P)-\bm{a}\right]+\left[\bm{C}(P)-\bm{V}(P)\right]) \nonumber\\
\leq &  g_2(\bm{V}(P)-\bm{a})+g_2(\bm{C}(P)-\bm{V}(P))\nonumber\\
=& f(\bm{V}(P))+g_2(\bm{C}(P)-\bm{V}(P)).\label{eq_lem_ratio_3}
\end{align}
At time $V_i(P)$, all tasks of job $i$ have started service. If $k_i> m$, then job $i$ has at most $m$ incomplete tasks at time $V_i(P)$ because there are only $m$ servers. If $k_i\leq m$, then job $i$ has at most $k_i$ incomplete tasks at time $V_i(P)$. Therefore, at most $k_i\wedge m$ tasks of job $i$ are in service at time $V_i(P)$. Let $X_{i,l}$ denote the random service time of the $l$-th remaining task of job $i$. 
We will prove that for all $\mathcal{I}$
\begin{align}\label{eq_order_good}
[\bm{C}(P)-\bm{V}(P) | \mathcal{I}]\leq_{\text{st}}\left[\bigg(\max_{l=1,\ldots,k_1 \wedge m} X_{1,l},\ldots,\max_{l=1,\ldots,k_n \wedge m} X_{n,l}\bigg)\bigg| k_1,\ldots,k_n\right].
\end{align}
Without loss of generality, suppose that at time $V_i(P)$, the remaining tasks of job $i$ are being executed by the set of servers $\mathcal{S}_i\subseteq\{1,\ldots,m\}$, which satisfies $|\mathcal{S}_i|\leq k_i \wedge m$. Hence, the $X_{i,l}$'s are \emph{i.i.d.} In policy $P$, let $\chi_{i,l}$ denote the amount of time that was spent on executing the $l$-th remaining task of job $i$ before time $V_i(P)$, and let $R_{i,l}$ denote the remaining service time to complete this task after time $V_i(P)$. Then, $R_{i,l}$ can be expressed as $R_{i,l} = [X_{i,l} - \chi_{i,l} | X_{i,l} > \chi_{i,l}]$. Suppose that in policy $P$, $V_{j_i}(P)$ associated with job $j_i$ is the $i$-th smallest component of the vector $\bm{V}(P)$, i.e., $V_{j_i}(P)=V_{(i)}(P)$. We prove \eqref{eq_order_good} by using an inductive argument supported by Theorem 6.B.3 of \cite{StochasticOrderBook}, which contains two steps.

\emph{Step 1: We first show that for all $\mathcal{I}$} 
\begin{align}\label{eq_order_good1}
[{C}_{j_1}(P)-V_{j_1}(P)|\mathcal{I}] \leq_{\text{st}}  \left[\max_{{l=1,\ldots,k_{j_1} \wedge m}} X_{j_1,l}\bigg|\mathcal{I}\right].
\end{align}
Because the $X_{i,l}$'s are \emph{i.i.d.} NBU, for all realizations of $j_1$ and $\chi_{j_1,l}$, we have
\begin{align}
[R_{j_1,l}|j_1,\chi_{j_1,l}] \leq_{\text{st}} [X_{j_1,l}| j_1],~\forall~l\in \mathcal{S}_{j_1}.\label{eq_order_good4}
\end{align}
Lemma \ref{lem_independent} tells us that 
the $R_{j_1,l}$'s are conditional independent for any given realization of $\{\chi_{{j_1},l},l\in \mathcal{S}_{j_1}\}$. Hence, for all realizations of $j_1$, $\mathcal{S}_{j_1}$, and $\{\chi_{{j_1},l},l\in \mathcal{S}_{j_1}\}$
\begin{align}
&~~[{C}_{j_1}(P)-V_{j_1}(P)|{j_1}, \mathcal{S}_{j_1},\{\chi_{j_1,l}, l\in \mathcal{S}_{j_1}\}] \nonumber\\
&=  [\max_{l\in \mathcal{S}_{j_1}} R_{j_1,l} |{j_1},\mathcal{S}_{j_1},\{\chi_{j_1,l}, l\in \mathcal{S}_{j_1}\}] \nonumber\\
&\leq_{\text{st}}  [\max_{l\in \mathcal{S}_{j_1}} X_{j_1,l} |{j_1},\mathcal{S}_{j_1}]\label{eq_order_good2}\\
& \leq [\max_{l=1,\ldots,k_{j_1} \wedge m} X_{j_1,l} |{j_1}],\label{eq_order_good3}
\end{align}
where in \eqref{eq_order_good2} we have used \eqref{eq_order_good4} and Theorem 6.B.14 of \cite{StochasticOrderBook}, and in \eqref{eq_order_good3} we have used $|\mathcal{S}_i|\leq k_i \wedge m$. Because ${j_1}$, $\mathcal{S}_{j_1}$, and $\{\chi_{j_1,l}, l\in \mathcal{S}_{j_1}\}$
 are random variables which depend on  the job parameters $\mathcal{I}$, by using Theorem 6.B.16(e) of \cite{StochasticOrderBook},  \eqref{eq_order_good1} is proven.

\emph{Step 2: We show that for all given $\mathcal{I}$ and $\{{C}_{j_i}(P),V_{j_i}(P), i=1,\ldots h\}$} 
\begin{align}\label{eq_order_good6}
[{C}_{j_{h+1}}(P)-V_{j_{h+1}}(P)|\mathcal{I},\{{C}_{j_i}(P),V_{j_i}(P), i=1,\ldots h\}] \leq_{\text{st}}  \left[\max_{{l=1,\ldots,k_{j_{h+1}} \wedge m}} X_{j_{h+1},l}\bigg| \mathcal{I}\right].
\end{align}
Similar with \eqref{eq_order_good3}, for all realizations of $j_{h+1}$, $\mathcal{S}_{j_{h+1}}$, and $\{\chi_{j_{h+1},l}, l\in \mathcal{S}_{j_{h+1}}\}$, we can get
\begin{align}
[{C}_{j_{h+1}}(P)-V_{j_{h+1}}(P)|j_{h+1},\mathcal{S}_{j_{h+1}},\{\chi_{j_{h+1},l}, l\in \mathcal{S}_{j_{h+1}}\}] \leq_{\text{st}} [\max_{{l=1,\ldots,k_{j_{h+1}} \wedge m}} X_{j_{h+1},l}|{j_{h+1}}].\nonumber
\end{align}
Because $j_{h+1}$, $\mathcal{S}_{j_{h+1}}$, and $\{\chi_{j_{h+1},l}, l\in \mathcal{S}_{j_{h+1}}\}$
 are random variables which are determined by $\mathcal{I}$ and $\{{C}_{j_i}(P),V_{j_i}(P), i=1,\ldots h\}$, 
by using Theorem 6.B.16(e) of \cite{StochasticOrderBook}, \eqref{eq_order_good6} is proven.
By \eqref{eq_order_good1}, \eqref{eq_order_good6}, and Theorem 6.B.3 of \cite{StochasticOrderBook}, we have
 \begin{align}
&[\bm{C}(P)-\bm{V}(P) | \mathcal{I}]\nonumber\\
\leq_{\text{st}} &\left[\bigg(\max_{l=1,\ldots,k_1 \wedge m} X_{1,l},\ldots,\max_{l=1,\ldots,k_n \wedge m} X_{n,l}\bigg)\bigg| \mathcal{I}\right] \nonumber\\
=~ & \left[\bigg(\max_{l=1,\ldots,k_1 \wedge m} X_{1,l},\ldots,\max_{l=1,\ldots,k_n \wedge m} X_{n,l}\bigg)\bigg| k_1,\ldots,k_n\right].\nonumber
\end{align}
%where in the last step we have used that given $(k_1,\ldots, k_n)$, $\mathcal{I}$ is independent of $(\max_{l=1,\ldots,k_1 \wedge m} X_{1,l},$ $\ldots,\max_{l=1,\ldots,k_n \wedge m} X_{n,l})$. 
Hence, \eqref{eq_order_good} holds in policy $P$.

In policy $\pi$, $k_i$ tasks of job $i$ must be accomplished to complete job $i$. Hence, using the above arguments again, yields   
\begin{align}\label{eq_order_good7}
\left[\bigg(\max_{l=1,\ldots,k_1 \wedge m} X_{1,l},\ldots,\max_{l=1,\ldots,k_n \wedge m} X_{n,l}\bigg)\bigg| k_1,\ldots,k_n\right]\leq_{\text{st}} [\bm{C}(\pi) - \bm{a}| \mathcal{I}].
\end{align}
Combining \eqref{eq_order_good1} and \eqref{eq_order_good7}, we have
\begin{align}
[\bm{C}(P)-\bm{V}(P) | \mathcal{I}]\leq_{\text{st}} [\bm{C}(\pi) - \bm{a}| \mathcal{I}].\nonumber\end{align}
Because $g_2$ is increasing, by Theorem 6.B.16(a) of \cite{StochasticOrderBook}
\begin{align}\label{eq_order_good8}
[g_2(\bm{C}(P)-\bm{V}(P))|\mathcal{I}] \leq_{\text{st}}  [g_2(\bm{C}(\pi) - \bm{a})|\mathcal{I}] = [f(\bm{C}(\pi))|\mathcal{I}].
\end{align}
By substituting \eqref{eq_ratio_0} and \eqref{eq_order_good8} into \eqref{eq_lem_ratio_3}, \eqref{eq_ratio_1} is proven. This completes the proof.
\end{proof}

\section{Proof of Proposition~\ref{ordering_2}}\label{app_lem2}
Let $j$ be any integer chosen from $\{1,\ldots,n\}$, and $y_{j}$ be the number of jobs that have arrived by the time  $c_{(j)}(\pi)$, where $y_{j}\geq j$. Because $j$ jobs are completed by the time $c_{(j)}(\pi)$ in policy $\pi$, 
there are exactly $(y_{j}-j)$ incomplete jobs in the system at time $c_{(j)}(\pi)$. By the definition of the system state, we have $\xi_{[i],\pi}(c_{(j)}(\pi))=0$ for $i=y_{j}-j+1,\ldots,n$. Hence,
%the system state of policy $\pi$ satisfies 
\begin{align}
\sum_{i=y_{j}-j+1}^n\xi_{[i],\pi}(c_{(j)}(\pi))=0.\nonumber
\end{align}
Combining this with \eqref{eq_ordering_2_1}, yields that policy $P$ satisfies 
%Hence, there are $y-1$ unfinished jobs at time $c_{(1)}(\pi)$ such that
%Invoking Lemma \ref{lemG4}, we can obtain
\begin{align}\label{eq_proof_1}
\sum_{i=y_{j}-j+1}^n \gamma_{[i],P}\left(c_{(j)}(\pi)\right)\leq 0.
\end{align}
Further, the definition of the system state tells us that $ \gamma_{i,P}\left(t\right)\geq0$ holds for all $i=1,\ldots,n$ and $t\geq0$. Hence, we have
\begin{align}\label{eq_proof_2}
\gamma_{[i],P}\left(c_{(j)}(\pi)\right)=0, ~\forall~i=y_j-j+1,\ldots,n.
\end{align}
Therefore, there are at most $y_j-j$ jobs which have unassigned tasks at time  $c_{(j)}(\pi)$ in policy $P$.
Because  the sequence of job arrival times $a_1,a_2,\ldots,a_n$ are invariant under any policy, $y_j$ jobs have arrived by the time  $c_{(j)}(\pi)$ in policy $P$. Thus, there are at least $j$ jobs which have no unassigned tasks  at the time  $c_{(j)}(\pi)$  in policy $P$, which can be equivalently expressed as
\begin{align}\label{eq_proof_222}
v_{(j)}(P)\!  \leq c_{(j)}(\pi).
\end{align}
Because $j$ is arbitrarily chosen, \eqref{eq_proof_222} holds for all $j=1,\ldots,n$, which is exactly \eqref{eq_ordering_2_2}. In addition, \eqref{eq_ordering_2_3} follows from \eqref{eq_ordering_2_2}, which completes the proof.


%Suppose that there are $l$ unfinished jobs at time $t$ in policy $\pi$, then $\sum_{i=l+1}^n {\xi}_{[i],\pi}(t)=0$. By \eqref{eq_ordering_1_1}, we get $\sum_{i=l+1}^n {\xi}_{[i],P}(t)=0$ and hence there are at most $l$ unfinished jobs in policy $P$. In other words, there are at least as many unfinished jobs in policy $\pi$ as in policy $P$ at any time $t\in[0,\infty)$. This implies \eqref{eq_ordering_1_1_2}, because the sequence of job arrival times $a_1,a_2,\ldots$ are invariant under any policy. In addition, \eqref{eq_ordering_1_2} follows from \eqref{eq_ordering_1_1_2}, which completes the proof.

%In policy $P$, there are at most $y_1$ jobs in the system at time $c_{(1)}(\pi)$ because only $y_1$ jobs have arrived by time $c_{(1)}(\pi)$. Hence, the system state of policy $P$ must satisfy
%\begin{align}\label{eq_proof_2}
% \gamma_{[i],P}\left(c_{(1)}(\pi)\right)=0,\forall~i=y_1\!+\!1,y_1\!+\!2,\ldots \!\!
%\end{align}
%Combining \eqref{eq_proof_1}, \eqref{eq_proof_2}, and the fact that $ \gamma_{i,P}\left(t\right)\geq0$ for all $i=1,\ldots,n$ and $t\geq0$, we can obtain
%%Combining \eqref{eq_proof_0}, \eqref{eq_proof_1}, and the fact that $\alpha_h(t)\geq\delta_h(t)$ for all $i,t$, yields
%\begin{align}\label{eq_proof_3}
% \gamma_{[y_1],P}\left(c_{(1)}(\pi)\right)=0.
%\end{align}
%Let $w_1$ be the index of the job associated to the $y_1$-th largest component of $\bm{\gamma}_P(t)$ at time $c_{(1)}(\pi)$. Then, \eqref{eq_proof_3} tells us that in policy $P$, all tasks of job $w_1$ are either completed or under service at time $c_{(1)}(\pi)$. Hence, \eqref{eq_Condition_3_1} is proven.
%
%Then, by using similar arguments in \eqref{eq_proof_1}-\eqref{eq_proof_3}, we can obtain that at time $c_{(j+1)}(\pi)$ the system state of policy $P$ satisfies
%\begin{align}\label{eq_proof_4}
%\gamma_{[i],P}(c_{(j+1)}(\pi))=0
%\end{align}
%for each $i=y_{j+1}\!-\!j,y_{j+1}\!-\!j+1,\ldots,y_{j+1}$.
%Notice that there are $j+1$ jobs satisfying \eqref{eq_proof_4}. Hence, at least one of these $j+1$ jobs is different from the jobs $w_1,w_2,\ldots,w_j$. Let $w_{j+1}$ be the index of this job. Then, \eqref{eq_proof_4} tells us that in policy $P$, all tasks of job $w_{j+1}$ are either completed or under service at time $c_{(j+1)}(\pi)$. Hence, \eqref{eq_proof_9} is proven.
%
%By induction, we can obtain
%\begin{align}
%v_{w_{j}}(P) \leq c_{(j)}(\pi),~j=1,\ldots,n. \nonumber
%\end{align}
%By the construction of $w_1,w_2,\ldots, w_{n}$, we have 
%\begin{align}\label{eq_proof_101}
%v_{w_{1}}(P)\leq v_{w_{2}}(P)\leq
%\ldots\leq v_{w_{n}}(P).
%\end{align}
%Because $v_{(j)}(P)$ is the $j$-th smallest components of $\bm{v}(P)$, it follows that 
%\begin{align}
%v_{(j)}(P)\! \leq \!\max_{i=1,\ldots,j}v_{w_{i}}(P) = v_{w_{j}}(P)\leq c_{(j)}(\pi),~j=1,\ldots,n.\nonumber
%\end{align}
%Hence, \eqref{eq_ordering_2_2} is proven. Form this, \eqref{eq_ordering_2_3} follows directly, which completes the proof.
%
%
%We prove \eqref{eq_ordering_2_2} by induction. 
%
%\emph{Step 1: We first show that there exists a job $w_1$ such that}
%\begin{align}\label{eq_Condition_3_1}
%v_{w_1}(P) \leq c_{(1)}(\pi).
%\end{align}
%
%In policy $\pi$, the first job departure occurs at time $c_{(1)}(\pi)$. Let $y_1$ be the number of jobs that have arrived by time $c_{(1)}(\pi)$. Then, there are $y_1-1$ incomplete jobs at time $c_{(1)}(\pi)$ in policy $\pi$. Hence, the system state of policy $\pi$ satisfies ${\xi}_{[i],\pi}\left(c_{(1)}(\pi)\right)=0$ for all $i=y_1,y_1+1,\ldots,n$ at time $c_{(1)}(\pi)$. By taking the summation, we have
%\begin{align}\label{eq_proof_0}
%\sum_{i=y_1}^n {\xi}_{[i],\pi}\left(c_{(1)}(\pi)\right)=0.
%\end{align}
%This and  \eqref{eq_ordering_2_1} imply that the system state of policy $P$ satisfies 
%%Hence, there are $y-1$ unfinished jobs at time $c_{(1)}(\pi)$ such that
%%Invoking Lemma \ref{lemG4}, we can obtain
%\begin{align}\label{eq_proof_1}
%\sum_{i=y_1}^n \gamma_{[i],P}\left(c_{(1)}(\pi)\right)\leq 0.
%\end{align}
%In policy $P$, there are at most $y_1$ jobs in the system at time $c_{(1)}(\pi)$ because only $y_1$ jobs have arrived by time $c_{(1)}(\pi)$. Hence, the system state of policy $P$ must satisfy
%\begin{align}\label{eq_proof_2}
% \gamma_{[i],P}\left(c_{(1)}(\pi)\right)=0,\forall~i=y_1\!+\!1,y_1\!+\!2,\ldots \!\!
%\end{align}
%Combining \eqref{eq_proof_1}, \eqref{eq_proof_2}, and the fact that $ \gamma_{i,P}\left(t\right)\geq0$ for all $i=1,\ldots,n$ and $t\geq0$, we can obtain
%%Combining \eqref{eq_proof_0}, \eqref{eq_proof_1}, and the fact that $\alpha_h(t)\geq\delta_h(t)$ for all $i,t$, yields
%\begin{align}\label{eq_proof_3}
% \gamma_{[y_1],P}\left(c_{(1)}(\pi)\right)=0.
%\end{align}
%Let $w_1$ be the index of the job associated to the $y_1$-th largest component of $\bm{\gamma}_P(t)$ at time $c_{(1)}(\pi)$. Then, \eqref{eq_proof_3} tells us that in policy $P$, all tasks of job $w_1$ are either completed or under service at time $c_{(1)}(\pi)$. Hence, \eqref{eq_Condition_3_1} is proven.
%%\begin{align}%\label{eq_proof_9}
%%U_{w_1}(P) \leq c_{(1)}(\pi),\nonumber
%%\end{align}
%%which implies \eqref{eq_Condition_3_1}.
%
%\emph{Step 2: Assume that there exist $j$ jobs indexed by $w_1,w_2,$ $\ldots,w_j$ such that
%\begin{align}
%v_{w_i}(P) \leq c_{(i)}(\pi),~i=1,\ldots,j,\nonumber
%\end{align}
%we will show that there exists a job $w_{j+1}$ such that  $w_{j+1}$ is different from $w_1,w_2,\ldots,w_j$ and}
%\begin{align}\label{eq_proof_9}
%v_{w_{j+1}}(P) \leq c_{(j+1)}(\pi).
%\end{align}
%%Since preemption is not allowed, these $\delta_y\left(c_{(1)}(\pi)\right)$ tasks will be under service in policy $P$ until completion. Let $w_1$ be the index of the job associated to the coordinate $y$ at time $c_{(1)}(\pi)$. According to \eqref{eq_def_state}, we can obtain $\delta_y\left(c_{(1)}(\pi)\right)\leq \min[k_{w_1},M].$ Therefore, the time duration between $c_{(1)}(\pi)$ and $c_{w_1,\text{FUT-NR}}$ is no more than the time to complete $\min[k_{w_1},M]$ tasks of job $w_1$.
%Let $y_{j+1}$ denote the number of jobs that have arrived by time  $c_{(j+1)}(\pi)$, where $y_{j+1}\geq j+1$. Because $(j+1)$ jobs are completed during $[0,c_{(j+1)}(\pi)]$ in policy $\pi$, 
%there are $(y_{j+1}-j-1)$ incomplete jobs at time $c_{(j+1)}(\pi)$. Hence, the system state of policy $\pi$ satisfies 
%\begin{align}
%\sum_{i=y_{j+1}-j}^n\xi_{[i],\pi}(c_{(j+1)}(\pi))=0.\nonumber
%\end{align}
%Then, by using similar arguments in \eqref{eq_proof_1}-\eqref{eq_proof_3}, we can obtain that at time $c_{(j+1)}(\pi)$ the system state of policy $P$ satisfies
%\begin{align}\label{eq_proof_4}
%\gamma_{[i],P}(c_{(j+1)}(\pi))=0
%\end{align}
%for each $i=y_{j+1}\!-\!j,y_{j+1}\!-\!j+1,\ldots,y_{j+1}$.
%Notice that there are $j+1$ jobs satisfying \eqref{eq_proof_4}. Hence, at least one of these $j+1$ jobs is different from the jobs $w_1,w_2,\ldots,w_j$. Let $w_{j+1}$ be the index of this job. Then, \eqref{eq_proof_4} tells us that in policy $P$, all tasks of job $w_{j+1}$ are either completed or under service at time $c_{(j+1)}(\pi)$. Hence, \eqref{eq_proof_9} is proven.
%
%By induction, we can obtain
%\begin{align}
%v_{w_{j}}(P) \leq c_{(j)}(\pi),~j=1,\ldots,n. \nonumber
%\end{align}
%By the construction of $w_1,w_2,\ldots, w_{n}$, we have 
%\begin{align}\label{eq_proof_101}
%v_{w_{1}}(P)\leq v_{w_{2}}(P)\leq
%\ldots\leq v_{w_{n}}(P).
%\end{align}
%Because $v_{(j)}(P)$ is the $j$-th smallest components of $\bm{v}(P)$, it follows that 
%\begin{align}
%v_{(j)}(P)\! \leq \!\max_{i=1,\ldots,j}v_{w_{i}}(P) = v_{w_{j}}(P)\leq c_{(j)}(\pi),~j=1,\ldots,n.\nonumber
%\end{align}
%Hence, \eqref{eq_ordering_2_2} is proven. Form this, \eqref{eq_ordering_2_3} follows directly, which completes the proof.


==> v3/appendices_lem2_0.tex <==
\section{Proof  of Proposition \ref{lem2_0}} \label{app_lem2_0}

The proof of Proposition \ref{lem2_0} requires the following two lemmas:

\begin{lemma}\label{lem_non_prmp1_thm3_0}
Suppose that, in policy $P$, $\{\bm{\xi}_P',\bm{\gamma}_P'\}$ is obtained by completing $b_P$ tasks in the system whose state is $\{\bm{\xi}_P,\bm{\gamma}_P\}$. Further, suppose that, in policy $\pi$, $\{\bm{\xi}_\pi',\bm{\gamma}_\pi'\}$ is obtained by completing $b_\pi$ tasks in the system whose state is $\{\bm{\xi}_\pi,\bm{\gamma}_\pi\}$.
If $b_P\geq b_\pi$, condition 3 of Proposition \ref{lem2_0} is satisfied in policy $P$, and
\begin{eqnarray}
\sum_{i:d_i\leq\tau} \xi_{i,P}\leq \sum_{i:d_i\leq\tau} \xi_{i,\pi}, ~\tau\in[0,\infty),\nonumber
\end{eqnarray}
then
\begin{eqnarray}\label{eq_non_prmp_40_thm3_0}
\sum_{i:d_i\leq\tau} \xi_{i,P}'\leq \sum_{i:d_i\leq\tau} \xi_{i,\pi}', ~\tau\in[0,\infty).\end{eqnarray}
\end{lemma}

\begin{proof}
If $\sum_{i:d_i\leq\tau} \xi_{i,P}'=0$, then the inequality \eqref{eq_non_prmp_40_thm3} follows naturally. 
If $\sum_{i:d_i\leq\tau} \xi_{i,P}'>0$, then there exist some remaining tasks. 
In policy $P$, each task completing service is from the job with the earliest due time. Hence,
$\sum_{i:d_i\leq\tau} \xi_{i,P}'=\sum_{i:d_i\leq\tau} \xi_{i,P} - b_P \leq \sum_{i:d_i\leq\tau} \xi_{i,\pi} -b_\pi \leq \sum_{i:d_i\leq\tau} \xi_{i,\pi}'$.
\end{proof}


\begin{lemma}\label{lem_non_prmp2_thm3_0}
Suppose that under policy $P$, $\{\bm{\xi}_P',\bm{\gamma}_P'\}$ is obtained by adding a job with $b$ tasks and due time $d$ to the system whose state is $\{\bm{\xi}_P,\bm{\gamma}_P\}$. Further, suppose that under policy $\pi$, $\{\bm{\xi}_\pi',\bm{\gamma}_\pi'\}$ is obtained by adding a job with $b$ tasks and due time $d$ to the system whose state is $\{\bm{\xi}_\pi,\bm{\gamma}_\pi\}$.
If
\begin{eqnarray}
\sum_{i:d_i\leq\tau} \xi_{i,P}\leq \sum_{i:d_i\leq\tau} \xi_{i,\pi}, ~\tau\in[0,\infty),\nonumber
\end{eqnarray}
then
\begin{eqnarray}
\sum_{i:d_i\leq\tau} \xi_{i,P}'\leq \sum_{i:d_i\leq\tau} \xi_{i,\pi}', ~\tau\in[0,\infty).\nonumber\end{eqnarray}
\end{lemma}

\begin{proof}
If $d\leq\tau$, then
$\sum_{i:d_i\leq\tau} \xi_{i,P}'\leq \sum_{i:d_i\leq\tau} \xi_{i,P} + b\leq \sum_{i:d_i\leq\tau} \xi_{i,\pi}+b \leq \sum_{i:d_i\leq\tau} \xi_{i,\pi}'$.

If $d>\tau$, then
$\sum_{i:d_i\leq\tau} \xi_{i,P}'\leq \sum_{i:d_i\leq\tau} \xi_{i,P} \leq \sum_{i:d_i\leq\tau} \xi_{i,\pi} \leq \sum_{i:d_i\leq\tau} \xi_{i,\pi}'$.
\end{proof}


\begin{proof}[Proof of Proposition \ref{lem2_0}]

Because policy $P$ is more work-efficient than policy $\pi$, the task completion times in policy $P$ are smaller  than those in policy $\pi$, i.e., 
\begin{align}
(t_{1,P},\ldots, t_{k_{\text{sum}},P}) \leq(t_{1,\pi},\ldots, t_{k_{\text{sum}},\pi}). \nonumber
\end{align} 

We modify the sample-path of policy $P$ as follows:  Suppose that for each $i=1,\ldots, k_{\text{sum}}$  a task of job $j_i$ is completed at time $t_{i,P}$ on the original sample-path of policy $P$, then on the modified sample-path of policy $P$ a task of job $j_i$ is completed at time $t_{i,\pi}$. Hence, the task completion times of policy $P$ are postponed after the modification, but the order of completed tasks remain the same. 
Let $\hat{\bm{\xi}}_{P}(t) =(\hat{\xi}_{1,P}(t),\ldots,\hat{\xi}_{n,P}(t))$ and $\hat{\bm{\gamma}}_{P}(t) =(\hat{\gamma}_{1,P}(t),\ldots,\hat{\gamma}_{n,P}(t))$ denote the system state on the modified sample-path of policy $P$. Then, at any time $t$ we can get ${\xi}_{i,P}(t)  \leq \hat{\xi}_{i,P}(t) $ for $i=1,\ldots,n$ and hence
\begin{align}\label{eq_lem2_0_proof_1}
\sum_{i:d_i\leq\tau} {\xi}_{i,P}(t)\leq \sum_{i:d_i\leq\tau} \hat{\xi}_{i,P}(t), ~\tau\in[0,\infty).
\end{align}

Next, we compare policy $\pi$ with the modified sample-path of policy $P$. By the foregoing construction, \emph{the task completion times are identical on the sample-path of policy $\pi$ and on the modified sample-path of policy $P$.}
 
On the original sample-path of policy $P$, each task completing service  is from the job with the earliest due time among all jobs in the queue. Furthermore, because $k_1\leq k_2\leq \ldots\leq k_n$, later arrived jobs have more tasks. Hence, on the modified sample-path of policy $P$, each task completing service  is also from the job with the earliest due time among all jobs in the queue. In other words, \emph{condition 3 of Proposition \ref{lem2_0} is satisfied on the modified sample-path of policy $P$}. 

Because $\hat{\bm{\xi}}_{P}(0) = {\bm{\xi}}_{\pi}(0) =\bm{0}$, by using Lemma \ref{lem_non_prmp1_thm3_0} and Lemma \ref{lem_non_prmp2_thm3_0}, and taking an induction on the job arrival events and task completion events over time, we can obtain for all $t\in[0,\infty)$
% Then, by using the arguments in \cite{Smith78} we can show 
\begin{align}\label{eq_lem2_0_proof_2}
\sum_{i:d_i\leq\tau} \hat{\xi}_{i,P}(t)\leq \sum_{i:d_i\leq\tau} {\xi}_{i,\pi}(t), ~i=1,2,\ldots,n.
\end{align}
Combining \eqref{eq_lem2_0_proof_1} and \eqref{eq_lem2_0_proof_2}, yields \eqref{eq_ordering_3_1}. Then, \eqref{eq_ordering_3_2} follow from Lemma \ref{ordering_3}, which completes the proof. \end{proof}



==> v3/appendices_lem3.tex <==
\section{Proofs of Proposition~\ref{ordering_3} and Proposition~\ref{ordering_3_1}}\label{app_lem3}
\begin{proof}[Proof of Proposition~\ref{ordering_3}]
Let $w_i$ be the index of the job associated with the job completion time $c_{(i)}(P)$. In order to prove \eqref{eq_ordering_3_2}, it is sufficient to show that for each $j=1,2,\ldots,n$,
\begin{align}\label{eq_Condition_3_12_thm3}
c_{w_j}(P)-d_{w_j} \leq \max_{i=1,2,\ldots,n }[c_{i}(\pi)-d_i].
\end{align}
We prove \eqref{eq_Condition_3_12_thm3} by contradiction. \emph{For this, let us assume that 
\begin{align}\label{eq_proof_9_thm3}
c_{i}(\pi)< c_{w_j}(P) 
\end{align}
holds for all job $i$ satisfying $a_i\leq c_{w_j}(P)$ and $d_i\leq d_{w_j}$.} That is, if job $i$ arrives before time $c_{w_j}(P)$ and its due time is no later than $d_{w_j}$, then  job $i$ is completed before time $c_{w_j}(P)$ in policy $\pi$.
Define  
\begin{align}\label{eq_def}
\tau_j=\max_{i:a_i\leq c_{w_j}(P),d_i\leq d_{w_j}} c_{i}(\pi).
\end{align} 
According to \eqref{eq_proof_9_thm3} and \eqref{eq_def}, we can obtain
\begin{align}\label{eq_proof_19_thm3}
\tau_j<c_{w_j}(P).
\end{align}


On the other hand, \eqref{eq_def} tells us that all job  $i$ satisfying $d_i\leq d_{w_j}$ and $a_i\leq c_{w_j}(P)$ are completed by time $\tau_j$ in policy $\pi$. 
By this,
%$d_i> d_{w_j}$ holds for all job $i$ in the queue in policy $\pi$. 
the system state of policy $\pi$ satisfies  
\begin{align}
\sum_{i:d_i\leq d_{w_j}}\xi_{i,\pi}(\tau_j) =0.\nonumber
\end{align}
Combining this with \eqref{eq_ordering_3_1}, yields
%Hence, there are $y-1$ unfinished jobs at time $C_{w_1}(\pi)$ such that
%Invoking Lemma \ref{lemG4}, we can obtain
\begin{align}\label{eq_proof_1_thm3}
\sum_{i:d_i\leq d_{w_j}} \xi_{i,P}(\tau_j)\leq 0.
\end{align}
Further, the definition of the system state tells us that $\xi_{i,P}(t)\geq0$ for all $i=1,\ldots,n$ and $t\geq0$. Using this and \eqref{eq_proof_1_thm3}, we get that job $w_j$ satisfies
\begin{align}
\xi_{w_j,P}(\tau_j)= 0.\nonumber
\end{align}
That is, all tasks of job $w_j$ are completed by time $\tau_j$ in policy $P$. Hence, $c_{w_j}(P)\leq \tau_j$, where contradicts with \eqref{eq_proof_19_thm3}. Therefore, there exists at least one job $i$ satisfying the conditions 
$a_i\leq c_{w_j}(P)$, $d_i\leq d_{w_j}$, and $c_{w_j}(P) \leq c_{i}(\pi)$. This can be equivalently expressed as
\begin{align}\label{eq_proof_3_thm3}
c_{w_j}(P) \leq \max_{i:a_i\leq c_{w_j}(P),d_i\leq d_{w_j} }c_{i}(\pi).
\end{align}
Hence, for each $j=1,2,\ldots,n$,
\begin{align}
c_{w_j}(P)-d_{w_j} &\leq \max_{i:a_i\leq c_{w_j}(P),d_i\leq d_{w_j} }c_{i}(\pi)-d_{w_j} \nonumber\\
& \leq \max_{i:a_i\leq c_{w_j}(P),d_i\leq d_{w_j} }[c_{i}(\pi)-d_{i}]\nonumber\\
&\leq \max_{i=1,2,\ldots,n }[c_{i}(\pi)-d_i].\nonumber
\end{align}
This implies \eqref{eq_ordering_3_2}. Hence, Proposition~\ref{ordering_3} is proven.
\end{proof}
The proof of Proposition~\ref{ordering_3_1} is almost identical with that of 
Proposition~\ref{ordering_3}, and hence is not repeated here. The only difference is that $c_{w_j}(P)$ and $\bm{\xi}_{P}(\tau_j)$ in the proof of Proposition~\ref{ordering_3} should be replaced by $v_{w_j}(P)$ and $\bm{\gamma}_{P}(\tau_j)$, respectively.



==> v3/appendices_version2.tex <==
% !TEX root = ./replication.tex
\section{Proof of Proposition \ref{lem1}} \label{app0}

The following two lemmas are needed to prove Proposition \ref{lem1}:  

\begin{lemma}\label{lem_non_prmp1}
Suppose that under policy $P$, $\{\bm{\xi}_{P}',\bm{\gamma}_{P}'\}$ is obtained by allocating $b_P$ unassigned tasks to the servers in the system whose state is $\{\bm{\xi}_{P},\bm{\gamma}_{P}\}$. Further, suppose that under policy $\pi$, $\{\bm{\xi}_{\pi}',\bm{\gamma}_{\pi}'\}$ is obtained by completing $b_\pi$ tasks in the system whose state is $\{\bm{\xi}_{\pi},\bm{\gamma}_{\pi}\}$.
If $b_P\geq b_\pi$, condition 2 of Proposition \ref{lem1} is satisfied in policy $P$, and
\begin{eqnarray}\label{eq_non_prmp_41}
\sum_{i=j}^n {\gamma}_{[i],P}\leq \sum_{i=j}^n {\xi}_{[i],\pi}, ~\forall~j = 1,2,\ldots,n,\nonumber
\end{eqnarray}
then
\begin{eqnarray}\label{eq_non_prmp_40}
\sum_{i=j}^n {\gamma}_{[i],P}'\leq \sum_{i=j}^n {\xi}_{[i],\pi}', ~\forall~j = 1,2,\ldots,n.
\end{eqnarray}
\end{lemma}

\begin{proof}
%The proof is similar to that of Lemma 2 in \cite{Smith78}.
If $\sum_{i=j}^n {\gamma}_{[i],P}'=0$, then the inequality \eqref{eq_non_prmp_40} follows naturally. 
If $\sum_{i=j}^n {\gamma}_{[i],P}'>0$, then there exist  unassigned tasks which have not been assigned to any server. 
In policy $P$, each task allocated to the servers is from the job with the minimum positive ${\gamma}_{i,P}$. Hence,
$\sum_{i=j}^n {\gamma}_{[i],P}'=\sum_{i=j}^n {\gamma}_{[i],P} - b_P \leq \sum_{i=j}^n {\xi}_{[i],\pi} - b_\pi \leq \sum_{i=j}^n {\xi}_{[i],\pi}'$.
\end{proof}


\begin{lemma}\label{lem_non_prmp2}
Suppose that, under policy $P$, $\{\bm{\xi}_{P}',\bm{\gamma}_{P}'\}$ is obtained by adding a job with $b$ tasks to the system whose state is $\{\bm{\xi}_{P},\bm{\gamma}_{P}\}$. Further, suppose that, under policy $\pi$, $\{\bm{\xi}_{\pi}',\bm{\gamma}_{\pi}'\}$ is obtained by adding a job with $b$ tasks to the system whose state is $\{\bm{\xi}_{\pi},\bm{\gamma}_{\pi}\}$.
If
\begin{eqnarray}
\sum_{i=j}^n {\gamma}_{[i],P}\leq \sum_{i=j}^n {\xi}_{[i],\pi}, ~\forall~j = 1,2,\ldots,n,\nonumber
\end{eqnarray}
then
\begin{eqnarray}
\sum_{i=j}^n {\gamma}_{[i],P}'\leq \sum_{i=j}^n {\xi}_{[i],\pi}', ~\forall~j = 1,2,\ldots,n.\nonumber
\end{eqnarray}
\end{lemma}

\begin{proof}
%The proof is similar to that of Lemma 3 in \cite{Smith78}.
Without loss of generalization, we suppose that after the job arrival, $b$ is the $l$-th largest component of $\bm{\gamma}_{P}'$ and the $m$-th largest component of $\bm{\xi}_{\pi}'$, i.e., $\gamma'_{[l],P} = \xi'_{[m],\pi}= b$. We consider the following four cases:

{Case 1}: $l<j, m<j$. We have $\sum_{i=j}^n {\gamma}_{[i],P}' =\sum_{i=j-1}^n {\gamma}_{[i],P} \leq \sum_{i=j-1}^n {\xi}_{[i],\pi}= \sum_{i=j}^n {\xi}_{[i],\pi}'$.

{Case 2}: $l<j, m\geq j$. We have $\sum_{i=j}^n {\gamma}_{[i],P}' =\sum_{i=j-1}^n {\gamma}_{[i],P} \leq b + \sum_{i=j}^n {\gamma}_{[i],P} \leq b + \sum_{i=j}^n {\xi}_{[i],\pi} = \sum_{i=j}^n {\xi}_{[i],\pi}'$.

{Case 3}: $l\geq j, m<j$. We have $\sum_{i=j}^n {\gamma}_{[i],P}' = b + \sum_{i=j}^n {\gamma}_{[i],P} \leq \sum_{i=j-1}^n {\gamma}_{[i],P} \leq \sum_{i=j-1}^n {\xi}_{[i],\pi} = \sum_{i=j}^n {\xi}_{[i],\pi}'$.

{Case 4}: $l\geq j, m\geq j$. We have $\sum_{i=j}^n {\gamma}_{[i],P}' = b + \sum_{i=j}^n {\gamma}_{[i],P} \leq b + \sum_{i=j}^n {\xi}_{[i],\pi} = \sum_{i=j}^n {\xi}_{[i],\pi}'$.
\end{proof}

We now use Lemma \ref{lem_non_prmp1} and Lemma \ref{lem_non_prmp2} to prove Proposition \ref{lem1}.
\ifreport
\begin{proof}[Proof of Proposition \ref{lem1}]
\else
\begin{proof}[of Proposition \ref{lem1}]
\fi

Assume that no task is completed at the job arrival times $a_i$ for $i=1,\ldots,n$. This does not lose any generality, because if a task is completed at time $t_j=a_i$, Proposition \ref{lem1} can be proven by first proving for the case $t_j=a_i+\epsilon$ and then taking the limit $\epsilon\rightarrow 0$. 
We prove \eqref{eq_ordering_2_1} by induction. 

\emph{Step 1: We will show that \eqref{eq_ordering_2_1} holds during $[0,a_2)$.\footnote{Note that $a_1=0$.}} 

Because $\bm{\xi}_{P}(0^-) = \bm{\gamma}_{P}(0^-) =\bm{\xi}_{\pi}(0^-) = \bm{\gamma}_{\pi}(0^-)=\bm{0}$, \eqref{eq_ordering_2_1} holds at time $0^-$. Job 1 arrives at time $a_1=0$. By Lemma \ref{lem_non_prmp2}, \eqref{eq_ordering_2_1} holds at time $0$. Let $t$ be an arbitrarily chosen time during $(0,a_{2})$. Suppose that  $b_\pi$ tasks start execution and also complete execution during $[0,t]$ in policy $\pi$. We need to consider two cases: 

Case 1: The queue is not empty (there exist unassigned tasks in the queue) during $[0,t]$ in policy $P$. By the weak work-efficiency ordering condition, no fewer than $b_\pi$ tasks start execution during $[0,t]$ in policy $P$. Because \eqref{eq_ordering_2_1} holds at time $0$, by Lemma \ref{lem_non_prmp1}, \eqref{eq_ordering_2_1} also holds at time $t$. 

Case 2: The queue is empty (all tasks in the system are in service) by time $t'\in[0,t]$ in policy $P$. Because $t\in(0,a_{2})$ and there is no task arrival during $(0,a_2)$, there is no task arrival during $(t',t]$. Hence, it must hold that all tasks in the system are in service at time $t$. Then, the system state of policy $P$ satisfies $\sum_{i=j}^n {\gamma}_{[i],P}(t)=0$ for all $j=1,2,\ldots,n$ at time $t$. Hence, \eqref{eq_ordering_2_1} holds at time $t$. 




In summary of these two cases, \eqref{eq_ordering_2_1} holds for all $t\in[0,a_2)$.  



 


\emph{Step 2: Assume that for some integer $i\in\{2,\ldots, n\}$, the conditions of Proposition \ref{lem1} imply that \eqref{eq_ordering_2_1} holds for all $t\in[0,a_i)$. We will prove that the conditions of Proposition \ref{lem1} imply that  \eqref{eq_ordering_2_1} holds for all $t\in[0,a_{i+1})$.}


Let $t$ be an arbitrarily chosen time during $(a_i,a_{i+1})$. We modify the task completion times in policy $\pi$ as follows: For each pair of corresponding task $j$ and task $j'$ mentioned in the definition of the weak work-efficiency ordering, if 
%After this modification, the following three properties are true:
\begin{itemize}
\item In policy $\pi$, task $j$ starts execution at time $\tau\in[0,a_i]$ and completes execution at time $\nu\in(a_i,t]$,
\item In policy $P$, the queue is not empty (there exist unassigned tasks in the queue) during $[\tau,\nu]$,
\item In policy $P$, the corresponding task $j'$ starts execution at time $t'\in[0,a_i]$,
\end{itemize}
then the completion time of task $j$ is modified from $\nu$ to $a_i^-$ in policy $\pi$, as illustrated in Fig. \ref{fig_modification}.

This modification satisfies the following three claims:
\begin{itemize}
\item[1.] The system state of policy $\pi$ at time $t$ remains the same before and after this modification;
\item[2.] Policy $P$ is still weakly more work-efficient than policy $\pi$ after this modification;
\item[3.] If $b_\pi$ tasks complete execution during $[a_i,t]$ on the modified sample path of policy $\pi$, and  the queue is not empty (there exist unassigned tasks in the queue) during $[a_i,t]$ in policy $P$, then no fewer than $b_\pi$ tasks start execution during $[a_i,t]$ in policy $P$.
\end{itemize}
We now prove these three claims. Claim 1 follows from the fact that the tasks completed during $[0,t]$ remain the same before and after this modification. It is easy to prove Claim 2 by checking the definition of work-efficiency ordering. For Claim 3, notice that if a task $j$ starts execution and completes execution during $[a_i,t]$ on the modified sample path of policy $\pi$, then by Claim 2, its corresponding task $j'$ must start execution during $[a_i,t]$ in policy $P$. On the other hand, if a task $j$ starts execution during $[0,a_i]$ and completes execution during $[a_i,t]$ on the modified sample path of policy $\pi$, then by the modification, its corresponding task $j'$ must start execution during $[a_i,t]$ in policy $P$. By combining these two cases, Claim 3 follows.




\ifreport
\begin{figure}
\centering 
\includegraphics[width=0.7\textwidth]{Figures/modification} \caption{Illustration of the modification of task completion times in policy $\pi$: If in policy $\pi$, task $j$ starts execution at time $\tau\in[0,a_i]$ and completes execution at time $\nu\in(a_i,t]$, and in policy $P$, task $j'$ starts execution at time $t'\in[0,a_i]$, then the completion time of task $j$ is changed from $\nu$ to $a_i^-$ in policy $\pi$.}
\label{fig_modification} 
\end{figure} 
\fi





We use these three claims to prove the  statement of \emph{Step 2}. According to Claim 2, policy $P$ is weakly more work-efficient than policy $\pi$ after the modification. By the assumption of \emph{Step 2}, \eqref{eq_ordering_2_1} holds during $[0,a_i)$ for the modified sample path of policy $\pi$. Job $j$ arrives at time $a_i$. By Lemma \ref{lem_non_prmp2}, \eqref{eq_ordering_2_1} holds at time $a_i$ for the modified sample path of policy $\pi$. Suppose that $b_\pi$ tasks complete execution during $[a_i,t]$ on the modified sample path of policy $\pi$.
We need to consider two cases: 

Case 1: The queue is not empty (there exist unassigned tasks in the queue) during $[a_i,t]$ in policy $P$. By Claim 3, no fewer than $b_\pi$ tasks start execution during $[a_i,t]$ in policy $P$. Because \eqref{eq_ordering_2_1} holds at time $a_i$, by Lemma \ref{lem_non_prmp1}, \eqref{eq_ordering_2_1} also holds at time $t$ for the modified sample path of policy $\pi$. 

Case 2: The queue is empty (all tasks in the system are in service) at  time $t'\in[a_i,t]$ in policy $P$. Because $t\in(a_i,a_{i+1})$ and $t'\in[a_i,t]$, there is no task arrival during $(t',t]$. Hence, it must hold that all tasks in the system are in service at time $t$. Then, the system state of policy $P$ satisfies $\sum_{i=j}^n {\gamma}_{[i],P}(t)=0$ for all $j=1,2,\ldots,n$  at time $t$. Hence, \eqref{eq_ordering_2_1} holds at time $t$ for the modified sample path of policy $\pi$. 






In summary of these two cases, \eqref{eq_ordering_2_1} holds at time $t$ for the modified sample path of policy $\pi$. By Claim 1, the system state of policy $\pi$ at time $t$ remains the same before and after this modification. Hence, \eqref{eq_ordering_2_1} holds at time $t$ for the original sample path of policy $\pi$. Therefore, if  the assumption of \emph{Step 2} is true, then \eqref{eq_ordering_2_1} holds for all $t\in[0,a_{i+1})$. 

% each task (index by $j$) completed during $[0,t]$ in policy $\pi$, we modify the completion time of task $j$ as follows
%
%
%Suppose that $g$ tasks are assigned to the servers during $[a_i,t]$ in policy $P$, and $h$ tasks are completed during $[a_i,t]$ in policy $\pi$. 
%
%If $g\geq h$, then by Lemma \ref{lem_non_prmp1} tells us that \eqref{eq_ordering_2_1} holds for all $t\in(a_i,a_{i+1})$. 
%
%If $g< h$, suppose that $h'$ tasks ($h'\leq h$) are assigned to the servers during $[a_i,t]$ and are  completed during $[a_i,t]$ in policy $\pi$. Hence, $h-h'$ tasks are assigned to the servers during $[0,a_i)$ and are completed during $[a_i,t]$ in policy $\pi$. Because policy $P$ is more work-efficient than policy $\pi$,  in policy $P$ one of the following cases holds: (i) no fewer than $h'$ unassigned tasks are allocated to the servers during $[a_i,t]$, i.e., $h'\leq g$, (ii) all the remaining tasks are in service at time $t'\in[a_i,t]$, or (iii) the queue is empty at time $t'\in[a_i,t]$.
%
%
%If case (i) happens, %we can obtain that $h-h'$ tasks are assigned to the servers during $[0,a_i)$ and are completed during $[a_i,t]$ in policy $\pi$. 
% We modify the completion times of these $h-h'$ tasks such that these $h-h'$ tasks are completed at time $a_i^-$ on the modified sample path of policy $\pi$. After this modification, the conditions of Proposition \ref{lem1} still hold and the system state $\bm{\beta}(t)$ of policy $\pi$ at time $t$ remains the same. Hence, we only need to prove \eqref{eq_ordering_2_1} at time $t$ on this modified sample path of policy $\pi$. In particular, by the assumption of \emph{Step 2}, \eqref{eq_ordering_2_1} holds during $[0,a_i)$ on this modified sample path of policy $\pi$. Job $j$ arrives at time $a_i$. By Lemma \ref{lem_non_prmp2}, \eqref{eq_ordering_2_1} holds at time $a_i$ on this modified sample path of policy $\pi$. By Lemma \ref{lem_non_prmp1} and $h'\leq g$, we can obtain that \eqref{eq_ordering_2_1} holds at time $t$ on the modified sample path of policy $\pi$. Hence, \eqref{eq_ordering_2_1} also holds at time $t$ on the original sample path of policy $\pi$.
%
%
%If case (ii) happens, because there is no task arrival during $(t',t]$, it must hold that all the remaining tasks are in service at time $t$. Then, the system state of policy $P$ at time $t$ satisfies $\sum_{i=j}^n [\alpha_h(t)- \delta_h(t)]=0$ for all $h=1,2,\ldots$ Hence, \eqref{eq_ordering_2_1} holds at time $t$. If case (iii) happens, because there is no task arrival during $(t',t]$, it must hold that the queue is empty at time $t$. Similar with case (ii), we can show that \eqref{eq_ordering_2_1} holds at time $t$. In summary, if  the assumption of \emph{Step 2} is true, then \eqref{eq_ordering_2_1} holds for all $t\in[0,a_{i+1})$. 
By induction, \eqref{eq_ordering_2_1} holds at time $t\in[0,\infty)$. Then, \eqref{eq_ordering_2_2} and \eqref{eq_ordering_2_3} follow from Proposition \ref{ordering_2}.
This completes the proof.\end{proof}





==> v3/conclusion.tex <==
\section{Conclusions}\label{sec_conclusion}
In this paper, we present a comprehensive study on near delay-optimal scheduling of batch jobs in queueing systems with parallel servers. We prove that for NBU task service time distributions and for arbitrarily given job parameters, the FUT policy, EDD  policy, and the  FCFS  policy are near delay-optimal in stochastic ordering for minimizing average delay, maximum lateness, and maximum delay, respectively, among all causal and non-preemptive policies. If the job parameters satisfy some additional conditions, we can further show that these policies are near delay-optimal in stochastic ordering for minimizing three general classes of delay metrics. 


The key tools for showing these results are some novel sample-path conditions for comparing the delay performance of different policies. 
These sample-path conditions do not need to specify the queueing system model and hence can potentially be  applied to obtain near delay-optimal results for other queueing systems. One application of these sample-path conditions is in \cite{Yin_report2016}, which considered the problem of scheduling batch jobs in multi-server queueing systems with replications. 

\section*{Acknowledgements}

The authors are grateful to Ying Lei, Eytan Modiano, R. Srikant, and Junshan Zhang for helpful
discussions.




%This paper establishes delay optimality or near delay optimality in the scheduling of queueing systems with replications. As replication is a special type of codes, it is possible to generalize these results to coded queueing systems. %Some preliminary results on this are available in \cite{Sun2015}. 
%The system settings and delay metrics considered here are quite general, some of which are analyzed in the study of replications for the first time. In order to establish these results, sufficient conditions are developed to compare the delay performance of different policies on sample-path. These sufficient conditions are general and can be applied to any queueing system. 
%
%
%
%One limitation in existing delay optimality analysis of replications is that the service time distributions are assumed to be either NBU or NWU. %\footnote{Note that this limitation exists for delay minimization, but not for delay characterization.} 
%Recent measurements \cite{addShengboOriginal,Liang2013_2} in some systems show that the service times follow a shifted exponential distribution, which is a NBU distribution. However, the service time distribution may not be NBU or NWU in other systems. An interesting topic for future research is delay-optimal scheduling of replications and coding under general service time distributions that are not NBU or NWU. In addition, service time correlation across the servers has significant influence on the delay performance of replications and coding, which requires further investigation.  


==> v3/distributed.tex <==
% !TEX root = ./replication.tex

\section{Replications in Distributed Queueing Systems}\label{sec_distributed}
In this section, we propose replication policies for distributed queueing systems with data-locality constraints,\footnote{Note that if there is no data-locality constraints, each task can be replicated on all servers. In this case, a distributed queueing system can be equivalently viewed as a centralized queueing system and all results in Section \ref{sec_analysis} apply.} and prove that these policies are near delay-optimal for minimizing several classes of delay metrics. To the extent of our knowledge, these are the first results on delay-optimal replications in distributed queueing systems with data-locality constraints.

%, and more general  delay metrics. 


%We will not use study the FUT scheduling principle 

%\subsection{Equivalent System Model}
%First 


\subsection{An Equivalent Hierarchical Distributed Queueing Model}
%The sufficient conditions obtained in Section \ref{sec_sufficient} cannot be directly applied to distributed queueing systems with  data-locality constraints, because these sufficient conditions require policy $P$ to be work-conserving. However, due to data-locality constraints, some groups of servers may be idle while the other groups of servers are busy, and hence policy $P$ cannot be work-conserving. 

%In order to resolve this problem, we propose a hierarchical distributed queueing model of the system, as illustrated in Fig. \ref{fig1model_distri_eq}, which is equivalent with the distributed queueing model in Section \ref{sec:model}. 
There are two types of data locality constraints: per-task constraints and per-job constraints \cite{Sparrow:2013}. In per-task  constraints, the tasks of one job may have a different group of servers on which it can run; while in per-job constraints, all tasks of one job must be executed on the same group of servers. Per-task constraints are more general than per-job constraints, and are also more difficult to handle. Both types of constraints play an important role in cloud computing clusters \cite{taskplacement2011}. We will consider both types of data locality constraints in our study.


For the convenience of analysis, we consider a hierarchical distributed queueing model depicted in Fig. \ref{fig1model_distri_eq}. In this model, there are two levels of job queues: the job queues at the schedulers, and the sub-job queues at the server groups. At the scheduler side, each incoming job is split into $g$ sub-jobs, where the $h$-th sub-job consists of the tasks to be executed by server group $h$ and $h=1,\ldots,g$. Each sub-job is routed its corresponding server group, and stored in a sub-job queue. Then, a local scheduler assigns tasks to the servers within the group. 
In this hierarchical distributed queueing model, each sub-job queue for a group of servers can be considered as a centralized queueing system in Fig. \ref{fig1model_central}. 
It is important to note that this hierarchical distributed queueing model is equivalent with the original distributed queueing model in Fig. \ref{fig1model_distri}. In particular, according to the discussions in Section \ref{sec:model}, each task assignment policy of the local scheduler in the hierarchical distributed queueing model can be equivalently implemented in the original distributed queueing model, and vice versa.


% the task assignments by the local scheduler can be  
% each sub-job queue in Fig. \ref{fig1model_distri_eq}, and further utilize \eqref{eq_sub_job_relation} to obtain near delay optimality results for .

Let $k_{ih}$ denote the number of tasks in sub-job $h$ of job $i$, where $\sum_{h=1}^g k_{ih} = k_i>0$. If no task of job $i$ should be executed by $h$-th group of the servers, then $k_{ih}=0$. 
The arrival time and due time of each sub-job of job $i$ are $a_i$ and $d_i$, respectively. Define $\mathcal{I}_h = \{n,(a_i,d_i,k_{ih})_{i=1}^n\}$ as the parameters of the sub-jobs of server group $h$.
For sub-job $h$ of job $i$, $V_{ih}$ is the earliest time that all tasks of the sub-job have entered the servers, $C_{ih}$ is the completion time, $D_{ih}= C_{ih}-a_i$ is the delay, and $L_{ih} = C_{ih}-d_i$ is the {lateness} after the due time $d_i$. If $k_{ih}=0$, then $V_{ih}=C_{ih}=0$. Then, we have $V_{ih}\leq C_{ih}$.
A job is completed when all of its sub-jobs are completed. Hence, 
\begin{align}\label{eq_sub_job_relation}
C_i = \max_{h=1,\ldots,g}C_{ih}, V_i=\max_{h=1,\ldots,g}V_{ih}, D_i = \max_{h=1,\ldots,g} D_{ih},  L_i = \max_{h=1,\ldots,g}L_{ih},
\end{align}
where $V_i$ and $C_i$  depend only on the sub-jobs with positive sizes $k_{ih}>0$. Define $\bm{V}_h = (V_{1h},\ldots,V_{nh})$ and $\bm{C}_h = (C_{1h},\ldots,C_{nh})$. Let  $V_{(i),h}$ and $C_{(i),h}$ denote the $i$-th smallest components of $\bm{V}_h$ and $\bm{C}_h$, respectively. 
%, and Let $v_{ih}$ and $c_{ih}$ denote the realizations of $V_{ih}$ and $C_{ih}$.
%Let $u_{ih}$ and $c_{ih}$ denote the realization of $U_{ih}$ and $C_{ih}$, respectively. 
All these quantities are functions of the adopted scheduling policy $\pi$. 



Next, we will use the results obtained in Section \ref{sec_analysis} to study the delay performance of replications in distributed queueing systems.

%In this model, each sub-job queue for a group of servers can be considered as a centralized queue system in Fig. \ref{fig1model_central}. 


\begin{figure}
\centering
%\captionsetup{justification=centering}
\includegraphics[width=0.9\textwidth]{Figures/equivalent_distributed_queue}  
\caption{A hierarchical distributed queueing model, which is equivalent with the distributed queueing model in Fig. \ref{fig1model_distri}. } \label{fig1model_distri_eq} 
\end{figure} 

\subsection{Per-Task Data Locality Constraints}
We first consider delay minimization with per-task data locality constraints.
%, which is known to be a difficult scheduling problem \cite{Sparrow:2013}. 
For minimizing the maximum lateness $L_{\max}(\cdot)$, we propose one policy called \textbf{Earliest Due Date first with Group-based Replication (EDD-GR)}: For each local scheduler in the hierarchical distributed queueing model, if the task service times are NBU (but not exponential), the tasks are assigned to this group of servers by following policy EDD-FR; if the task service times are NWU, the tasks are assigned to the this group of servers by following policy EDD-R. The local schedulers of different server group operates independently. Note that in the original distributed queueing systems, policy EDD-FR and policy EDD-R can be implemented by first placing multiple copies of a task to all the servers in one group, and then letting the servers to communicate with each other to cancel the redundant task copies; on each server, the priority of a task is determined by the due time of the job it belongs to. Hence, policy EDD-GR is a fully distributed scheduling policy. The delay performance of policy EDD-GR is provided as follows. 
\begin{theorem}\label{thm_dis4}
If (i) the task service times are independent across the servers, (ii) each server group $h$ and its sub-job parameters $\mathcal{I}_h$ satisfy the conditions of Theorem \ref{thm3}, Theorem \ref{thm4}, or Theorem \ref{thm4_exp}, and (iii) the task assignment is subject to per-task data locality constraints, then for all \emph{$\pi\in\Pi$} and $\mathcal{I}$
\emph{
\begin{align}\label{eq_delaygap3_thm4_dis}
[L_{\max}(\bm{V}(\text{EDD-GR}))|\mathcal{I}] \leq_{\text{st}} [L_{\max}(\bm{C}(\pi))|\mathcal{I}].
\end{align}}
\end{theorem}
\begin{proof}
%See Appendix \ref{app_dis_EDD}.
%Consider the $h$-th group of servers in the distributed queue system. If the task service times of these servers are independent NBU, then EDD-NIR policy and  EDD-NR policy are more work-efficient than any policy $\pi\in\Pi$ for this group of servers. If the task service times of these servers are independent NWU, then EDD-R policy is more work-efficient than any policy $\pi\in\Pi$ for this group of servers. 
By using Theorem \ref{thm3}, Theorem \ref{thm4}, Theorem \ref{thm4_exp}, and the fact that $V_{ih}(\text{EDD-GR})\leq C_{ih}(\text{EDD-GR})$, we obtain that for all $h=1,\ldots,g$, $\pi\in\Pi$
and $\mathcal{I}$
\begin{align}
\Big[\max_{i=1,\ldots,n}[V_{ih}(\text{EDD-GR})-d_i]\Big|\mathcal{I}\Big] \leq_{\text{st}} \Big[\max_{i=1,\ldots,n}[C_{ih}(\pi)-d_i]\Big|\mathcal{I}\Big]. \nonumber
\end{align}
In addition, according to \eqref{eq_sub_job_relation}, we can get  
\begin{align}
&L_{\max}(\bm{V}(\text{EDD-GR})) = \max_{i=1,\ldots,n}[V_{i}(\text{EDD-GR})-d_i] = \max_{h=1,\ldots, g} \max_{i=1,\ldots,n}[V_{ih}(\text{EDD-GR})-d_i], \nonumber\\
&L_{\max}(\bm{C}(\pi)) = \max_{i=1,\ldots,n}[C_{i}(\pi)-d_i] = \max_{h=1,\ldots, g} \max_{i=1,\ldots,n}[C_{ih}(\pi)-d_i].\nonumber
\end{align}
Then, by using Theorem 6.B.16.(b) of \cite{StochasticOrderBook} and the independence of the task service times across the servers, it follows that
\begin{align}
\Big[\max_{i=1,\ldots,n}[V_{i}(\text{EDD-GR})-d_i]\Big|\mathcal{I}\Big] \leq_{\text{st}} \Big[\max_{i=1,\ldots,n}[C_{i}(\pi)-d_i]\Big|\mathcal{I}\Big]. \nonumber
\end{align}
By this, Theorem \ref{thm_dis4} is proven.
\end{proof}


For minimizing the maximum delay $D_{\max}(\cdot)$, we propose one policy called  \textbf{First-Come, First-Served with Group-based Replication (FCFS-GR)}: 
For each local scheduler in the hierarchical distributed queueing model, if task service times are NBU (but not exponential), the tasks are assigned to this group of servers by following policy FCFS-FR; if task service times are NWU, the tasks are assigned to this group of servers by following policy FCFS-R. Similar with policy EDD-GR, policy FCFS-GR can also be implemented distributedly in the original distributed queueing systems.
By choosing $d_i=a_i$ for all $i$, it follows from Theorem \ref{thm_dis4} that



\begin{theorem}\label{thm_dis5}
If (i) the task service times are independent across the servers, (ii) each server group $h$ and its sub-job parameters $\mathcal{I}_h$ satisfy the conditions of Theorem \ref{thm5} or Theorem \ref{thm6}, and (iii) the task assignment is subject to per-task data locality constraints, then for all \emph{$\pi\in\Pi$} and $\mathcal{I}$
\emph{
\begin{align}\label{eq_delaygap3_thm5_dis}
[D_{\max}(\bm{V}(\text{FCFS-GR}))|\mathcal{I}] \leq_{\text{st}} [D_{\max}(\bm{C}(\pi))|\mathcal{I}].
\end{align}}
\end{theorem}




%In policy EDD-GR and policy FCFS-GR, the arrival time and due time are used to determine the priority of a sub-job. However, it is difficult to use the number of unassigned tasks to determine the priority of a job, because the number of unassigned tasks decreases over time and is difficult to track in a distributed queueing system. One important open question is whether policy EDD-GR and policy FCFS-GR are optimal for minimizing more general delay metrics. 

\subsection{Per-Job Data Locality Constraints}
It appears that under per-task constraints it is difficult to generalize Theorem \ref{thm_dis4} and Theorem \ref{thm_dis5} for minimizing other delay metrics. However, under per-job constraints such generalizations are possible, which are discussed in the sequel.

For minimizing the average delay $D_{\text{avg}}(\cdot)$ and the delay metrics in $\mathcal{D}_{\text{sym}}$, we propose one policy called \textbf{Fewest Unassigned Tasks first with Group-based Replication (FUT-GR)}: For each local scheduler, if task service times are NBU (but not exponential), the tasks are assigned to this group of servers by following policy FUT-FR; if task service times are NWU, the tasks are assigned to this group of servers by following policy FUT-R. Hence, the priority of a sub-job is determined by the number of unassigned tasks in this sub-job. If $\max_{i,h} k_{ih}>1$, the local scheduler needs to track the number of unassigned tasks of each sub-job by communicating with each server in the group. If $\max_{i,h} k_{ih}=1$, policy FUT-GR can be implemented distributedly in the original distributed queueing systems. 
%For each server group, if the task service times are NBU (but not exponential) and independent across the servers in this group, the tasks of the sub-jobs are assigned to the servers by following policy FUT-FR; if the task service times are NWU and independent across the servers in this group, the tasks are assigned to the servers by following policy FUT-R. Therefore, each group of servers is treated as an independent centralized queueing system in policy FUT-GR. 
The delay performance of policy FUT-GR is provided as follows. 


\begin{theorem}\label{thm2_dist}
If (i) the task service times are independent across the servers, (ii) each server group $h$ and its sub-job parameters $\mathcal{I}_h$ satisfy the conditions of Theorem \ref{thm1}, %Theorem \ref{coro3}, 
Theorem \ref{thm2}, or Theorem \ref{thm2_exp}, and (iii) the task assignment is subject to per-job data locality constraints, then for all \emph{$f\in\mathcal{D}_{\text{sym}}$},  \emph{$\pi\in\Pi$}, and $\mathcal{I}$
\emph{
\begin{align}\label{eq_delaygap2_dist}
[f(\bm{V}(\text{FUT-GR}))|\mathcal{I}] \leq_{\text{st}} [f(\bm{C}(\pi))|\mathcal{I}].
\end{align}}
\end{theorem}
\begin{proof}
For any policy $\pi\in\Pi$, suppose that policy FUT-GR$_1$  (policy $\pi_1$) satisfies the same queueing discipline and stochastic law with policy FUT-GR (policy $\pi$).
By using the proof arguments of  Theorems \ref{thm1}-\ref{thm2_exp} and the fact that $V_{ih}(\text{FUT-GR}_1)\leq C_{ih}(\text{FUT-GR}_1)$, we can couple policy FUT-GR$_1$ and policy $\pi_1$ to show that 
\begin{align}\label{eq_thm2_dist}
V_{(i),h}(\text{FUT-GR}_1)\leq C_{(i),h}(\pi_1) 
\end{align}
holds with probability one for $h=1,\ldots,g$ and $i=1,\ldots,n$. Under per-job data locality constraints, each job can be only executed by one group of the servers. In addition, if $k_{ih}=0$, $V_{ih}(\text{FUT-GR}_1)=C_{ih}(\pi_1)=0$. By sorting the non-zero elements $V_{ih}(\text{FUT-GR}_1)$ and $C_{ih}(\pi_1)$ with $h=1,\ldots,g$ and $i=1,\ldots,n$, we can obtain  that
\begin{align}%\label{eq_thm2_dist1}
V_{(i)}(\text{FUT-GR}_1)\leq C_{(i)}(\pi_1)\nonumber
\end{align}
holds with probability one for $i=1,\ldots,n$.
Then, by using the proof arguements of Proposition \ref{lem1_1}, we get that for all $f\in\mathcal{D}_{\text{sym}}$
\begin{align}%\label{eq_thm2_dist1}
f(\bm{V}(\text{FUT-GR}_1))\leq f(\bm{C}(\pi_1))\nonumber
\end{align}
holds with probability one.
Then, by the property of stochastic ordering \cite[Theorem 1.A.1]{StochasticOrderBook}, we can obtain \eqref{eq_delaygap2_dist}. This completes the proof.
\end{proof}


Let us further consider the delay metrics in the set $\mathcal{D}_{\text{sym}}\cup\mathcal{D}_{\text{Sch-1}}$, for which we can obtain the following result.

\begin{theorem}\label{thm3_dist}
If (i) the task service times are independent across the servers, (ii) each server group $h$ and its sub-job parameters $\mathcal{I}_h$ satisfy the conditions of Theorem \ref{coro_thm3_1}, Theorem \ref{coro4_1}, or Theorem \ref{coro_thm3_1_exp}, and (iii) the task assignment is subject to per-job data locality constraints, then for all \emph{$f\in\mathcal{D}_{\text{sym}}\cup\mathcal{D}_{\text{Sch-1}}$},  \emph{$\pi\in\Pi$}, and $\mathcal{I}$
\emph{
\begin{align}\label{eq_delaygap3_dist}
[f(\bm{V}(\text{EDD-GR}))|\mathcal{I}] \leq_{\text{st}} [f(\bm{C}(\pi))|\mathcal{I}].
\end{align}}
\end{theorem}
\begin{proof}
If each server group $h$ and its sub-job parameters $\mathcal{I}_h$ satisfy the conditions of Theorem \ref{coro_thm3_1}, Theorem \ref{coro4_1}, or Theorem \ref{coro_thm3_1_exp}, then we can obtain
\begin{itemize}
\item[1.] The job with the earliest due time among all jobs with unassigned tasks is also the jobs with fewest unassigned tasks,

\item[2.] Each server group $h$ and its sub-job parameters $\mathcal{I}_h$  satisfy the conditions of Theorem \ref{thm1}, Theorem \ref{thm2}, or Theorem \ref{thm2_exp}.
\end{itemize}
Then, by using Theorem \ref{thm2_dist}, yields that \eqref{eq_delaygap3_dist} holds for all $f\in\mathcal{D}_{\text{sym}}$. 

Next, we consider the delay metrics in $\mathcal{D}_{\text{Sch-1}}$.
For any policy $\pi\in\Pi$, suppose that policy EDD-GR$_1$  (policy $\pi_1$) satisfies the same queueing discipline and stochastic law with policy EDD-GR (policy $\pi$).
By using the proof arguments of Proposition \ref{coro2_0} and Proposition \ref{coro2} (which are used in the proofs of Theorem \ref{coro_thm3_1}, Theorem \ref{coro4_1}, or Theorem \ref{coro_thm3_1_exp})  and the fact that $V_{ih}(\text{EDD-GR}_1)\leq C_{ih}(\text{EDD-GR}_1)$, we can couple policy EDD-GR$_1$ and policy $\pi_1$ to show that 
\begin{align}%\label{eq_thm3_dist}
\bm{V}_h(\text{EDD-GR}_1)-\bm{d}\prec_{\text{w}} \bm{C}_h (\pi_1)-\bm{d}\nonumber
\end{align}
holds with probability one for $h=1,\ldots,g$. Then, Theorem 5.A.7 of \cite{Marshall2011} tells us that
\begin{align}\label{eq_thm3_dist}
(\bm{V}_1(\text{EDD-GR}_1)-\bm{d}, \ldots,\bm{V}_g(\text{EDD-GR}_1)-\bm{d})\prec_{\text{w}} (\bm{C}_1 (\pi_1)-\bm{d},\ldots,\bm{C}_g (\pi_1)-\bm{d})
\end{align}
holds with probability one. Under per-job data locality constraints, each job can be only executed by one group of the servers. 
In addition, if $k_{ih}=0$, $V_{ih}(\text{EDD-GR}_1)=C_{ih}(\pi_1)=0$. If the elements satisfying $V_{ih}(\text{EDD-GR}_1)=0$  on LHS of \eqref{eq_thm3_dist} and the elements satisfying $C_{ih}(\pi_1)=0$ on RHS of \eqref{eq_thm3_dist} are removed, the obtained inequality still holds with probability one. By this, we get that
%Hence, 
%\begin{align}
%&\bm{V}(\text{EDD-GR}_1) = \sum_{h=1}^g\bm{V}_h(\text{EDD-GR}_1),\nonumber\\
%&\bm{C}(\pi_1) = \sum_{h=1}^g\bm{C}_h(\pi_1).\nonumber
%\end{align}
%By taking the summation over $h$ in \eqref{eq_thm3_dist} and use Theorem \ref{} of \cite{Marshall2011}, we get that
\begin{align}
\bm{V}(\text{EDD-GR}_1)-\bm{d}\prec_{\text{w}} \bm{C} (\pi_1)-\bm{d}\nonumber
\end{align}
holds with probability one.
In addition, by Theorem 3.A.8 of \cite{Marshall2011},
\begin{align}%\label{eq_thm2_dist1}
f(\bm{V}(\text{EDD-GR}_1))\leq f(\bm{C}(\pi_1)) \nonumber
\end{align}
holds with probability one for all $f\in\mathcal{D}_{\text{Sch-1}}$.
Then, by the property of stochastic ordering \cite[Theorem 1.A.1]{StochasticOrderBook}, we can obtain \eqref{eq_delaygap3_dist}. This completes the proof.
\end{proof}

Finally, if $d_i=a_i$ for all job $i$, it follows from Theorem 
\ref{thm3_dist} that 
\begin{theorem}\label{thm4_dist}
If (i) the task service times are independent across the servers, (ii) each server group $h$ and its sub-job parameters $\mathcal{I}_h$ satisfy the conditions of Theorem \ref{coro5_1} or Theorem \ref{coro6_1}, and (iii) the task assignment is subject to per-job data locality constraints, then for all \emph{$f\in\mathcal{D}_{\text{sym}}\cup\mathcal{D}_{\text{Sch-2}}$},  \emph{$\pi\in\Pi$}, and $\mathcal{I}$
\emph{
\begin{align}\label{eq_delaygap4_dist}
[f(\bm{V}(\text{FCFS-GR}))|\mathcal{I}] \leq_{\text{st}} [f(\bm{C}(\pi))|\mathcal{I}].
\end{align}}
\end{theorem}

% \textbf{Earliest Due Date first with Group-based Replication (EDD-GR)}: 
%Each group of servers is treated as an independent centralized queueing system. Consider one particular group of servers. If the task service times of this group of servers are independent NBU, the tasks of the sub-jobs in the sub-job queue are assigned to the servers by following EDD-NIR or EDD-NR policy; if the task service times of this group of the servers are independent NWU, the tasks are assigned to the servers by following EDD-R policy. The delay performance of policy EDD-GR is provided as follows. 

%\begin{theorem}\label{thm_dis4_1}
%If (i) the task service times in each group of servers are either NBU or NWU and independent across the servers, and (ii) ${O}_l={0}$ for each NWU server $l$, then for all \emph{$\pi\in\Pi$} and $\mathcal{I}$
%\emph{
%\begin{align}\label{eq_delaygap3_thm4_dis}
%[L_{\max}(\bm{U}(\text{EDD-GR}))|\mathcal{I}] \leq_{\text{st}} [L_{\max}(\bm{C}(\pi))|\mathcal{I}].
%\end{align}}
%\end{theorem}
%\begin{proof}
%%See Appendix \ref{app_dis_EDD}.
%Consider the $h$-th group of servers in the distributed queue system. If the task service times of these servers are independent NBU, then EDD-NIR policy and  EDD-NR policy are more work-efficient than any policy $\pi\in\Pi$ for this group of servers. If the task service times of these servers are independent NWU, then EDD-R policy is more work-efficient than any policy $\pi\in\Pi$ for this group of servers. 
%By applying Theorem \ref{lem2} for the $h$-th group of servers, we can obtain that for all $\mathcal{I}$ and all $\pi\in\Pi$
%\begin{align}
%\big[\max_{i=1,\ldots,n}[U_{ih}(\text{EDD-GR})-d_i]\big|\text{EDD-GR},\mathcal{I}\big] \leq_{\text{st}} \big[\max_{i=1,\ldots,n}[C_{ih}(\pi)-d_i]\big|\pi,\mathcal{I}\big]. \nonumber
%\end{align}
%Because the task service times are independent across the servers, by \eqref{eq_sub_job_relation} and Theorem 6.B.16.(b) of \cite{StochasticOrderBook}, it follows that
%\begin{align}
%\big[\max_{i=1,\ldots,n}[U_{i}(\text{EDD-GR})-d_i]\big|\mathcal{I}\big] \leq_{\text{st}} \big[\max_{i=1,\ldots,n}[C_{i}(\pi)-d_i]\big|\mathcal{I}\big]. \nonumber
%\end{align}
%By this, Theorem \ref{thm_dis4} is proven.
%\end{proof}


%For minimizing the maximum delay $D_{\max}(\cdot)$, we propose one policy called  \textbf{First-Come, First Served with Group-based Replication (FCFS-GR)}: 
%Consider one particular group of servers, if task service times of this group of servers are independent NBU, the tasks of the sub-jobs in the sub-job queue are assigned to the servers by following FCFS-NIR or FCFS-NR policy; if task service times of this group of servers are independent NWU, the tasks are assigned to the servers by following FCFS-R policy. By choosing $d_i=a_i$ for all $i$, it directly follows from Theorem \ref{thm_dis4} that
%
%\begin{theorem}\label{thm_dis5_1}
%If (i) the task service times of each group of servers are either independent NBU or independent NWU, and (ii) ${O}_l=\bm{0}$ for each NWU server $l$, then for all \emph{$\pi\in\Pi$} and $\mathcal{I}$
%\emph{
%\begin{align}\label{eq_delaygap3_thm5_dis}
%[D_{\max}(\bm{U}(\text{FCFS-GR}))|\mathcal{I}] \leq_{\text{st}} [D_{\max}(\bm{C}(\pi))|\mathcal{I}].
%\end{align}}
%\end{theorem}
%
%In policy EDD-GR and policy FCFS-GR, we have use the arrival time and due time to determine the priority of a job. However, it is difficult to use the number of unassigned tasks to determine the priority of a job, because the number of unassigned tasks decreases over time and is difficult to track in a distributed queueing system. One important open question is whether policy EDD-GR and policy FCFS-GR are optimal for minimizing more general delay metrics. 

%The sub-jobs are allocated to sub-job queues, each for a server group.  

% in Fig. \ref{fig1model_distri}, 



==> v3/intro.tex <==
% !TEX root = ./parallel_servers.tex


\section{Introduction}
%Low latency has become one major concern across a variety of industries. %
%It is imperative that modern computer systems are designed for achieving low latency.
%Achieving low latency is imperative in modern computer systems. 
%Google has found that increasing the latency of Web searching from 0.4 seconds to 0.9 seconds decreases the traffic and ad revenues by 20\% \cite{Linden2006}. Similar results were reported by Amazon, where every 100 milliseconds of extra response time was shown to decrease the sales by 1\% \cite{LindenStanfordtalk}. 
%These results imply that prompt responses not only allow users to view more pages in the same period of time, but also provide instant gratification to motivate them to spend more time online \cite{Farber2006}. 
%In addition, low latency is critically important for the 
%%Another important example is 
%stock market, where the fastest trading decisions are made within a few milliseconds. It was  estimated that a 1-millisecond advantage in trading can be worth 100 million dollars a year for a major brokerage firm \cite{Martin2007}. 
%%These examples implies
%%It has been observed
%%These evidences suggest that
%Therefore, 
%%These evidences imply that
%even small changes in latency can have a significant impact on business success. 

Achieving low service latency is imperative in cloud computing and data center systems. 
As the user population and data volume scale up, the running times of service jobs grow quickly. 
%maintaining low latency becomes increasingly challenging. 
In  practice, 
long-running jobs are broken into a batch of short tasks which can be executed separately by a number of parallel servers  \cite{mapreduce}. We study the scheduling of such batch jobs in multi-server queueing systems. 
The jobs arrive over time according to a  general arrival process, where the number, batch sizes, arrival times, and due times of the jobs are \emph{arbitrarily} given. A scheduler determines how to assign the tasks of incoming jobs to the servers, based on the casual information (the history and current information) of the system. 
We assume that each task is of one unit of work and can be flexibly assigned to any server. The service times of the tasks follow New-Better-than-Used (NBU) distributions, and are \emph{independent} across the servers and \emph{i.i.d.} across the tasks assigned to the same server. % but the servers may have random service times to execute the tasks. In particular, the task service times are assumed to be \emph{independent} across the servers and \emph{i.i.d.} across the tasks assigned to the same server. 
Our goal is to seek for low-complexity scheduling policies that optimize the delay performance of the jobs.

Many delay-optimal scheduling results have been established in single-server queueing systems. In the deterministic scheduling models, the preemptive Shortest Remaining Processing Time first (SRPT) policy, the preemptive Earliest Due Date first (EDD) policy, and the First-Come, First-Served  (FCFS) policy were proven to minimize the average delay \cite{Schrage68,Smith78}, maximum lateness \cite{Jackson55}, and maximum delay \cite{Baccelli:1993}, respectively. In addition,  index policies are shown to be delay-optimal in many stochastic scheduling problems, e.g., \cite{Smith56,Rothkopf66,Gittins79banditprocesses,Klimov74,Gittins2011}. 

Unfortunately, generalizing these delay-optimal results to the parallel-server case is quite challenging. In particular, minimizing the average delay in deterministic scheduling problems with more than one servers is $NP$-hard \cite{Leonardi:1997}. Similarly, delay-optimal stochastic scheduling in multi-class multi-server queueing systems is deemed to be notoriously difficult \cite{Weiss:1992,Weiss:1995}. Prior attempts on solving the delay-optimal stochastic scheduling problem have met with little success, except in some limiting regions such as large system limits, e.g., \cite{Ying2015}, and heavy traffic limits, e.g.,\cite{Dacre1999, Stolyar_heavy2004}. However, these results may not apply either outside of these limiting regions, or for a non-stationary job arrival process under which the steady state distribution of the system does not exist.


%Prior attempts on solving the delay-optimal scheduling problem have met little success, except in some limiting regions such as large system limits, e.g., \cite{Ying2015}, and heavy traffic limits, e.g.,\cite{Stolyar_heavy2004}. However, these results may not apply outside of these limiting regions or when the stationary distribution of the system does not exist.





%In addition, replications add a further layer of difficulty to this problem. If a task is replicated on multiple servers, its service time is reduced, but at a cost of longer waiting times of other tasks. In general, it is difficult to determine whether the gain of shorter service time would exceed the loss of longer waiting times. Hence, ``to replicate or not  to replicate'' is a fundamental dilemma that needs to be resolved in order to design an optimal scheduler. We note that each task has many replication modes (i.e., it can be replicated on different servers and at different time instants), which require different amounts of service time. Thus, the work conservation law \cite{Leonard_Kleinrock_book,Jose2010} does not hold in the queueing systems that we consider. Hence, some powerful delay minimization methods, such as the achievable region approach \cite{Gittins:11}, cannot be directly applied in our study.

%



% As a result, the job service latency is constrained by the slowest straggling tasks, which may cause long latency tail. 
%In some systems, it was observed that the 99.9\% percentile latency can be as long as 42 times of the 95\% percentile latency\cite{Google_Rapid}.



%An efficient technique used to tame the latency tail is \emph{replications} \cite{Ghare:2004,Cirne2007213,vulimiri13latency,ShengboInfocom,Wang:2014,Wang2015}, which is also called \emph{redundant requests} in \cite{shah-Allerton-2013,Kristen2015,Lee-Allerton-2015} and \emph{cloning} in \cite{Ananthanarayanan11,Ananthanarayanan13}. In this technique, multiple replicas of a task are dispatched to different servers and the first completed replica is considered as the valid execution of the task. After that, the remaining replicas of this task can be cancelled to release the servers. 
%%When each server has a  distributed queueing systems, it was replications 
%%Recently, the delay performance of replications has been extensively explored in empirical studies  \cite{mapreduce,Zaharia:2008,Ananthanarayanan:2010,Dremel2010,Dean:2013:Tail,Ananthanarayanan11,Ananthanarayanan13,Ananthanarayanan2014, vulimiri12latency,vulimiri13latency,addShengboOriginal,Liang2013_2,DTN-delay}. In some systems, replications can significantly reduce the job latency tail. 
%The potential benefits of replications are huge.
%For example, in Google's BigTable service which has a high degree of parallelism, replications can reduce the 99.9\%-th percentile delay from 1,800 milliseconds to 74 milliseconds \cite{Dean:2013:Tail}. However, in some other systems, replications may worsen the delay performance, e.g., \cite{Liang2013_2,vulimiri13latency}. In particular, the delay performance of replications depends heavily on the scheduling decisions of when to replicate, which servers to replicate on, and which task to serve first. So far, little is understood on how to optimally schedule replications for minimizing the delay to complete the jobs.
%
%In this paper, we study delay-optimal scheduling of replications for both centralized and distributed queueing systems, which are illustrated in Fig. \ref{fig1model_central} and Fig. \ref{fig1model_distri}, respectively. In centralized queueing systems, the jobs arrive at a scheduler and are stored in a job queue. Each job is a batch of tasks. The scheduler queries the idle/busy state of each server, and assigns tasks to the available servers over time. In distributed queueing systems, the jobs arrive at multiple parallel schedulers and each scheduler independently assigns tasks to the servers. The schedulers is subject to {data locality} constraints \cite{taskplacement2011,Sparrow:2013}. More specifically, the servers  are divided into multiple server groups and each task can be only executed by one group of servers, each of which stores one copy of the data necessary for executing the task.\footnote{The data locality constraints considered here are \emph{hard} constraints, where the servers are not allowed to process remote tasks belonging to other groups. There exists another form of \emph{soft} data locality constraints, where a server can execute remote tasks belonging to other groups by first retrieving the necessary data and then processing the task. Therefore, remote tasks are executed at a slower speed than local tasks. In practical systems, hard data locality constraints are more appropriate for interactive Web services, which need to respond within a few seconds; while soft data locality constraints are usually used in offline services, where the tasks are executed at a slower time scale and hence there is sufficient time to retrieve the necessary data.} 

%\begin{figure}
%\centering
%\includegraphics[width=0.5\textwidth]{Figures/queue_model_1}
%\caption{A centralized queueing system, where a scheduler assigns the tasks of incoming jobs to the servers.} \label{fig1model_central}
%\end{figure}
%\begin{figure}
%\centering
%%\captionsetup{justification=centering}
%\includegraphics[width=0.8\textwidth]{Figures/queue_model_3}
%\caption{A distributed queueing system with data locality constraints, where multiple schedulers independently assign tasks to the servers. Each task can be only assigned to a group of servers, each of which stores one copy of the data necessary for executing the task.} \label{fig1model_distri}
%\end{figure}

\subsection{Our Contributions}
Because of the difficulty in establishing delay optimality in the considered queueing systems, we investigate near delay-optimal scheduling in this paper.
We prove that %for New-Better-than-Used (NBU) task service time distributions and 
for arbitrarily given job parameters (including the number,  batch sizes, arrival times, and due times of the jobs), the Fewest Unassigned Tasks first (FUT) policy, the EDD  policy, and the  FCFS  policy are near delay-optimal in  stochastic ordering
%distribution\footnote{In this paper, ``in distribution" is equivalent to ``in stochastic ordering''.} 
for minimizing average delay, maximum lateness, and maximum delay, respectively, among all causal and non-preemptive\footnote{We consider task-level non-preemptive policies: Processing of a task cannot be interrupted until the task is completed. However, after completing a task from one job, a server can switch to process another task from any job.} policies. If the job parameters satisfy some additional conditions, we can further show that these policies are near delay-optimal in stochastic ordering for minimizing three  general classes of delay metrics. In particular, we  show that the FUT policy is within a constant additive delay gap from the optimum  for minimizing the mean average delay (Theorem \ref{lem7_NBU})\footnote{As we will see in Section \ref{sec_analysis}, the FUT policy is a nice approximation of the Shortest Remaining Processing Time (SRPT) first policy \cite{Schrage68,Smith78}.}; and  
the FCFS policy within twice of the optimum for minimizing the mean maximum delay and mean $p$-norm of delay (Theorems \ref{thm_max_delay_ratio} and \ref{thm_max_delay_ratio_1}). 

We develop a unified sample-path method to establish these results, where the key proof tools are several novel sample-path orderings for comparing the delay performance of different policies in a near-optimal sense. These sample-path orderings are very general because they do not need to specify the queueing system model, and hence can be potentially used for establishing near delay optimality results in other queueing systems.





%The near delay-optimal scheduling results obtained in this paper are summarized in Table \ref{tab:policy}.



 
%The proposed scheduling policies are \emph{non-anticipative} in the sense that the scheduling decisions are made without using any information about the future job arrivals. These scheduling policies are rigorously proven to be delay-optimal or near delay-optimal among all \emph{non-preemptive} and \emph{causal} policies, as well as \emph{anticipative} policies that have access to the information about future job arrivals. 
%These delay optimality and near delay optimality results are established in very general system settings, which allow for arbitrary arrival processes, arbitrary job sizes, arbitrary soft deadlines, and heterogeneous servers with data locality constraints. The delay metrics optimized in this study include average delay, maximum delay, maximum lateness, and more generally, three classes of delay metrics with diverse fairness and deadline concerns. Each of these delay metrics is a random variable and our goal is to minimize any moments and the complementary CDF (i.e., the tail distribution) of these delay metrics.


% We prove that for arbitrary job parameters (including the arrival times, due times, and batch sizes of the jobs) and New-Better-than-Used (NBU) task service time distributions, the Fewest Unassigned Tasks first (FUT) policy, Earliest Due Date first (EDD) policy, and the First-Come, First-Served  (FCFS) policy are near delay-optimal in distribution for minimizing average delay, maximum lateness, and maximum delay, respectively, among all non-preemptive and causal policies. In addition, these results are generalized to minimize several classes of delay metrics if the job parameters satisfy certain conditions. 
%
%
%
% delay-optimal scheduling with replications. Specifically, low-complexity scheduling policies are designed for both centralized and distributed queueing systems. 
%The proposed scheduling policies are \emph{non-anticipative} in the sense that the scheduling decisions are made without using any information about the future job arrivals. These scheduling policies are rigorously proven to be delay-optimal or near delay-optimal among all \emph{non-preemptive} and \emph{causal} policies, as well as \emph{anticipative} policies that have access to the information about future job arrivals. 
%These delay optimality and near delay optimality results are established in very general system settings, which allow for arbitrary arrival processes, arbitrary job sizes, arbitrary soft deadlines, and heterogeneous servers with data locality constraints. The delay metrics optimized in this study include average delay, maximum delay, maximum lateness, and more generally, three classes of delay metrics with diverse fairness and deadline concerns. Each of these delay metrics is a random variable and our goal is to minimize any moments and the complementary CDF (i.e., the tail distribution) of these delay metrics.
%
%\begin{itemize}
%\item[1.] Sample-Path Ordering: We first present a few sample-path orderings for comparing the system states of two policies on sample-path, where each of these sample-path orderings can be used to obtain an inequality between the values of one delay metric of these two policies (Lemmas \ref{ordering_1}-\ref{ordering_4_1}). This builds a strong connection between system state inequality and delay inequality. The remaining problem is how to establish these sample-path orderings.
%\item[2.]  Sufficient Conditions for Delay Comparison: As we have mentioned, each task has many replication modes, which require different amounts of service time. In order to minimize the delay, the scheduler needs to choose efficient replication modes to execute the tasks. Motivated by this, two work-efficiency orderings are introduced to compare the efficiency of task service in different replication policies. By combining these work-efficiency orderings with appropriate priority queueing disciplines, we obtain a number of sufficient conditions for the foregoing sample-path orderings and delay inequality (Propositions \ref{lem1_0}-\ref{coro3_1}). 
%Note that these sufficient conditions hold for any queueing system, and are not limited to the study of replications. 
%\item[3.]  Coupling Arguments: The final step is to prove the work-efficiency orderings. In the queueing systems that we consider, it is hard to prove the work-efficiency orderings on a sample-path. Because of this, we use coupling arguments to prove the work-efficiency orderings in the sense of stochastic ordering, which enables us to establish delay optimality and near delay optimality in distribution (Theorems \ref{thm1}-\ref{coro6_1}).  
%\end{itemize}
%
%
%



%we have obtained delay-optimality This requires our study to be not limited to  is not limited to 

%Prior theoretical studies of task replications can be classified into two categories: The first category characterizes the average delay of different task replication policies, and then uses the obtained delay characterizations to compare these policies. The second category focuses on delay minimization among a class of task replication policies. 

%These studies compare different task replication policies without relying on accurate delay characterizations. Compared with the first category of research, these studies aim to establish delay optimality for more general system settings (e.g., arbitrary arrival process and heterogeneous servers) and in a larger policy space (e.g., all causally feasible task replication policies).
%
%
% which task replication policy can achieve the optimal delay performance.
%In the existing delay optimality analyses of task replications \cite{Borst2003,Righter2008,Kim2010,shah-Allerton-2013,ShengboInfocom,Sun2015}, the proof techniques are usually combinatorial and vary from case to case, which makes them difficult to follow and manage.
%%To some extent, this has limited the development of scheduling theory in this area.
%In addition, most existing analyses focus on finding low-complexity scheduling policies that are delay-optimal. However, delay optimality can be only shown in a few limited system settings. In many general system settings, what one can hope is a low-complexity scheduling policy of task replications which deviates from the optimum delay by at most a small gap. 












%In interactive cloud computing and data analytics, the slowest straggling task delays job completion. One efficient approach to mitigation stragglers is \emph{task replications}: straggling tasks are dynamically replicated and executed on multiple servers to curb long latency \cite{Dean:2004,Zaharia:2008,Ananthanarayanan:2010,Dremel2010,Ananthanarayanan13,Dean:2013:Tail,Ananthanarayanan2014}. 

%data is redundant stored  \cite{addShengboOriginal,ShengboInfocom,Sun2015},


%If a job is replicated to $w$ copies and processed on $w$ servers (possibly starting at $w$ different time instants), then the job is completed as long as one of its $w$ replicated copies is accomplished. After that, the remaining $w-1$ copies are cancelled, which is called \emph{service cancellation}, to release the server resources. By this, the processing time of the head-of-line job can be reduced. On the other hand, service replication may also increase the waiting time of the other jobs in the queue. Therefore, the design of replication-control policy provides a tradeoff between faster job processing and a longer waiting time. It is difficult to understand which replication-control policy has the optimum delay performance.

%\subsection{Notations}




%\subsection{Our Contributions} 
%\subsubsection{Design of Scheduling Policies} 
%For centralized queueing systems, scheduling policies are developed by combining the following replication disciplines and priority queueing disciplines:
%
%There are two different replication disciplines. If the task service times of the servers follow independent New-Better-than-Used (NBU) distributions, regardless of the delay overhead for cancelling the redundant tasks, the following principles should be used for replication and cancellation operations, which we refer to as the Flexible Replication (FR) discipline:
%\begin{itemize}
%\item[1.] {Replication:} {Replicate a task on an idle server only when all tasks are under service on other servers, or not replicate this task at all.}
%\item[2.] {Cancellation:} {Cancel a redundant task copy only when the time to cancel the task is stochastically shorter than the remaining service time to complete the task, or not cancel this task at all.}  
%\end{itemize}
%If the task service times of the servers follow independent New-Worse-than-Used (NWU) distributions and the cancellation delay is zero, the following principles should be used for replication and cancellation operations, which are simply referred to as the Replication (R) discipline:
%\begin{itemize}
%\item[1.] {Replication:} {Replicate each task on as many servers as possible, even if there are tasks not assigned to any server.}
%\item[2.] {Cancellation:} {When one copy of a task is completed, cancel the remaining task copies immediately.}  
%\end{itemize}
%The priority queueing disciplines for minimizing average delay, maximum lateness, and maximum delay are Fewest Unassigned Tasks (FUT) first, Earliest Due Date (EDD) first, and First-come First-Served (FCFS), respectively. Each of these three delay metrics can be generalized to a class of delay metrics, which can be also optimized by the FUT, EDD, and FCFS priority queueing disciplines under certain conditions. 


%For example, if the task service times of the servers follow independent NBU distributions and the concerned delay metric is the maximum lateness, we suggest to use a scheduling policy named Earliest Due Date first with Flexible Replication (EDD-FR).
%
%The scheduling policies of distributed queueing systems can be obtained by applying the foregoing scheduling policies of centralized queueing systems in each group of servers. For example, if one group of servers have independent NBU service time distributions, the second group of servers have independent NWU service time distributions, and the concerned delay metric is the maximum delay, then  we suggest to use policy First-come First-Served with Flexible Replication (FCFS-FR) to schedule the tasks associated with server group one, and use policy First-come First-Served with  Replication (FCFS-R) to schedule the tasks associated with server group two. More details of the scheduling policy design are available in  
%Section \ref{sec_analysis} and  Section \ref{sec_distributed}.

%\subsubsection{Outline of Proof Methodology} The proposed scheduling policies are shown to be delay-optimal or near delay-optimal. Our proof approach consists of three major steps:
%
%\begin{itemize}
%\item[1.] Sample-Path Ordering: We first present a few sample-path orderings for comparing the system states of two policies on sample-path, where each of these sample-path orderings can be used to obtain an inequality between the values of one delay metric of these two policies (Lemmas \ref{ordering_1}-\ref{ordering_4_1}). This builds a strong connection between system state inequality and delay inequality. The remaining problem is how to establish these sample-path orderings.
%\item[2.]  Sufficient Conditions for Delay Comparison: As we have mentioned, each task has many replication modes, which require different amounts of service time. In order to minimize the delay, the scheduler needs to choose efficient replication modes to execute the tasks. Motivated by this, two work-efficiency orderings are introduced to compare the efficiency of task service in different replication policies. By combining these work-efficiency orderings with appropriate priority queueing disciplines, we obtain a number of sufficient conditions for the foregoing sample-path orderings and delay inequality (Propositions \ref{lem1_0}-\ref{coro3_1}). 
%Note that these sufficient conditions hold for any queueing system, and are not limited to the study of replications. 
%\item[3.]  Coupling Arguments: The final step is to prove the work-efficiency orderings. In the queueing systems that we consider, it is hard to prove the work-efficiency orderings on a sample-path. Because of this, we use coupling arguments to prove the work-efficiency orderings in the sense of stochastic ordering, which enables us to establish delay optimality and near delay optimality in distribution (Theorems \ref{thm1}-\ref{coro6_1}).  
%\end{itemize}
%%As we will see in Section \ref{sec_analysis} and Section \ref{sec_distributed}, 
%These theoretical results can be further generalized to distributed queueing systems with replications and data locality constraints (Theorems \ref{thm_dis4}-\ref{thm4_dist}).

%\subsection{Related Research}
%\subsubsection{Systems Research} 
%The benefits of exploiting replications to reduce latency have been empirically studied for several applications  \cite{mapreduce,Zaharia:2008,Ananthanarayanan:2010,Dremel2010,Dean:2013:Tail,Ananthanarayanan11,Ananthanarayanan13,Ananthanarayanan2014, vulimiri12latency,vulimiri13latency,addShengboOriginal,Liang2013_2,DTN-delay}. In communication networks, multiple replicated copies of a message can be sent over different routing paths to reduce delay \cite{DTN-delay,vulimiri13latency}. 
%In cloud computing systems, the task execution time is highly random and it was shown that replicating straggling tasks can significantly reduce the job service latency \cite{mapreduce,Zaharia:2008,Ananthanarayanan:2010,Dremel2010,Ananthanarayanan13,Ananthanarayanan2014,Dean:2013:Tail}. In \cite{vulimiri12latency,vulimiri13latency}, the authors observed that the latency of DNS queries can be reduced by sending multiple replications of a query to multiple servers. 
%
%Replications and more general coding techniques have been proposed to reduce communication delay in cloud storage and information retrieval systems. In \cite{addShengboOriginal,Liang2013_2}, the authors performed experiments on Amazon S3, and found that one can exploit storage redundancy to issue multiple downloading connections to reduce delay. 
%%In many systems, it is observed that task replications  reduce latency in some scenarios and increase latency in others. This underlines a need for theoretical guidance on the design and control of task replication policies, to avoid harming the delay performance of the system.
%Recently, coding techniques were introduced to speedup distributed algorithms such as MapReduce and machine learning \cite{Li-Allerton-2015, Lee-NIPS-2015}. Significant performance improvement was shown through experiments on Amazon EC2  \cite{Lee-NIPS-2015}.
%
%\subsubsection{Theoretical Research} 
%There has been a growing interest in understanding and characterizing the delay performance of replication and coding techniques. One focus in this area is fast data retrieval in distributed storage systems. In \cite{huang-isit-2012}, Huang et al. showed that codes can reduce the queueing delay in distributed storage systems. In \cite{Joshi-2012,shah-mdsq-2012,Kumar2014}, the authors obtained bounds on the mean average delay of redundant data downloading policies. In \cite{addShengboOriginal,Liang2013_2}, Liang and Kozat provided an approximate analysis for the delay performance of redundant data downloading policies, based on their measurements on Amazon S3. 
%There also exist some analytical studies on distributed computing systems.
%In \cite{Wang:2014,Wang2015}, Wang et al. studied the tradeoff between delay and computing cost in cloud computing systems.
%For Poisson arrivals and exponential service times, Gardner et al. \cite{Kristen2015} characterized the response time distribution for several replication policies in distributed queueing systems. Recently, the delay performance of replications was analyzed in the context of load-balancing \cite{BinInfoCom2016,Gardner2016}, where the number of servers may potentially grow to infinity.  
%
%In addition to the aforementioned studies that focus on delay analysis and characterization, there also exist a few works which aim to find delay-optimal scheduling policies of replications and coding. If the task service times are geometrically distributed and each job has a single task, it was shown in \cite{Borst2003} that distributing the tasks over the servers as evenly as possible is delay-optimal among all admissible policies. 
%Later, delay-optimal scheduling of replications was studied for more general service time distributions, such as New-Better-than-Used (NBU) distributions and New-Worse-than-Used (NWU) distributions \cite{Righter2008,Kim2010}. In \cite{shah-Allerton-2013,Lee-Allerton-2015,Joshi2015}, the delay performance of replication policies was analyzed in a few different models, where the optimal policies were obtained for minimizing the mean average delay within a specific family of policies.
%In \cite{ShengboInfocom}, Chen et al. presented some similar results with \cite{shah-Allerton-2013}, where the difference is that the delay optimality results in  \cite{ShengboInfocom} were established among all admissible policies. 
%
%This paper differs from the existing works in two aspects: First, our study is carried out for very general system settings and  delay metrics, some of which are considered in the study of replications for the first time. Second, in our study, delay optimality results are established  when it is possible; and in some more general scenarios where delay optimality is inherently difficult to achieve, alternative near delay optimality results with small sub-optimality gaps are obtained. 
%
%Some preliminary ideas of this paper were presented in \cite{Sun2015}.

\subsection{Organization of the Paper}
%The rest of the paper is organized as follows: 
We describe the system model and problem formulation in Section \ref{sec_model}, together with the notations that we will use throughout the paper. Some near delay optimality results are introduced in Section \ref{sec_analysis}, which are proven in Section \ref{sec_proofmain}.
%In Section \ref{sec_sufficient}, some novel sample-path orderings are introduced, which can be used to obtain delay inequalities. Further, sufficient conditions for these sample-path orderings and delay inequalities are presented in Section \ref{sec_delay_ineq}.  
Finally, some conclusion discussions are presented in Section \ref{sec_conclusion}. 



%In order to understand how close the considered policies are from delay optimality, we further characterize the sub-optimal delay gap for some important delay metrics: It is show that the FUT policy is within a constant additive gap from the optimum for minimizing the mean average delay (Theorem \ref{lem7_NBU}), and the FCFS policy is within twice of the optimum for minimizing the mean maximum delay and the mean $p$-norm of delay (Theorems \ref{thm_max_delay_ratio}-\ref{thm_max_delay_ratio_1}). 

%The FUT policy is a nice approximation of the SRPT policy in the considered queueing systems: The FUT policy utilizes the number of unassigned tasks of a job to approximate its remaining processing time. While there exist many different ways to approximate the remaining processing time of a job, it is not easy to find an approximation that leads to a provable and tight sub-optimal delay gap. 






%Traditional sample-path methods --- such as forward induction, backward induction, and interchange arguments \cite{Liu1995} ---  can be used to establish delay optimality when possible. However, in the considered parallel-server scenarios where delay optimality is inherently difficult to achieve, it is challenging to relax the delay inequalities in these methods and prove near delay-optimal results. On the other hand, the sample-path orderings, weak work-efficiency orderings, and coupling arguments in this paper form an ingenious and powerful framework for showing near delay optimality.






==> v3/model.tex <==
% !TEX root = ./parallel_servers.tex
%\ifreport
%\begin{table*}
%\centering
%\footnotesize
%\begin{tabular}{|c| c | c | c | c | c | c | c|} \hline
%           & \!Arrival\!  & Job&  Delay               & Distributions of   & Queueing   & Proposed      &  Delay  \\
%\!\!Theorem\!\!  & \!process\!&\!size\! &  \!metrics\!       & task service time  & buffers & scheduling policies &  optimality \\
%\hline
%\ref{thm1} & any & any &  $D_{\text{avg}}$     & independent NBU  & centralized   & FUT-NR, FUT-NIR    & near optimal \\
%\hline
%\ref{thm2} & any & any &  $D_{\text{avg}}$      & independent NWU  & centralized   & FRT-R            & near optimal  \\
%\hline
%\ref{thm3} & any & any &  $L_{\max}$    &  independent NBU   & centralized  & EDD-NR, EDD-NIR  & near optimal \\
%\hline
%\ref{thm4} & any & any &  $L_{\max}$        & independent NWU & centralized    & EDD-R            & near optimal  \\
%\hline
%\ref{thm5} & any & any &  $D_{\max}$   & independent NBU & centralized & \!\!FCFS-NR, FCFS-NIR\!\! & near optimal\\
%\hline
%\ref{thm6} & any & any &  $D_{\max}$     & independent NWU & centralized &  FCFS-R  & near optimal  \\
%\hline
%\ref{thm_dis4} & any & any &  $L_{\max}$    & \!\!independent NBU/NWU\!\!     & distributed  & EDD-GR & near optimal \\
%&  &  &         & for each group of servers &  with data locality   &            &   \\
%\hline
%\ref{thm_dis5} & any & any &  $D_{\max}$   & \!\!independent NBU/NWU\!\!  & distributed & FCFS-GR  & near optimal\\
%&  &  &      & for each group of servers & with data locality &    & \\
%%\ref{thm5} & any & $k_i =1$, $d_{\min}\geq L$   &Multivariate  NBU& SEDPT-R            & near optimal\\
% \hline
%\end{tabular}
%\caption{Summary of delay optimality results in this paper, where New-Better-than-Used (NBU) and  New-Worse-than-Used (NWU) distributions are defined in Section \ref{sec:model}, the delay metrics are defined in Section \ref{sec:metrics}, and near delay optimality is defined in Section \ref{sec_optimality}. The average delay $D_{\text{avg}}$, maximum lateness $L_{\max}$, and maximum delay $D_{\max}$ are analyzed in Theorems \ref{thm1}-\ref{thm_dis5}, and more general delay metrics are studied in the corollaries of these theorems.
% }\label{tab2}
%%\hspace{-0.8cm}
%\end{table*}
%\fi

%\section{Related Works}
%In storage clouds, data is stored across numerous disks by using erasure codes. Suppose that an $(n_i,k_i)$ code is used to stored file $i$, the system can launch more than $k_i$ downloading connections to fetch coded chunks such that file $i$ is retrieved if any $k_i$ out of $n_i$ chunks are downloaded.
%
% The requested file is fetched if any $k$ coded chunks  are  connections to download data chunks. The requested data
%To reduce data retrieval latency,
%
%
%Suppose that file $i$ is stored by using a $(n_i,k_i)$ code, then file $i$ is retrieved
%
%Suppose the $i$-th requested file is stored by  A front-end proxy server may launch $m$ connections to retrieve coded data chunks for different storage disks.
\section{Model and Formulation}\label{sec_model}
\subsection{Notations and Definitions}
We will use lower case letters such as $x$ and $\bm{x}$, respectively, to represent deterministic scalars and vectors.
In the vector case, a subscript will index the components of a vector, such as $x_i$.
%; on the other hand, a superscript will index scalars and vectors, e.g., ${x}^{\pi}$ and $\bm{x}^{\pi}$.
We use $x_{[i]}$ and $x_{(i)}$, respectively, to denote the $i$-th largest and the $i$-th smallest components of $\bm{x}$.  %If $\mathcal{S}\subseteq\{1,\ldots,n\}$, let $\bm{x}_\mathcal{S}$ denote the vector of the $x_i$'s such that $i\in \mathcal{S}$.
For any $n$-dimensional vector $\bm{x}$, let $\bm{x}_{\uparrow}=(x_{(1)},\ldots,x_{(n)})$ %and $\bm{x}_{\downarrow}=(x_{[1]},\ldots,x_{[n]})$, respectively,
denote the increasing %and decreasing
rearrangement of $\bm{x}$.  Let $\bm{0}$
% and $\bm{e}$, respectively,
denote the vector %s
with all 0 %and all 1
components.
%denote the vector composed of the components of $\bm{x}$ indexed by $\mathcal{S}$.

Random variables and vectors will be denoted by upper case letters such as $X$ and $\bf{X}$, respectively, with the subscripts and superscripts following the same conventions as in the deterministic case. %Matrices will be also denoted by upper case letters such as $W$ and $U$, which will not be confused with random variables from the content.
Throughout the paper, ``increasing/decreasing'' and ``convex/concave'' are used in the non-strict sense. LHS and RHS denote, respectively, ``left-hand side'' and ``right-hand side''.

For any $n$-dimensional vectors $\bm{x}$ and $\bm{y}$, the elementwise vector ordering $x_i\leq y_i$, $i=1,\ldots,n$, is denoted by $\bm{x} \leq \bm{y}$. Further, $\bm{x}$ is said to be \emph{majorized} by $\bm{y}$, denoted by $\bm{x}\prec\bm{y}$, if (i) $\sum_{i=1}^j x_{[i]} \leq \sum_{i=1}^j y_{[i]}$, $j=1,\ldots,n-1$ and (ii) $\sum_{i=1}^n x_{[i]} = \sum_{i=1}^n y_{[i]}$ \cite{Marshall2011}. In addition, $\bm{x}$ is said to be  \emph{weakly majorized by $\bm{y}$ from below}, denoted by $\bm{x}\prec_{\text{w}}\bm{y}$, if $\sum_{i=1}^j x_{[i]} \leq \sum_{i=1}^j y_{[i]}$, $j=1,\ldots,n$; $\bm{x}$ is said to be  \emph{weakly majorized by $\bm{y}$ from above}, denoted by $\bm{x}\prec^{\text{w}}\bm{y}$, if $\sum_{i=1}^j x_{(i)} \geq \sum_{i=1}^j y_{(i)}$, $j=1,\ldots,n$ \cite{Marshall2011}.
A function that preserves the majorization order is called a Schur convex function. Specifically, $f: \mathbb{R}^n\rightarrow \mathbb{R}$ is termed \emph{Schur convex} if $f(\bm{x})\leq f(\bm{y})$ for all $\bm{x}\prec\bm{y}$ \cite{Marshall2011}. A function $f: \mathbb{R}^n\rightarrow \mathbb{R}$ is termed \emph{symmetric} if $f(\bm{x})= f(\bm{x}_{\uparrow})$ for all $\bm{x}$. A function $f: \mathbb{R}^n\rightarrow \mathbb{R}$ is termed \emph{sub-additive} if $f(\bm{x}+\bm{y})\leq f(\bm{x})+f(\bm{y})$ for all $\bm{x},\bm{y}$. The composition of functions $\phi$ and $f$ is denoted by $\phi \circ f (\bm{x}) = \phi(f (\bm{x}))$. Define $x\wedge y=\min\{x,y\}$.

Let $\mathcal{A}$ and $\mathcal{S}$ denote sets and events, with $|\mathcal{S}|$ denoting the cardinality of $\mathcal{S}$.
For all random variable ${X}$ and event $\mathcal{A}$, let $[{X}|\mathcal{A}]$ denote a random variable whose distribution is identical to the conditional distribution of ${X}$ for given $\mathcal{A}$. A random variable ${X}$ is said to be stochastically smaller than another random variable ${Y}$, denoted by ${X}\leq_{\text{st}}{Y}$, if $\Pr({X}>x) \leq \Pr({Y}>x)$ for all~$x\in \mathbb{R}$.
A set $\mathcal{U} \subseteq \mathbb{R}^n$ is called \emph{upper}, if $\bm{y} \in \mathcal{U}$ whenever $\bm{y}\geq \bm{x}$ and $\bm{x} \in \mathcal{U}$. 
A random vector $\bm{X}$ is said to be \emph{stochastically smaller} than another random vector $\bm{Y}$, denoted by $\bm{X}\leq_{\text{st}}\bm{Y}$, if $\Pr(\bm{X}\in \mathcal{U}) \leq \Pr(\bm{Y}\in \mathcal{U})$ for all upper sets ~$\mathcal{U}\subseteq \mathbb{R}^n$. If $\bm{X}\leq_{\text{st}}\bm{Y}$ and $\bm{X}\geq_{\text{st}}\bm{Y}$, then $\bm{X}$ and $\bm{Y}$ follow the same distribution, denoted by $\bm{X}=_{\text{st}}\bm{Y}$. We remark that $\bm{X}\leq_{\text{st}}\bm{Y}$  if, and only if,
\begin{align}\label{eq_order_property}
 \mathbb{E}[\phi(\bm{X})] \leq \mathbb{E}[\phi(\bm{Y})]
\end{align}
holds for all increasing $\phi: \mathbb{R}^n\rightarrow \mathbb{R}$ for which the expectations in \eqref{eq_order_property} exist.

%It is worth noting that $\bm{X}\leq_{\text{st}}\bm{Y}$ if, and only if, there exist two random vectors $\bm{\hat{X}}$ and $\bm{\hat{Y}}$ such that $\bm{\hat{X}}=_{\text{st}}\bm{X}$, $\bm{\hat{Y}}=_{\text{st}}\bm{Y}$, and $\bm{\hat{X}}\leq\bm{\hat{Y}}$ with probability one.
%Stochastic ordering of stochastic processes can be defined similarly \cite{StochasticOrderBook}.
%Define $1_{A}$ as the indicator function of event $A$, i.e.,
%\begin{align}
%1_{A}(x) =\left\{\begin{array}{l l} 1& \text{if}~x\in A;\\ 0 &\text{if}~x\notin A.\end{array}\right.
%\end{align}
%Let $|S|$ denote the cardinality of set $\mathcal{S}$ and $a\wedge b=\min[a,b]$.

%It is known that $\bm{X}\leq_{\text{st}}\bm{Y}$ if and only if \cite{StochasticOrderBook}
%\begin{align}\label{eq_property}
%\mathbb{E}[\phi(\bm{X})] \leq \mathbb{E}[\phi(\bm{Y})]
%\end{align}
%holds for all non-decreasing function $\phi$ for which the expectations exist.
%%\end{property}
%We say $\bm{X}=_{\text{st}}\bm{X}$ if $\bm{X}\leq_{\text{st}}\bm{Y}$ and $\bm{X}\geq_{\text{st}}\bm{Y}$.

% let $\bf{x}_{\uparrow}=(x_{(1)},x_{(2)},\ldots, x_{(m)})$ denote increasing rearrangement of $\bm{x}$.

%A set $U \subseteq \mathbb{R}^m$ is called \emph{upper}, if for all $\bm{x} \in U$ and $\bm{y}\geq \bm{x}$ it holds that $\bm{y} \in U$.
%\begin{definition}
%\textbf{Stochastic Ordering of Random Variables \cite[p. 1]{StochasticOrderBook}}:
%Let ${X}$ and ${Y}$ be two random variables. Then, ${X}$ is said to be \emph{stochastically smaller} than ${Y}$ (denoted by ${X}\leq_{\text{st}}{Y}$), if
%\begin{eqnarray}
%\Pr({X}>t) \leq \Pr({Y}>t),~\forall~t\in \mathbb{R}.
%\end{eqnarray}
%\end{definition}
%
%
%
%\begin{definition}\label{def_vector}
%\textbf{Stochastic Ordering of Random Vectors \cite[p. 266]{StochasticOrderBook}}:
%Let $\bm{X}$ and $\bm{Y}$ be two random vectors. Then, $\bm{X}$ is said to be \emph{stochastically smaller} than $\bm{Y}$ (denoted by $\bm{X}\leq_{\text{st}}\bm{Y}$), if
%\begin{eqnarray}
%\Pr(\bm{X}\in U) \leq \Pr(\bm{Y}\in U)~\text{for all upper sets}~U\subseteq \mathbb{R}^m.
%\end{eqnarray}
%\end{definition}
%
%It is known that $\bm{X}\leq_{\text{st}}\bm{Y}$ if and only if \cite{StochasticOrderBook}
%\begin{align}\label{eq_property}
%\mathbb{E}[\phi(\bm{X})] \leq \mathbb{E}[\phi(\bm{Y})]
%\end{align}
%holds for all non-decreasing function $\phi$ for which the expectations exist.
%%\end{property}
%We say $\bm{X}=_{\text{st}}\bm{X}$ if $\bm{X}\leq_{\text{st}}\bm{Y}$ and $\bm{X}\geq_{\text{st}}\bm{Y}$.
%
%\begin{definition}\label{def_process}
%\textbf{Stochastic Ordering of Stochastic Processes \cite[p. 281]{StochasticOrderBook}}:
%Let $\{X(t),t\in \mathcal{T} \}$ and $\{X(t),t\in \mathcal{T} \}$ be two stochastic processes with time parameter space $\mathcal{T}$ (usually $\mathcal{T}=[0,\infty)$ or $\mathcal{T}=\mathbb{n}_+$). Then, $\{X(t),t\in \mathcal{T} \}$ is said to be \emph{stochastically smaller} than $\{X(t),t\in \mathcal{T} \}$ (denoted by $\{X(t),t\in \mathcal{T} \}\leq_{\text{st}}\{Y(t),t\in \mathcal{T} \}$), if for all integer $m$ and $t_1< t_2<\ldots<t_m$ in $\mathcal{T}$, it holds that
%\begin{eqnarray}
%\!\!(X(t_1),X(t_2),\ldots,X(t_m)) \!\leq_{\text{st}}\! (Y(t_1),Y(t_2),\ldots,Y(t_m)),\!\!\!
%\end{eqnarray}
%where $\leq_{\text{st}}$ is in the sense of \emph{Definition \ref{def_vector}}.
%\end{definition}



%NBU distributions can be used to characterize the service times of healthy servers: The longer a healthy server has worked on a task, the more likely it will finish soon \cite{Righter2008}.
%NBU distributions include log-concave distributions and increasing hazard rate (IHR) distributions as special cases \cite{StochasticOrderBook}. {\red One example is the discrete distribution of $X\in \{1, 2\}$ with probability 0.5, which is NBU but neither log-concave nor IHR.}

%For a healthy server, the processing time of a new task that has not been served is usually longer than the remaining processing time of a task that has been served for $\tau$ time units in distributions, which is expressed in \eqref{eq_light}.

%\begin{definition} \textbf{New-Worse-than-Used:} \cite{StochasticOrderBook}
%We say that a random variable $X$ is \emph{New-Worse-than-Used (NWU)}, if for all $t,\tau\geq 0$ and $\Pr(X>\tau)>0$
%\begin{eqnarray}\label{eq_heavy}
%\Pr[X>t]\leq\Pr[X-\tau>t|X>\tau].
%\end{eqnarray}
%Hence, the remaining processing time of a task that has been served for $\tau$ time units is \emph{stochastically larger} than the processing time of a new task that has not been served.
%\end{definition}
%NWU distributions can be used to characterize occasional slow responses that is commonly observed in cloud computing systems \cite{Dean:2013:Tail,C3:2015}: The longer a server has processed a task, the more likely it has experienced a malfunction and will complete late. NWU distributions include the classes of log-convex distributions and decreasing  hazard rate (DHR) distributions \cite{StochasticOrderBook}.



\begin{figure}
\centering
\includegraphics[width=0.5\textwidth]{Figures/queue_model_1}
\caption{A centralized queueing system, where a scheduler assigns the tasks of arrived jobs to the servers.} \label{fig1model_central}
\end{figure}

\subsection{Queueing System Model}\label{sec:model}
Consider a queueing system with $m$ parallel servers, as shown in Fig. \ref{fig1model_central}, which starts to operate at time $t=0$. %, denoted by $\mathcal{M}=\{1,2,$ $\ldots,m\}$.
A sequence of $n$ jobs arrive at time instants $a_1,\ldots,$ $a_n$ and are stored in a job queue, where $n$ is an arbitrary positive integer, no matter finite or infinite, and $0=a_1\leq a_2\leq\cdots\leq a_n$. %If $n$ is finite, denote $a_{n+1}=\infty$. The inter-arrival time is denoted by $T_i = a_{i+1}-a_i$. %If $n$ is finite, denote $a_{n+1}=\infty$. %The incoming jobs are admitted into a queue, where they wait to be served.
The $i$-th arrived job, called job $i$, brings with it a batch of $k_i$ tasks.
%, where $k_i$ can be larger or smaller than $m$.\footnote{Previous delay analyses of task replications\cite{Borst2003,Righter2008,Kim2010,Joshi-2012,shah-Allerton-2013,Wang:2014,Wang2015,Joshi2015,Lee-Allerton-2015} focused on the case $k_i\leq m$. However, $k_i$ can be larger than $m$ in real systems \cite{Ananthanarayanan:2012,Sparrow:2013}.}
Each task is of one unit of work, and can be flexibly assigned to any server.  Job $i$ is completed when all $k_i$ tasks of job $i$ are completed. The maximum job size is\footnote{If $n\rightarrow\infty$, then the $\max$ operator in \eqref{eq_0} is replaced by $\sup$.}
\begin{align}\label{eq_0}
k_{\max} = \max_{i=1,\ldots,n}k_i.
\end{align}
%We consider a centralized queueing model, where 
%In a centralized queueing system, 
%the jobs arrive at a scheduler and are stored in a job queue. 

%The scheduler queries the idle/busy state of each server, and assigns tasks to the available servers over time.


 

%\ifreport
%\begin{figure*}
%\captionsetup{justification=centering}

%\caption{Queueing models.} \label{fig1model}
%\end{figure*}
%\else
%\begin{figure*}
%\centering
%\begin{subfigure}[b]{0.4\textwidth}
%\centering
%\includegraphics[width=\textwidth]{Figures/queue_model_1} \caption{Centralized queueing model.}
%\end{subfigure}
%~~~~
%\begin{subfigure}[b]{0.55\textwidth}
%\includegraphics[width=\textwidth]{Figures/queue_model_3} \caption{Distributed queueing model.}
%\end{subfigure}
%\caption{Queueing model.} \label{fig1model}
%\end{figure*}
%\fi
%In practical systems, the task service times are highly random and may have a long latency tail due to many reasons, including resource sharing, network interference, cache misses,  database blocking, background activities, hardware/software failures, and so on \cite{Dean:2013:Tail}. In addition, the servers may operate at different speeds, because they have diverse amounts of resources, e.g., CPU, memory, and I/O bandwidth \cite{Googletrace2012,C3:2015}. We assume that the tasks are statistically identical, but the servers can have different speeds, or in general different service time distributions. Therefore, the service time distribution of a task depends only on which server is assigned to execute the task. In addition, 


 %, which are invariant for all scheduling policy of the system. 


%\subsubsection{Service Time Distributions} 
\label{sec_Multivariate}
%Existing delay optimality analyses of task replications \cite{Borst2003,Righter2008,Kim2010,shah-Allerton-2013,ShengboInfocom,Sun2015} assumed that the task service times are NBU (or NWU), and are \emph{independent} across time and servers.
%The task service times of the servers are assumed to be NBU and NWU distributions

%Let  $X_l$ and $O_l$ represent the random service time and cancellation overhead of server $l$, respectively. The  service rate of server $l$ is $\mu_l= 1/\mathbb{E}[X_l]$. Denote $\bm{X}=(X_1,\dots,X_m)$ and $\bm{O}=(O_1,\dots,O_m)$, which are  assumed to be \emph{mutual independent}.

A scheduler assigns the tasks of arrived jobs to the servers over time. The service times of the tasks  are assumed to be \emph{independent} across the servers and \emph{i.i.d.} across the tasks assigned to the same server.
%While each task is of the same amount of work, the servers can have different service times to execute the tasks. %To model this, we assume that
%The task service times are \emph{independent} across the servers and \emph{i.i.d.} across the tasks assigned to the same server. 
Let $X_l$ represent the random service time of server $l$. The service rate of server $l$ is $\mu_l= 1/\mathbb{E}[X_l]$, which may vary across the servers. Denote $\bm{X}=(X_1,\dots,X_m)$.
We consider the classes of NBU task service time distributions.
\begin{definition}
Consider a non-negative random variable $X$ with complementary cumulative distribution function (CDF)  $\bar{F}(x)=\Pr[X>x]$. Then, $X$ is \textbf{New-Better-than-Used (NBU)} if for all $t,\tau\geq 0$
\begin{eqnarray}\label{eq_NBU}
\bar{F}(\tau+t)\leq \bar{F}(\tau)\bar{F}(t).
\end{eqnarray}
%On the other hand, $X$ is \textbf{New-Worse-than-Used (NWU)} if $\bar{F}$ is \emph{absolutely continuous} and for all $t,\tau\geq 0$
%\begin{eqnarray}\label{eq_NWU}
%\bar{F}(\tau+t)\geq\bar{F}(\tau)\bar{F}(t).
%\end{eqnarray}
%In the language of stochastic ordering, this can be ex $X \geq_{\text{st}} (\leq_{\text{st}}) [X-\tau| X>\tau]$ .
\end{definition}
%%We note that the definition of NWU distributions in \eqref{eq_NWU} is different from the traditional definition of NWU distributions in reliably theory \cite[p. 1]{StochasticOrderBook}, because of an additional condition on the absolutely continuity of $\bar{F}$. The res
%
%NBU distributions include increasing failure rate (IFR) distributions and log-concave distributions as special cases. %\footnote{If a random variable has log-concave (log-convex) density function, then it is IHR (DHR).}
%Examples of NBU distributions include constant service time, shifted exponential distribution, geometrical distribution, Erlang distribution, etc. Recent measurements \cite{addShengboOriginal,Liang2013_2} show that the data downloading time in Amazon AWS can be approximated as a shifted exponential distribution. 
%NWU distributions include the classes of decreasing failure rate (DFR) distributions and log-convex distributions. Examples of NWU distributions include hyperexponential distribution, Pareto type II (Lomax) distribution \cite{Arnold99}, gamma distributions with $m<1$, Weibull distribution with $c<1$, etc. Task execution time can be modeled as a hyperexponential distribution in some systems \cite{Christodoulopoulos2008}. 
%A random variable is both NBU and NWU if, and only if, it is exponential. %More general service time distributions will be studied in our future work.

%In real systems, task executions exhibit \emph{spatial correlation} across the servers
%\cite{Rish2004,Fu2007,Googletrace2012,Liang2013_2}, which was not considered in prior theoretical studies \cite{Borst2003,Righter2008,Kim2010,shah-Allerton-2013,ShengboInfocom,Sun2015}.
%To model this, we generalize the above univariate NBU and NWU distributions %of univariate service time distributions %in \cite{Borst2003,Righter2008,Kim2010,shah-Allerton-2013,ShengboInfocom,Sun2015}
%to multivariate NBU and NWU distributions. % with spatial correlation. %and cancellation overheads $\bm{O}$.
%We will use these generalized distributions to answer some open questions.
%
%\begin{definition}\label{independent NBU}
%Consider an $m$-dimensional non-negative random vector $\bm{X}$ with survival function $\bar{F}(\bm{x})=\Pr[\bm{X}>\bm{x}]$, $\bm{X}$ is \emph{Multivariate-New-Better-than-Used (independent NBU)}, if for all ${t}\geq0,\bm{\tau}\geq \bm{0}$ and $i=1,\ldots,m$
%%\begin{align}\label{eq_independent NBU}
%%\bar{F}(\bm{\tau}+t \bm{e})\leq \bar{F}(\bm{\tau})\bar{F}(t\bm{e}),
%%\end{align}
%\begin{align}\label{eq_independent NBU}
%&\bar{F}(\tau_1+t,\!\ldots\!,\taV_i+t,\!\ldots\!,\tau_{m}+t)\bar{F}(\tau_1,\!\ldots\!,\tau_{i-1},0,\tau_{i+1},\!\ldots\!,\tau_{m})\nonumber\\
%\leq& \bar{F}(\tau_1+t,\!\ldots\!,\tau_{i-1}+t,t,\tau_{i+1}+t,\!\ldots\!,\tau_{m}+t)\nonumber\\
%&~\times\bar{F}(\tau_1,\ldots,\taV_i,\ldots,\tau_{m}). \!\!\!\!
%\end{align}
%%with $\bm{e}=(1,\ldots,1)$, and (ii) the condition (i) holds for all lower dimensional marginals of $\bar{F}$.
%On the other hand, $\bm{X}$ is \emph{Multivariate-New-Worse-than-Used (independent NWU)}, if for all ${t}\geq0,\bm{\tau}\geq \bm{0}$ and $i=1,\ldots,m$
%\begin{align}\label{eq_independent NWU}
%&\bar{F}(\tau_1+t,\!\ldots\!,\taV_i+t,\!\ldots\!,\tau_{m}+t)\bar{F}(\tau_1,\!\ldots\!,\tau_{i-1},0,\tau_{i+1},\!\ldots\!,\tau_{m})\nonumber\\
%\geq& \bar{F}(\tau_1+t,\!\ldots\!,\tau_{i-1}+t,t,\tau_{i+1}+t,\!\ldots\!,\tau_{m}+t)\nonumber\\
%&~\times\bar{F}(\tau_1,\ldots,\taV_i,\ldots,\tau_{m}), \!\!\!\!
%\end{align}
%%(i') for all ${t}\geq0,\bm{\tau}\geq \bm{0}$
%%\begin{align}\label{eq_independent NWU}
%%\bar{F}(\bm{\tau}+t \bm{e})\geq \bar{F}(\bm{\tau})\bar{F}(t\bm{e}),
%%\end{align}
%%(ii') the condition (i') holds for all lower dimensional margin-als of $\bar{F}$, and (iii')
%and $\bar{F}$ is absolutely continuous.
%\end{definition}
%
%
%
%Unlike the univariate case, various possibilities of independent NBU and independent NWU notions have been proposed in the literature; see \cite{Buchanan1977,marshall1982,Neweihi1983,Marshall1986,Roy1994,Belzunce2014} and the references therein. We will see that the independent NBU and independent NWU distributions defined in \emph{Definition \ref{independent NBU}} fit well with the delay optimality analysis of task replications. To the extent of our knowledge, the independent NBU and independent NWU distributions defined in \emph{Definition \ref{independent NBU}} are novel. Special cases of independent NBU (independent NWU) distributions include multivariate increasing failure rate or MIFR (multivariate decreasing failure rate or MDFR) distributions of Brindley and Thompson \cite{Brindley1972}, with an additional requirement on absolutely continuity of $\bar{F}$ for MDFR distributions.
%%A key property of independent NBU (independent NWU) distributions is as follows:
%
%
%\begin{lemma}\label{lem_ass1}
%independent NBU and independent NWU distributions have the following properties:
%\begin{itemize}
%\itemsep0em
%\item[1.] An NBU (NWU) random variable is independent NBU (independent NWU).
%\item[2.] The union of two mutually independent sets of independent NBU (independent NWU) random variables is independent NBU (independent NWU).
%%\item[3.] Any subset of independent NBU (independent NWU) random variables is independent NBU (independent NWU).
%\item[3.] Suppose that the components of $\bm{X}$ and $\bm{Y}$ satisfy $Y_i =\min_{j\in\mathcal{S}_i} X_j$ for all $i$. If $\bm{X}$ is independent NBU, then $\bm{Y}$ is independent NBU. If $\bm{X}$ is independent NWU and the
%$\mathcal{S}_i$'s are disjoint sets, then $\bm{Y}$ is independent NWU.
%
%%\item[6.] A set of random variables is both independent NBU and independent NWU if, and only if, they are independent exponentials.
%
%\item[4.]\label{lem_property_independent NBUindependent NWU} If an $m$-vector $\bm{X}$ is
%independent NBU (independent NWU), then for all $t\geq0$, $\bm{\tau}\geq \bm{0}$, and $\mathcal{S}\subseteq\{1,\ldots,m\}$
%%\emph{\begin{align}\label{eq_property_independent NBUindependent NWU}
%%&\Big[\min_{l=1,\ldots,m}(X_l-\tau_l)\Big| \bm{X}> \bm{\tau} \Big]\nonumber\\
%%\leq_{\text{st}}(\geq_{\text{st}})&\Big[\min\Big\{\min_{l\in\mathcal{S}}(X_l-\tau_l),\min_{l\in\mathcal{S}^c}X_l\Big\} \Big| \bm{X}_{\mathcal{S}}> \bm{\tau}_{\mathcal{S}}\Big].
%%\end{align}}
%\emph{\begin{align}\label{eq_property_independent NBUindependent NWU}
%&\Pr\Big[\min_{l=1,\ldots,m}(X_l-\tau_l)>t\Big| \bm{X}> \bm{\tau} \Big]\nonumber\\
%\leq(\geq)&\Pr\!\Big\{\min\Big[\min_{l\in\mathcal{S}}(X_l-\tau_l),\min_{l\in\mathcal{S}^c}X_l\Big]>t \Big| \bm{X}_{\mathcal{S}}> \bm{\tau}_{\mathcal{S}}\Big\}.\!\!
%\end{align}}
%\end{itemize}
%\end{lemma}
%\begin{proof}
%See Appendix \ref{app_independent NBUproperty}.
%\end{proof}
%%Some properties of independent NBU and independent NWU distributions are provided in Appendix \ref{app_independent NBUproperty}.
%
%%\item[5.]
%The $n$-dimensional multivariate exponential distribution of Marshall and Olkin \cite{Marshall1967} with $\bar{F}$ defined in \eqref{MOexp} is independent NBU, where
%\begin{align}\label{MOexp}
%\!\!\!\!\bar{F}(\bm{x}) = \exp\Bigg(-\sum_{\mathcal{S}\subseteq \{1,\ldots,n\}} \lambda_{\mathcal{S}}\max_{l\in \mathcal{S}} x_l\Bigg),~~\lambda_{\mathcal{S}}\geq0.%\nonumber
%\end{align}
%

%\subsubsection{Queueing Model}\label{eq_model_heter}

%\subsubsection{Task Assignment}




%\textbf{Centralized queueing model:}



%In order to reduce response latency, a task can be \textbf{replicated} on multiple servers, possibly at different time instants.
%The task is deemed complete when one copy of the task is completed. After that, the other redundant copies of the task are either cancelled, which may incur a delay overhead, or executed until completion. %One example of centralized queueing system with and without task replication operations are illustrated in Fig. \ref{fig2central_replication}.
% We assume that the cancellation overheads are \emph{independent} across the servers and \emph{i.i.d.} across the  cancellation operations occurring on a server. 

%\ifreport
%\begin{figure*}
%%\captionsetup{justification=centering}
%\centering
%\begin{subfigure}[b]{\textwidth}
%\centering
%\includegraphics[width=0.9\textwidth]{Figures/replicates_1}
%\caption{\textbf{The Power of $k$ Choices policy:} The scheduler queries the queue lengths of $k=2$ servers, and assigns a task to the server with the shortest queue length.}
%\end{subfigure}
%\begin{subfigure}[b]{\textwidth}
%\centering
%\includegraphics[width=0.9\textwidth]{Figures/replicates_3}
%\caption{\textbf{Cancel-After-Execution policy:} Each task is replicated in both queues and can be assigned to both servers. If one copy of task 1 completes execution on one server, a message is sent to cancel the other copy of task 1, which is being executed on the other server.}
%\end{subfigure}
%\begin{subfigure}[b]{\textwidth}
%\centering
%\includegraphics[width=0.9\textwidth]{Figures/replicates_2}
%\caption{\textbf{Cancel-Before-Execution policy:} Each task is replicated in both queues, but can be only assigned to one server. If one copy of task 2 starts execution on one server, a message is sent to cancel the other copy of task 2, which is waiting in the queue on the other server.}
%\end{subfigure}
%\caption{Task assignment policies for a distributed queueing system with two task queues on two servers. This system is a part of the distributed queueing system in Fig. \ref{fig1model_distri}.} \label{fig3_distri_replication}
%\end{figure*}
%\else
%\fi

 



%When task replication occurs, a task is redundantly assigned to multiple servers, at possibly different time instants when the servers are available.

%which might be  they are idle.



%. A task dispatcher assigns tasks to the servers

%The job queue is connected to a task dispatcher, which has access to the idle/busy state of the servers. The task dispatcher assigns tasks to servers which are idle.

%A task dispatcher assigns tasks to the servers over time The task dispatcher has access to the idle/busy state of the servers, and hence only tasks to idle servers.
%This model can be used to characterize centralized machine scheduling in a cloud computing cluster\cite{Zaharia2012}, the control of TCP ports on a Web server \cite{Borg2015}, multipath routing in communication networks \cite{DTN-delay}, and core scheduling in a multi-core processor \cite{Ranger2007}.

%\textbf{Distributed queueing model:}
%In a distributed queueing system, the jobs arrive at a number of parallel schedulers, and are stored in  
%the job queues associated to the schedulers, as depicted in Fig. \ref{fig1model_distri}. Each scheduler independently assigns tasks to the servers.
%The servers  are divided into $g$ groups, where each group has $v=m/g$ servers.  Each server has a task queue, which stores the tasks assigned from different schedulers.
%The task assignment of the schedulers is subject to \textbf{data locality} constraints \cite{taskplacement2011,Sparrow:2013}. More specifically, each task can be only executed by one group of servers, each of which stores one copy of the data necessary for executing the task.
%Based on our communications with some Web service companies, such group-based data locality constraints are used in their Web-searching systems.


%There are multiple ways to assign a task to its required group of the servers. \textbf{The Power of $k$ Choices} load balancing policy is illustrated in Fig. \ref{fig3_distri_replication}(a), where the scheduler queries the queue lengths of $k$ servers in one group ($k\leq v$), and selects the server with the shortest queue length. In this policy, it may happen that some queues in the group are empty and the other queues in the group are not, which reduces the efficiency of the system.
%Two alternative task assignment policies are depicted in Fig. \ref{fig3_distri_replication}(b) and Fig. \ref{fig3_distri_replication}(c), where the scheduler simultaneously places multiple copies of a task to all the servers in one group, and the servers are allowed to communicate with each other to cancel the redundant task copies. Such an approach is advocated in \cite{Dean:2013:Tail}. In Fig. \ref{fig3_distri_replication}(b), when one copy of a task starts execution, a message is sent to cancel the other redundant task copies. This policy is called the \textbf{Cancel-After-Execution} policy. In Fig. \ref{fig3_distri_replication}(c), when one copy of a task completes execution, a message is sent to cancel the other redundant task copies. This policy is called the \textbf{Cancel-Before-Execution} policy, which was also named ``tied-requests'' in \cite{Dean:2013:Tail} and ``late-bindling'' in \cite{Sparrow:2013}.
%% the redundant task copies are cancelled when one  copy of the task starts execution; which in Fig. \ref{fig3_distri_replication}(b) the redundant task copies are cancelled when one  copy of the task completes execution. %The technique in Fig. \ref{fig3_distri_replication}(b) was termed ``tied-requests'' in \cite{Dean:2013:Tail} and ``late-bindling'' in \cite{Sparrow:2013}. 
%It was pointed out in \cite{Dean:2013:Tail,Sparrow:2013} that the Cancel-Before-Execution policy
%%in Fig. \ref{fig3_distri_replication}(c) %and Fig. \ref{fig3_distri_replication}(c) are implementable in real systems and
%can potentially achieve a better delay performance than the Power of $k$ Choices load balancing policy.

%By comparing Fig. \ref{fig3_distri_replication} and Fig. \ref{fig3_distri_replication},
%\ifreport
%\begin{figure*}
%%\captionsetup{justification=centering}
%\centering
%\begin{subfigure}[b]{\textwidth}
%\centering
%\includegraphics[width=0.6\textwidth]{Figures/centralized_replications_1}
%\caption{\textbf{Assign-When-Enqueueing policy:} Each task is assigned to one of the two servers when it arrives to the task queue, and cannot be re-assigned to the other server. In this example, tasks 1-4 are assigned to one server when enqueueing. If the other server is idle, only a new arriving task can be assigned to the idle server.}
%\end{subfigure}
%\begin{subfigure}[b]{\textwidth}
%\centering
%\includegraphics[width=0.6\textwidth]{Figures/centralized_replications_3}
%\caption{\textbf{Replication policy:} Each task is replicated on both servers. If one copy of task 1 completes execution on one server, a message is sent to cancel the other copy of task 1, which is being executed on the other server.}
%\end{subfigure}
%\begin{subfigure}[b]{\textwidth}
%\centering
%\includegraphics[width=0.6\textwidth]{Figures/centralized_replications_2}
%\caption{\textbf{No-replication policy:} Each task can be only assigned to one server. If one copy of task 2 starts execution on one server, a message is sent to cancel the other copy of task 2, which is waiting in the queue on the other server.}
%\end{subfigure}
%\caption{Task assignment policies for a centralized queueing system with one task queue and two servers. These policies are equivalent with the policies in Fig. \ref{fig3_distri_replication} for a distributed queueing system.} \label{fig2central_replication}
%\end{figure*}
%\else
%\fi
%
%We note that each task assignment policy in Fig. \ref{fig3_distri_replication} for distribution queueing systems has one equivalent task assignment policy for centralized queueing systems.
%% task assignment policies in Fig. \ref{fig3_distri_replication} for a distributed queueing system are equivalent with the task replication policies in Fig. \ref{fig2central_replication} for a centralized queue system.
%In particular, the Power of $k$ Choices load balancing policy in Fig. \ref{fig3_distri_replication}(a) is equivalent to one instant of the \textbf{Assign-When-Enqueueing policy} in Fig. \ref{fig2central_replication}(a),
%the Cancel-After-Execution policy in Fig. \ref{fig3_distri_replication}(b) is equivalent with the \textbf{Replication policy} in Fig. \ref{fig2central_replication}(b), and the Cancel-Before-Execution policy in Fig. \ref{fig3_distri_replication}(c) is equivalent with the \textbf{No-Replication policy} in Fig. \ref{fig2central_replication}(c). In this paper, we will establish a unified framework to study delay-optimal scheduling in centralized and distributed queueing systems with replications.


%In this sequel, the task assignment operations in Fig. \ref{fig3_distri_replication}(a) is termed ``task replication'', and the task assignment operations in Fig. \ref{fig3_distri_replication}(b) is termed ``non task replication''. We will establish a unified framework to study task replications in centralized and distributed queue systems. Recently, task replications for distributed queueing systems were studied in \cite{Joshi2015}, which did not consider data locality constraints.
%\ifreport

%This model is used in many data-intensive applications, e.g., \cite{Dean:2013:Tail,C3:2015}.
%Each server has a task queue which stores the tasks assigned by different task dispatchers.
%Data locality constraints are common in data-intensive applications, such as web-searching \cite{Dean:2013:Tail}, advertisements \cite{Thusoo:2010}, data analytics \cite{Chang:2006}, etc. 

%In conventional load balancing techniques, the task dispatcher randomly selects two servers from the server group and queries the queue lengths of  sample the queue length at a few server nodes from a group, and place tasks to the server with the shortest queue.

%each group of servers store the data necessary for processing a particular type of tasks. Therefore, .


%In distributed queueing systems, many task dispatchers may simultaneously assign tasks to the same server. These task are buffered in a task queue.




% Each task can be only assigned to the servers of a certain group, which possess the data necessary for processing the task.  Because multiple task dispatchers may route




%In the centralized queue
%
%
%, and $O_l$ dentoe .
%%Experiments on real systems further show that the task service times exhibit correlation across time and servers \cite{Rish2004,Fu2007,Googletrace2012,Liang2013_2}.
%
%
%
%Let $\bm{X}=(X_1,\dots,X_m)$ denote the random vector of the task service times of the $m$ servers, with a joint probability measure $\mu$. For all $\mathcal{A}\subseteq\mathcal{M}$, let $\bm{X}_\mathcal{A}$ denote the vector of $X_l$'s such that $l\in\mathcal{A}$. The servers are allowed to be asynchronized such that different servers may start to process new tasks/replicas at different time instants.
%%where $\bm{\theta}$ is a parameter vector representing the individual and common states of the servers (e.g., healthy/unhealthy state, network congestion, and the availability of shared resources \cite{Rish2004,Fu2007,Isard:2007:AAD:1243418.1243426}). Let $\mathcal{F}_t=\sigma(\bm{\theta}(\tau),\tau\in[0,t])$ denote the $\sigma$-field generated by the parameter vector before time $t$.
%%\footnote{Our analysis applies readily to the general scenario where the server state vector $\{\bm{\theta}(t),[0,\infty)\}$ is a slow-varying stationary process; see Section \ref{} for the details. For ease of presentation, we fix $\bm{\theta}(t)=\bm{\theta}$ at this moment.}
%More specifically, suppose that at a particular time, the servers indexed by $\mathcal{S}\subseteq\mathcal{M}$ are assigned to process new tasks, the servers in $\mathcal{U}\subseteq \mathcal{S}^c= \mathcal{M}/\mathcal{S}$ are busy, and the servers in $\mathcal{S}^c/\mathcal{U}$ are idle. For any given realization of $\bm{X}_{\mathcal{U}}=\bm{x}_{\mathcal{U}}$, $\bm{X}_{\mathcal{S}}$ is \emph{independently} drawn according to the conditional distribution %$p(\mathcal{A}|\bm{x}_{\mathcal{U}})%)=
%$\mu(\bm{X}_{\mathcal{S}}\in \mathcal{A}|\bm{X}_{\mathcal{U}}=\bm{x}_{\mathcal{U}})$ associated with the joint probability measure $\mu$. Let $\bm{O}=(O_1,\dots,O_m)$ denote the random cancellation overhead vector of the $m$ servers. For all $\mathcal{A}\subseteq\mathcal{M}$, let $\bm{O}_\mathcal{A}$ denote the vector of $O_l$'s such that $l\in\mathcal{A}$. We assume that $\bm{X}$ and $\bm{O}$ are independent.

%(t)=\bm{\theta})$ associated with $\mu$.
%Hence, the tasks that are simultaneously served at any time follows the joint probability measure  $\mu$.
% is the joint distribution of  being processed on the $m$ servers at any time.
%The parameter process $\{\bm{\theta}(t),[0,\infty)\}$ is stationary, and
%
%Similarly, let $\bm{O}=(O_1,\dots,O_m)$ denote the random cancellation overhead vector of the $m$ servers with a joint probability measure $\nu$, and $\bm{O}_{\mathcal{S}}$ denote the cancellation overhead vector of the servers indexed by $\mathcal{S}$. We assume that $\bm{X}$ and $\bm{O}$ are independent. For any realization of $\bm{O}_{\mathcal{U}}=\bm{o}_{\mathcal{U}}$, $\bm{O}_{\mathcal{S}}$ is {independently} drawn according to the conditional distribution $p(\mathcal{A}|\bm{o}_{\mathcal{U}})= \nu(\bm{O}_{\mathcal{S}}\in \mathcal{A}|\bm{O}_{\mathcal{U}}=\bm{o}_{\mathcal{U}})$ associated with $\nu$.

\subsection{Scheduling Policies}
%In the distributed queue model, the scheduling policy determines both the task assignments of each dispatcher and determines task assgi and task replications  scheduler assigns tasks to servers over time.

%In conventional load balancing technique, the task dispatcher queries the queue lengths at multiple servers, and assign the task to the server with the shortest queue length.


%A scheduling policy, denoted by $\pi$, or scheduler assigns tasks to servers over time. In order to minimize service delay, the scheduler needs to carefully determine \emph{which task of which job to serve next, when to replicate a task, and replicate on which servers}.
A scheduling policy, denoted by $\pi$, determines the task assignments %and replication operations
 in the system.
We consider the class of \textbf{causal} policies, in which scheduling decisions are made based on the history and current state of the system; the realization of task service time is unknown until the task is completed (unless the service time is deterministic). 
In practice, service preemption is costly and may leads to complexity and reliability issues \cite{Sparrow:2013,Borg2015}. Motivated by this, we assume that \textbf{preemption is not allowed}. Hence, if a server starts to process a task, it must complete this task before switching to process another task. 
We use $\Pi$ to denote the set of causal and non-preemptive policies. Let us define several sub-classes of policies within $\Pi$:

A policy is said to be \textbf{non-anticipative}, if the scheduling decisions are made without using any information about the future job arrivals; and is said to be \textbf{anticipative}, if it has access to the parameters $(a_i,{k}_i,d_i)$ of future arriving jobs. For periodic and pre-planned services, future job arrivals can be predicted in advance. To cover these scenarios, we abuse the definition of causal policies a bit and include anticipative policies into the policy space $\Pi$. However, the policies that we propose in this paper are all {non-anticipative}. 

A policy is said to be \textbf{work-conserving}, if no server is idle when there are tasks waiting to be processed. 


 %For some tightly monitored systems with
%In distributed queueing systems, a load balancing policy is determined by its task assignment and replication operations. Hence, all non-preemptive feasible load balancing policies are contained in $\Pi$.


%A feasible policy can be preemptive or non-preemptive. In a \emph{preemptive} policy, a server can switch to another task at any time, and resume to process the previous task later. In a \emph{non-preemptive} policy, a server must complete (or cancel) the current task before switching to another task.
%In work-conserving policies, some of the servers can be idle if all tasks are being processed by the remaining servers.
%all the remaining tasks are being processed on some servers, the remaining servers can be idle. %We use $\Pi_{\text{non-prmp}}\subset\Pi$ to denote the set of work-conserving, non-preemptive, and feasible policies.
%Examples of static list policies include First-Come-First-Served (FCFS), Last-Come-First-Served (LCFS), and Head-of-the-line (HOL) priority policies \cite{Leonard_Kleinrock_book}. Let $PL$ denote a static priority list and $\Pi_{{PL}}\subset \Pi$ denote the set of static list policies for given priority list $PL$, but with different task replication operations.
%A policy is said to be a \textbf{priority} policy, if the jobs are ordered according to a priority list of all $n$ jobs. At any time, an idle server is assigned to process a task from the job with the highest priority among the jobs in the queue. The relative priority ordering of the jobs in the queue are determined based on their arrival time, due time, and current state, without requiring any information of the jobs that have departed or have not arrived to the system. %A priority policy is said to be \textbf{static (dynamic)} if the priority list remains constant (varies) during the evolution of the system. 
%Let $p_i\geq 0$ denote the priority of job $i$, and $PL=(p_1,\ldots,p_n)$ denote a priority list, where $p_i>p_j$ means that job $i$ has a higher priority then job $j$. Two examples of priority list $PL$ are $(n,n-1,\ldots,1)$ for First-Come-First-Served (FCFS) policies, and $(1,2,\ldots,n)$ for Last-Come-First-Served (LCFS) policies. Let $\Pi_{{PL}}\subset \Pi$ denote the set of {static priority policies} with a fixed priority list $PL$ and different task replication operations, and $\Pi_{\text{FCFS}}\subset \Pi$ denote the set of First-Come-First-Served (FCFS) policies with different task replication operations.

%Hence, any priority policy is online.

The goal of this paper is to design low-complexity non-anticipative scheduling policies that are near delay-optimal among all policies in $\Pi$, even compared to the anticipative policies with knowledge about future arriving jobs.

%All policies proposed in this paper are  policies within $\Pi$. We





%In practice, non-preemptive online policies are desirable, because preemption is costly %and may leads to complexity and reliability issues
%\cite{Sparrow:2013,Borg2015} and information about the future may not be available.
%%maguluri2012,

%\begin{definition}\textbf{Work Conservation:}
%In a \emph{work-conserving} policy, no server is idle when there exists at least one remaining task that is not under service.
%\end{definition}
%
%\begin{definition}\textbf{Static Priority Policy:} In a \emph{static priority} policy  the scheduler orders the jobs at time zero according to a priority list. This priority list includes jobs to arrive after time zero. This priority list does not change during the evolution of the system and the servers are assigned to tasks from the jobs with the highest priorities.
%\end{definition}
%
%
%Let $PL$ denote a priority list and $\Pi_{PL}\subseteq \Pi$ denote the set of static list policies with fixed priority list $PL$ and different task replication operations.

%there exist a class of policies

%




%Hence, a feasible policy can have access to parameters $(a_i,k_i)$ of future jobs.
%
%Our goal is to develop {online} scheduling policies and prove they are
%
%scheduling decisions are made based on history and current information of system evolutions, and the service time distributions of the servers. %In addition, the scheduling decisions of a casual policy is \emph{independent} of the random task service times.
%The service time of a task is unknown to the decision maker before task completion (unless the service time is deterministic). In a \emph{preemptive} policy, a server can switch to process another task at any time, and resume the previous chunk at a later time, continuing from the interrupted point.
%
%We focus on \emph{non-preemptive task service} which {preemption} of tasks from a lower priority job is not allowed when a high priority job arrives.

\subsection{Delay Metrics}\label{sec:metrics}
Each job $i$ has a \textbf{due time} $d_i\in[0,\infty)$, also called {due date}, which is the time that job $i$ is promised to be completed \cite{michael2012book}. %\cite{Wang:2011}.
Completion of a job after its due time is allowed, but then a penalty is incurred. Hence, the due time can be considered as a soft deadline. 

For each job $i$, $C_i$ is the job completion time, $D_i= C_i-a_i$ is the delay, $L_i = C_i-d_i$ is the {lateness} after the due time $d_i$, and $T_i = \max[C_i-d_i,0]$ is the  {tardiness} (or positive lateness). %Hence, $V_i-a_i$ is the longest waiting time among all tasks of job $i$.
%Because preemption is not allowed, the time difference $C_i-V_i$ is small.
% upper bounds of $C_i-V_i$ will be studied in Section \ref{sec_average_delay}.
%all tasks of job $i$ have already started their service on some servers. %Hence, %A superscript $\pi$ denotes the quantities in policy $\pi$
Define the vectors $\bm{a} =(a_1,\ldots,a_n)$,
$\bm{d} =(d_1,\ldots,d_n)$, $\bm{C}=(C_1,$ $\ldots,C_n)$, $\bm{D}=(D_1,\ldots, D_n)$,  $\bm{L}=(L_1,\ldots,$ $ L_n)$, and $\bm{C}_{\uparrow}\! =\! (C_{(1)},\ldots,C_{(n)})$. %In addition, let $\bm{C}_{\uparrow} = (C_{(1)},\ldots,$ $C_{(n)})$ denote the increasing completion sequence of the jobs.
%These quantities obtained policy $\pi$ are denoted as, e.g., ${C}_i(\pi)$ and $V_i(\pi)$.
%In particular, let $\bm{d}_{\uparrow} =(d_{(1)},\ldots,d_{(n)})$, and  $\bm{C}_{\uparrow}\! =\! (C_{(1)},\ldots,C_{(n)})$.
Let $\bm{c}=(c_1,$ $\ldots,c_n)$ and $\bm{c}_{\uparrow}\! =\! (c_{(1)},\ldots,c_{(n)})$, respectively, denote the realizations of $\bm{C}$ and $\bm{C}_{\uparrow}$. All these quantities are functions of the  scheduling policy $\pi$.


%Let $k_{\text{sum}}=\sum_{i=1}^nk_i$ denote the total number of tasks, $\bm{t}(\pi)=(t_{1}(\pi),\ldots, t_{k_{\text{sum}}}(\pi))$ denote the realizations of task completion times on a sample path of policy $\pi$. The components of $\bm{t}(\pi)$ are arranged in the increasing order such that $\bm{t} (\pi)=\bm{t}_{\uparrow}(\pi)$.

%It is easy to show that $C_i(\pi)-V_i(\pi)$ is upper bounded by the maximum service time of the $m$ servers. Using stochastic ordering, this can be expressed as
%\begin{align}\label{eq_difference}
%[C_i(\pi)-V_i(\pi)|\pi,\mathcal{I}] \leq_{\text{st}} \max_{l=1,\ldots,m}X_l,
%\end{align}
%where the RHS is independent of $i$, $\pi$, and $\mathcal{I}$.
%%Tighter upper bounds of $C_i(\pi)-V_i(\pi)$ will be studied later.
%In the sequel, we will omit mentioning the condition of given policy $\pi$ to emphasize on the dependences that we wish to focus on.
%

Several important delay metrics are introduced in the following: For any policy $\pi$, the \textbf{average delay} ${D}_{\text{avg}}: \mathbb{R}^n\rightarrow \mathbb{R}$ is defined by\footnote{If $n\rightarrow\infty$, then a $\limsup$ operator is enforced on the RHS of \eqref{eq_2}, and the $\max$ operator in \eqref{eq_1} and \eqref{eq_11} is replaced by $\sup$.
%, \eqref{eq_10}, \eqref{eq_12}, \eqref{eq_1111}, and \eqref{eq_1112}.
}
\begin{align}
{D}_{\text{avg}}(\bm{C}(\pi))=\frac{1}{n}\sum_{i=1}^{n}\left[C_i(\pi)-a_i\right]. \label{eq_2}
\end{align}
%In addition, the \textbf{mean square of tardiness} ${T}_{\text{ms}}: \mathbb{R}^n\rightarrow \mathbb{R}$ is given by
%\begin{align}
%T_{\text{ms}}(\bm{C}(\pi)) \!= \frac{1}{n}\sum_{i=1}^{n} \max[L_i(\pi),0]^2=\frac{1}{n}\sum_{i=1}^{n} \max\left[C_i(\pi)-d_i,0\right]^2.\label{eq_10}
%\end{align}
%If $d_i=a_i$, $T_{\text{ms}}$ reduces to the \textbf{mean square of delay}  ${D}_{\text{ms}}: \mathbb{R}^n\rightarrow \mathbb{R}$, i.e.,
%\begin{align}
%D_{\text{ms}}(\bm{C}(\pi)) \!= \frac{1}{n}\sum_{i=1}^{n} D_i^2(\pi)=\frac{1}{n}\sum_{i=1}^{n} \left[C_i(\pi)-a_i\right]^2.\label{eq_12}
%\end{align}
%Note that $C_i(\pi)\geq a_i$ for all $i$ and $\pi$. 
%Note that ${D}_{\text{ms}}(\bm{C}(\pi))$ is different from ${D}_{\text{avg}}(\bm{C}(\pi))^2$.
%In many systems, fairness is an important aspect of the quality-of-service. We define two delay metrics related to   \emph{min-max fairness}. In particular, 
The \textbf{maximum lateness}  ${L}_{\max}: \mathbb{R}^n\rightarrow \mathbb{R}$ is defined by
\begin{align}
L_{\max}(\bm{C}(\pi)) \!= \!\max_{i=1,2,\ldots,n} L_i(\pi)=\max_{i=1,2,\ldots,n} \left[C_i(\pi)-d_i\right],\label{eq_1}
\end{align}
if $d_i=a_i$, $L_{\max}$ reduces to the \textbf{maximum delay}  ${D}_{\max}: \mathbb{R}^n\rightarrow \mathbb{R}$, i.e.,
\begin{align}
D_{\max}(\bm{C}(\pi))\!=\! \max_{i=1,2,\ldots,n} D_i(\pi)= \max_{i=1,2,\ldots,n} \left[C_i(\pi)-a_i\right].\!\!\label{eq_11}
\end{align}
The \textbf{$p$-norm of delay} ${D}_{p}: \mathbb{R}^n\rightarrow \mathbb{R}$  is defined by
\begin{align}
D_p(\bm{C}(\pi)) = || \bm{D}(\pi) ||_p = \left[\sum_{i=1}^n D_i(\pi)^p\right]^{1/p},~ ~p\geq 1.
\end{align}
%In addition, two delay metrics related to \emph{proportional fairness} \cite{Kushner2004} are defined by
%\begin{align}\label{eq_1111}
%&T_{\text{PF}}(\bm{C}(\pi)) \!= \! -\frac{1}{n}\sum_{i=1}^n \log (\max[L_i(\pi),0]+\epsilon)=-\frac{1}{n}\sum_{i=1}^n \log(\max[C_i(\pi)-d_i,0]+\epsilon),\\
%&D_{\text{PF}}(\bm{C}(\pi)) \!= \! - \frac{1}{n}\sum_{i=1}^n \log (D_i(\pi)+\epsilon)=-\frac{1}{n}\sum_{i=1}^n \log(C_i(\pi)-a_i+\epsilon),\label{eq_1112}
%\end{align}
%where $\epsilon$ is a positive number, which can be as small as we wish. 


%if $d_i=a_i$, $L_{\max}$ reduces to the \textbf{maximum delay}  ${D}_{\max}: \mathbb{R}^n\rightarrow \mathbb{R}$, i.e.,
%\begin{align}
%D_{\max}(\bm{C}(\pi))\!=\! \max_{i=1,2,\ldots,n} D_i(\pi)= \max_{i=1,2,\ldots,n} \left[C_i(\pi)-a_i\right].\!\!\label{eq_11}
%\end{align}
%In some studies, people are interested in the second moment delay performance. 




In general, a \textbf{delay metric} can be expressed as a function $f(\bm{C}(\pi))$ of the job completion time vector $\bm{C}(\pi)$, where $f: \mathbb{R}^n\rightarrow \mathbb{R}$ is increasing. In this paper, we consider three classes of delay metric functions:
\begin{align}
%\mathcal{D} &= \{f : f \text{ is increasing}\},\nonumber\\
\mathcal{D}_{\text{sym}} &= \{f : f \text{ is symmetric and increasing}\},\nonumber\\
\mathcal{D}_{\text{Sch-1}} &= \{f:  f (\bm{x}+\bm{d}) \text{ is Schur convex and increasing in $\bm{x}$}\},\nonumber\\
\mathcal{D}_{\text{Sch-2}} &= \{f:  f (\bm{x}+\bm{a}) \text{ is Schur convex and increasing in $\bm{x}$}\}.\nonumber\end{align}
Consider two alternative expressions of the delay metric function $f$:
\begin{align}
&f_1(\bm{L}(\pi))=f(\bm{L}(\pi)+\bm{d})=f(\bm{C}(\pi)),\label{eq_expression_1}\\
&f_2(\bm{D}(\pi))=f(\bm{D}(\pi)+\bm{a})=f(\bm{C}(\pi)).\label{eq_expression_2}\end{align}
%as two alternative expressions of the delay metric function $f$. 
Then, $f_1(\bm{L}(\pi))$ is Schur convex in the lateness vector $\bm{L}(\pi)$ for each $f\in \mathcal{D}_{\text{Sch-1}}$, and $f_2(\bm{D}(\pi))$ is Schur convex in the delay vector $\bm{D}(\pi)$ for each $f\in \mathcal{D}_{\text{Sch-2}}$. Furthermore, every convex and symmetric function is Schur convex. Using these properties, it is easy to show that
\begin{align}
&{D}_{\text{avg}}\in\mathcal{D}_{\text{sym}}\cap \mathcal{D}_{\text{Sch-1}} \cap \mathcal{D}_{\text{Sch-2}},\nonumber \\
%&T_{\text{ms}}\in\mathcal{D}_{\text{Sch-1}}, ~D_{\text{ms}}\in\mathcal{D}_{\text{Sch-2}},\nonumber\\
&L_{\max}\in\mathcal{D}_{\text{Sch-1}}, D_{\max}\in\mathcal{D}_{\text{Sch-2}}, D_p \in \mathcal{D}_{\text{Sch-2}}.\nonumber
%&T_{\text{PF}}\in\mathcal{D}_{\text{Sch-1}}, ~D_{\text{PF}}\in\mathcal{D}_{\text{Sch-2}}.\nonumber
\end{align}


%For all $f\in\mathcal{D}_{\text{Sch}}$, $f(\bm{C})=f(\bm{L}+\bm{d})$ is Schur convex and increasing in $\bm{L}$.
%, and $D_{\max}\in\mathcal{D}_{\text{Sch-2}}$.



%Any \emph{delay metric} can be expressed as $f (\bm{C})$ with function $f: \mathbb{R}^n\rightarrow \mathbb{R}$.
%For any function $f: \mathbb{R}^n\rightarrow \mathbb{R}$, $f (\bm{C})$ is said to be a \emph{delay metric}. %In this paper, we will study three classes of delay metrics where the function $f$ is increasing, increasing and symmetric, increasing and Schur convex, respectively.
%\begin{definition}
%A function $D$ is said to be a \emph{delay metric} if
%\begin{align}
%D_{\pi} = f (C_{1,\pi},C_{2,\pi},\ldots,C_{N,\pi}),\label{eq_metric}
%\end{align}
%where $f$ is a non-decreasing function.
%\end{definition}


\subsection{Near Delay Optimality}\label{sec_optimality}

Define $\mathcal{I}=\{n,(a_i,{k}_i,d_i)_{i=1}^n\}$ as the parameters of the jobs, which include the number, batch sizes, arrival times, and due times of the jobs.
The job parameters $\mathcal{I}$ and random task service times are determined by two external processes, which are \emph{mutually independent} and do not change according to the scheduling policy. % adopted in the system.
For delay metric function $f$ and policy space $\Pi$, a policy $P\in \Pi$ is said to be \textbf{delay-optimal in stochastic ordering}, if for all $\pi\in \Pi$ and $\mathcal{I}$% and $\bm{\Theta}$
\begin{align}\label{eq_optimal}
[f (\bm{C}(P))|P,\mathcal{I}]\leq_{\text{st}} [f (\bm{C}(\pi))|\pi,\mathcal{I}].%\nonumber
\end{align}
%an equivalent definition of delay-optimal in distribution is: %\eqref{eq_optimal} is equivalent with that
%In particular, policy $P\in \Pi$ is {delay-optimal in distribution} if, and only if,
or equivalently, if for all $\mathcal{I}$
\begin{align}\label{eq_optimal1}
\mathbb{E}[\phi \circ f (\bm{C}(P))|P,\mathcal{I}]=\min_{\pi\in\Pi}\mathbb{E}[\phi \circ f (\bm{C}(\pi))|\pi,\mathcal{I}]%\nonumber
\end{align}
holds for all increasing function $\phi: \mathbb{R}\rightarrow \mathbb{R}$ for which the conditional expectations in \eqref{eq_optimal1} exist.
%We will seek for non-preemptive {online} policies $P$ and $Q$ which satisfy
%\begin{align}\label{delay optimal1}
%&\mathbb{E}[{D}_{\text{avg},P}|\mathcal{I}] = \min_{\pi\in\Pi} \mathbb{E}[{D}_{\text{avg}}(\pi)|\mathcal{I}],~\forall~\mathcal{I},\\
%&\mathbb{E}[L_{\max,Q}|\mathcal{I}] = \min_{\pi\in\Pi} \mathbb{E}[L_{\max}(\pi)|\mathcal{I}],~\forall~\mathcal{I},\label{delay optimal2}
%\end{align}
The equivalence between \eqref{eq_optimal} and \eqref{eq_optimal1} follows from \eqref{eq_order_property}. 
For notational simplicity, we will omit the mention of the condition that policy $\pi$ or policy $P$ is adopted in the system in the rest of the paper. Note that this definition of delay optimality is quite strong because the optimal policy $P$ needs to satisfy \eqref{eq_optimal} and \eqref{eq_optimal1} for \emph{arbitrarily given} job parameters  $\mathcal{I}$.

%Note that because the job parameters 
%the conditional expectations in \eqref{eq_optimal1} are taken with respect to the random task service times for given scheduling policy and job parameters $\mathcal{I}$, and .
%Therefore, \emph{if policy $P\in \Pi$ is {delay-optimal in distribution}, then for all number, sizes, arrival times, and due times of the jobs denoted by $\mathcal{I}$ and all increasing function $\phi$, policy $P$ minimizes $\mathbb{E}[\phi \circ f  (\bm{C}(\pi))| \mathcal{I}]$ among all policies $\pi\in\Pi$.} 


%Note that policies $P$ and $Q$ are online and hence require no information about future jobs. However, they are no worse than the policies having access to $(a_i,{k}_i)$ of future jobs.
%{\blue Examples of the delay metric function $f$ include the average delay $D_{\text{avg}}$, the maximum lateness $L_{\max}$, and the maximum delay $D_{\max}$ defined in \eqref{eq_2}-\eqref{eq_11}. Examples of the increasing function $\phi$ include:
%\begin{itemize}
%\itemsep0em
%\item[1.] Linear function $\phi_1(x)=x$. Hence, the expected average delay can be expressed as $\mathbb{E}[D_{\text{avg}} (\bm{C}(\pi))|\mathcal{I}]=\mathbb{E}[\phi_1 \circ D_{\text{avg}} (\bm{C}(\pi))|\mathcal{I}]$.
%
%\item[2.] Indicator function $\phi_d(x)$, which equals to 1 if $x>d$ and equals to 0 if $x\leq d$. Hence, the delay tail probability can be expressed as $\Pr[D_{\max} (\bm{C}(\pi)) > d|\mathcal{I}] = \mathbb{E}[ \phi_d  \circ f (\bm{C}(\pi))  |\mathcal{I}]$.
%\end{itemize}}

In multi-class multi-server queueing systems, delay optimality is extremely difficult to achieve,
%. It may happen that no policy is delay-optimal,
even with respect to some definitions of delay optimality that are weaker than \eqref{eq_optimal}. 
In deterministic scheduling problems, it was shown that minimizing the average delay in multi-server queueing systems is $NP$-hard %and has no constant competitive ratio if the number of servers $m\geq 2$ 
\cite{Leonardi:1997}. Similarly, delay-optimal stochastic scheduling in multi-server queueing systems with multiple job classes is deemed to be notoriously difficult \cite{Weiss:1992,Weiss:1995,Dacre1999}.
%Therefore, delay optimality is inherently difficult to achieve in queueing systems with parallel servers. 
This motivated us to study whether there exist policies that can come close to delay optimality. We will show that this is possible in the following sense:

\ifreport
\begin{figure}
\centering
\includegraphics[width=0.55\textwidth]{Figures/definitionofUi2} \caption{An illustration of $V_i$ and $C_i$. There are 2 servers, and job $i$ has 3 tasks denoted by $(i,1)$, $(i,2)$, $(i,3)$. Tasks $(i,1)$ and $(i,3)$ are assigned to Server 1, and Task $(i,2)$ is assigned to Server 2. By time $V_i$, all tasks of job $i$ have started service. By time $C_i$, all tasks of job $i$ have completed service. Therefore, $V_i\leq C_i$.}
% and their different $C_i-V_i$ is small.}
\label{V_i}
\end{figure}
\else
\begin{figure}
\centering
\includegraphics[width=0.35\textwidth]{Figures/ordering_1} \caption{An illustration of $V_i$ and $C_i$. There are 2 servers, and job $i$ has 3 tasks denoted by $(i,1)$, $(i,2)$, $(i,3)$. Task $(i,1)$ is replicated on both servers, tasks $(i,2)$ and $(i,3)$ are assigned to the two servers separately. By time $V_i$, all tasks of job $i$ have entered the servers. By time $C_i$, all tasks of job $i$ have completed service. Therefore, $V_i\leq C_i$.}
\label{V_i}
\end{figure}
\fi


{Define $V_i$ as the earliest time that all tasks of job $i$ have entered the servers. In other words, all tasks of job $i$ are either completed or under service   at time $V_i$. One illustration of $V_i$ is provided in Fig. \ref{V_i}, from which it is easy to see 
\begin{align}\label{eq_V_i_small}
V_i\leq C_i.
\end{align}
Denote $\bm{V}=(V_1,\ldots, V_n)$, $\bm{V}_{\uparrow} \!=\! (V_{(1)},\ldots,V_{(n)})$. Let $\bm{v}=(v_1,\ldots, v_n)$ and $\bm{v}_{\uparrow} \!=\! (v_{(1)},\ldots,v_{(n)})$ be the realization of $\bm{V}$ and $\bm{V}_{\uparrow}$, respectively. All these quantities are functions of the  scheduling policy $\pi$.
A policy $P\in \Pi$ is said to be \textbf{near delay-optimal in stochastic ordering}, if for all $\pi\in \Pi$ and $\mathcal{I}$% and $\bm{\Theta}$
\begin{align}\label{eq_nearoptimal}
[f (\bm{V}(P))|\mathcal{I}]\leq_{\text{st}} [f (\bm{C}(\pi))|\mathcal{I}],%\nonumber
\end{align}
%or equivalently, for all increasing $\phi: \mathbb{R}\rightarrow \mathbb{R}$ and $\mathcal{I}$
%\begin{align}%\label{eq_optimal1}
%\mathbb{E}[\phi \circ f (\bm{V}(P))|\mathcal{I}]= \min_{\pi\in\Theta}\mathbb{E}[\phi \circ f (\bm{C}(\pi))|\mathcal{I}].\nonumber
%\end{align}
%which is similar with \eqref{eq_optimal}, except that $\bm{C}(P)$  on the LHS  is replaced by $\bm{V}(P)$.
%The difference $\bm{C}(P)-\bm{V}(P)$ is characterized by \eqref{eq_difference}. %Tighter bounds will be provided later.
%According to \eqref{eq_order_property}, policy $P\in \Pi$ is {near delay-optimal in distribution} if, and only
or equivalently, if for all $\mathcal{I}$
\begin{align}\label{eq_nearoptimal1}
\mathbb{E}[\phi \!\circ\! f (\bm{V}(P))|\mathcal{I}] \!\leq\! \min_{\pi\in\Pi}\mathbb{E}[\phi \!\circ\! f (\bm{C}(\pi))|\mathcal{I}] \!\leq\!\mathbb{E}[\phi \!\circ\! f (\bm{C}(P))|\mathcal{I}]
\end{align}
holds for all increasing function $\phi$ for which the conditional expectations in \eqref{eq_nearoptimal1} exist. There exist many ways to approximate \eqref{eq_optimal} and \eqref{eq_optimal1}, and obtain various forms of near delay optimality.
We find that the form in \eqref{eq_nearoptimal} and \eqref{eq_nearoptimal1} is convenient, because it is analytically 
provable and leads to tight sub-optimal delay gap, as we will see in the subsequent sections.
 
% the remaining processing time of a job, it is not easy to find an approximation that leads to a provable and tight sub-optimal delay gap.


% There are many possible expressions of near delay optimality. We choose this form of definition because it is 
% it is not easy to find an approximation that leads to a provable and tight sub-optimal delay gap

 
%Hence, $\mathbb{E}[\phi \circ f (\bm{V}(P))|\mathcal{I}]$ and $\mathbb{E}[\phi \circ f (\bm{C}(P))|\mathcal{I}]$, respectively, are lower and upper bounds of the optimum expected delay $\min_{\pi\in\Pi}\mathbb{E}[\phi \circ f (\bm{C}(\pi))|\mathcal{I}]$. 
%The tightness of these bounds will be characterized in Section \ref{sec_analysis} for some important delay metrics. 



%Some examples of \eqref{eq_optimal1} are provided as follows:
%\begin{itemize}
%\itemsep0em
%\item[1.] If $f(\cdot)=D_{\text{avg}}(\cdot)$ and $\phi(x)=x$, then \eqref{eq_optimal1} implies
%%\begin{align}
%%\mathbb{E}[D_{\text{avg}} (\bm{C}(P))|\mathcal{I}]= \min_{\pi\in\Pi}\mathbb{E}[D_{\text{avg}} (\bm{C}(\pi))|\mathcal{I}],\nonumber
%%\end{align}
%\begin{align}
%\mathbb{E}\bigg[\frac{1}{n}\sum_{i=1}^{n}\left[C_i(P)-a_i\right]\bigg|\mathcal{I}\bigg]= \min_{\pi\in\Pi}\mathbb{E}\bigg[\frac{1}{n}\sum_{i=1}^{n}\left[C_i(\pi)-a_i\right]\bigg|\mathcal{I}\bigg],\nonumber
%\end{align}
%that is, policy $P$ minimizes the mean average delay.
%
%\item[2.] If $f(\cdot)=D_{\text{ms}}(\cdot)$ and $\phi(x)=x$, then \eqref{eq_optimal1} implies
%%\begin{align}
%%\mathbb{E}[D_{\text{ms}} (\bm{C}(P))|\mathcal{I}]= \min_{\pi\in\Pi}\mathbb{E}[D_{\text{ms}} (\bm{C}(\pi))|\mathcal{I}],\nonumber
%%\end{align}
%\begin{align}
%\mathbb{E}\bigg[\frac{1}{n}\sum_{i=1}^{n} \left[C_i(P)-a_i\right]^2\bigg|\mathcal{I}\bigg]= \min_{\pi\in\Pi}\mathbb{E}\bigg[\frac{1}{n}\sum_{i=1}^{n} \left[C_i(\pi)-a_i\right]^2\bigg|\mathcal{I}\bigg],\nonumber
%\end{align}
%that is, policy $P$ minimizes the second moment of delay.
%
%\item[3.] If $f(\cdot) = L_{\max}(\cdot)$ and $\phi$ is an indicator function of the interval $[t,\infty)$, such that  $\phi(x)=1$ if $x>t$ and $\phi(x)=0$ if $x\leq t$. Then, \eqref{eq_optimal1} implies
%%\begin{align}
%%\Pr[D_{{\max}} (\bm{C}(P))>d|\mathcal{I}]= \min_{\pi\in\Pi}\Pr[D_{\max} (\bm{C}(\pi))>d |\mathcal{I}],\nonumber
%%\end{align}
%\begin{align}
%\Pr\Big[\max_{i=1,2,\ldots,n} [C_i(P)-d_i]>t\Big|\mathcal{I}\Big]= \min_{\pi\in\Pi}\Pr\Big[\max_{i=1,2,\ldots,n} [C_i(\pi)-d_i]>t \Big|\mathcal{I}\Big],\nonumber
%\end{align}
%that is, policy $P$ minimizes the complementary CDF of the maximum lateness.
%\end{itemize}


% through theoretical analysis and numerical results.
% results are provided in Section \ref{sec_numerical} to illustrate t.

%The numerical results show that these lower and upper bounds are tight when the system load is high. When the system load is low, the lower bound $\mathbb{E}[\phi \circ f (\bm{C}(P))|\mathcal{I}]$ is still tight. In this sense, policy $P$ is near delay-optimal.

%Numerical results are provided in in Section \ref{sec_numerical} to illustrated the tightness of these bounds.
% will be studied in Section \ref{sec_numerical}.
%Our numerical results suggest that
%These lower and upper bounds are tight when the system load is high. When the system load is low, the upper bound $\mathbb{E}[\phi \circ f (\bm{C}(P))|\mathcal{I}]$ is still tight. In this sense, policy $P$ is near delay-optimal.


%the lower bound $\mathbb{E}[\phi \circ f (\bm{V}(P))|\mathcal{I}]$ is not tight, but




%The tightness of these bounds will be studied in Section \ref{sec_}

%Therefore, \emph{if policy $P\in \Pi$ is {near delay-optimal in distribution}, then for all number, sizes, arrival times, and due times of the jobs denoted by $\mathcal{I}$ and all increasing functions $\phi$, policy $P$ is near-optimal in minimizing $\mathbb{E}[\phi \circ f  (\bm{C}(\pi))|\mathcal{I}]$ among all policies $\pi\in\Pi$.}

%Our research suggest that these lower and upper bounds are tight when the system load is high. When the system load is low, the lower bound $\mathbb{E}[\phi \circ f (\bm{V}(P))|\mathcal{I}]$ is not tight, but the upper bound $\mathbb{E}[\phi \circ f (\bm{C}(P))|\mathcal{I}]$ is still tight. In this sense, policy $P$ is near delay-optimal. Tighter lower bounds of the optimum delay $\min_{\pi\in\Pi}\mathbb{E}[\phi \circ f (\bm{C}(\pi))|\mathcal{I}]$ will be studied in our future work.

% the upper bound $\mathbb{E}[\phi \circ f (\bm{C}(P))|\mathcal{I}]$ is tight for both high and low system load, and hence



%   lower bound may not be sufficiently tight, and one can use
%\begin{align}
%C_i(\pi) \geq_{\text{st}} a_i + \min_{l=1,\ldots,m} X_m,~\forall~\pi\in\Pi,i=1,\ldots,n\nonumber
%\end{align}
%to improve the lower bound.
%Therefore, \emph{if policy $P\in \Pi$ is {near delay-optimal in distribution}, then for all number, sizes, arrival times, and due times of the jobs denoted by $\mathcal{I}$ and all increasing functions $\phi$, policy $P$ is near-optimal in minimizing $\mathbb{E}[\phi \circ f  (\bm{C}(\pi))|\mathcal{I}]$ among all policies $\pi\in\Pi$.


%\footnote{We remark that it is possible to obtained tighter lower and upper bounds. For example, tighter  lower bounds are obtained in Corollaries \ref{coro3} and \ref{coro4} where delay optimality holds.}



%holds for  for which the conditional expectations exist.


%According to \eqref{eq_difference}, $[{C}_i(P)-{U}_i(P)|\mathcal{I}]$ is uniformly upper bounded for all $i$ and $\mathcal{I}$ in the stochastic ordering. We will use properties like this to characterize delay sub-optimality gap.

%\begin{definition}\textbf{Near Delay Optimality:}
%Consider the delay metric $D$ defined in \eqref{eq_metric} and policy space $\Theta$, a policy $P\in \Theta$ is said to be \emph{near delay-optimal in distribution}, if there exist non-negative $f_1,\ldots, G_N$ and $G$ such that for all $\pi\in \Theta$ and $\mathcal{I}$
%\begin{align}\label{eq_nearoptimal}
%&[D_P|\mathcal{I}]\leq_{\text{st}} [f (C_{1,\pi}+f_1,\ldots,C_{N,\pi}+G_N)|\mathcal{I}],\\
%&G_i\leq_{\text{st}} G,~i=1,\ldots,n,
%\end{align}
%where $G$ is independent of $\pi$ and $\mathcal{I}$.
%%That is, \emph{compared to any policy $\pi\in\Pi$, the job complete time contributed to the delay metric $D$ is increased in policy $P$ by no more than a time duration with the distribution of $G$.}
%% Hence, for all non-decreasing function $\phi$ and all $\mathcal{I}$
%%\begin{align}
%%\mathbb{E}[\phi(D(P))|\mathcal{I}]\leq_{\text{st}} \mathbb{E}[\phi (f (C_{1,\pi}+f_1,\ldots,C_{N,\pi}+G_N))|\mathcal{I}].
%%\end{align}
%%, and $\bm{\Theta}$.
%%We are particularly interested in the case that %$f_1,\ldots, G_N$ are uniformly small in distribution such that
%\end{definition}

%It is worth noting that if
%\begin{align}
%&~~~~[(C_{1,P}+f_1,\ldots,C_{N,P}+G_N)|\mathcal{I}]\nonumber\\
%&\leq_{\text{st}}  [(C_{1,\pi}+f_1,\ldots,C_{N,\pi}+G_N)|\mathcal{I}],~\forall~\pi\in \Theta,\mathcal{I},
%\end{align}
%then \eqref{eq_nearoptimal} holds for all non-decreasing $f$; but the reverse is not true.

% in the sense of
%\begin{align}\label{delay nearoptimal1}
%&\mathbb{E}[{D}_{\text{avg},P}|\mathcal{I}] \leq \min_{\pi\in\Pi} \mathbb{E}[{D}_{\text{avg}}(\pi)|\mathcal{I}] + g,~\forall~\mathcal{I},\\
%&\mathbb{E}[L_{\max,Q}|\mathcal{I}] \leq \min_{\pi\in\Pi} \mathbb{E}[L_{\max}(\pi)|\mathcal{I}] +h,~\forall~\mathcal{I},\label{delay nearoptimal2}
%\end{align}
%where $g$ and $h$ are constants and independent of $n$. The formulations \eqref{delay nearoptimal1} and \eqref{delay nearoptimal2} apply to more system settings than \eqref{delay optimal1} and \eqref{delay optimal2}. However, great efforts are needed to show that the sub-optimality gaps are small and independent of $n$.



==> v3/numerical.tex <==
% !TEX root = ./replication.tex

\section{Numerical Results}\label{sec_numerical}
In this section, we present some numerical results to illustrate the delay
performance of different scheduling policies and validate our
theoretical results.
\subsection{Centralized Queueing Systems}
Consider a centralized queueing system consisting of 3 servers with heterogeneous service time distributions, 
%50\% jobs are of the size $k_i=1$ and the other 50\% jobs are of the size $k_i = 10$. 
The inter-arrival time of the jobs $T_i=a_{i+1}-a_i$ is exponentially distributed for even $i$; and is zero for odd $i$. 
\ifreport
\begin{figure}
\centering \includegraphics[width=0.6\textwidth]{Figures/figure1_shifted_exp} \caption{Expected average delay $\mathbb{E}[D_{\text{avg}} (\bm{C}(\pi))|\mathcal{I}]$ versus traffic intensity $\rho$ in a centralized queueing system with heterogeneous NBU service time distributions.}
\label{fig1} \vspace{-0.cm}
\end{figure}
\else
\begin{figure}
\centering \includegraphics[width=0.4\textwidth]{Figures/figure1_shifted_exp} \caption{Expected average delay $\mathbb{E}[D_{\text{avg}} (\bm{C}(\pi))|\mathcal{I}]$ versus traffic intensity $\rho$ in a centralized queueing system with heterogeneous NBU service time distributions.}
\label{fig1} \vspace{-0.cm}
\end{figure}
\fi
\subsubsection{Average Delay}
Figure \ref{fig1} plots the expected average delay $\mathbb{E}[D_{\text{avg}} (\bm{C}(\pi))|\mathcal{I}]$ versus traffic intensity $\rho$ in a centralized queueing system with heterogeneous NWU service time distributions. The number of incoming jobs is $n=3000$, the job size $k_i$ is chosen to be either $1$ or $10$ with equal probability.
The task service time $X_l$ follows a shifted exponential distribution:
\begin{align}
\Pr[X_l>x] = \left\{\begin{array}{l l}1,&\text{if}~x<\frac{1}{3\mu_l};\\
\exp[-\frac{3\mu_l}{2}(x-\frac{1}{3\mu_l})],&\text{if}~x\geq \frac{1}{3\mu_l},
\end{array}\right.
\end{align}
and the service rate of the 3 servers are $\mu_1=1.4$, $\mu_2=1$, and $\mu_3=0.6$, respectively. 
%Hence, the total task service rate is $\mu_1+\mu_2+\mu_3=3$, and 
The traffic intensity can be computed as $\rho = 
2\mathbb{E}[T_2] \frac{1+10}{2} (\mu_1+\mu_2+\mu_3) =33 \mathbb{E}[T_2]$. The cancellation overhead $O_l$ of server $l$ is exponentially distributed with rate $3\mu_l/2$. %The numerical results are averaged over 100 random samples for the downloading times of data chunks.
The ``Low bound'' curve is generated by using $\mathbb{E}[D_{\text{avg}}(\bm{V}(\text{FUT-NR}))|\mathcal{I}]$ which, according to Theorem \ref{thm1}, is a lower bound of the optimum expected average delay.
We can observe from Fig. \ref{fig1} that the policies FCFS-NR, FUT-NR, and FUT-NIR are throughput-optimal, while the policies FCFS-R and  FUT-R have a smaller throughput region.  The average delays of policies FUT-NR and FUT-NIR are quite close to the lower bound, while the other policies are far from the lower bound.
%Hence, when the queue length is large, no task should be replicated for NBU service time distributions. In addition, the job with the fewest unassigned tasks should be executed first to reduce the average delay.


  %These results are in accordance with Theorem \ref{thm1}.

\ifreport
\begin{figure}
\centering \includegraphics[width=0.6\textwidth]{Figures/figure2_Pareto} \caption{Expected average delay $\mathbb{E}[D_{\text{avg}} (\bm{C}(\pi))|\mathcal{I}]$ versus traffic intensity $\rho$ in a centralized queueing system with heterogeneous NWU service time distributions.}
\label{fig2} \vspace{-0.cm}
\end{figure}
\else
\begin{figure}
\centering \includegraphics[width=0.4\textwidth]{Figures/figure2_Pareto} \caption{Expected average delay $\mathbb{E}[D_{\text{avg}} (\bm{C}(\pi))|\mathcal{I}]$ versus traffic intensity $\rho$ in a centralized queueing system with heterogeneous NWU service time distributions.}
\label{fig2} \vspace{-0.cm}
\end{figure}
\fi


Figure \ref{fig2} illustrates the expected average delay $\mathbb{E}[D_{\text{avg}} (\bm{C}(\pi))|\mathcal{I}]$ versus traffic intensity $\rho$ in a centralized queueing system with heterogeneous NWU service time distributions. The number of incoming jobs is $n=3000$, the job sizes are $k_i=10$ for all $i$. The task service time $X_l$ follows a Pareto type II (Lomax) distribution \cite{ParetoDis}:
\begin{align}
\Pr[X_l>x] = \left[1+\frac{x}{\sigma}\right]^{-\alpha_l},
\end{align}
where $\sigma = 14/3$, $\alpha_1 = 7$, $\alpha_2 = 5$, and $\alpha_3 = 3$. The cancellation overhead $O_l$ is zero for all servers. According to the property of Pareto type II (Lomax) distribution \cite{ParetoDis}, the maximum task service rate is $1/\mathbb{E}[\min_{l=1,2,3}X_l] = (\alpha_1+\alpha_2+\alpha_3-1)/\sigma=3$, which is achieved when each task is replicated on all 3 servers. Hence, the traffic intensity can be computed as $\rho = 2\mathbb{E}[T_2] \times\frac{1+10}{2}\frac{1}{\mathbb{E}[\min_{l=1,2,3}X_l]} =33 \mathbb{E}[T_2]$. Because all jobs are of the same size, the FUT discipline is identical with the FCFS discipline. %i FCFS-R (policy FCFS-NR, or policy FCFS-NIR)
We can observe that policy FUT-R, which is identical with policy FCFS-R, is throughput-optimal, while  policy FUT-NR and policy FUT-NIR have a smaller throughput region. 
In addition, policy FUT-R achieves better delay performance than the other policies, which is in accordance with Theorem \ref{thm2}. 

%According to Theorem \ref{thm2}, policy FUT-R achieves the optimum delay performance. 

\begin{figure}
\centering \includegraphics[width=0.6\textwidth]{Figures/figure2_exp} \caption{Expected average delay $\mathbb{E}[D_{\text{avg}} (\bm{C}(\pi))|\mathcal{I}]$ versus traffic intensity $\rho$ in a centralized queueing system with heterogeneous exponential service time distributions.}
\label{fig2_exp} \vspace{-0.cm}
\end{figure}

Figure \ref{fig2_exp} depicts the expected average delay $\mathbb{E}[D_{\text{avg}} (\bm{C}(\pi))|\mathcal{I}]$ versus traffic intensity $\rho$ in a centralized queueing system with heterogeneous exponential service time distributions. The number of incoming jobs is $n=3000$, the job size $k_i$ is chosen to be either $1$ or $10$ with equal probability. The service rate of the 3 servers are $\mu_1=1.4$, $\mu_2=1$, and $\mu_3=0.6$, respectively. The cancellation overhead $O_l$ is zero for all servers. The maximum task service rate is $1/\mathbb{E}[\min_{l=1,2,3}X_l] = \mu_1+\mu_2+\mu_3=3$. Hence, the traffic intensity can be computed as $\rho = 2\mathbb{E}[T_2] \times\frac{1+10}{2}\frac{1}{\mathbb{E}[\min_{l=1,2,3}X_l]} =33 \mathbb{E}[T_2]$. The ``Low bound'' curve is generated by using $\mathbb{E}[D_{\text{avg}}(\bm{V}(\text{FUT-R}))|\mathcal{I}]$ which, according to Theorem \ref{thm1}, is a lower bound of the optimum expected average delay. We can observe that the delay performance of policy FUT-R is close to the lower bound, compared with the other policies.


% quite close to the delay lower bound. Hence, for any queue length, each task should be replicated on all servers for NWU service time distributions. 

%These results are in accordance with Theorem \ref{thm1}.

\ifreport
\begin{figure}
\centering \includegraphics[width=0.6\textwidth]{Figures/figure3_lateness_shifted_exp} \caption{Complementary CDF of the maximum lateness $\Pr[L_{\max} (\bm{C}(\pi))>t|\mathcal{I}]$ versus $t$ in a centralized queueing system with heterogeneous NBU service time distributions.}
\label{fig3} \vspace{-0.cm}
\end{figure}
\else
\begin{figure}
\centering \includegraphics[width=0.4\textwidth]{Figures/figure3_lateness_shifted_exp} \caption{Complementary CDF of the maximum lateness $\Pr[L_{\max} (\bm{C}(\pi))>t|\mathcal{I}]$ versus $t$ for different policy $\pi$ in a centralized queueing system  with heterogeneous NBU service time distributions.}
\label{fig3} \vspace{-0.cm}
\end{figure}
\fi

\subsubsection{Maximum Lateness}


Figure \ref{fig3} evaluates the complementary CDF of maximum lateness $\Pr[L_{\max} (\bm{C}(\pi))$ $>t|\mathcal{I}]$ versus $t$ in a centralized queueing system with heterogeneous NBU service time distributions. The number of incoming jobs is $n=100$, the job size $k_i$ is chosen to be either $1$ or $10$ with equal probability, and the due time $d_i$ is chosen to be either $a_i$ or $a_i+50$ with equal probability. 
The distributions of task service times and cancellation overheads are the same with those in Fig. \ref{fig1}. The traffic intensity is set as $\rho = 0.8$.  
The ``Low bound'' curve is generated by using $\Pr[L_{\max}(\bm{V}(\text{EDD-NR}))>t|\mathcal{I}]$, which, according to Theorem \ref{thm3}, is a lower bound of the optimum delay performance.
We can observe that the complementary CDF of the maximum lateness of policies EDD-NR and EDD-NIR are close to the lower bound curve. In addition, the delay performance of policy FCFS-NR is better than that of FCFS-R and EDD-R. This is because policy FCFS-NR  has a larger throughput region than policy  FCFS-R and policy EDD-R. 
%In addition, the job with the earliest due time should be executed first to reduce the maximum lateness.

%Hence, when the queue length is large, no task should be replicated for NBU service time distributions.


\ifreport
\begin{figure}
\centering \includegraphics[width=0.6\textwidth]{Figures/figure4_lateness_Pareto} \caption{Complementary CDF of the maximum lateness $\Pr[L_{\max} (\bm{C}(\pi))>t|\mathcal{I}]$ versus $t$ in a centralized queueing system with heterogeneous service time NWU distributions.}
\label{fig4} \vspace{-0.cm}
\end{figure}
\else
\begin{figure}
\centering \includegraphics[width=0.4\textwidth]{Figures/figure4_lateness_Pareto} \caption{Complementary CDF of the maximum lateness $\Pr[L_{\max} (\bm{C}(\pi))>t|\mathcal{I}]$ versus $t$ for different policy $\pi$ in a centralized queueing system with heterogeneous service time NWU distributions.}
\label{fig4} \vspace{-0.cm}
\end{figure}
\fi

Figure \ref{fig4} shows the complementary CDF of maximum lateness $\Pr[L_{\max} (\bm{C}(\pi))>t|\mathcal{I}]$ versus $t$ for a centralized queueing system with heterogeneous NWU service time distributions. The number of incoming jobs is $n=100$, the job size $k_i$ is chosen to be either $1$ or $10$ with equal probability, and the due time $d_i$ is $a_i+5$. 
The distributions of task service times and cancellation overheads are the same with those in Fig. \ref{fig2}. The traffic intensity is set as $\rho = 0.8$. 
Because $d_1\leq d_2\leq\ldots\leq d_n$, the EDD discipline is identical with the FCFS discipline. %i FCFS-R (policy FCFS-NR, or policy FCFS-NIR)
We can observe that policy EDD-R, which is identical with policy FCFS-R, achieves better  performance than the other policies, which is in accordance with Theorem \ref{thm4}. 

%We can observe that the complementary CDF of the maximum lateness of policy EDD-R is close to the lower bound curve. In addition, the delay performance of policy FCFS-R is better than those of policies EDD-NR, EDD-NIR, and FCFS-NR, which have a smaller throughput region.

\ifreport
\begin{figure}
\centering \includegraphics[width=0.6\textwidth]{Figures/figure4_lateness_exp} \caption{Complementary CDF of the maximum lateness $\Pr[L_{\max} (\bm{C}(\pi))>t|\mathcal{I}]$ versus $t$ in a centralized queueing system with heterogeneous exponential service time distributions.}
\label{fig4_exp} \vspace{-0.cm}
\end{figure}
\else
\begin{figure}
\centering \includegraphics[width=0.4\textwidth]{Figures/figure4_lateness_exp} \caption{Complementary CDF of the maximum lateness $\Pr[L_{\max} (\bm{C}(\pi))>t|\mathcal{I}]$ versus $t$ for different policy $\pi$ in a centralized queueing system with heterogeneous exponential service time  distributions.}
\label{fig4_exp} \vspace{-0.cm}
\end{figure}
\fi

Figure \ref{fig4_exp} provides the complementary CDF of maximum lateness $\Pr[L_{\max} (\bm{C}(\pi))>t|\mathcal{I}]$ versus $t$ for a centralized queueing system with heterogeneous exponential service time distributions. The number of incoming jobs is $n=100$, the job size $k_i$ is chosen to be either $1$ or $10$ with equal probability, and the  due time $d_i$ is chosen to be either $a_i$ or $a_i+50$ with equal probability. 
The distributions of task service times and cancellation overheads are the same with those in Fig. \ref{fig2_exp}. The traffic intensity is set as $\rho = 0.8$. The ``Low bound'' curve is generated by using $\Pr[L_{\max}(\bm{V}(\text{EDD-R}))>t|\mathcal{I}]$.
We can observe that the delay performance of policy EDD-R is quite close to the lower bound curve. The delay performance of policy EDD-NR and policy EDD-NIR is a bit farther than from the lower bound curve. 
Policy FCFS-R and policy FCFS-NR have the worse performance. 
These results are in accordance with  Theorem \ref{thm3} and Theorem \ref{thm4_exp}.

%In addition, the delay performance of policy FCFS-R is better than those of policies EDD-NR, EDD-NIR, and FCFS-NR, which have a smaller throughput region.

%\begin{figure}
%\centering \includegraphics[width=0.6\textwidth]{Figures/figure1_square_lateness_shifted_exp} \caption{Root mean square of tardiness $\mathbb{E}[T_{\text{ms}} (\bm{C}(\pi))|\mathcal{I}]^{1/2}$ versus traffic intensity $\rho$ for different policy $\pi$ in a centralized queueing system, where the task service times of the servers follow {independent} NBU distributions.}
%\label{fig1_1} \vspace{-0.cm}
%\end{figure}

\ifreport
\begin{figure}
\centering \includegraphics[width=0.6\textwidth]{Figures/figure5_maximum_delay_shifted_exp} \caption{Complementary CDF of the maximum delay $\Pr[D_{\max} (\bm{C}(\pi))>t|\mathcal{I}]$ versus $t$  in a centralized queueing system with heterogeneous NBU service time distributions.}
\label{fig5} \vspace{-0.cm}
\end{figure}
\else
\begin{figure}
\centering \includegraphics[width=0.4\textwidth]{Figures/figure5_maximum_delay_shifted_exp} \caption{Complementary CDF of the maximum delay $\Pr[D_{\max} (\bm{C}(\pi))>t|\mathcal{I}]$ versus $t$  in a centralized queueing system with heterogeneous NBU  service time distributions.}
\label{fig5} \vspace{-0.cm}
\end{figure}
\fi
\ifreport
\begin{figure}
\centering \includegraphics[width=0.6\textwidth]{Figures/figure6_maximum_delay_Pareto} \caption{Complementary CDF of the maximum delay $\Pr[D_{\max} (\bm{C}(\pi))>t|\mathcal{I}]$ versus $t$  in a centralized queueing system with heterogeneous NWU service time distributions.}
\label{fig6} \vspace{-0.cm}
\end{figure}
\else
\begin{figure}
\centering \includegraphics[width=0.4\textwidth]{Figures/figure6_maximum_delay_Pareto} \caption{Complementary CDF of the maximum delay $\Pr[D_{\max} (\bm{C}(\pi))>t|\mathcal{I}]$ versus $t$  in a centralized queueing system with heterogeneous NWU service time distributions.}
\label{fig6} \vspace{-0.cm}
\end{figure}
\fi

\subsubsection{Maximum Delay}
Figure \ref{fig5} plots the complementary CDF of maximum delay $\Pr[D_{\max} (\bm{C}(\pi))>t|\mathcal{I}]$ versus $t$ in a centralized queueing system with heterogeneous NBU service time distributions. The system model is the same with that of Fig. \ref{fig3}.
%number of incoming jobs is $n=100$, the job size $k_i$ is chosen to be either $1$ or $10$ with equal probability, and the  due time $d_i$ is chosen to be either $a_i$ or $a_i+50$ with equal probability.  The distributions of task service times and cancellation overheads are the same with those in Fig. \ref{fig1}. The traffic intensity is set as $\rho = 0.8$.  
The ``Low bound'' curve is generated by using $\Pr[D_{\max}(\bm{V}(\text{FCFS-NR}))$ $>t|\mathcal{I}]$,  which, according to Theorem \ref{thm5}, is a lower bound of the optimum delay performance.
We can observe that the delay performance of policy FCFS-NR and policy FCFS-NIR is close to the lower bound curve. In addition, the delay performance of policy EDD-NR is better than that of FCFS-R and EDD-R because policy EDD-NR has a larger throughput region than policy  FCFS-R and policy EDD-R. 
%In addition, the job with the earliest arrival time should be executed first to reduce the maximum delay.



Figure \ref{fig6} illustrates the complementary CDF of maximum delay $\Pr[D_{\max} (\bm{C}(\pi))>t|\mathcal{I}]$ versus $t$ in a centralized queueing system with heterogeneous NWU service time distributions. The system model is almost the same with that of Fig. \ref{fig4}, except that the  due time $d_i$ is chosen to be either $a_i$ or $a_i+50$ with equal probability. 
We can observe that the delay performance of policy FCFS-R is much better than that of the other policies, which validates Theorem \ref{thm6}. 

\ifreport
\begin{figure}
\centering \includegraphics[width=0.6\textwidth]{Figures/figure_3root_mean_square_lateness_shifted_exp} \caption{Root mean square of tardiness $\mathbb{E}[T_{\text{ms}} (\bm{C}(\pi))|\mathcal{I}]^{0.5}$ versus traffic intensity $\rho$ in a centralized queueing system with heterogeneous NBU service time distributions.}
\label{fig5_RMS_tardiness} \vspace{-0.cm}
\end{figure}
\else
\begin{figure}
\centering \includegraphics[width=0.4\textwidth]{Figures/figure_3root_mean_square_lateness_shifted_exp} \caption{Root mean square of tardiness $\mathbb{E}[T_{\text{ms}} (\bm{C}(\pi))|\mathcal{I}]^{0.5}$ versus traffic intensity $\rho$ in a centralized queueing system with heterogeneous NBU  service time distributions.}
\label{fig5_RMS_tardiness} \vspace{-0.cm}
\end{figure}
\fi

\ifreport
\begin{figure}
\centering \includegraphics[width=0.6\textwidth]{Figures/figure_4root_mean_square_lateness_exp} \caption{Root mean square of tardiness $\mathbb{E}[T_{\text{ms}} (\bm{C}(\pi))|\mathcal{I}]^{0.5}$ versus traffic intensity $\rho$ in a centralized queueing system with heterogeneous exponential service time distributions.}
\label{fig6_RMS_tardiness} \vspace{-0.cm}
\end{figure}
\else
\begin{figure}
\centering \includegraphics[width=0.4\textwidth]{Figures/figure_4root_mean_square_lateness_exp} \caption{Root mean square of tardiness $\mathbb{E}[T_{\text{ms}} (\bm{C}(\pi))|\mathcal{I}]^{0.5}$ versus traffic intensity $\rho$ in a centralized queueing system with heterogeneous exponential  service time distributions.}
\label{fig6_RMS_tardiness} \vspace{-0.cm}
\end{figure}
\fi

\subsection{Some Other Delay Metrics}
Figure \ref{fig5_RMS_tardiness} shows the root mean square of tardiness $\mathbb{E}[T_{\text{ms}} (\bm{C}(\pi))|\mathcal{I}]^{0.5}$ versus traffic intensity $\rho$ in a centralized queueing system with heterogeneous NBU service time distributions, where 
\begin{align}
T_{\text{ms}}(\bm{C}(\pi)) \!= \frac{1}{n}\sum_{i=1}^{n} \max[L_i(\pi),0]^2=\frac{1}{n}\sum_{i=1}^{n} \max\left[C_i(\pi)-d_i,0\right]^2.\nonumber
\end{align}
The system model is similar with that of Fig. \ref{fig5}, except that $k_i=1$ for all job $i$ and the due time $d_i$ is either $a_i$ or $a_i+10$ with equal probability.
%number of incoming jobs is $n=100$, the job size $k_i$ is chosen to be either $1$ or $10$ with equal probability, and the  due time $d_i$ is chosen to be either $a_i$ or $a_i+50$ with equal probability.  The distributions of task service times and cancellation overheads are the same with those in Fig. \ref{fig1}. The traffic intensity is set as $\rho = 0.8$.  
The ``Low bound'' curve is generated by using $\mathbb{E}[T_{\text{ms}} (\bm{V}(\text{EDD-NR}))|\mathcal{I}]^{0.5}$, which, according to Theorem \ref{coro_thm3_1}, is a lower bound of the optimum delay performance.
We can observe that the delay performance of policy EDD-NR and policy EDD-NIR is close to the lower bound curve, and is better than that of the other policies. Notice that as  $\rho\rightarrow 0$, policy EDD-R and policy EDD-NIR tends become the same policy, and hence has the same delay performance.

%can achieve a smaller delay than policy EDD-NR and policy EDD-NIR, because replication is beneficial when  low system load. 
% performance 
%In addition, the job with the earliest arrival time should be executed first to reduce the maximum delay.



Figure \ref{fig6_RMS_tardiness} presents the root mean square of tardiness $\mathbb{E}[T_{\text{ms}} (\bm{C}(\pi))|\mathcal{I}]^{0.5}$ versus traffic intensity $\rho$ in a centralized queueing system with heterogeneous exponential service time distributions. The system model is similar with that of Fig. \ref{fig6}, except that $k_i=1$ for all job $i$ and the due time $d_i$ is either $a_i$ or $a_i+10$ with equal probability. 
The ``Low bound'' curve is generated by using $\mathbb{E}[T_{\text{ms}} (\bm{V}(\text{EDD-R}))|\mathcal{I}]^{0.5}$, which, according to Theorem \ref{coro_thm3_1_exp}, is a lower bound of the optimum delay performance.
We can observe that the delay performance of policy EDD-R is close to the lower bound curve, and is better than that of the other policies.


\ifreport
\begin{figure}
\centering \includegraphics[width=0.6\textwidth]{Figures/figure_1root_mean_square_delay_shifted_exp} \caption{Root mean square of delay $\mathbb{E}[D_{\text{ms}} (\bm{C}(\pi))|\mathcal{I}]^{0.5}$ versus traffic intensity $\rho$ in a centralized queueing system with heterogeneous NBU service time distributions.}
\label{fig5_RMS} \vspace{-0.cm}
\end{figure}
\else
\begin{figure}
\centering \includegraphics[width=0.4\textwidth]{Figures/figure_1root_mean_square_delay_shifted_exp} \caption{Root mean square of delay $\mathbb{E}[D_{\text{ms}} (\bm{C}(\pi))|\mathcal{I}]^{0.5}$ versus traffic intensity $\rho$ in a centralized queueing system with heterogeneous NBU  service time distributions.}
\label{fig5_RMS} \vspace{-0.cm}
\end{figure}
\fi

\ifreport
\begin{figure}
\centering \includegraphics[width=0.6\textwidth]{Figures/figure_2root_mean_square_delay_Pareto} \caption{Root mean square of delay $\mathbb{E}[D_{\text{ms}} (\bm{C}(\pi))|\mathcal{I}]^{0.5}$ versus traffic intensity $\rho$ in a centralized queueing system with heterogeneous NWU service time distributions.}
\label{fig6_RMS} \vspace{-0.cm}
\end{figure}
\else
\begin{figure}
\centering \includegraphics[width=0.4\textwidth]{Figures/figure_2root_mean_square_delay_Pareto} \caption{Root mean square of delay $\mathbb{E}[D_{\text{ms}} (\bm{C}(\pi))|\mathcal{I}]^{0.5}$ versus traffic intensity $\rho$ in a centralized queueing system with heterogeneous NWU  service time distributions.}
\label{fig6_RMS} \vspace{-0.cm}
\end{figure}
\fi


Figure \ref{fig5_RMS} illustrates the root mean square of delay $\mathbb{E}[D_{\text{ms}} (\bm{C}(\pi))|\mathcal{I}]^{0.5}$ versus traffic intensity $\rho$ in a centralized queueing system with heterogeneous NBU service time distributions, where 
\begin{align}
D_{\text{ms}}(\bm{C}(\pi)) \!= \frac{1}{n}\sum_{i=1}^{n} D_i^2(\pi)=\frac{1}{n}\sum_{i=1}^{n} \left[C_i(\pi)-a_i\right]^2.\nonumber
\end{align}
The system model is almost the same with that of Fig. \ref{fig5}, except that $k_i=10$ for all job $i$.
%number of incoming jobs is $n=100$, the job size $k_i$ is chosen to be either $1$ or $10$ with equal probability, and the  due time $d_i$ is chosen to be either $a_i$ or $a_i+50$ with equal probability.  The distributions of task service times and cancellation overheads are the same with those in Fig. \ref{fig1}. The traffic intensity is set as $\rho = 0.8$.  
The ``Low bound'' curve is generated by using $\mathbb{E}[D_{\text{ms}} (\bm{V}(\text{FCFS-NR}))|\mathcal{I}]^{0.5}$, which, according to Theorem \ref{coro5_1}, is a lower bound of the optimum delay performance.
We can observe that the delay performance of policy FCFS-NR and policy FCFS-NIR is close to the lower bound curve, and is much better than the other policies. 

%In addition, the job with the earliest arrival time should be executed first to reduce the maximum delay.



Figure \ref{fig6_RMS} presents the root mean square of delay $\mathbb{E}[D_{\text{ms}} (\bm{C}(\pi))|\mathcal{I}]^{0.5}$ versus traffic intensity $\rho$ in a centralized queueing system with heterogeneous NWU service time distributions. The system model is almost the same with that of Fig. \ref{fig6}, except that $k_i=10$ for all job $i$. 
We can observe that the delay performance of policy FCFS-R is much better than that of the other policies, which validates Theorem \ref{coro6_1}. 

\ifreport
\begin{figure}
\centering \includegraphics[width=0.6\textwidth]{Figures/figure7_maximum_lateness_distributed} \caption{Complementary CDF of the maximum lateness $\Pr[L_{\max} (\bm{C}(\pi))>t|\mathcal{I}]$ versus $t$ in a distributed queueing system with per-task data locality constraints.}
\label{fig7} \vspace{-0.cm}
\end{figure}
\else
\begin{figure}
\centering \includegraphics[width=0.4\textwidth]{Figures/figure7_maximum_lateness_distributed} \caption{Complementary CDF of the maximum lateness $\Pr[L_{\max} (\bm{C}(\pi))>t|\mathcal{I}]$ versus $t$ in a distributed queueing system with per-task data locality constraints.}
\label{fig7} \vspace{-0.cm}
\end{figure}
\fi
\subsection{Distributed Queueing Systems}

%The distributions of task service times and cancellation overheads are the same with those in Fig. \ref{fig1}. 


Next, we provide some numerical results for the delay performance of replications in distributed queueing systems with data locality constraints. The inter-arrival time of the jobs $T_i=a_{i+1}-a_i$ is exponentially distributed for even $i$; and is zero for odd $i$. The number of incoming jobs is $n=100$. The due time $d_i$ of job $i$ is $a_i$ or $a_i+50$ with equal probability. The traffic intensity is set as $\rho = 0.8$.  
%\subsubsection{Per-Task Data Locality Constraints}

Figure \ref{fig7} evaluates the complementary CDF of maximum lateness $\Pr[L_{\max} (\bm{C}(\pi))$ $>t|\mathcal{I}]$ versus $t$ in a distributed queueing system with per-task data locality constraints. The system has $g=2$ groups of servers, each consisting of 3 servers. The size of each sub-job $k_{ih}$ is  $1$ or $10$ with equal probability. The distributions of task service times and cancellation overheads of one group of servers are the same with those in Fig. \ref{fig1}, and the distributions of task service times and cancellation overheads of the other  group of servers are the same with those in Fig. \ref{fig2_exp}. 
The ``Low bound'' curve is generated by using $\Pr[L_{\max}(\bm{V}(\text{EDD-GR}))>t|\mathcal{I}]$, which, according to Theorem \ref{thm_dis4}, is a lower bound of the optimum delay performance. We can observe that The delay performance of  policy EDD-GR is close to the lower bound curve. In addition, policy EDD-NR and EDD-GR have similar performance. This is because exponential distribution is also NBU. Hence, both groups of servers have NBU service time distributions.
% and is much better than that of the other policies. 

\ifreport
\begin{figure}
\centering \includegraphics[width=0.6\textwidth]{Figures/figure8_maximum_delay_distributed} \caption{Complementary CDF of the maximum delay $\Pr[D_{\max} (\bm{C}(\pi))>t|\mathcal{I}]$ versus $t$ in a distributed queueing system with per-task data locality constraints.}
\label{fig8} \vspace{-0.cm}
\end{figure}
\else
\begin{figure}
\centering \includegraphics[width=0.4\textwidth]{Figures/figure8_maximum_delay_distributed} \caption{Complementary CDF of the maximum delay $\Pr[D_{\max} (\bm{C}(\pi))>t|\mathcal{I}]$ versus $t$ in a distributed queueing system with per-task data locality constraints.}
\label{fig8} \vspace{-0.cm}
\end{figure}
\fi
Figure \ref{fig8} depicts the complementary CDF of maximum delay $\Pr[D_{\max} (\bm{C}(\pi))$ $>t|\mathcal{I}]$ versus $t$ in a distributed queueing system with per-task data locality constraints. This system has $g=3$ groups of servers, each consisting of 3 servers. The size of each sub-job $k_{ih}$ is  $1$ or $10$ with equal probability. The distributions of task service times and cancellation overheads of two groups of servers are the same with those in Fig. \ref{fig7}, and the distributions of task service times and cancellation overheads of the third group of servers are the same with those in Fig. \ref{fig2}. 
The ``Low bound'' curve is generated by using $\Pr[D_{\max}(\bm{V}(\text{FCFS-GR}))>t|\mathcal{I}]$, which, according to Theorem \ref{thm_dis5}, is a lower bound of the optimum delay performance. We can see that the delay performance of  policy FCFS-GR is quite close to the lower bound curve and is much better than that of the other policies. 
%\subsubsection{Per-Job Data Locality Constraints}
%Figure \ref{fig8_RMS_tardiness_locality} plots the root mean square of tardiness $\mathbb{E}[T_{\text{ms}} (\bm{C}(\pi))|\mathcal{I}]^{0.5}$ versus traffic intensity $\rho$ in a distributed queueing system with per-job data locality constraints. The system model is similar with that of Fig. \ref{fig8}, except that each job has only one task and the due time $d_i$ is either $a_i$ or $a_i+10$ with equal probability.
%%number of incoming jobs is $n=100$, the job size $k_i$ is chosen to be either $1$ or $10$ with equal probability, and the  due time $d_i$ is chosen to be either $a_i$ or $a_i+50$ with equal probability.  The distributions of task service times and cancellation overheads are the same with those in Fig. \ref{fig1}. The traffic intensity is set as $\rho = 0.8$.  
%The ``Low bound'' curve is generated by using $\mathbb{E}[T_{\text{ms}} (\bm{V}(\text{EDD-GR}))|\mathcal{I}]^{0.5}$, which, according to Theorem \ref{thm3_dist}, is a lower bound of the optimum delay performance.
%We can observe that the delay performance of policy EDD-GR is close to the lower bound curve, and is better than that of the other policies. 
%%Notice that as  $\rho\rightarrow 0$, policy EDD-R and policy EDD-NIR tends become the same policy, and hence has the same delay performance.
%
%
%
% The distributions of task service times and cancellation overheads of two groups of servers are the same with those in Fig. \ref{fig7}, and the distributions of task service times and cancellation overheads of the third group of servers are the same with those in Fig. \ref{fig2}. 
%The ``Low bound'' curve is generated by using $\Pr[D_{\max}(\bm{V}(\text{FCFS-GR}))>t|\mathcal{I}]$, which, according to Theorem \ref{thm_dis5}, is a lower bound of the optimum delay performance. We can see that the delay performance of  policy FCFS-GR is quite close to the lower bound curve and is much better than that of the other policies. 
%


==> v3/sufficient_conditions.tex <==
% !TEX root = ./replication.tex

%\section{Sufficient Conditions for Delay Optimality and Near-Optimality}


\section{Sufficient Conditions for Near Delay Optimality}\label{sec_sufficient}
%\section{Proof Structure}
%The existing proof techniques for the delay optimality or near optimality of task replication policies are combinatorial and  difficult to understand. There is a lack of unify framework to unify different proof techniques.  As an attempt to alleviate this difficulty, 

%Existing delay optimality and near delay optimality analyses of task replications \cite{Borst2003,Righter2008,Kim2010,shah-Allerton-2013,ShengboInfocom,Sun2015} focused on the average delay ${D}_{\text{avg}}(\cdot)$, and their proof techniques vary from case to case. 
%There is a lack of unified treatment for minimizing different delay metrics in various system settings. 
In this section, we establish a unified framework for minimizing several classes of delay metrics in various system settings. In particular, sufficient conditions are proposed for proving that a scheduling policy is near delay-optimal, %These sufficient conditions do not need to specify the queueing model or service time distribution, and hence provide a unified treatment for various system settings. 
%In addition, 
%These sufficient conditions can handle not only the average delay ${D}_{\text{avg}}(\cdot)$, but also more general delay metric functions in $\mathcal{D}_{\text{sym}}$, $\mathcal{D}_{\text{Sch-1}}$, and $\mathcal{D}_{\text{Sch-2}}$. 
% for various system settings.
%These sufficient conditions
which will be used to establish our main results in later sections. These sufficient conditions are proven by using stochastic ordering and majorization.
%A \textbf{sample-path ordering} technique is developed to prove 
 %Note that the bounds that we will describe are by no means the tightest that are available from the sample-path ordering technique. In particular, different bounds can be obtained from different forms of sample-path ordering, which will be studied in our future work.
%for centralized queue systems in Section \ref{sec_analysis}, and for distributed queue systems in Section \ref{sec_distributed}.
% for distribued delay metrics and system settings.

%which provide a unified framework in minimizing a number of delay metrics. These sufficient conditions do not depend on a specific system setting, independent, The existing proof techniques for the delay optimality or near optimality results of task replication policies  
%are combinatorial and 
%vary from case to case, 
%which makes them difficult to understand, 
%which do not provide a unified treatment for different system settings.
% and do not provide a unified treatment. 
% combinatorial and  difficult to understand. There is a lack of unify framework to unify different proof techniques.  
%As an attempt to alleviate this difficulty, 


%These sufficient conditions will be used in later sections to %outline the key proof steps of 
%which will be used later sections to prove near delay optimality results in various system settings. 


%We will see that the sufficient conditions for different delay metrics can be expressed in similar forms to provide a unified treatment for different delay metrics, but their proof techniques are different. 
%

%Moreover, in order to compare the task completion times among different scheduling policies, we develop a \emph{sample-path ordering} technique, which enables us to  prove near delay optimality results in the form of \eqref{eq_nearoptimal}. 
%The results of this section are proven in Appendix \ref{app0}.

%When using these sufficient conditions, one key difficulty is to prove that a scheduling policy is near-optimal in terms of \eqref{eq_nearoptimal}. To that end, we develop a novel technique called \emph{sample-path ordering}, which can effectively characterize the delay gap from the optimum. 
%\subsection{} 


%In this section, we propose novel sufficient conditions for proving that a scheduling policy is  delay-optimal or near-optimal. These sufficient conditions reveal the key ideas in delay optimality analysis of task replications and can greatly simplify the corresponding proof arguments.  The proofs of these sufficient conditions are provided in Appendix \ref{app0}.

% showing the existence of a low-complexity policy that is within a finite gap from the optimum delay.
%There is a lack of uniform methodology for bounding the sub-optimality gap from the optimum delay performance.

%Their usage will be illustrated in later sections when studying task replications across heterogeneous servers.

%In this section, we present a general analysis framework of
%redundant executions which serves two purposes: (i) to provide
%sufficient conditions for identifying scheduling policies that
%are delay-optimal or near-optimal, and (ii) to simplify and
%unify the proof techniques for establishing delay optimalityalleviate
%and near-optimality. These analysis tools will be used later tocumbersome
%study redundancy scheduling across heterogeneous servers.

 
%Define $\bm{s}=(s_{1},\ldots, s_{k_{\text{sum}}})$ as the sequence of task arrival times of the system, and $\bm{T}(\pi)=(T_{1}(\pi),\ldots, T_{k_{\text{sum}}}(\pi))$ as the sequence of task completion times of the system. The components of $\bm{s}$ and $\bm{T}(\pi)$ are arranged in the increasing order such that $\bm{s} =\bm{s}_{\uparrow}$ and $\bm{T}(\pi)=\bm{T}_{\uparrow}(\pi)$.~Then, $\bm{s}$ is uniquely determined by $\mathcal{I}$, while $\bm{T}(\pi)$ is determined by $\mathcal{I}$, the scheduling policy $\pi$, and random task service times.
\subsection{Work-Efficiency Ordering}

In traditional queueing systems without task replications, the service delay is largely governed by the following work conservation law (or its generalizations): At any time, the expected total amount of time for completing the jobs in the queue is invariant among all work-conserving policies \cite{Leonard_Kleinrock_book,Gittins:11}. However, this work conservation law does not hold in queueing system with task replications.
%, because each task has multiple replication modes. 
In particular, each task has multiple replication modes (i.e., it can be replicated on different numbers of servers and at different time instants), which require different amounts of service time. In order to minimize delay, the scheduler needs to choose efficient replication modes to execute the tasks. Motivated by this, we define a work-efficiency ordering to compare the efficiency of task executions in different task replication policies, where the job indices of the tasks are not concerned. 
%One illustration of this is provided in Fig. \ref{Work_Efficiency_Ordering}.



% Consider two non-preemptive feasible policies $\pi_1,\pi_2\in\Pi$. Suppose that the 


% in policy $\pi_1$ the tasks are executed in a more efficient replication mode than in policy $\pi_2$, then one would expect the . If , then in policy $\pi_1$ no fewer than $b$ tasks start execution during $[\tau,\nu]$, which may complete execution after time $\nu$ because 







%Define $\bm{s}=(s_{1},\ldots, s_{k_{\text{sum}}})$ as the sequence of task arrival times of the system, and $\bm{T}(\pi)=(T_{1}(\pi),\ldots,$ $ T_{k_{\text{sum}}}(\pi))$ as the sequence of task completion times of the system. The components of $\bm{s}$ and $\bm{T}(\pi)$ are arranged in the increasing order such that $\bm{s} =\bm{s}_{\uparrow}$ and $\bm{T}(\pi)=\bm{T}_{\uparrow}(\pi)$.~Then, $\bm{s}$ is uniquely determined by $\mathcal{I}$, while $\bm{T}(\pi)$ is determined by $\mathcal{I}$, the scheduling policy $\pi$, and random task service times.

%Let $k_{\text{sum}}=\sum_{i=1}^nk_i$ denote the total number of tasks, $\bm{t}(\pi)=(t_{1}(\pi),\ldots, t_{k_{\text{sum}}}(\pi))$ denote the realizations of task completion times on a sample path of policy $\pi$. The components of $\bm{t}(\pi)$ are arranged in the increasing order such that $\bm{t} (\pi)=\bm{t}_{\uparrow}(\pi)$.

%A relationship between two policies $\pi_1$ and $\pi_2$ is said to \textbf{hold on sample path}, if there is a measure preserving one-to-one correspondence between the sample paths of policies $\pi_1$ and $\pi_2$, such that  the relationship holds between each pair of corresponding sample paths of policies $\pi_1$ and $\pi_2$.

%We define a \emph{work efficiency order}:

%For any time interval $[\tau,\nu]$ and policy $\pi$, let $n_{{s}}^{\pi}(\tau,\nu)$ denote the number of tasks that start execution during $[\tau,\nu]$, and $n_{sc}^{\pi}(\tau,\nu)$ denote the number of tasks that start and complete execution during $[\tau,\nu]$. 

A relationship between policy $\pi_1$ and policy $\pi_2$ is said to \textbf{hold in stochastic ordering}, if for each sample path of policy $\pi_1$ there is a corresponding sample path of policy $\pi_2$, such that (i) these two sample paths of policy $\pi_1$ and policy $\pi_2$ have the same probability density, and (ii) the relationship holds between these two sample paths of policy $\pi_1$ and policy $\pi_2$.

\begin{definition} \label{def_order} \textbf{Work-Efficiency Ordering:}
A work-conserving policy $\pi_1\in\Pi$ is said to be \textbf{more work-efficient} than policy $\pi_2\in\Pi$, if 
the following relationship between policy $\pi_1$ and policy $\pi_2$ holds in stochastic ordering: For each task $j$ executed in  policy $\pi_2$, if 
\begin{itemize}
\item[1.] Task $j$ starts execution at time $\tau$ and completes execution at time $\nu$ on the sample path of policy $\pi_2$ where $\nu\geq\tau$, 
\item[2.] There exist unassigned tasks in the queue during $[\tau,\nu]$ on the corresponding sample path of policy $\pi_1$, 
\end{itemize}
then  on the sample path of policy $\pi_1$ there exists one corresponding task $j'$ which starts execution during $[\tau,\nu]$. 
\end{definition}

An illustration of the work-efficiency ordering is provided in Fig. \ref{Work_Efficiency_Ordering}. Informally speaking, policy $\pi_1$ is said to be more work-efficient than policy $\pi_2$, if the tasks are executed faster in policy $\pi_1$ than in policy $\pi_2$. In particular, if the service duration of task $j$ is $[\tau,\nu]$ on the sample path of policy $\pi_2$, then there  exists one task $j'$ whose service time is shorter than $\nu-\tau$ on the corresponding sample path of policy $\pi_1$. Because the task service of policy $\pi_1$ and policy $\pi_2$ is asynchronized, the executions of task $j$ and task $j'$ may start at different time instants. Hence, task $j'$ may start execution during $[\tau,\nu]$, and complete execution either before or after time $\nu$. We note that work-efficiency ordering is defined on task-level, which is not related to the service priority of different jobs. For this reason, the job indices of task $j$ and task $j'$ are not specified in the definition.

% speed  determined by the job indices of task $j$ and task $j'$ are not specified because they do not affect the efficiency of policy $\pi_1$ and policy $\pi_2$.


% the task service of policy $\pi_1$ and policy $\pi_2$ is asynchronized

%If on the sample path of policy $\pi_2$, one server starts to process a task at time $\tau$ and completes this task at time $\nu$ ($\tau\leq\nu$), then  on the sample path of policy $\pi_1$ there exists a time $t\in[\tau,\nu]$ such that one of the following three cases holds:  (i) the same server starts to process a corresponding task at time $t$ (as illustrated in Fig. \ref{Work_Efficiency_Ordering}), (ii) all the remaining tasks are under service at time $t$, or (iii) the queue is empty at time $t$.


%for any time interval $[\tau,\nu]$ if $b$ tasks start execution and also complete execution during $[\tau,\nu]$ in policy $\pi_2$, then one would expect that in policy $\pi_1$ no fewer than $b$ tasks start execution during $[\tau,\nu]$ (unless there are not enough tasks to execute in policy $\pi_1$); however, these tasks may complete execution after time $\nu$ in policy $\pi_1$, because the task service of policy $\pi_1$ and policy $\pi_2$ is asynchronized. 
%By this, the work-efficiency ordering can be defined as follows:


%This definition can be understood as follows: If each task is executed in a more efficient mode in policy $\pi_1$ than policy $\pi_2$, then the service duration of the task is shorter in policy $\pi_1$ than policy $\pi_2$. Because policy $\pi_1$ and policy $\pi_2$ are asynchronized, if $b$ tasks start and complete execution during $[\tau,\nu]$ on the sample path of policy $\pi_2$, than at least $b$ 


% $\pi_1\in\Pi$ is said to be \textbf{more work-efficient} than policy $\pi_2\in\Pi$


% $[\tau,\nu]$ and all servers are busy execution during $[\tau,\nu]$
%
%
%, if all servers are busy during $[\tau,\nu]$  on the sample path of policy $\pi_1$, then
%\begin{align}
%n_{{s}}^{\pi_1}(\tau,\nu)\geq_{\text{st}}  n_{sc}^{\pi_2}(\tau,\nu),
%\end{align}
%where $n_{{s}}^{\pi_1}(\tau,\nu)$ is the number of tasks that start execution during $[\tau,\nu]$  on the sample path of policy $\pi_1$, and $n_{sc}^{\pi_2}(\tau,\nu)$ is the number of tasks that start and complete execution during $[\tau,\nu]$  on the corresponding sample path of policy $\pi_2$.
% all servers are busy and $b$ tasks start execution in a time interval on the sample path of policy $\pi_1$, then no more than $b$ tasks start and complete execution in the same time interval on the sample path of policy $\pi_2$.
%$b$ tasks start and complete execution during $[\tau,\nu]$ on the sample path of policy $\pi_2$, then on the sample path of policy $\pi_1$, it holds that either $b$ tasks start execution during $[\tau,\nu]$ or all the remaining tasks are under service at some time $t\in[\tau,\nu]$.

%for all time interval $[\tau,\nu]\subseteq[0,\infty)$ and job parameters $\mathcal{I}$
%\begin{align}
%[N_{{a}}^{\pi_1}(\tau,\nu)| \mathcal{I}]\geq_{\text{st}}  [N_{ac}^{\pi_2}(\tau,\nu)| \mathcal{I}].
%\end{align}
%the following relationship holds on sample path: 
%\begin{itemize}
%\item[1.] $\bm{t}(\pi_1)\leq\bm{t}(\pi_2)$ holds on sample path.
%
%\item[2.] 
%For all $j=1,\ldots,n$ and $t\in[a_j,a_{j+1})$, 

%If on the sample path of policy $\pi_2$, one server starts to process a task at time $\tau$ and completes this task at time $\nu$ ($\tau\leq\nu$), then  on the sample path of policy $\pi_1$ there exists a time $t\in[\tau,\nu]$ such that one of the following three cases holds:  (i) the same server starts to process a corresponding task at time $t$ (as illustrated in Fig. \ref{Work_Efficiency_Ordering}), (ii) all the remaining tasks are under service at time $t$, or (iii) the queue is empty at time $t$.

\begin{figure}
\centering 
\includegraphics[width=0.4\textwidth]{Figures/work_efficiency_ordering} \caption{Illustration of work-efficiency ordering, where the service duration of a task is indicated by a rectangle. If on the sample path of policy $\pi_2$, task $j$ starts execution at time $\tau$ and completes execution at time $\nu$, then on the sample path of policy $\pi_1$ one corresponding task $j'$ starts execution at some time $t\in[\tau,\nu]$. The job indices of task $j$ and task $j'$ are not specified because they do not affect the efficiency of policy $\pi_1$ and policy $\pi_2$.}
% work--efficiency ordering holds for any priorities of the jobs.
\label{Work_Efficiency_Ordering} 
\end{figure} 
%or (ii') {one server is idle at time $\tau$}.\footnote{Note that the difference between these two definitions are in condition (ii) and condition (ii').}


%$b$ unassigned tasks are allocated to the servers and completed by the servers during $[a_j,t]$ on the sample path of policy $\pi_2$, then on the corresponding sample path of policy $\pi_1$ one of the following cases holds: (i) no fewer than $b$ unassigned tasks are allocated to the servers  during $[a_j,t]$, (ii) all the remaining tasks are under service at time $t$, or (iii) the queue is empty at time $t$.
%\end{itemize}
%in policy $\pi_2$ the system starts to process a task at time $\tau$ and completes the task at time $\nu$ ($\tau\leq\nu$), then in policy $\pi_1$ it holds that (i) a task is completed at some time during $[\tau,\nu]$, or (ii) {the queue is empty at time $\tau$}.
%for any sample path of policy $\pi_2$, there exists a sample path of policy $\pi_1$ with the same probability density such that $\bm{t}(\pi_1)\leq\bm{t}(\pi_2)$.
%Policy $\pi_1$ is said to be \emph{weakly more work-efficient} than policy $\pi_2$, if the following relationship holds on sample path: If in policy $\pi_2$ the system starts to process a task at time $\tau$ and completes the task at time $\nu$ ($\tau\leq\nu$), then in policy $\pi_1$ it holds that (i) a task is completed at some time during $[\tau,\nu]$, or (ii') {one server is idle at time $\tau$}.\footnote{Note that the difference between these two definitions are in condition (ii) and condition (ii').}


%The proof of the following lemma is straightforward and thus omitted: 
%\begin{theorem}\label{lemma_work_efficiency}
%If policy $\pi_1$ is {more work-efficient} than policy $\pi_2$, then
%\begin{itemize}
%\itemsep0em 
%\item[1.] policy $\pi_1$ is {weakly more work-efficient} than policy $\pi_2$;
%\item[2.] $\bm{t}(\pi_1)\leq\bm{t}(\pi_2)$ holds on sample path.
%\end{itemize} 
%\end{lemma}


%
\subsection{Sample-Path Ordering and Sufficient Conditions for Near Optimality}
In the special case that each job has one task, sufficient conditions are provided in \cite{Borst2003,Righter2008,Kim2010,shah-Allerton-2013} for minimizing 
%if policy $P\in\Pi$ is more {work-efficient} than all $\pi\in\Pi$, then policy $P$ minimizes 
the average delay ${D}_{\text{avg}}(\cdot)$% in distribution (or on sample path) 
. However, %as one can imagine, 
it is extremely difficult to establish delay optimality or near delay optimality results when the job sizes are arbitrarily given. 
By using work-efficiency ordering, we obtain the following sufficient condition for near delay optimality in minimizing ${D}_{\text{avg}}(\cdot)$ for general job sizes.

%In Sec. \ref{sec_analysis}, we will use this sufficient condition to study near delay-optimal scheduling of task replications for arbitrary job sizes.  


\begin{theorem}\label{lem1}
If there exists a work-conserving policy $P\in\Pi$ such that for all $\mathcal{I}$
\begin{itemize}
\itemsep0em 
\item[1.] Policy $P$ is {more work-efficient} than any policy $\pi\in\Pi$,
\item[2.] In policy $P$, each task allocated to the servers belongs to the job with the fewest unassigned tasks, whenever there exist unassigned tasks in the queue,
\end{itemize} 
then \emph{$[{D}_{\text{avg}}(\bm{V}_{}(P))|\mathcal{I}]\leq_{\text{st}} [{D}_{\text{avg}}(\bm{C}_{}(\pi))|\mathcal{I}]$} holds for all $\pi\in\Pi$ and $\mathcal{I}$.
\end{theorem}

%The sufficient condition of Theorem \ref{lem1} provides a unified treatment for minimizing ${D}_{\text{avg}}(\cdot)$ in various system settings. 


We note that, in Theorem \ref{lem1} and other sufficient conditions of this section, model-specific information (such as the number of servers and service time distribution) and policy-specific information (such as when to replicate a task and replicate on which servers) is summarized in the work-efficiency ordering. 
%In Section \ref{sec_analysis} and Section \ref{sec_distributed}, 
When applying these sufficient conditions, one needs to first prove the work-efficiency ordering between policy $P$ and any policy $\pi\in\Pi$ for the specified system setting, and then uses these sufficient conditions to show that policy $P$ is near delay-optimal. 

%When using this sufficient condition i
%does not specify one particular queueing model or service time distribution, because such 

%This sufficient condition not depend on the specific queueing model or service time distribution. For each specific system setting, this  as long as a work-efficiency ordering can be established between 



The difficulties in proving Theorem \ref{lem1} are as follows: First, policy $P$ is a dynamic priority policy where the job with the fewest unassigned tasks has the highest priority. Hence, the priority of a job increases as more tasks of this job are assigned to the servers. On the other hand, policy $\pi$ could be any policy in $\Pi$, which may follow a  different priority rule. Therefore,  the servers might be processing completely different jobs in policy $P$ and policy $\pi$, which makes it difficult to compare these two policies. Second, policy $P$ is an online policy, where the scheduling decisions are made without using any information about the future job arrivals. However, policy $\pi$ is allowed to have access to the parameters $(a_i,{k}_i,d_i)$ of future arriving jobs. Hence, the comparison between these two policies is unfair for policy $P$. Third, all policies in $\Pi$ are non-preemptive and server-idleness is allowed for some policies in $\Pi$. These conditions are adversary for finding a delay-optimal or near-optimal policy in $\Pi$ \cite{michael2012book,Gittins:11}. 

%Even if Lemma \ref{thm1} switches to seek for near-delay optimality result, it is unclear 

%suggests that in such adverse scenarios, it is still possible to establish near-delay optimality results.  
%The difficulties in Theorem \ref{lem1} are as follows: 

%



%we consider preemption is not allowed and server-idleness is allowed for the policies in $\Pi$, which makes it extremely difficult to find a delay-optimal policy in $\Pi$ \cite{michael2012book,Gittins:11}. Lemma \ref{thm1} suggests that it is still possible to seek for near delay optimality in such adverse scenario.  of delay optimality, it is still possible to prove Lemma \ref{thm1}. 


%Second,  Second, while policy $P$ is an online policy, policy $\pi$ may have access to the parameters $(a_i,{k}_i,d_i)$ of future arriving jobs. Hence, the comparison between these two policies is unfair for policy $P$. Third, in $\Pi$ are , which is usually 

In order to prove Theorem \ref{lem1}, we need to first define the system state for any policy $\pi\in\Pi$. 

\begin{definition}\label{def_state_thm3}
At any time $t$, the system state of policy $\pi$ is specified by a pair of $n$-vectors $\bm{\xi}_{\pi}(t)=(\xi_{1,\pi}(t),\ldots,\xi_{n,\pi}(t))$ and $\bm{\gamma}_{\pi}(t)=(\gamma_{1,\pi}(t),\ldots,\gamma_{n,\pi}(t))$ %and $\bm{\zeta}=(\zeta_1,\ldots,\zeta_n)$ 
with non-negative components, where $n$ is the number of arriving jobs which can be either finite or infinite. The components of $\bm{\xi}_{\pi}(t)$ and $\bm{\gamma}_{\pi}(t)$ are interpreted as follows:
if job $i$ is present in the system at time $t$, then $\xi_{i,\pi}(t)$ is the number of remaining tasks (which are stored in the queue or being executed  by the servers) of job $i$, and $\gamma_{i,\pi}(t)$ is the number of unassigned tasks (which are stored in the queue and not being executed  by the servers) of job $i$; if job $i$ is not present in the system at time $t$ (i.e., job $i$ has not arrived at the system or has departed from the system), then $\xi_{i,\pi}(t)=\gamma_{i,\pi}(t)=0$. Hence, for all $i=1,\ldots,n$, $\pi\in\Pi$, and $t\in[0,\infty)$
\begin{align}%\label{eq_def_state_thm3}
0\leq \gamma_{i,\pi}(t)\leq \xi_{i,\pi}(t)\leq k_i.
\end{align}
Let $\{\bm{\xi}_{\pi}(t),\bm{\gamma}_{\pi}(t),t\geq0\}$ be the state process of policy $\pi$, which is assumed to be right-continuous. 
\end{definition}





A proof sketch of Theorem \ref{lem1} is provided as follows.
\begin{proof}[Proof sketch of Theorem \ref{lem1}]
%Here is a proof sketch of Theorem \ref{lem1}.
The proof contains two parts: In the first part, we use the conditions of Theorem \ref{lem1} to establish the following stochastic ordering result:
\begin{lemma}[Stochastic Ordering]\label{lemG4}
Suppose that $\bm{\xi}_{P}(0^-) = \bm{\gamma}_{P}(0^-) =\bm{\xi}_{\pi}(0^-) = \bm{\gamma}_{\pi}(0^-)=\bm{0}$ and the conditions of Theorem \ref{lem1} are satisfied. Then, the following relationship holds in stochastic ordering:
\begin{eqnarray}\label{eq_lemG4}
\sum_{i=j}^n {\gamma}_{[i],P}(t)\leq \sum_{i=j}^n {\xi}_{[i],\pi}(t),~j = 1,2,\ldots,n
\end{eqnarray}
for all $t\geq0$, where ${\xi}_{[i],\pi}(t)$ is the $i$-th largest component of vector $\bm{\xi}_{\pi}(t)$, and ${\gamma}_{[i],\pi}(t)$ is the $i$-th largest component of vector $\bm{\gamma}_{\pi}(t)$. 
\end{lemma}
From the perspective of majorization, \eqref{eq_lemG4} can be equivalent expressed as: $\bm{\xi}_{\pi}(t)$ is weakly majorized by $\bm{\gamma}_{P}(t)$ from above, i.e., $\bm{\xi}_{\pi}(t)\prec^{\text{w}}\bm{\gamma}_{P}(t)$ \cite{Marshall2011}. Note that Lemma \ref{lemG4} is a strong statement, because it holds for all $j = 1,2,\ldots,n$, time $t\in[0,\infty)$, job parameters $\mathcal{I}$, and policy $\pi\in\Pi$. In addition, Lemma \ref{lemG4} holds even if  the scheduling decisions of policy $\pi$ are made by using the parameters $(a_i,{k}_i,d_i)$ of future arriving jobs. In the second part of the proof, we use Lemma \ref{lemG4} to show that 
\begin{align}\label{eq_sketch1}
v_{(i)}(P) \leq c_{(i)}(\pi), ~i=1,\ldots,n
\end{align}
holds in stochastic ordering (Lemma \ref{lem_sample_path_ordering}).\footnote{Recall that $c_{(i)}(\pi)$ is the $i$-th smallest job completion time on the sample path of policy $\pi$, $v_{(i)}(P)$ is the $i$-th smallest component of the vector $(v_1(P),\ldots,v_n(P))$, and  $v_{i}(P)$ is the earliest time that all tasks of job $i$ are either completed or under service on the sample path of policy $P$.} Hence, Lemma \ref{lemG4} characterizes the timeline of job
executions on the sample paths of policy $P$ and policy $\pi$. Finally, Theorem \ref{lem1} follows from \eqref{eq_sketch1}. 
The proof details are provided in Appendix \ref{app0}. 
\end{proof}

%In Appendix \ref{app0}, we develop a  {sample-path ordering} technique to prove Theorem \ref{lem1}. 

%The first part of this {sample-path ordering} technique, i.e., 
The stochastic ordering result in Lemma \ref{lemG4} is motivated by \cite{Smith78}, which provided a proof of the optimality of Shortest-Remaining-Processing-Time (SRPT) first policy for single-server queueing systems. The generalization from \cite{Smith78} to Lemma \ref{lemG4} for multiple-server queueing systems with parallel processing and task replications is highly non-trivial. A preliminary version of this {sample-path ordering} technique was proposed in \cite{Sun2015}.  


%Nonetheless, this technique is able to establish a dominance between $v_{(i)}(P)$ and $c_{(i)}(\pi)$ on sample-path, hence the name. 




% but the generalization from \cite{Smith78} to this {sample-path ordering} technique is non-trivial. % and unexpected when this research started. 


%While existing delay optimality analyses of task replications \cite{Borst2003,Righter2008,Kim2010,shah-Allerton-2013,ShengboInfocom,Sun2015} focused on the average delay ${D}_{\text{avg}}(\cdot)$, 
First, Theorem \ref{lem1} can be generalized to all delay metrics in $\mathcal{D}_{\text{sym}}$.
\begin{corollary}\label{coro1}
If \emph{${D}_{\text{avg}}(\cdot)$} is replaced by any \emph{$f\in\mathcal{D}_{\text{sym}}$}, Theorem \ref{lem1} still holds.
\end{corollary}

\begin{proof}
See Appendix \ref{app0}.
\end{proof}

\ifreport
\else
Due to space limitation, the proofs of the remaining results are relegated to our technical report \cite{report2015}.
\fi
In addition, a sufficient condition can be obtained for near optimality in minimizing the maximum lateness $L_{\max}(\cdot)$.
\begin{theorem}\label{lem2}
If there exists a work-conserving policy $P\in\Pi$ such that for all $\mathcal{I}$
\begin{itemize}
\itemsep0em 
\item[1.] Policy $P$ is {more work-efficient} than any policy $\pi\in\Pi$,
\item[2.] In policy $P$, each task allocated to the servers belongs to the job  with the earliest due time, whenever there exist unassigned tasks in the queue,
\end{itemize} 
then \emph{$[L_{\max}(\bm{V}_{}(P))|\mathcal{I}]\leq_{\text{st}} [L_{\max}(\bm{C}_{}(\pi))|\mathcal{I}]$} holds for all $\pi\in\Pi$ and $\mathcal{I}$.
\end{theorem}
%For the ease of understanding, Theorem \ref{lem1} and Theorem \ref{lem2} are expressed in similar forms. However, some parts of their proofs are quite different. In particular, because the delay metric is changed from average delay ${D}_{\text{avg}}(\cdot)$ to maximum lateness $L_{\max}(\cdot)$, a different form of sample-path ordering is required to prove Theorem \ref{lem2}. 
\ifreport
\begin{proof}[Proof sketch of Theorem \ref{lem2}]
The proof contains two parts: In the first part, we use the conditions of Theorem \ref{lem2} to establish a second form of  stochastic ordering:

\begin{lemma}[Stochastic Ordering --- The Second Form]\label{lemG4_thm3}
Suppose that $\bm{\xi}_P(0^-)=\bm{\gamma}_P(0^-)=\bm{\xi}_{\pi}(0^-)=\bm{\gamma}_{\pi}(0^-)=\bm{0}$ and the conditions of Thoerem \ref{lem2} are satisfied. Then, the following relationship holds in stochastic ordering:
\begin{eqnarray}\label{eq_lemG4_thm3}
\sum_{i:d_i\leq\tau} \gamma_{i,P}(t)\leq \sum_{i:d_i\leq\tau} \xi_{i,\pi}(t), ~\forall~\tau\in[0,\infty)
\end{eqnarray}
holds for all $t\geq0$.
\end{lemma}
In the second part of the proof, we use Lemma \ref{lemG4_thm3} to show that 
\begin{align}
v_{i}(P)-d_i \leq \max_{j=1,\ldots,n}[c_{j}(\pi)-d_j],~i=1,\ldots,n
\end{align}
holds in stochastic ordering (Lemma \ref{lem_sample_path_ordering_thm3}). By this, Theorem \ref{lem2} follows. The details are provided in Appendix \ref{app0_1}.
\end{proof}
\fi




If each job has one task, Theorem \ref{lem2} can be generalized to all delay metrics in $\mathcal{D}_{\text{sym}}\cup\mathcal{D}_{\text{Sch-1}}$ by using the rearrangement inequality in \cite[Theorem 6.F.14]{Marshall2011} and\cite{Chang93rearrangement_majorization}. 
%This result is motivated by .
%, but the proof technique is different.
\begin{corollary}\label{coro2}
If $k_1=\ldots=k_n=1$ and \emph{$L_{\max}(\cdot)$} is replaced by any \emph{$f\in\mathcal{D}_{\text{sym}}\cup\mathcal{D}_{\text{Sch-1}}$}, Theorem \ref{lem2} still holds.
\end{corollary}
\ifreport
\begin{proof}[Proof sketch of Corollary \ref{coro2}]
For all $f\in\mathcal{D}_{\text{sym}}$, we use Corollary \ref{coro1} to prove that the statement of Theorem \ref{lem2} holds if \emph{$L_{\max}(\cdot)$} is replaced by any $f\in\mathcal{D}_{\text{sym}}$. For all $f\in\mathcal{D}_{\text{Sch-1}}$, we show that there exists an $n$-vector $\bm{u}'$ satisfying 
%In order to prove \eqref{eq_coro2_3}, 
%it is sufficient to show that there exists an  such that 
\begin{align}\label{eq_coro2_6}
\bm{u}(P)-\bm{d}\prec \bm{u}'- \bm{d} \leq \bm{c} (\pi)-\bm{d},
\end{align}
which further implies 
\begin{align}\label{eq_coro2_3}
\bm{u}(P)-\bm{d}\prec_{\text{w}} \bm{c} (\pi)-\bm{d}. 
\end{align} 
Using this, we can show that the statement of Theorem \ref{lem2} holds if \emph{$L_{\max}(\cdot)$} is replaced by any $f\in\mathcal{D}_{\text{Sch-1}}$.
The details are provided Appendix \ref{app0_1}.
\end{proof}
\fi

If $d_i=a_i$ for all job $i$, $L_{\max}(\cdot)$ reduces to the {maximum delay} $D_{\max}(\cdot)$. In this case, we can obtain
\begin{theorem}\label{lem3}
If there exists a work-conserving policy $P\in\Pi$ such that for all $\mathcal{I}$
\begin{itemize}
\itemsep0em 
\item[1.] Policy $P$ is {more work-efficient} than any policy $\pi\in\Pi$,
\item[2.] In policy $P$, each task allocated to the servers belongs to the job  with the earliest arrival time, whenever there exist unassigned tasks in the queue,
\end{itemize} 
then \emph{$[D_{\max}(\bm{V}_{}(P))|\mathcal{I}]\leq_{\text{st}} [D_{\max}(\bm{C}_{}(\pi))|\mathcal{I}]$} holds for all $\pi\in\Pi$ and $\mathcal{I}$.
\end{theorem}
\ifreport
\begin{proof}
%Because $D_{\max}(\cdot)$ is a special case of $L_{\max}(\cdot)$. 
See Appendix \ref{app0_2}.
\end{proof}
\fi

If each job has $k$ tasks, Theorem \ref{lem3} can be generalized to all delay metrics in $\mathcal{D}_{\text{sym}}\cup\mathcal{D}_{\text{Sch-2}}$.
\begin{corollary}\label{coro3_1}
If $k_1=\ldots=k_n=k$ and \emph{$D_{\max}(\cdot)$} is replaced by any \emph{$f\in\mathcal{D}_{\text{sym}}\cup\mathcal{D}_{\text{Sch-2}}$}, Theorem \ref{lem3} still holds.
\end{corollary}
\ifreport
\begin{proof}
See Appendix \ref{app0_2}.
\end{proof}
\fi

